Practical Verifiable In-network Filtering for DDoS defense

In light of ever-increasing scale and sophistication of modern DDoS attacks, it is time to revisit in-network filtering or the idea of empowering DDoS victims to install in-network traffic filters in the upstream transit networks. Recent proposals show that filtering DDoS traffic at a handful of large transit networks can handle volumetric DDoS attacks effectively. However, the innetwork filtering primitive can also be misused. Transit networks can use the in-network filtering service as an excuse for any arbitrary packet drops made for their own benefit. For example, transit networks may intentionally execute filtering services poorly or unfairly to discriminate their competing neighbor ASes while claiming that they drop packets for the sake of DDoS defense. We argue that it is due to the lack of verifiable filtering - i.e., no one can check if a transit network executes the filter rules correctly as requested by the DDoS victims. To make in-network filtering a more robust defense primitive, in this paper, we propose a verifiable in-network filtering, called VIF, that exploits emerging hardware-based trusted execution environments (TEEs) and offers filtering verifiability to DDoS victims and neighbor ASes. Our proof of concept demonstrates that a VIF filter implementation on commodity servers with TEE support can handle traffic at line rate (e.g., 10 Gb/s) and execute up to 3,000 filter rules. We show that VIF can easily scale to handle larger traffic volume (e.g., 500 Gb/s) and more complex filtering operations (e.g., 150,000 filter rules) by parallelizing the TEE-based filters. As a practical deployment model, we suggest that Internet exchange points (IXPs) are the ideal candidates for the early adopters of our verifiable filters due to their central locations and flexible software-defined architecture.

==> Makefile <==
export TEXINPUTS:=.:formatting:$(TEXINPUTS)

CROSSTEX := crosstex
CROSSTEX_ARGS := --titlecase lower --add-in --short=author --short=conference

BIBTEX   := bibtex

FIGFIGS :=
EPSFIGS := 
PNGFIGS :=
PDFFIGS :=
SVGFIGS := 
GNUPLOTFIGS :=
FIGS    := $(FIGFIGS) $(EPSFIGS) $(PDFFIGS) $(SVGFIGS) $(GNUPLOTFIGS) \
           $(PNGFIGS)

TEX_SOURCES := paper.tex 

.SUFFIXES:

all: 
	pdflatex -shell-escape paper
	bibtex paper
	pdflatex -shell-escape paper
	
pdf: paper.pdf

commit: 
	git commit -m "Added stuff" -a
	git push origin master


spell: $(TEX_SOURCES)
	detex $^ | spell | env LANG=C sort -u | env LANG=C comm -23 - ok-words

clean:
	rm -f *~ *.log *.bbl *.dvi paper.pdf *.blg *.aux *.ps *.out


==> algo/inference-attack.tex <==
\begin{algorithm}[t]
	\footnotesize
	\caption{\PSD Inference Attack}
	\label{algo:class-boundary-search}
	\begin{algorithmic}[1]
		\Function{InferenceAttack}{}
		\State $C \gets$ SearchClassBoundary()
		\State $R \gets$ MeasureAverageRates($C$)
		\State \Return $C$, $R$
		\EndFunction		\Function{SearchClassBoundary}{}
		\State $U \gets \{0, 1\}^H, C \gets \emptyset, R \gets \emptyset$
		\While{$|U| > 0$}
		\State $h \overset{\$}{\gets} U$, $C \gets c \cup C$, $c \gets$ FindClass($h$), $U \gets U - c$
		\EndWhile
		\State \Return $C$
		\EndFunction
		\Function{FindClass}{$h$}
		\State $b \gets 0$                              \Comment{bitmask}
		\For{$i \gets 0$ to $H-1$}
		\State $h' \gets h \mathrel{\oplus} 2^i$    \Comment{flip the bit (bitwise xor)}
		\If{PairwiseFlooding($h$,$h'$) $= 1$}
		\State $b \gets b \mathrel{|} 2^i$      \Comment{mark the bit (bitwise or)}
		\EndIf
		\EndFor
		\State \Return $c \gets \{x | \text{ $x$ is coverd by header $h$ and mask $b$} \}$
		\EndFunction
		\Function{MeasureAverageRates}{$C$}
		\State $R \gets \emptyset, W \gets \emptyset$
		\State select a random class $c_0$ from $C$ \Comment{choose the reference class}
		\For{each class $c_i$ in $C$}
			\State choose a random header $h_i$ from $c_i$, $h_0$ from $c_0$
			\State $w_i \gets \textrm{PairwiseFlooding}(h_0, h_i)$
			\State $W \gets W \cup \{w_i\}$
		\EndFor
		\State $w_{\textrm{total}} = \sum\nolimits_{w_i \in W} w_i$
		\For{each class $w_i$ in $W$}
			\State $R \gets R \cup \{\frac{w_i}{w_{\textrm{total}}}L\}$ \Comment{$L$ is the total throughput limit}
		\EndFor
		\State \Return $R$
		\EndFunction
		\Function{PairwiseFlooding}{$h$,$h'$}
		\State Flood with packets of header $h$ and $h'$. Measure their rates $m$ and $m'$.
		\State \Return $\frac{m'}{m}$
		% \If{$m = m'$}
		% \State \Return True
		% \Else
		% \State \Return False
		% \EndIf
		\EndFunction		
	\end{algorithmic}    
\end{algorithm}

==> chapters/1intro.tex <==
\section{Introduction}
%
%In spite of extensive efforts (e.g.,~\cite{mirkovic2004taxonomy,moore2006inferring,parno2007portcullis}), distributed denial-of-service (DDoS) attacks continue to plague the Internet.  
Over the last few years, we have observed an escalation in {\em volume} of DDoS attack
%traffic; e.g., four times increase in the last three years~\cite{computerworld2013biggest,guardian2016ddos}. This stems from a growing attack-defense cost asymmetry --- generating attack
%traffic now costs much lesser than buying bandwidth to absorb it~\cite{kang2016defending},
%given the proliferation of attack sources (e.g., IoT devices~\cite{guardian2016ddos}).
During a volumetric attack, a victim autonomous system (AS) is flooded with unmanageably large svolume of packets to process.  
A primary defense against DDoS today is {\em filtering} (or blocking) of packets at the destination AS or {\em outsourced} filtering at third-party networks (e.g., cloud-based scrubbing).
%Unlike application-layer DDoS attacks that surgically target a
%particular resource of a targeted server, 
Volumetric attacks
congest bandwidth resources of targeted servers, their networks, and often
one or more of their upstream ASes~\cite{arbornetwork2016}.
Thus, by their very nature, defenses against volumetric attacks often demand {\em inter-domain collaboration} for filtering packets.
In fact, collaborative filtering has long been practiced via manual, on-demand interaction between administrators of ASes~\cite{dots-working-group}.  
Recently, there have been increasing interests in inter-domain collaborative filtering by major carriers (e.g., AT\&T and CenturyLink's collaborative filtering system~\cite{levy2017operationalizing}), a standards organization (e.g., IETF's DOTS~\cite{dots-use-case-7}), and equipment manufacturers (e.g., Huawei's Cloud Clean Alliance~\cite{}).
%
%two large ASes in the
%US\,---\,AT\&T and CenturyLink\,---\,have proposed a systematic,
%automated collaboration system for DDoS mitigation based on their
%institutional trust and pre-negotiated policies~\cite{levy2017operationalizing}.  
%An IETF standard working group called
%the DDoS Open Threat Signalling group (or DOTS) is working on a
%proposal for collaboration between two adjacent ASes with direct peering
%relationships~\cite{dots-use-case-7}.
%Some network equipment manufacturers advocate collaborative filtering among more than two ASes with a trusted third party that orchestrates large-scale DDoS mitigations (see Huawei's Cloud Clean Alliance~\cite{}).

%\paragraph{Source-end filtering.} 
Ideally, inter-domain collaboration is {\em most} effective when an attack-targeted destination AS {\em directly requests} a source AS, which hosts suspicious traffic, to filter suspicious or unwanted packets.  
Such {\em source-end filtering} has
clear technical and economical benefits: (1) it can significantly
reduce the bandwidth waste (thus cost saving for participating ASes) for
suspicious packets that would otherwise unnecessarily traverse to
downstream ASes; (2) ASes near the sources see lower traffic volume
than the destination ASes and thus can perform more complicated,
resource-demanding filtering operations (e.g., finer-grained rate
limiting); and (3) some local contexts about the traffic sources
(e.g., list of historically poorly protected client machines) can be utilized for better DDoS mitigation.  Many prior work has already highlighted these
benefits of source-end filtering~\cite{huawei-CCA,mirkovic2002attacking, liu2008filter,
  alwabel2015senss,zargar2013survey}.


Despite its advantages, however, source-end filtering has {\em not} found
wide-scale deployment due to the security and incentive problems. First, two ASes may
be {\em mutually distrusting} because they are likely to have no direct business relationship. 
Outsourcing filtering operations between untrusted ASes may pose some
security issues; e.g., a source AS may falsely claim that it is performing the 
requested filtering operation correctly, or, it may leak the filtering policy submitted by the destination AS, which may include sensitive information about the destination AS. 
Second, even if two ASes somehow establish some level of trust, there exist
{\em no explicit incentive} for the source ASes to perform filtering operations, which 
incur non-negligible costs, solely on behalf of other ASes. 
Moreover, even if the source AS somehow finds incentive to help (or decided
to be altruistic), it may find some clear risks of being criticized for dropping its own customers' packets without any evidence of congestion in its network, which further disincentivizes such filtering operations. 


\smallskip
%\paragraph{Secure Collaborative Source-End Filtering.} 
In this paper, we propose a novel collaborative source-end filtering framework (which we call {\em \name}) that, perhaps surprisingly, demonstrates that we can effectively filter suspicious or unwanted packets during DDoS attacks while providing {\em strong incentives} to the source AS (which actually performs packet filtering) and nicely handling potential attacks between the {\em mutually-untrusted} source and destination ASes.
Unlike most, if not all, source-end filtering proposals that {\em outsource} the filtering functionality of a destination AS to a source AS, \name requires {\em mutual participation} from two ASes for determining the final filtering policy that is impartial to the both participating ASes.
To be specific, {\em both} the destination and source ASes submit their packet filtering policies to the {\em filtering function} located in the source AS (let us consider a logical function until we clearly define it later). 
Then the filtering function combines the two policies to create and enforces the final policy for filtering packets from the source AS to the destination AS. 

\name can offer unprecedentedly strong {\em incentives} to source ASes becuase it allows a source AS to explicitly control the filtering policy when a remote destination AS is experiencing congestion. 
In existing DDoS mitigation, source ASes are {\em not} allowed to participate in a packet filtering decision but to solely rely on the destination AS's discretion (or cloud scrubber's decision) on which packets should be dropped when congestion occurs. 

%
%\smallskip
%\paragraph{Necessary security properties.}
\name also offers strong {\em security guarantees} against potential attacks between the untrusted ASes:
%\begin{enumerate}
%\item[(1)] {\bf Verifiably fair policy composition and enforcement.}
(1) \name guarantees the {\em verifiably fair policy composition} between untrusted ASes. 
%When the two independently-generated policies are combined, the final composed filtering policy should be a {\em fair} policy between the two. 
%To be specific, two policies may have rules that are conflicting (or even contradictory) to each other and thus both cannot be included in the final policy. 
The \name's policy composition logic guarantees that the final policy is determined as the middle ground between the two, which favors neither parties.
Moreover, \name allows two ASes to verify whether the policy composition is fairly composed and enforced; 
%
%\item[(2)] {\bf Negotiable privacy guarantees.}
(2) \name enables two ASes to {\em negotiate} the desired level of {\em privacy guarantees}. 
Network filtering policies are inherently sensitive information (e.g., policies may include information about private contracts, private white/black policies, or even vulnerable points of the networks) and thus any excessive policy leakages can be detrimental to their businesses. 
In \name, two ASes negotiate the desired upper-bound of the privacy leakage for their policies before they start filtering packets; and
%In particularly, the ASes should be able to sdecide the upper-bound of policy leakages (e.g., minimum anonymity set size) during the negotiation stage. 
% the minimum guaranteed degree of anonymity (e.g., anonymity set size) for the given two policies based on the inherent fairness-anonymity {\em trade-off}\,---\,that is, fairness must decrease to increase the degree of anonymity of the policies. 
%
%\item[(3)] {\bf Effective bypass detection.}
(3) \name effectively {\em detects any circumvention} attempt by source ASes.
A source AS may try to bypass the filtering function outside of the \name system; e.g., detour the \name system via rerouting.
The \name's detection is fast and accurate (e.g., extremely low false alarm rates).  
%\end{enumerate}


To make \name practical for mitigating large-scale DDoS attacks in today's Internet, we utilize several emerging secure hardwares capabilities and network management techniques available for commodity server platforms.  
First, we utilize a {\em trusted execution environment} (TEE) capability available in many CPUs for commodity servers (e.g., ARM TrustZone, Intel SGX).
With the TEE support, \name offers {\em isolated executions} for the filtering operations, protecting them from a potentially malicious source ASes. 
Second, to make it practical for backbone operations (e.g., 10--100 Gb/s packet filtering) with dynamic bandwidth provisioning at a low operational cost, we take advantage of {\em software-defined networking} (SDN) and {\em network functions virtualization} (NFV), which already have been embraced by major industry players (e.g., Verizon, AT\&T)~\cite{1,1,1,1}.

\smallskip
\paragraph{Challenges.} 
However, there are two main practical challenges that need to be addressed to realize a secure and practical defense mechanism with these emerging security and network capabilities:
\begin{enumerate}
	\item {\bf Fairness and privacy dilemma.} 
	First, there exists an undesirable, inherent trade-off between the fairness of policy composition and the privacy guarantees for the input policies. 
	Thus, it is fundamentally hard to achieve both the fairness and privacy of policies. 
	Worse yet, finding a right balance between them is non-trivial.
	Therefore, it is highly desired to build a negotiation protocol that guarantees quantifiably reasonable fairness and privacy bounds for practical operations between two mutually untrusted ASes.
	
	\item {\bf Secure and fast packet processing rate.} 
	Second, the desired security properties require heavy security checks for large volume of traffic.
	Particularly, for bypass detection, per-packet checks in the secure processor become necessary.
	However, such heavy use of secure processors makes it hard to achieve line-rate (e.g., 10s or 100s Gb/s) packet processing in commodity computing platforms.
	
\end{enumerate}

In this paper, we focus on how the TEE-based \name design can address these practical challenges. 
To address (1), \name analyzes the fairness-anonymity trade-off for a selected generic policy language and then presents a negotiation protocol that draws up an agreement on the balanced fairness-anonymity point between two untrusted parties. 
Moreover, to address (2), \name carefully designs the per-packet security checks to minimize the secure/non-secure-world context switching and achieves the near zero-copy operation for line-rate packet processing. 



Seen in a broader network security context, \name is a unique proof point that answers the question ``What is the emerging trusted hardware capability good for Internet security?'' in a wide-area context beyond simple trust extensions to existing distributed applications; e.g.,~\cite{kim2017enhancing,han2017sgx}.
Specifically, \name's TEE-based verifiably fairness, negotiable privacy guarantees, and circumvention detections form the basis for the first secure and practical source-end filtering against volumetric DDoS attacks.   
In the scope of this paper, \name demonstrates the first trusted collaborative filtering only between two ASes; yet, this design philosophy can be easily applied to existing systems (e.g.,~\cite{att}) and protocols (e.g.,~\cite{dots-working-group}), and extended to multiple-AS collaboration platforms (e.g.,~\cite{huawei}).


%TEE capabilities (e.g., isolated executions, remote attestation) of \name enable the two ASes to verify the \name's guarantees (i.e., fair policy composition, negotiated degree of privacy) and to detect bypass attacks.
%However, building an effective TEE based filtering system poses several design challenges. 
%First it requires the rigorous evaluation of privacy leakage of the submitted filtering policies based on adversary's capabilities/strategies and the fairness notions. 
%To be specific, the trade-off between the fairness of the policy composition and the degree of anonymity of the input policies need to be clearly analyzed for different policy definitions (e.g., simple allow/block rule sets, prioritized flow lists). 
%In addition, we should develop attacks that maximize the privacy leakages of the policies and demonstrate their feasibility and effectiveness. 
%
%Furthermore, designing a TEE based collaborative filtering system entails several non-trivial architectural challenges. 
%Particularly, achieving line-rate packet processing (e.g., rate limiting per traffic class, per-packet bypass detection) with per-packet verification operations by securely executed functions in the secure world seems non-viable due to the expected significant context switching overheads. 


\smallskip
\paragraph{Contributions.}
In this paper, we have the following contributions:
\begin{enumerate}
	\item Identify the security and incentivization problems of source-end outsourced filtering.
	\item First proposal. Fair collaboration. that offers new control to source networks.
	\item TEE based design for verifiably fair policy composition.
	\item Privacy guaranteed negotiation. Attacks. Tradeoff.
	\item Accurate and efficient bypass detection. Line rate. 
	\item SDN/NFV implementation. 
\end{enumerate}


==> chapters/3attack.tex <==
\section{Privacy Negotiation between Untrusted Autonomous Systems}
\label{sec:privacy}
In \name, there exist clear concerns for privacy when a destination AS hands over its own filtering policy to another untrusted AS~\cite{levy2017operationalizing}. 
Inherently, some filtering policies of an AS can be privacy-sensitive information that can be abused if they are leaked to other untrusted ASes. 
Filtering policies may include information about private contracts (e.g., which customer networks are `premium' subscribers), proprietary algorithms (e.g., mechanisms that prioritize certain services over the others when under congestion), internal white/black policies (e.g., usual suspects, mission-critical services), or even the vulnerable points of the networks (e.g., which links or subnetworks are under attacks).
In this section, we discuss how \name implements strong privacy mechanism that guarantees a certain level of privacy for both ASes based on the negotiation between them. 

\paragraph{Overview of the section.}
In this section, we first spend enough space to describe a number of policy inference attacks.
Privacy properties (e.g., degree of anonymity) are often the direct outcomes of particular attack instances and thus we first analyze privacy attacks in depth, focusing on their effectiveness and the attack outcomes. 
We devise an optimal adversary strategy and analyze the maximum attack effectiveness in terms of the anonymity set size.
Our policy inference attacks first try to learn the composed policy $P_{S,D}$ of \name and then the policy of the other party ($P_D$ in $S$'s perspective and $P_S$ in $D$'s perspecdtive).

Then, we describe how \name guarantees the desired level of privacy that is negotiable between the two ASes.
For this, we analyze the observed fairness-anonymity tradeoff that enables us to design a negotiable anonymity guarantee mechanism at the cost of reduced fairness. 
We demonstrate a simple, verifiable negotiation mechanism that can guarantee adequate level of privacy with limited fairness degradation.


\subsection{Policy inference attacks}
The ultimate goal of policy inference attacks is to accurately infer the other party's private policy ($P_D$ in $S$'s perspective and $P_S$ in $D$'s perspective). 
In more formal terms, the attack goal is to reduce the degree of anonymity of the other party's policy as much as possible. 
For example, a source AS $S$ may begin observing the behavior of \name to finally infer a number of possible policies of $D$, $\widehat{\mathcal{P}_D} = \{P_D^1,\cdots,P_D^n\}$, which constitutes the anonymity set for $P_D$.
We set the goal of the policy inference attacks to reduce the anonymity set size.

\input{figures/attack-overview.tex}

Note that due to the \name's isolated execution of the policy composition, an adversary cannot direct read the policies (that is, \PS, \PD, \PSD). 
Thus, instead, as shown in Figure~\ref{fig:attack-overview}, an adversary takes two-stage approach: 
(1) an adversary first observes the execution $\psi(\cdot)$ of the composed policy $P_{S,D}$ by monitoring packets entering/leaving the \name system and infer $P_{S,D}$ (Section~\ref{sec:PSD-inference-attack}); and
(2) the adversary infers the other party's policy by reversing the known policy composition function $\phi(\cdot)$ with the estimated $P_{S,D}$ and its own policy (Section~\ref{sec:PD-inference-attack}). 

For simpler illustration, in this section, we focus only on the attacks launched by a source AS $S$ to infer the destination AS $D$'s policy $P_D$. 
The vice versa is also possible (though with less attack effectiveness) and is summarized at the end of this section.
Moreover, as we discussed in Section~\ref{sec:policy-languages}, in this paper, we only consider the {\em soft preference} action type of our policy language.

\subsubsection{\bf Attack 1: $P_{S,D}$ inference attack}
\label{sec:PSD-inference-attack}
In this section, we design an effective attack that can accurately measure \PSD.
This, in fact, may sound {\em counter-intuitive} because the policy composition and the execution of it are {\em isolated} and thus no adversary directly read them.
However, with strong adversary capabilities of controlling all the inputs and outputs of our filtering function, adversaries can accurately infer the filtering policy.

Inferring \PSD is essentially the task of estimating the {\em average rates} of the token buckets for each traffic classes. 
Flach et al.~\cite{flach2016internet} recently proposes a simple algorithm to infer the average rates of token buckets only by monitoring the outgoing packets from a rate limiter.
When a constant flat outgoing rate is observed, it is the telltale sign of the specified average rate because it is highly likely that the incoming rate to the rate limiter is higher than the specified average rate and thus the rate has been policed.
Our \PSD inference attack may utilize this estimation technique to infer the average rate of each traffic class (i.e., token bucket) and reconstruct the policy \PSD.

Having said that, inferring \PSD is not trivial due to the following remaining challenges:
(1) the adversary does {\em not} know the {\em exact} traffic-class set \CSD and thus cannot determine which traffic-class identifier (e.g., five tuple) to measure for the flat outgoing rate; and
(2) the passive mechanism may be inaccurate when tokens in multiple token buckets are {\em shared} to achieve some {\em priority} policies (e.g., hard or soft preference among multiple traffic classes).

To that end, we propose a set of algorithms that detect the traffic class definition \CSD and then estimate the average rate of each traffic class.

\paragraph{Algorithm overview.}
Our algorithm picks one specific five-tuple identifier $h$ (say, $srcIP$=100.100.100.51, $dstIP$=200.200.200.133\footnote{For simplicity of discussion, we consider only IP addresses.}) at a time and tries to find if a slightly different identifier $h'$ (say, $srcIP$=100.100.100.38, $dstIP$=200.200.200.70) is also in the same traffic class or not (see below for details) until identifying the class definition $h$ is included in (say, $srcIP$=100.100.100.0/24, $dstIP$=200.200.200.0/24).
The algorithm continues until it finds all traffic classes specified in \PSD.
In the last step, it measures the average rates of all the identified traffic classes and then finally reconstructs \PSD.


\input{algo/inference-attack}

The full algorithms of the \PSD inference attack is described in Algorithm~\ref{algo:class-boundary-search}. 
The algorithm first runs the function \textsc{SearchClassBoundary} to accurately detect the traffic class definition of \PSD, that is, \CSD. 
The function random selects a flow identifier $h$ from the not-yet-classified flow identifier set ($U$) and then finds its class definition via the function \textsc{FindClass}.
Then, the algorithm brute-forces the position of masked bits of $h$; that is, for each bit in $h$, the algorithm flips the bit, obtains a new header $h'$, and tests whether $h$ and $h'$ are of same class.
To test, in the function \textsc{PairwiseFlooding} the algorithm floods \name with large enough input traffic rate with only packets of two types: $h$ and $h'$.
Then, it measures the output rates $m$ for $h$ and $m'$ for $h'$. 
If they are close enough, the algorithm determines that they are in the same traffic class (i.e., equally treated by \name); otherwise, they are in a different traffic class.
Once the traffic class set \CSD is inferred, the algorithm measures the rates of each traffic class in the function \textsc{MeasureAverageRates($C$)}.


\begin{figure}[ht]
	\centering
	\includegraphics[width=\columnwidth]{figures/attack_cost_analysis.pdf}
	\caption{Time cost evaluation of pairwise flooding (PF) and class boundary searching (CBS)}
	\label{fig:learn_psd_attack_eval}
\end{figure}

This inference attack algorithm is efficient. 
We use the number of calls of the PairwiseFlooding function as the metric for time cost analysis because it is the dominant time-consuming task in the entire algorithm. 
With this metric, the time cost comparison of two attacks is illustrated in Fig.~\ref{fig:learn_psd_attack_eval}. 
The figures shows that the class boundary searching is not only efficient (linear to $H$ and $|C|$) but also practical, even with a growing $H$ and an extremely large $|C|$ (e.g. 1000).
The estimated real time cost for class boundary searching is around 2.7 hours, assuming $|C| = 100$, $H = 100$ and 1s for running flooding-and-measuring once.



\subsubsection{\bf Attack 2: $P_{D}$ inference attack}
\label{sec:PD-inference-attack}

\input{chapters/attack-part2}

\subsection{Negotiation for the desired level of privacy}

As we saw in the policy inference attacks, when the policy composition aims to achieve the fairness between policies, the anonymity of policies can be quite restricted.
In this section, we first analyze this fundamental {\em fairness-anonymity trade-off}; that is, both fairness and anonymity of policies cannot be achieved in their ideal forms and some reduction of one is required to increase the other. 
Then, we utilize this trade-off and achieve much larger anonymity set by compromising relatively small amount of fairness. 

For the guaranteed level of privacy, \name allows untrusted ASes to negotiate on an agreed level of fairness degradation for a desired level of privacy before starting the filtering operation. 
Then, \name lets the two ASes to verify the correct negotiation operations in its control plane $\phi(\cdot)$ throughout the execution of the policies via remote attestation. 

\subsubsection{\bf Fairness-anonymity trade-off}
Let us first illustrate why both the fairness and anonymity properties {\em cannot} be achieved in their ideal forms.
As we saw in the previous section, any policy instance can be mapped into a unique policy point in the entire policy space. 
To achieve the ideal anonymity, when one policy (say, \PS) and the composed policy \PSD are given {\em all} the policy points in the universe must be equally possible for the other policy (say, \PD). 
This essentially implies that our composition function should be a random function that outputs any policy point in the space uniformly at random.
The random function, however, does not guarantee any fairness.
Conversely, to achieve the ideal fairness between \PS and \PD, \name should achieve $\mathcal{F}(\phi) =  |d(P_S,P_{S,D}) - d(P_D,P_{S,D})| = 0$\footnote{Or, $\mathcal{F}(\phi)=1$ when $|d(P_S,P_D)|$ is odd. For simplicity, we assume  $|d(P_S,P_D)|$ is even.} and such strict fairness enforcement allows only a small number of composed policy \PSD.
Therefore when one of the two input policies (say, \PS) and the composed policy \PSD are given, the number of possible \PD's can be quite limited; that is, the anonymity of \PD is limited.

The only way to increase the anonymity set of the input policies is to {\em enlarge} the possible composed policy set beyond the optimally fair policy solutions. 
In other words, \name needs to allow the composition algorithm to choose {\em sub-optimally fair} policies in addition to the optimal ones.

Note that this trade-off is a {\em inherent} property of any policy composition problem and thus cannot be removed via a new composition logic design. 
Instead, in \name, we exploit this trade-off and provide a negotiation mechanism for two untrusted ASes to come to an agreed level of fairness-anonymity trade-off.
Note that all the functions for the policy (i.e., trade-off) negotiation are the control-plane functions of \name and thus can be easily verified by the two ASes.

\subsubsection{\bf Demonstration: guaranteed anonymity set size}
Demonstration of one simple way to implement fairness compromise. Evaluate in various settings -- reasonable anonymity is obtained with reasonable fairness compromise. 



==> chapters/algo-example-fig.tex <==
\begin{figure}[t]
    \centering
%       \subfloat[Choices of $P_{S,D}$ for given $P_S$ \& $P_D$.]{%
%          \includegraphics[width=0.66\columnwidth]{figures/eg1}%
%          \label{fig:eg1}%
%       } 
%       \subfloat[Choices of $P_D$ for given $P_S$ \& $P_{S,D}$. ]{%
%          \includegraphics[width=0.66\columnwidth]{figures/eg2}%
%          \label{fig:eg2}%
%       }
%       \subfloat[Permutonhedron of order 4.]{%
          \includegraphics[width=0.65\columnwidth]{figures/4-permutohedron-sage}%
          \label{fig:order_4_p_hedron}%
%       }
       \caption{Permutonhedron of order 4.}
%       \label{fig:algo-example}
\end{figure}

==> chapters/algorithm.tex <==
\alglanguage{pseudocode}
\begin{algorithm}
\caption{Composition to find the midpoint of $P_S$ and $P_D$}
\label{algo:fair-comp}
\begin{algorithmic}[1]
\scriptsize
\Procedure {FairComposition}{$P_S(a_1, a_2, ..., a_n)$, $P_D(b_1, b_2, ..., b_n)$} 
\State $dist \gets \lfloor d(P_S, P_{D}) / 2 \rfloor$, $P_{S,D} \gets P_D$
\For{$i \leftarrow 1, n-1$}
    \For{$j \leftarrow 1, n - i$}
        \If{$p > q$ where $a_p = b_j, a_q = b_{j+1}$}
            \State {SWAP} {$b_j, b_{j+1}$}, $dist \gets dist - 1$
            \If{$dist = 0$}
                \State $P_{SD} \gets P_D$
                \State \Return
            \EndIf
        \EndIf
    \EndFor
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

%
%\alglanguage{pseudocode}
%\begin{algorithm}
%	\caption{Composition to find the midpoints of $P_S$ and $P_D$}
%	\label{algo:fair-comp}
%	\begin{algorithmic}[1]
%		\scriptsize
%		\Procedure {FairComposition}{$P_S(s_1 .. s_n)$, $P_D(d_1 .. d_n)$} 
%		\State $dist \gets RAND(\lfloor d(P_S, P_{D}) / 2 \rfloor, \lceil d(P_S, P_{D}) / 2 \rceil)$
%		\State $P_{SD} \gets P_D$
%		\For{$i \leftarrow 1, n-1$}
%		\For{$j \leftarrow 1, n - i$}
%		\If{$s_m > s_n$ where $s_m = d_j, s_n = d_{j+1}$}
%		\State {SWAP} RAND({$d_j, d_{j+1}$})
%		\State $dist \gets dist - 1$
%		\If{$dist = 0$}
%		\State $P_{SD} \gets P_D$
%		\EndIf
%		\EndIf
%		\EndFor
%		\EndFor
%		\EndProcedure
%	\end{algorithmic}
%\end{algorithm}

==> chapters/as-path.tex <==
\section{Availability of Alternative AS Paths}
\label{sec:as-path}

\updated{As we discussed in Section~\ref{sec:filter-bypass-detection}, the
ASes along the default path from $S$ to $D$ can refuse to forward the traffic,
thus causing {\em false positives} to our bypass detection. Here, we show that
$S$ and $D$ can flexibly choose an alternative AS path rather than sticking
with the default one. In particular, we model the network topology and the BGP
processing using the AS inferred relationships dataset from
CAIDA~\cite{caida}.  Next, we choose $100$ ASes that contain the most number
of Mirai botnets~\cite{mirai} and $100$ ASes that contain the most number of
DNS resolvers~\cite{wessels2014open} and model them as the source ASes. We select Tier-2
ASes, i.e., have providers and customers, to be the destination ASes. For each
source and destination pair, we count the number of available BGP paths
between them. The results in Figure~\ref{fig:as-path}  show that in the
majority of the AS pairs (more than $80\%$), there is at least  one
alternative BGP path between the source and the destination ASes so that they
can move traffic around the intermediate ASes on the default path.}


\begin{figure}[h]
	\centering
	\includegraphics[width=0.40\textwidth]{figures/as-path.pdf}
	\vspace{-5pt}
	\caption{Availability of alternative paths from Mirai-affected ASes and ASes with DNS amplifiers to Tier-2 ASes.}
	\vspace{-5pt}
	\label{fig:as-path}
\end{figure}

==> chapters/attack-part2.tex <==
% overview
Once $P_{S, D}$ is learned, the adversary $S$ can use the knowledge of composition algorithm $\phi(\cdot)$ to further recover the destination AS $D$'s policy $P_{D}$. To continue the discussion, we focus on the attack strategy against the soft preference policy and the fair composition algorithm we propose in Section~\ref{sec:policy}. The attack targets only one execution of the composition, i.e., learning $P_D$ according to the corresponding $P_S$ and $P_{S, D}$.

First, the adversary calculates $d(P_D, P_{S, D})$ using the known distance function (e.g., Kendall tau function). It then enumerates all possible \PD's with the condition that can generate $P_{S, D}$ with $P_S$ following the composition algorithm~\ref{algo:fair-comp}. If the there are multiple $P_D$ satisfying the condition, all of the possible \PD's form the anonymity set of \PD.

\input{chapters/algo-example-fig}

%\paragraph{Permutohedron}
% permutohedron
To better illustrate how the attack works, we use \textit{permutohedron} to visualize the policy, the distance metric, and  the composition. Permutohedron is a graph model where each vertex represents one possible policy (one permutation) and each edge represents the transformation between two polices via a single swap of two adjacent elements in the policy. Figure~\ref{fig:order_4_p_hedron} gives an example of permutohedron of order 4, which contains all the possible polices on 4 rules from 1 to 4 and all the possible transformation among each pair of them.

%\paragraph{Attack on deterministic composition}. 
The visualization provides a new way of understanding the deterministic policy composition. The composition algorithm essentially forms a shortest path between $P_S$ and $P_D$ where $P_{S, D}$ is the middle point on the path. When there are multiple shortest paths in the permutohedron for some pairs of $P_S$ and $P_D$, one of the shortest path is selected and its middle point is chosen as the composed policy by the algorithm~\ref{algo:fair-comp}. 
%This deterministic algorithm unfortunately fail to protect the policy $P_D$ since the adversary can always find the correct $P_D$ out of all the possibilities.

%\paragraph{Attack on non-deterministic composition}. 
%For the non-deterministic version of algorithm~\ref{algo:fair-comp} where all the shortest paths are considered and only one is selected randomly, the anonymity set is improved because it is possible that two or more different $P_D$ generates to the same $P_{S, D}$ with the same $P_S$. 
%Now the attacker can only find out the anonymity set instead of the correct $P_D$.

Let us illustrate how an adversary easily compute the anonymity set when \PS and \PSD are known. 
Let say \PS is 1432 ($A$) and \PD is 3214 ($B$), and the algorithm $\phi(\cdot)$ selects \PSD 1324 ($C$). 
Given \PS and \PSD, the adversary can guess that (3214 or 2134) for $\mathcal{F}(\phi) =  |d(P_S,P_{S,D}) - d(P_D,P_{S,D})| = 0$, or (3124, 1234, 3241, 2314, 2143) for $\mathcal{F}(\phi) = 1$ can be \PD. 
Thus, \PD's anonymity set is \{3214, 2134, 3124, 1234, 3241, 2314, 2143\}. 


The anonymity set size varies with different $P_S$ and $P_D$. 
From the permutohedron, one can find that in general the longer distance between $P_S$ and $P_D$, the larger the anonymity set, as there tend to be more equal-length shortest paths. 
Note that in certain extreme cases, the anonymity set may have only one element, which directly reveals \PD; e.g., when \PS is 1432 ($A$) and \PSD is 3124 ($D$), the only possible \PD is 2341 ($E$); i.e., the anonymity has size of 1.

==> chapters/attacks-sigcomm.tex <==
\section{Defense against Malicious Sources}
\label{sec:attacks-defenses}

\msk{Three attacks. Occurred outside of the \name enclaves. }

%\input{chapters/policy-bias}

\subsection{Filter Bypass Attack}

\msk{Bypass is possible. $S$ controls the network outside of the \name enclave and thus our system cannot prevent it.}

\msk{We make this detectable via consistancy checks}

\msk{We admit we cannot immediately detect some bypasses}

\msk{In such cases, we let the source hosts detect it instead. Source hosts are the ones who can choose their upstream ISPs (except some places where local ISP market is monopolized.) We believe that this will give reasonable incentives to source ISP not to conduct such bypass.}

This fine-grained packet processing in the enclave is useful for the detection of bypass attacks launched by $S$ to circumvent the \name filtering.
With the per-packet logging functions before and after the rate limiter (see Figure~\ref{fig:near-zero-copy}(a)), the enclave later can proof (1) if it has received a certain packet and (2) if it has allowed/dropped a certain packet. 
For such filtering accountability, one can imagine an memory efficient data structure, such as Bloom filters~\cite{bloom1970space}.
In practice, $D$ can periodically download the secure per-packet logging to match its own logging to detect any bypass (e.g., packet injections or drop outside of the enclave) has been conducted. 
Also, any customer network of $S$ (or even source hosts themselves) can query the enclave to check if their packets have been safely processed without any bypass attempt (e.g., $S$ drops packets before they reach the enclave). 

\subsection{Invoice Inflation Attack}

\msk{We measure `Did I' but not `Should I.'~\cite{ccsw11}. In other words, was the filtering all that necessary? It is hard to answer. In some network functions, this may be answered but not for filtering functions.}

\msk{We admit that measuring Should I is not possible for filtering function}

\msk{Our approach. Make it fully transparent. All the history of sources are recorded in the immutable, write-only log.}

\msk{We admit that we do not provide any proof or analysis of the deterrence. But we believe that this is practically the best approach we could do.}


==> chapters/attacks.tex <==
\section{Attacks}
\label{sec:attacks}

In this section, we discuss several generic attacks arising from the current problem settings. To begin with, we first introduce several concepts that are necessary for our discussion.

\begin{itemize}
    \item \textbf{Class}. As we have seen in the motivating examples, \textit{traffic class} groups the packets into a virtual cluster and is a efficient way to express the policy on a large subset of traffic. 
    
    \item \textbf{Action}. The \textit{action} is closely bound to one class, describing the rules or parameters that the rate-limiter should adopt and enforce.
\end{itemize}

According to our observation, we assume that class and action are building blocks in defining policy. We also use \textit{policy language} to denote the principles that different type of policies follow. 

\subsection{Recovering initial policy}
\label{subsec:recover-policy}

% P_S \phi P_D  ---> P_{S, D}.                attack reverses the 
%  | original policy    | composed policy
% class, action/value
The initial policy is the most confidential information and will be destroyed after policy composition. Therefore, the adversary has no way but recovers the initial policy using the information it collects, such as:

\begin{enumerate}
    \item Composition function, $\phi$.
    \item Adversary initial policy, $P_{D}$ or $P_{S}$.
    \item Composite policy, $P_{S, D}$.
\end{enumerate}

Note that (1) and (2) are public to the relevant parties, including the adversary. For (3) composite policy, we assume it is already compromised and fully learned by the adversary, by means we discussed in this paper.

Now we introduce several attacks that target different scenarios. The difficulty of conducting such attacks varies because any factors in policy composition will more or less change the game that adversary is playing. The factors may include the choice of policy language (complexity, expressiveness, completeness), the choice of composition function (fairness, efficiency), and the level of protection on privacy (uncertainty, transparency).

\subsubsection{\textbf{Null- and full-policy attack}}

The adversary uses an empty set of policy (thus the name \textit{null-policy}) to participate the policy composition. A weak composition will immediately output the opponent policy as the composite one, and lets the adversary knows the initial policy. The adversary has zero cost in this attack, making it a free lunch the adversary will anyway try first prior to any other attacks.

Compared to null-policy attack, the other extreme is \textit{full-policy} attack. The fullness is reflected from the size of the policy, because the full-policy abuses the usage of class, treating each individual unit (e.g., packet or flow) as a class. This long list of policy poses a challenge to the composition function: The opponent policy usually has a handful of classes with each covering a large subset of the traffic, so the function has to solve class conflict first. Usually, two strategies are used: (1) It merges some of the single-unit classes according to the classes defined in the opponent policy; (2) It keeps single-unit classes but inevitably assigns same actions to some groups of single-unit classes. Either one reveals at least the class information in the initial policy. On the other hand, the leakage of action information depends on how the adversary codes the action regarding to single-unit classes, which we will not expand here.

\subsubsection{\textbf{Black-and-white attack}}

\textit{Black-and-white} represents the simplest action performed on the class in the policy. For example, ISPs allow or block the traffic belongs to different classes. Such binary decision on each class causes a dilemma in composition when two initial policy have exactly opposite action. Because of this, the \textit{black-and-white attack} exploits the fact that any composition to solve black-and-white conflicts will inevitably reveal the initial policy. A simple example is the adversary will immediately know the opponent initial policy when a black policy on a class eventually turns white in the composite policy.
% \subsubsection{Example 1} \textit{Black-and-white policy}. ISPs use such policy to completely block or allow the traffic falling in certain class. The composition over this policy is never easy as conflicts are common, and they are solved in a way that will aid in reversing the initial policy. Knowing the composition rule, the malicious side can start inferring from the policy that are overwritten, and even create conflicts to its advantage. This inferring is straightforward no matter it is the allow policy overwrites the block policy or vice versa. We can foresee that the policy alike is subject to the reversing attack, simply because the composition is deterministic and reversible.

\subsubsection{\textbf{Inverse function attack}}

\textit{Multi-valued policy} is a direct extension on black-and-white policy, where the policy language allows a range of values associated with the per-class action, such as "block 30\% traffic", "set rate upper bound at 1Gbps", etc. One prominent advantage is such languages permit more flexible merging strategies rather than a binary decision. However, a poorly designed composition is still vulnerable to reversing attack, given that the function $\phi$ has a inverse function $\phi^{-1}$, which will accept $P_{S, D}$ and $P_{S}$ as input and output $P_{D}$ (assume a malicious $S$). This is \textit{inverse function attack}.

In fact, the adversary can construct the inverse function $\phi^{-1}$ using the known information about $\phi$, which compromise a series of naive composition functions like sum, average, or other linear combination of the policy value on  same class. On the other hand, from the composition designer's view, this suggest a defense of running non-reversible or non-deterministic composition functions.

% \subsubsection{Example 2} \textit{Multi-valued policy}. A direct improvement on the policy language is using policy that allows more possibilities with a range over different values. This offers a possibility to have fairness in the composition as a distance function can be defined the quantify the conflicts, and further used to find the middlepoint when solving the conflicts. Yet the attack is still simple given the determinism of the composition.
\subsubsection{\textbf{Adaptive attack}}

The above attacks mostly target one specific composition procedure, whereas the more powerful attack can be mounted when the attack can adaptively change its policy and smartly select the initial policy to recover the opponent one during multiple composition. An assumption here is the target policy will not change frequently during the time of adaptive attack.

Assume the policy language is a rank-based policy where each class is associated to a rank value, and the composition function $\phi$ is supposed to find a fair rank to mediate the difference of two ranks. For example, $(1, 4, 3, 2)$, $(3, 4, 2, 1)$ and $(3, 1, 4, 2)$ are the policies given by the adversary, the opponent, and the composition function $\phi$ respectively. The adversary notice the change after composition, so she launches a second composition using the first composite policy as its input, i.e., $(3, 1, 4, 2)$. The second composite policy is $(3, 4, 1, 2)$, which is close enough to the target. By reusing the composite policy as the input for next iteration, the adversary exploits the fair function $\phi$ that tries to bridge the gap between two diverged policy. Gradually, it approaches the target policy and it can choose to stop the iterations when the composite policy is same as its input or the difference between them is acceptable to the adversary.

% 1432            3421
%     1342     3412
%         3142


\subsection{Learning class and rate}
\label{subsec:learn-class-n-rate}
Another category of attacks appears in the policy enforcement stage, where for each class in the $P_{S, D}$, a rate-limiter is shaping the traffic in the class limited by a per-class rate. The \textit{class partition} and the \textit{per-class rates} are derived secretly from the $P_{S, D}$ and safely used by rate-limiters inside the trusted execution environment, ruling out any direct unauthorized access. However, these parameters are in the adversary's interest. once learned by the adversary, they can be used to infer $P_{S, D}$, eventually resulting in the reversing of the opponent policy (Section \ref{subsec:reverse-policy}).

The main targets are class partition and per-class rates, and the basic tool used by the attacker is traffic \textit{meter}, measuring the traffic rate of a potential class, set according to the guess on the class partition. The meter outputs the rate in real time, plotting the rate variation over time, and if a rate-limiter were set on the same class, one or more horizontal lines pinning at fixed rate would appear on the rate-time plot. This signals a possible right guess of the class and also reveals the rate. Conversely, if there is not capped rate found, the guess could be wrong.

Armed with this observation tool, the adversary could launch various attacks with different difficulty, depending on its capability.

\subsubsection{Enumeration}
For a passive observer watching the output traffic, it can setup per-class meters based on one enumeration of the class partition, whose total number on $n$ elements is given by exponential generating function $\sum_{n=0}^{\infty}{\frac{B_{n}}{n!}}z^{n}=e^{e^{z}-1}$. The attack will succeed once all the meters get the capped rate (and they sum up to the overall limit $L$), meaning that the partition is also found correctly. One can see that this is not a very efficient attack given the huge number of enumeration to make. Note that, the difficulty will continue to increase with \textit{work-conserving} mechanism (Section \ref{}) activated as it allows fluctuation, thus reducing the chances of getting a constant rate.

\subsubsection{Same-rate flooding}
For an active attacker who not only sees the output traffic but also has the ability to control the input, the guessing is not longer necessary. By overwhelming each point with high-volume traffic at a substantially large rate, the work-conserving protection will not take effect because there will be no underutilized bandwidth. Tha adversary then operates meters for every single point, reads the policed rate, and classifies the points having same measured rate into one class. This same-rate clustering works because the bandwidth in same class is equally distributed among every point within the class. The only chance it will fail is when points from different classes happen to have same measured rate, leading to misclassification.

\subsubsection{Partitioned search}


\subsection{Bypassing middlebox}

The third category of attacks, \textit{bypassing middlebox}, mainly carried out by a malicious platform provider, is about manipulating the traffic volume before or after the middlebox. The rate-limiting middlebox is only sensitive to shape-related manipulation as it focuses on the size of packets and only affects the volume of traffic getting through. Any other kinds of manipulation (e.g., packet content manipulation) is no longer only targeting the middlebox but the eventually the recipient of the traffic.

\subsubsection{Pre-filtering} 
The adversary runs its own filters prior to the middlebox, changing the profile of the traffic, or discriminating against the traffic of certain end-users. This pre-filtering is stealthy and runs undercover, since the blame is shifted to the middlebox if the end-users experience any service degradation.

\subsubsection{Probing}
This is another reshaping of the input traffic in a way that not only removes packets but also actively injects to drastically force the profile on input traffic. Usually the probing packets are used for the purpose like inferring the internal state of the middlebox. The more advanced probing has anti-detection measures, (e.g. mirroring traffic, slow rate attack) that evades the monitoring from middlebox or from the receiver of the output traffic.

% traffic addition, traffic deletion.
\subsubsection{Post-manipulating}
At the output side of the middlebox, the adversary is able to inject or remove the traffic mostly for covering up any operations done previously. It can remove the probing traffic or forward the original traffic directly to the output link for a complete bypassing, or inject packets to cancel out any pre-filtering actions.





==> chapters/attestation.tex <==
\section{Remote Attestation Performance}
\label{sec:remote-attestation}
% \msk{Shweta?}

The \name filter needs to provide a proof of authenticity to the destination network, before
the destination can trust the filter with the filter rules. 
The filter bootstraps this process by
creating a pair of public and privates keys. It then registers the public key
with the IAS service. At runtime, the destination initiates the remote
attestation process. 
Then the
source enclaved filter creates the attestation report which includes the
enclave measurement, platform security version number, software version,
software vendor security version number, the software configuration and any
other auxiliary information specific to the application.  The filter enclave
then asks the quoting enclave on the same platform to  verify and signs the
report with the attestation (private) key to generate the quote. The source
then forwards this quote to the destination. The destination asks the IAS to
verify the quote. The IAS then uses the initially registered public key of the
filter enclave to verify the signed quote. If the IAS confirms to the
destination that the quote is authentic, the remote attestation process
completes successfully.  

\codename performs remote attestation for each new enclave that the source
launches on its infrastructure. Since \codename is expected to operate under
DDoS attacks, we want to ensure that the launching of multiple-enclaves
on demand does not become the bottleneck for our deployment model. 
Here, we measure
the total amount of time to complete an end-to-end remote attestation
process for one enclave. In our micro-benchmark for remote attestation for the conservative performance tests, we setup the filter enclave
and the destination on a cloud machine hosted in
South Asia, and the IAS service
hosted in Ashburn, Virginia, United States. For an enclave binary of size $1$
MB, the platform takes $28.8$ milliseconds and the total end-to-end latency of $3.04$ seconds with a standard deviation $9.2$ milliseconds.


==> chapters/background.tex <==
\section{Background}
\label{sec:background}

\paragraph{Intel SGX.} (.25 page)
--- To be written.
%\msk{Need a short overview of SGX}
%
%
%\msk{how widely available.}
%
%\msk{focus on isolated execution, remote attestation.} 
%
%\msk{threat model}
%
%\msk{we trust IAS}

\paragraph{Blockchain-based Smart Contracts.} (.25 page)
--- To be written.
%\msk{Need a short overview of blockchain, Ethereum, smart contracts}
%
%
%- assets or resources are managed efficiently...
%
%SC.. embodies ... involvement of each party...
%
%SC ... written by a community network operators (e.g., IETF)...
%


==> chapters/bypass.tex <==
\section{Scalable Filter Implementation}
\label{sec:data-plane-design}

\msk{(1) Single-enclave implementation. Two options: full packet copy vs. near-zero copy.}

\msk{(2) Multi-enclave implementation for scalable bandwidth handling}



Line-rate performance on commodity platform is a necessity for \name design. 
Without it, \name can handle large-scale DDoS only with either highly-specialized hardwares or large numbers of commodity servers and thus can be too costly to source ISPs. 
As more network function virtualization applications require high-speed packet processing on commodity platforms, line-rate on commodity ideas have been extensively studied. Most widely accepted solutions (e.g., DPDK\cite{dpdk}, Netmap\cite{rizzo2012netmap}, PF\_RING ZC\cite{pfring}) implement zero-copy networking and achieve minimum context switching by circumventing the use of kernel network stack. Netmap reports that with a single core of 900 MHz it achieves 14.88 Mpps sending or receiving rate on 10 GbE network adapters. Also, the performance report from DPDK shows the capability of zero packet loss forwarding with various packet size.

However, achieving line-rate speed seems quite challenging when we need to satisfy the two desired security properties of the data-plane operation of \name.

\begin{itemize}
    \item \textbf{Integrity of rate-limiting.} Each data packet's filtering decision (i.e., allow/block) must be made within the enclave to ensure the integrity of the filtering decision. 
    
    \item \textbf{Secure packet logging.} Every packet incoming to and leaving from \name should be recorded within the enclave for accountable billing and bypass detection.
\end{itemize}

The two security properties appear to require per-packet operation within the enclave as we can see in a naive data-plane design.

\subsection{Accountable per-packet processing} 

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.5\textwidth]{figures/near-zero-copy.pdf}
	\caption{Two packet copy approaches for SGX-based accountable rate limiting and logging functions. In the near zero-copy approach, we copy only the memory reference ($\ast$), the five tuple ($5T$), and the size ($s$) of the packet into the enclave.}
	\label{fig:near-zero-copy}
\end{figure}

%As briefly discussed in Section~\ref{sec:overview}, a simple implementation of \name would be to enclose all sensitive filtering operations and private information inside the enclave.
The two main secure functions implemented inside the enclave are the multi-class rate limiters and packet logging. 
To guarantee the accountable operation of these functions, a naive approach would be to make the entire copy of incoming packets into the enclave and operate these functions over the packet copies inside the enclave. 
Figure~\ref{fig:near-zero-copy}(a) illustrates this so-called full packet copy approach. 
Any data-plane packet is copied into the enclave memory for full packet logging and rate limiting operations. 
If the packet is determined to be allowed, it is logged again before being copied once again back to the untrusted memory pool for final forwarding through the NIC.
 
\paragraph{Prevention of bypass attacks with per-packet logging.}
This fine-grained packet processing in the enclave is useful for the detection of bypass attacks launched by $S$ to circumvent the \name filtering.
%The intuition behind this full packet copy approach is clear.
%... want to ... accountability of packet filtering decision and logging per incoming packet. 
%With this ... can detect bypass attempts by $S$. 
With the per-packet logging functions before and after the rate limiter (see Figure~\ref{fig:near-zero-copy}(a)), the enclave later can proof (1) if it has received a certain packet and (2) if it has allowed/dropped a certain packet. 
For such filtering accountability, one can imagine an memory efficient data structure, such as Bloom filters~\cite{bloom1970space}.
In practice, $D$ can periodically download the secure per-packet logging to match its own logging to detect any bypass (e.g., packet injections or drop outside of the enclave) has been conducted. 
Also, any customer network of $S$ (or even source hosts themselves) can query the enclave to check if their packets have been safely processed without any bypass attempt (e.g., $S$ drops packets before they reach the enclave). 

\paragraph{Performance challenges.}
Despite its clear security benefits, the per-packet processing inside the enclave incurs too much overhead for making full packet copies of all the data-plane packets, whose data rate can be even a few Gb/s or more. 
This full packet copy operation also would create too frequent context switching that is too expensive for such high-packet processing requirements.
Our evaluation confirms the poor performance of the per-packet processing approach; see Section~\ref{sec:eval}.

 
%
%\paragraph{Overview}. In this naive implementation, 
%
%\paragraph{Rate-limiting}
%
%\paragraph{Packet logging}
%
%\paragraph{Challenges}
% In this naive detector, our goal to make the each packet's {\em arrival} and {\em departure} (after the packet is processed and allowed) at and from \name {\em verifiable} by the source hosts and the destination ISP $D$, respectively.
% One natural idea is to log {\em all} the packets \name receives and all the packets it forwards to $D$.
% For the memory efficient operations, which are necessary for our high throughput networking applications, we use two sets of Bloom filters $b_{in}$ and $b_{out}$ for incoming packets and outgoing packets, respectively.
% These Bloom filter bit arrays are stored within a secure memory region, e.g., en SGX enclave, to prevent malicious \name operators from manipulating the logging and thus verification.
% We provide two functions, {\tt Add}$_{in}(\cdot)$ and {\tt Query}$_{in}(\cdot)$ also within the secure memory region for $b_{in}$ ({\tt Add}$_{out}(\cdot)$ and {\tt Query}$_{out}(\cdot)$ for $b_{out}$).
% {\tt Add}$_{in}(p)$ function updates $b_{in}$ based on the cryptographic hash outputs of the incoming packet $p$ and {\tt Query}$_{in}(p)$ returns a test result whether $p$ is in the Bloom filter $b_{in}$. {\tt Add}$_{out}(p)$ and {\tt Query}$_{out}(p)$ are similarly defined for the outgoing packet $p$. 

% With the full packet logging mechanism, external verifiers can easily check if a certain packet has been handled by \name by requesting the copy of the Bloom filter bit arrays $b_{in}$ and $b_{out}$ and comparing them with the local filter arrays.
% The destination ISP $D$ may maintain its own local Bloom filter for the packets from $S$ and compare it with the Bloom filter array obtained from \name.
% Provided the accurate time synchronization between \name and $D$\footnote{possible... via a secure channel between them...}, any discrepancy between their Bloom filter arrays indicates a potential bypass attack.
% For example, if an array index is set to 1 in the $D$'s local filter but set to 0 in \name's filter, it indicates the existence of one or more injected packets.
% Or, any index that is set to 0 in the $D$'s local filter but not in \name's filter implies that one ore more packets have been dropped against \name's policy. 
% Note that it is the verifier's discretion to determine these indications as the bypass attacks or the artifacts of normal network operations (e.g., natural bit errors or packet drops happened in the transit networks).

\subsection{Sufficiency of {\em per-traffic-class} processing}
%\subsection{Near zero-copy data-plane}
% \paragraph{Performance challenge.}
% Although the naive full packet logging can effectively detect bypass attacks by the malicious source ISP $S$, there still remains a serious performance challenge\,---\,that is, the {\em per-packet logging} operations of the Bloom filter requires \name to copy {\em all} the packets into the secure memory region, e.g., enclave.
% Such {\em full packet copy} operation is indeed the biggest throughput bottleneck since copying each full packet creates significant context switching overheads.

\paragraph{Per-packet guarantee is unnecessary.}
Regarding the necessity of the expensive per-packet processing in the enclave, we make an observation that even with the secure per-packet processing, $S$ still can affect the rate limiting operations of \name by simply re-ordering the incoming data-plane packets.
Our rate limiter implementation handles multiple traffic classes in individual token buckets and each token bucket maintains the time varying amount of tokens to determine if an incoming packet should be dropped or allowed. 
If $S$ re-orders the packets within the same traffic class, it can affect the filtering decisions of re-ordered packets. 
For example, let say two packets $p_1$ and $p_2$ arrive at \name in this order and only $p_1$ uses the available tokens and $p_2$ is dropped. 
If $S$ flipped the order of the two packets, $p_1$ would be dropped instead. 
Such packet re-ordering can be potentially exploited by $S$ to control the rate limiting decisions within the same traffic class. 
Unfortunately, such packet re-ordering that happens {\em outside} of the enclave cannot be detected by the \name system. 

\paragraph{Per-traffic-class processing is sufficient.}
Instead of building expensive but unnecessary per-packet processing inside the enclave, we choose to build a much coarse-grained, per-traffic-class processing for the enclave operations. 
Figure~\ref{fig:near-zero-copy}(b) illustrates how the per-traffic-class processing works with the enclave memory operation. 
When a packet is received, only a fraction of its header fields (the five tuple fields, $5T$, and the packet size, $s$) are copied into the enclave memory along with the memory reference ($\ast$) of the packet.
The copied fields $<\!5T,s\!>$ are then represents the packet and used for the logging functions and the rate limiter. 
The memory reference $\ast$ is used to perform the corresponding operation (e.g., forward or block) for the packet in the untrusted memory pool depending on the rate limiter decision. 

The per-traffic-class accountability still guarantees the incoming and forwarded traffic volume per traffic class, which is sufficient for bandwidth measurement for billing purposes. 
Moreover, this enables $D$ and the $S$'s customer networks to detect bypass attempts when $S$ violates the per-traffic-class volume enforced by the fairly composed filtering policy \PSD. 
For example, if $S$ drops or injects some packets in a traffic class outside of the enclave, $D$ or the $S$'s customer networks can detect it because the per-traffic-class volume should differ. 
Note that the per-traffic-class accountability allows $S$ to affect the packet filtering decisions within a traffic class (e.g., dropping $p_1$ instead of $p_2$ when both are in the same traffic class); however, as we discussed, this attack is also feasible when we enforce finer-grained, per-packet accountability and it is fundamentally undetectable by \name.
%
%Let us first take a look at a subtle adversary's action called packet modification. 
%So fare we have defined bypass attacks as the source AS's illegal packet removals and injections. 
%Thus, a packet {\em modification} (say packet $p$ is modified to $p'$) by $S$ seems to be considered as bypass attacks (since modification can be expressed as removal followed by injection).
%However, we observe that some packet modifications are in fact {\em not} necessarily considered as bypass of the rate limiting operations. % and thus our bypass detection requirements can be relaxed significantly.
%Let us consider a particular packet modification from $p$ to $p'$ with the two conditions: $p$ and $p'$ are in the same traffic class (i.e., $\texttt{class}(p)=\texttt{class}(p')$) and have the same packet length (i.e., $\texttt{len}(p)=\texttt{len}(p')$).
%
%We observe that this particular packet modification does {\em not} necessarily bypass the rate limiting operation of \name because it does not make any changes to the rate limiting operations. 
%Recalling that our rate limiter operates based on the traffic class and  the packet length of incoming packets, the modification attempt does not effectively bypass any rate limiting operation but only damage the integrity of packets, which we do not aim to guarantee (see Section~X. Packet integrity is a non-goal.)
%
%Note that any other packet modifications (e.g., $p$ and $p'$ are in different traffic class or their lengths are different) are indeed considered as bypass attacks since the modification does bypass the rate limiting decision of \name. 

%\paragraph{Relaxed detection requirements.}
\paragraph{Per-traffic-class operations enables {\em near zero copy}.}
%As we exclude the specific type of packet modifications from our definition of bypass attacks, we can relax our detection requirements significantly.
%Particularly, we can have larger granularity of packet logging as we do not need to consider unnecessary details of each incoming packet but only necessary information for rate limiting operations; i.e., five-tuple bits and packet length.
As Figure~\ref{fig:near-zero-copy}(b) illustrates, the per-traffic-class processing in the enclave significantly reduces the amount of bits we copy into the enclave and thus we achieve a {\em near zero-copy} packet processing. % where only a subset of packet headers (e.g., five tuple bits and packet length) are copied into the trusted memory region and used for per-packet logging.
%We use a simple byte counter per traffic class within a trusted execution environment that maintains the authentic copy of the per-class byte counts at \name. 
%The per-class byte counter values are later sent to the destination AS $D$ and compared with $D$'s own local per-class byte counter values. 
%Any discrepancy between the two implies the potential bypass attempt, as we discussed in the naive full packet logging, with the only difference that we have per-class detection granularity as opposed to per-packet granularity, which is unnecessarily too fine grained.
%
Our near zero-copy operation reduces the byte size of what we copy into the trusted environment significantly (e.g., reduced to about 1\% for 1.5 KByte packets and 20\% for 64 Byte packets).
We evaluate the efficiency of the near zero-copy operation of \name in Section~\ref{sec:eval}.

\subsection{Scalability in parallel deployment}
Given the architectural limitation of secure computing resources in currently available SGX hardware, \name's single-enclave deployment is hardly able to deal with the ever-growing attack volume. Therefore, we extend the \name design to allow a parallel deploying scheme with multiple instances while preserving the same level of security guarantee as in the single one. The core idea is to randomly and equally distribute the traffic load among multiple replicated \name instances - each instance runs independently with same supplied policies and same outbound traffic limit. 
With this design, we believe that the \name system is capable of filtering up to 100 Gb/s undesired traffic, which is a reasonable capacity goal for one \name contract to handle as more contracts can work together to rate-limit the multi-hundred-giga traffic in the real world. 

The idea of replicated instances aims to avoid any additional complexity in the design and to make keeping the security promise a more straightforward task - any bias in the system is detectable because each rate-limiter is intended to start with the same filtering policies and run against roughly same-sized traffic with a similar distribution among different traffic classes. With multiple instances behaving like a single instance of \name, the extended system still keeps the integrity of the per-traffic-class filtering decision even though each instance works independently. 

\paragraph{Parallel Deployment} The extended design consists of multiple \name instances and one load-balancer distributing the traffic among the instances in a random and even manner (see Figure~\ref{}). 
Unlike the \name instance, the load-balancer does not need to run on the trusted hardware, making it possible to handle 100 Gb/s traffic with commodity hardware or any other existing specialized hardware in $S$'s network. Another change is that the instances must identify each other by the Ethereum wallet address with the help of $D$ after their remote attestations with $D$ succeed. Also, they can further establish secure channels with the help of $S$ to ally themselves with others and detect misbehaviors as an alliance.

\paragraph{Detecting diverged policy}. As each instance accepts policies from $S$ and $D$ via separate channels, the polices one receives may differ from the others if any party intends to create difference among the instances, breaking the overall integrity of the policy composition. However, this inconsistency can be easily detected when all the instances share the hash of the policy they received at the beginning and find any mismatches among the hashes. As a defense, all the instance will cease and inform the other party to stop the contract.

\paragraph{Detecting biased traffic distribution}. Our design requires a high-speed and fair load-balancer entirely controlled by $S$,  making the traffic distribution prone to $S$'s manipulation for malicious purpose. For example, a biased traffic distribution can affect the rate-limiting decisions made in different instances and tamper the rate-limiting result in the view of the entire system. Luckily, this bias can be detected similarly by sharing the per-traffic-class packet logging information and comparing with each other. We will discuss the consequence of this later.

\paragraph{Generating consolidated proof with multiple signatures}. In the single instance scheme, the proof of contracted work is generated by the \name enclave along with the signature and submitted by $S$ to the \name contract on behalf of the enclave. The same approach still works in the parallel deployment with only one amendment: the proof has to be signed by all the others if no load-balancer misbehaviors are detected. Any missing signature will cause failure of the verification process in the smart contract, and $S$ will not get the reward for the submitted work. 
%---------OLD------------
%\subsection{Tradeoff between accountability granularity and packet processing speed}
%
%\deli{Performance comparison: A Mpps vs B Mpps}

% \paragraph{Privacy-preserving traffic class granularity.}
% For the channel between $M$ and $D$, we use the traffic classes of $D$. 

% This creates a subtle problem. $S$ may attempt to bypass its own traffic class while satisfying $D$'s classes. 
% We argue that this is okay as this act harms the adversary himself only.

% For the channel between the traffic sources and $M$, we use the source IPs.



==> chapters/class-partition.tex <==
\section{Traffic Class Partition}
\label{sebsec:class-partition}

ISPs determine their policies $P_S$ and $P_D$ by translating their internal
traffic management policies; e.g., proprietary agreement for premium access,
higher priority for mission-critical services, black-listed or suspicious
networks.  A resulting filtering policy has one or more traffic classes.  A
{\em traffic class} represents a group of packets (e.g., a five-
tuple\footnote{\{Source IP, destination IP, source port number, destination
port number, and protocol\}.} defined flow aggregate) that are treated with
the same filtering configuration; e.g., any web (port 80 or 443) packet from a
group of hosts in an IP prefix to a group of server clusters.  We require that
each traffic class set ($C_S$ or $C_D$) is an exact cover of $U$ (i.e.,
traffic classes in each set ($C_S$ or $C_D$) are pairwise disjoint and the
union of all the traffic classes in each set is equal to $U$) so that each
policy covers all the flows in the entire address space.

The sets of traffic classes $C_S$ and $C_D$ in two policies $P_S$ and $P_D$,
respectively, are independently decided by the two ISPs and thus they are
likely to be different.  When they are unequal, as in most cases, the \name
middlebox should further partition the traffic classes in $C_S$ and/or $C_D$
until the two sets become identical.  This traffic class partition is
necessary as one cannot easily compare two policies when their traffic class
sets are different.  For example, when we have eight flows ($f_1,\cdots,f_8$),
the two traffic class sets can be differently defined as
$C_S=\{{\{{f_1,f_2}\},\{{f_3,f_4,f_5}\},\{{f_6,f_7,f_8}\}}\}$ and
$C_D=\{{\{{f_1}\},\{{f_2,f_3}\},\{{f_4,f_5,f_6,f_7,f_8}\}}\}$, then the
partitioned traffic class set is calculated as
$C_{S,D}=\{{\{{f_1}\},\{{f_2}\},\{{f_3}\},\{{f_4,f_5}\},\{{f_6,f_7,f_8}\}}\}$.
Two policies $P_S$ and $P_D$ can be expressed with the same traffic class set
$C_{S,D}$ and thus they are comparable.  Note that, as we see in this example,
we want the number of traffic classes in the partitioned set $C_{S,D}$ to be
minimized to remove unnecessary traffic classes.

\subsection{Recovering $C_{victim}$ without a priori information}
\label{subsec:csd-attack-strong}

The attacker wants to learn the victim's policy. This comprises of the traffic
classes and their relationship. For this the attacker first learns the $C_{S,
D}$ and the recovers the rate-limit for each class.

\paragraph{Forcing $C_{SD} = C_{victim}$.}
The attacker specifies a policy where all the points belong to a one class
i.e., $C_{attacker} = C_U$. This policy is an identity policy because it does
not affect the victim's classification. Thus, $\mathcal{C}(C_U, C_{victim}) =
C_{victim}$. For example, lets say that the victim's classification is
$C_{victim} = \{\{f_1,f_2\},\{f_3,f_4,f_5\}\}$ and the attacker choses his
classification as $C_{attacker}=\{\{f_1,f_2, f_3,f_4,f_5\}\}$. The resultant
re-classification $C_{s,d} = \{\{f_1,f_2\},\{f_3,f_4,f_5\}\}$. Thus, the
attacker can always ensure that the classification used by the middlebox is
exactly the same as the victim.

\paragraph{Learning the limit-rate of a class.}
When the middlebox sees a packet, it first identifies which class the packet
belongs to and then refers to the composite policy to probabilistically decide
whether to drop or keep the packet. The rate of dropping a packet is directly
defined by the rate-limiting function and the rank of that packet's class in
the policy.  The attacker knows that the output rate of the packets being
transmitted is capped to a $L$ bps pre-specified and known to both the ISPs.

%without work-conserving rate-limiters
If the source ISP is the attacker, it controls the types and number of packets
it can deliver to the middlebox. To learn the composite policy, the source ISP
starts adaptively pre-filtering the traffic it sends to the middlebox.
Specifically, it starts filtering all the traffic and floods the middle box
only say 2L packets which belong to one class $C_3$ whose class rate is
$P_{C_3}$. The middlebox consults the policy and drops $(2L) * (1 - P_{C_3})$
of the input packets. The attacker measures the number of total packets that
are being forwarded which is $(2L) * P_{C_3}$. The attacker can easily reverse
engineer that the limit-rate for $C_3$ is $P_{C_3}$.

\paragraph{Work-conserving rate-limiters.}
One way to make this attack difficult is to always saturate the output link
and keep the output volume at a constant volume of $L$ bps. Such mechanism is
well known as {\em work-conserving rate-limiters}~\cite{}. Thus, when the
attacker floods the middlebox with $2L$ bps packets from the same class,
instead of limiting the traffic to  the rate limiter with limit the traffic to
$(2L) * P_{C_3}$ bps which is less than $L$, the middle box will send out
packets at the rate of $L$ bps. When such a measure is in place, our attack is
not effective because the attacker only sees a constant encrypted output
traffic of $L$ bps.

\paragraph{Probe packets.}
The attacker can still circumvent the effect of  work-conserving rate-limiters
and learn the rate at which the middlebox is dropping the packets. To do this,
the attacker prepares {\em probe packets}. If a probe packet is delivered to
the victim, the attacker sees a response packet; if the packet is dropped the
attacker does not see any response packet. For example, the attacker prepares
$L$ packets of each class and floods the channel. i.e., if we have $4$ classes
$c_1, c_2, c_3, c_4$, then the attacker creates $4L$ traffic.  He lets the
middlebox filter the traffic to maintain a rate of $L$ and observe $r_1, r_2,
r_3, r_4$ responses per class. Then he learns that the rate for each classes
is $r_i/L$.

\paragraph{Search for partition classes.}

\begin{itemize}
	
	\item {\bf Enumeration.}
	The total number of partitions of an n-element set is given by exponential
	generating function  $\sum_{n=0}^{\infty}{\frac{B_{n}}{n!}}z^{n}=e^{e^{z}-1}$.
	The attacker can enumerate each of these possible partition classes until it
	finds the right partition class of the victim. However, the enumeration size
	quickly grows from $15$ options for $4$ elements to $4140$ options for $8$
	elements.

	\item {\bf Clustering after learning rates for each point.}
	The attacker floods the network with packets with same header $h_i$
	(represents a single point in the header space) and observes what is the
	rate-limit for it, say $r_i$. The attacker does this for all points in the
	header space and collects all the $r_i$ for $0 < i < n$. The it clusters
	all the $i$ which have the same rate. This directly tells the attacker
	that all these $i$ belong to the same class, since they have the same
	rate-limit.
	
	\item {\bf Partitioned Search.}
	The attacker first learns the rate for point 1 to be $r_1$ by sending only
	packets with header $h_1$. The attacker now knows that the rate-limit of
	the class which $h_1$ belongs to, is $r_1$. Then it starts sending equal
	number of packets for $h_1, h_2$ and observes the total output rate. If it
	is $r_1$, then $h_1, h_2$ both belong to the same class. If the new rate
	is $r > r_1$, then $h_2$ belongs to a different class whose rate-limit
	$r_2 = r - r_1$. Now the attacker can repeat this process to check the
	membership of $h_3$: check the rate for $h_1, h_3$ and $h_2, h_3$ to see
	if $h_3$ belongs to $h_1$'s class or $h_2$'s class. This strategy is
	similar to finding the right path in a search graph.

\end{itemize}

\subsection{Recovering $P_{s, d}$}
\label{subsec:psd-attack}

So far, we have assumed that the attacker (source ISP or destination ISP)
knows the composite policy $P_{s,d}$ computed by any one of our algorithms.
Here we show how this is possible. The attacker can repeat the process in
Section~\ref{subsec:csd-attack-strong} for all the traffic classes and learn
all the $P_{C_i}$. This directly leaks the composite policy $P_{s, d}$ being
deployed by the middlebox.

% We know that each class in the order-based policy comprises of IP addresses.
% When the middlebox sees a packet, it first identifies which class the packet
% belongs to and then refers to the composite policy to probabilistically decide
% whether to drop or keep the packet. The rate of dropping a packet is directly
% defined by the rank of that packet's class in the policy.  The attacker knows
% that the output rate of the packets being transmitted is capped to a $L$ bps
% pre-specified and known to both the ISPs.

% If the source ISP is the attacker, it controls the types and number of packets
% it can deliver to the middlebox. To learn the composite policy, the source ISP
% starts adaptively pre-filtering the traffic it sends to the middlebox.
% Specifically, it starts filtering all the traffic and floods the middle box
% only say 2L packets which belong to one class $C_3$ whose class rate is
% $P_{C_3}$. The middlebox consults the policy and drops $(2L) * (1 - P_{C_3})$
% of the input packets. The attacker measures the number of total packets that
% are being forwarded which is $(SL) * P_{C_3}$. The attacker can easily reverse
% engineer that the class-rate for $C_3$ is $P_{C_3}$. The attacker can repeat
% this process for all the traffic classes and learn all the $P_{C_i}$. This
% directly leaks the composite policy $P_{s, d}$ being deployed by the
% middlebox.

==> chapters/design.tex <==
\section{Policy Composition}
\label{sec:policy-composition}

Policy composition takes two input policies $P_S$ and $P_D$, and creates a
resultant composed policy $P_{S,D}$. The \codename middlebox uses this composite
policy to filter incoming packets from the source ISP $S$. 
In our composition, we use the policy abstraction we propose (see Section~\ref{sec:proposed-policy}); 
particularly, traffic classes are marked with preference rankings and Kendall tau metric
is used to define the distance between any two policies.

In this section, we define the fairness and privacy properties we wish to achieve
in more formal terms and define the goals of the policy composition function $\phi$. 
Then, under that proposed policy abstraction, we propose a set of deterministic and non-deterministic algorithms
that maximize the fairness while ensuring an adequate level of policy privacy. 

%The first step in policy
%composition is to calculate the composite traffic classes. \codename
%calculates the composite traffic-class set $C_{s,d}$ by breaking the traffic
%classes in input policies into smaller (i.e., finer-grained) traffic classes
%until both $C_{s}$ and $C_{d}$ can be expressed by $C_{s,d}$.  The number of
%traffic classes in the final composite $C_{s,d}$ is in the range of
%$[\max(|C_s|,|C_d|),|C_s|\times|C_d|]$ (inclusive at both ends). Once
%\codename has converted input policies as order preferences over uniform
%traffic classes, it calculates the composite policy $P_{s,d}$ using a
%composition function $\phi$.

% \subsection{Balancing Fairness \& Privacy}
\subsection{Metrics for Fairness \& Privacy}
\label{subsec:metrics-tradeoff}

%As an example, consider input policies
%$P_S = (1, 3, 2, 4)$ (where $i$-th element represents the rank of the $i$-th traffic class)
%and $P_D = (2, 1, 3, 4)$. 

The fairness and privacy of the resulting composite policy is a sensitive to
the choice of composition algorithms. 
We can express fairness of a composition function $\phi$ as $\mathcal{F}(\phi) =  |d(P_S,P_{S,D}) -
d(P_D,P_{S,D})|^{-1}$. Our aim is to find a $\phi$ that maximizes
$\mathcal{F}(\phi)$ for all possible input policies $P_S$ and $P_D$.
Given $P_S$
and $P_{S,D}$ we can define our privacy function $\mathcal{P}_S(\phi)$  as the
set of unique $P_D$'s such that $\phi(P_S, P_D) = P_{S,D}$. 
Similarly, we define the privacy function $\mathcal{P}_D(\phi)$ for given $P_D$ and $P_{S,D}$ as the 
number of unique $P_S$'s such that $\phi(P_S, P_D) = P_{S,D}$.
Note that $\mathcal{P}_S(\phi)$ ($\mathcal{P}_D(\phi)$) are the anonymity set 
for $D$ ($S$) as the real input policy $P_D$ ($P_S$) can be indistinguishable
within these set of other possible policies.

By these definitions, an ideal composition function $\phi$ is one which
maximizes both fairness $\mathcal{F}(\phi)$ and privacy $\mathcal{P}(\phi)$. 
We can achieve ideal fairness where
$d(P_S,P_{S,D}) = d(P_D,P_{S,D})$ such that $|d(P_S,P_{S,D})- d(P_D,P_{S,D})|
= 0$ then $\mathcal{F}(\phi) = 0^{-1} = \infty$. Thus, an ideal fair $\phi$
function is the one which  finds a policy $P_{S,D}$ that is {\em equidistant} from
both the input policies $P_S$ and $P_D$. Ideal privacy is achieved when the 
composite policy $P_{S,D}$ is completely independent of the input policies i.e., the
attacker's anonymity set size equals all possible policies in the language.
We can say that the
ideal anonymity set of the composite policy is the number of unique policies
possible with a given language and the traffic classes. In case of the policies with
four traffic classes and strictly ordered preference ranks, 
the $\phi$ function which randomly choses a policy from $24$ (or $\mathtt{factorial}({4})$) choices
achieves maximum privacy because by observing the output policy, the attacker
learns nothing about the input policies. As it is evident from this example,
ideal privacy may not preserve any fairness.

\input{chapters/recon-algo}

\input{chapters/privacy}

\input{chapters/sec-analysis}

==> chapters/economic-incentive.tex <==
\section{\updated{Opportunities and Pitfalls of Economic Incentives}}
\label{sec:economic-incentive}

%\updated{
%As we argue in Section~\ref{sec:intro} and~\ref{sec:case-for-source-filtering}, {\em well-intentioned} source networks would {\em unilateral} incentives (e.g., reduced upstream cost, monitoring its users/tenants) for non-cooperative filtering and incremental incentives (e.g., filtering with accurate attack attribution) to deploy \name as an add-on service. 
%Thus, additional economic incentive is {\em unnecessary} for them and the \name system can remain as {\em unpaid} service.
%}

Source networks may have multiple internal and external incentives for source filtering.
Irrespective of the types of incentives, \name bootstraps trust between ISPs.
Although the study of incentive models is {\em not} the main scope of this paper, we believe it is worth discussing the feasibility of economic incentive models and their potential pitfalls.


%However, additional economic incentive via {\em payment channels} (e.g., the additional operating costs of destination-specific filtering is paid by the destination ISP) may be useful when source ISPs are willing but unable to bear the operating costs of \name.
%The paid \name service model may have a potential to create a new, economically-driven DDoS defense platform at larger scale.
%may also incentivize indifferent source ISPs that do not have enough unilateral incentive for source filtering because the additional costs of filtering can be compensated by the payment from the destination ISPs. 
%That said, one may consider a paid filtering model, where a destination ISP pays a source ISP for performing certain filter rules. 
For economic incentives, one can consider a {\em paid} \name filtering service, where a DDoS victim network is willing to pay a source network for the measured amount of filtering work. 
%This paid filtering service is indeed possible because of the verifiable filtering operation of \name and, particularly, the accountable billing report from the SGX-based filter design.  
%Without the verifiable \name system between distrusting ISPs, a paid DDoS filtering service is only a wishful thinking. 
Yet, the paid service model, although interesting, must be carefully designed to address two potential pitfalls:
\begin{packeditemize}
\item {\bf Moral hazard.} 
Providing economic incentives for filtering work may end up encouraging rational source ISPs {\em not to fix} the problems in their networks (e.g., compromised hosts, misconfigured DNS servers) because the longer the attack duration, the larger payout the source ISPs can collect. 
To mitigate this, we can strictly limit the economic incentive when the source ISP filters the same attack traffic for the extended period of time.
For example, \name can implement a {\em decreasing pricing scheme} for filtering operations within an SGX-protected billing function. 
This way, the payout for the same traffic filtering work tapers off, thus encouraging the source ISP to fix the underlying problems (e.g., patching compromised hosts, reconfiguring DNS servers).
\item {\bf Attack generating ISPs.} 
A determined malicious source ISP may even generate attack traffic by itself to increase the attack traffic volume and maximize its revenue.
The long-term revenue of the malicious source ISP may not be guaranteed if \name has a defense scheme against the moral hazard problem. 
However, the malicious ISP can still cause short-term bill inflation.
To raise the bar for this attack, we can let the two ISPs to agree on the maximum traffic volume to be filtered with payment and enforce this limit in the SGX-protected billing function.
The malicious source ISP then may have to attack several destination ISPs to maximize its revenue and fully utilize its available attack bandwidth, which may increase the risk of its network being blacklisted. 
%\item {\bf Incentivization for deployment.} 
%The deployment of non-cooperative filtering is justified by the unilateral incentive of source ISPs.
%Only the additional filtering for destination-specific filter rules are required to be paid by the destination ISPs.
%Thus, the payment for the incremental cost cannot be used to incentivize the deployment of the source filter system. 
\end{packeditemize}
We envision that a new line of work on more rigorous economic incentive studies for source filtering will follow.
In this paper, our main interest is in the design of the practical auditable filters, which become an enabling technology for economic incentive models. 

==> chapters/filter-design.tex <==
\section{Scalable Filter Implementation}
\label{sec:filter-implementation}

\msk{(1) Single-enclave implementation. Two options: full packet copy vs. near-zero copy.}

\msk{(2) Multi-enclave implementation for scalable bandwidth handling}



Line-rate performance on commodity platform is a necessity for \name design. 
Without it, \name can handle large-scale DDoS only with either highly-specialized hardwares or large numbers of commodity servers and thus can be too costly to source ISPs. 
As more network function virtualization applications require high-speed packet processing on commodity platforms, line-rate on commodity ideas have been extensively studied. Most widely accepted solutions (e.g., DPDK\cite{dpdk}, Netmap\cite{rizzo2012netmap}, PF\_RING ZC\cite{pfring}) implement zero-copy networking and achieve minimum context switching by circumventing the use of kernel network stack. Netmap reports that with a single core of 900 MHz it achieves 14.88 Mpps sending or receiving rate on 10 GbE network adapters. Also, the performance report from DPDK shows the capability of zero packet loss forwarding with various packet size.

However, achieving line-rate speed seems quite challenging when we need to satisfy the two desired security properties of the data-plane operation of \name.

\begin{itemize}
    \item \textbf{Integrity of rate-limiting.} Each data packet's filtering decision (i.e., allow/block) must be made within the enclave to ensure the integrity of the filtering decision. 
    
    \item \textbf{Secure packet logging.} Every packet incoming to and leaving from \name should be recorded within the enclave for accountable billing and bypass detection.
\end{itemize}

The two security properties appear to require per-packet operation within the enclave as we can see in a naive data-plane design.

\subsection{Accountable per-packet processing} 

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.5\textwidth]{figures/near-zero-copy.pdf}
	\caption{Two packet copy approaches for SGX-based accountable rate limiting and logging functions. In the near zero-copy approach, we copy only the memory reference ($\ast$), the five tuple ($5T$), and the size ($s$) of the packet into the enclave.}
	\label{fig:near-zero-copy}
\end{figure}

%As briefly discussed in Section~\ref{sec:overview}, a simple implementation of \name would be to enclose all sensitive filtering operations and private information inside the enclave.
The two main secure functions implemented inside the enclave are the multi-class rate limiters and packet logging. 
To guarantee the accountable operation of these functions, a naive approach would be to make the entire copy of incoming packets into the enclave and operate these functions over the packet copies inside the enclave. 
Figure~\ref{fig:near-zero-copy}(a) illustrates this so-called full packet copy approach. 
Any data-plane packet is copied into the enclave memory for full packet logging and rate limiting operations. 
If the packet is determined to be allowed, it is logged again before being copied once again back to the untrusted memory pool for final forwarding through the NIC.
 
\paragraph{Prevention of bypass attacks with per-packet logging.}
This fine-grained packet processing in the enclave is useful for the detection of bypass attacks launched by $S$ to circumvent the \name filtering.
%The intuition behind this full packet copy approach is clear.
%... want to ... accountability of packet filtering decision and logging per incoming packet. 
%With this ... can detect bypass attempts by $S$. 
With the per-packet logging functions before and after the rate limiter (see Figure~\ref{fig:near-zero-copy}(a)), the enclave later can proof (1) if it has received a certain packet and (2) if it has allowed/dropped a certain packet. 
For such filtering accountability, one can imagine an memory efficient data structure, such as Bloom filters~\cite{bloom1970space}.
In practice, $D$ can periodically download the secure per-packet logging to match its own logging to detect any bypass (e.g., packet injections or drop outside of the enclave) has been conducted. 
Also, any customer network of $S$ (or even source hosts themselves) can query the enclave to check if their packets have been safely processed without any bypass attempt (e.g., $S$ drops packets before they reach the enclave). 

\paragraph{Performance challenges.}
Despite its clear security benefits, the per-packet processing inside the enclave incurs too much overhead for making full packet copies of all the data-plane packets, whose data rate can be even a few Gb/s or more. 
This full packet copy operation also would create too frequent context switching that is too expensive for such high-packet processing requirements.
Our evaluation confirms the poor performance of the per-packet processing approach; see Section~\ref{sec:eval}.

 
%
%\paragraph{Overview}. In this naive implementation, 
%
%\paragraph{Rate-limiting}
%
%\paragraph{Packet logging}
%
%\paragraph{Challenges}
% In this naive detector, our goal to make the each packet's {\em arrival} and {\em departure} (after the packet is processed and allowed) at and from \name {\em verifiable} by the source hosts and the destination ISP $D$, respectively.
% One natural idea is to log {\em all} the packets \name receives and all the packets it forwards to $D$.
% For the memory efficient operations, which are necessary for our high throughput networking applications, we use two sets of Bloom filters $b_{in}$ and $b_{out}$ for incoming packets and outgoing packets, respectively.
% These Bloom filter bit arrays are stored within a secure memory region, e.g., en SGX enclave, to prevent malicious \name operators from manipulating the logging and thus verification.
% We provide two functions, {\tt Add}$_{in}(\cdot)$ and {\tt Query}$_{in}(\cdot)$ also within the secure memory region for $b_{in}$ ({\tt Add}$_{out}(\cdot)$ and {\tt Query}$_{out}(\cdot)$ for $b_{out}$).
% {\tt Add}$_{in}(p)$ function updates $b_{in}$ based on the cryptographic hash outputs of the incoming packet $p$ and {\tt Query}$_{in}(p)$ returns a test result whether $p$ is in the Bloom filter $b_{in}$. {\tt Add}$_{out}(p)$ and {\tt Query}$_{out}(p)$ are similarly defined for the outgoing packet $p$. 

% With the full packet logging mechanism, external verifiers can easily check if a certain packet has been handled by \name by requesting the copy of the Bloom filter bit arrays $b_{in}$ and $b_{out}$ and comparing them with the local filter arrays.
% The destination ISP $D$ may maintain its own local Bloom filter for the packets from $S$ and compare it with the Bloom filter array obtained from \name.
% Provided the accurate time synchronization between \name and $D$\footnote{possible... via a secure channel between them...}, any discrepancy between their Bloom filter arrays indicates a potential bypass attack.
% For example, if an array index is set to 1 in the $D$'s local filter but set to 0 in \name's filter, it indicates the existence of one or more injected packets.
% Or, any index that is set to 0 in the $D$'s local filter but not in \name's filter implies that one ore more packets have been dropped against \name's policy. 
% Note that it is the verifier's discretion to determine these indications as the bypass attacks or the artifacts of normal network operations (e.g., natural bit errors or packet drops happened in the transit networks).

\subsection{Sufficiency of {\em per-traffic-class} processing}
%\subsection{Near zero-copy data-plane}
% \paragraph{Performance challenge.}
% Although the naive full packet logging can effectively detect bypass attacks by the malicious source ISP $S$, there still remains a serious performance challenge\,---\,that is, the {\em per-packet logging} operations of the Bloom filter requires \name to copy {\em all} the packets into the secure memory region, e.g., enclave.
% Such {\em full packet copy} operation is indeed the biggest throughput bottleneck since copying each full packet creates significant context switching overheads.

\paragraph{Per-packet guarantee is unnecessary.}
Regarding the necessity of the expensive per-packet processing in the enclave, we make an observation that even with the secure per-packet processing, $S$ still can affect the rate limiting operations of \name by simply re-ordering the incoming data-plane packets.
Our rate limiter implementation handles multiple traffic classes in individual token buckets and each token bucket maintains the time varying amount of tokens to determine if an incoming packet should be dropped or allowed. 
If $S$ re-orders the packets within the same traffic class, it can affect the filtering decisions of re-ordered packets. 
For example, let say two packets $p_1$ and $p_2$ arrive at \name in this order and only $p_1$ uses the available tokens and $p_2$ is dropped. 
If $S$ flipped the order of the two packets, $p_1$ would be dropped instead. 
Such packet re-ordering can be potentially exploited by $S$ to control the rate limiting decisions within the same traffic class. 
Unfortunately, such packet re-ordering that happens {\em outside} of the enclave cannot be detected by the \name system. 

\paragraph{Per-traffic-class processing is sufficient.}
Instead of building expensive but unnecessary per-packet processing inside the enclave, we choose to build a much coarse-grained, per-traffic-class processing for the enclave operations. 
Figure~\ref{fig:near-zero-copy}(b) illustrates how the per-traffic-class processing works with the enclave memory operation. 
When a packet is received, only a fraction of its header fields (the five tuple fields, $5T$, and the packet size, $s$) are copied into the enclave memory along with the memory reference ($\ast$) of the packet.
The copied fields $<\!5T,s\!>$ are then represents the packet and used for the logging functions and the rate limiter. 
The memory reference $\ast$ is used to perform the corresponding operation (e.g., forward or block) for the packet in the untrusted memory pool depending on the rate limiter decision. 

The per-traffic-class accountability still guarantees the incoming and forwarded traffic volume per traffic class, which is sufficient for bandwidth measurement for billing purposes. 
Moreover, this enables $D$ and the $S$'s customer networks to detect bypass attempts when $S$ violates the per-traffic-class volume enforced by the fairly composed filtering policy \PSD. 
For example, if $S$ drops or injects some packets in a traffic class outside of the enclave, $D$ or the $S$'s customer networks can detect it because the per-traffic-class volume should differ. 
Note that the per-traffic-class accountability allows $S$ to affect the packet filtering decisions within a traffic class (e.g., dropping $p_1$ instead of $p_2$ when both are in the same traffic class); however, as we discussed, this attack is also feasible when we enforce finer-grained, per-packet accountability and it is fundamentally undetectable by \name.
%
%Let us first take a look at a subtle adversary's action called packet modification. 
%So fare we have defined bypass attacks as the source AS's illegal packet removals and injections. 
%Thus, a packet {\em modification} (say packet $p$ is modified to $p'$) by $S$ seems to be considered as bypass attacks (since modification can be expressed as removal followed by injection).
%However, we observe that some packet modifications are in fact {\em not} necessarily considered as bypass of the rate limiting operations. % and thus our bypass detection requirements can be relaxed significantly.
%Let us consider a particular packet modification from $p$ to $p'$ with the two conditions: $p$ and $p'$ are in the same traffic class (i.e., $\texttt{class}(p)=\texttt{class}(p')$) and have the same packet length (i.e., $\texttt{len}(p)=\texttt{len}(p')$).
%
%We observe that this particular packet modification does {\em not} necessarily bypass the rate limiting operation of \name because it does not make any changes to the rate limiting operations. 
%Recalling that our rate limiter operates based on the traffic class and  the packet length of incoming packets, the modification attempt does not effectively bypass any rate limiting operation but only damage the integrity of packets, which we do not aim to guarantee (see Section~X. Packet integrity is a non-goal.)
%
%Note that any other packet modifications (e.g., $p$ and $p'$ are in different traffic class or their lengths are different) are indeed considered as bypass attacks since the modification does bypass the rate limiting decision of \name. 

%\paragraph{Relaxed detection requirements.}
\paragraph{Per-traffic-class operations enables {\em near zero copy}.}
%As we exclude the specific type of packet modifications from our definition of bypass attacks, we can relax our detection requirements significantly.
%Particularly, we can have larger granularity of packet logging as we do not need to consider unnecessary details of each incoming packet but only necessary information for rate limiting operations; i.e., five-tuple bits and packet length.
As Figure~\ref{fig:near-zero-copy}(b) illustrates, the per-traffic-class processing in the enclave significantly reduces the amount of bits we copy into the enclave and thus we achieve a {\em near zero-copy} packet processing. % where only a subset of packet headers (e.g., five tuple bits and packet length) are copied into the trusted memory region and used for per-packet logging.
%We use a simple byte counter per traffic class within a trusted execution environment that maintains the authentic copy of the per-class byte counts at \name. 
%The per-class byte counter values are later sent to the destination AS $D$ and compared with $D$'s own local per-class byte counter values. 
%Any discrepancy between the two implies the potential bypass attempt, as we discussed in the naive full packet logging, with the only difference that we have per-class detection granularity as opposed to per-packet granularity, which is unnecessarily too fine grained.
%
Our near zero-copy operation reduces the byte size of what we copy into the trusted environment significantly (e.g., reduced to about 1\% for 1.5 KByte packets and 20\% for 64 Byte packets).
We evaluate the efficiency of the near zero-copy operation of \name in Section~\ref{sec:eval}.

\subsection{Scalability in parallel deployment}
Given the architectural limitation of secure computing resources in currently available SGX hardware, \name's single-enclave deployment is hardly able to deal with the ever-growing attack volume. Therefore, we extend the \name design to allow a parallel deploying scheme with multiple instances while preserving the same level of security guarantee as in the single one. The core idea is to randomly and equally distribute the traffic load among multiple replicated \name instances - each instance runs independently with same supplied policies and same outbound traffic limit. 
With this design, we believe that the \name system is capable of filtering up to 100 Gb/s undesired traffic, which is a reasonable capacity goal for one \name contract to handle as more contracts can work together to rate-limit the multi-hundred-giga traffic in the real world. 

The idea of replicated instances aims to avoid any additional complexity in the design and to make keeping the security promise a more straightforward task - any bias in the system is detectable because each rate-limiter is intended to start with the same filtering policies and run against roughly same-sized traffic with a similar distribution among different traffic classes. With multiple instances behaving like a single instance of \name, the extended system still keeps the integrity of the per-traffic-class filtering decision even though each instance works independently. 

\paragraph{Parallel Deployment} The extended design consists of multiple \name instances and one load-balancer distributing the traffic among the instances in a random and even manner (see Figure~\ref{}). 
Unlike the \name instance, the load-balancer does not need to run on the trusted hardware, making it possible to handle 100 Gb/s traffic with commodity hardware or any other existing specialized hardware in $S$'s network. 
%Another change is that the instances must identify each other by the Ethereum wallet address with the help of $D$ after their remote attestations with $D$ succeed. 
Also, they can further establish secure channels with the help of $S$ to ally themselves with others and detect misbehaviors as an alliance.

\paragraph{Detecting diverged policy}. As each instance accepts policies from $S$ and $D$ via separate channels, the polices one receives may differ from the others if any party intends to create difference among the instances, breaking the overall integrity of the policy composition. However, this inconsistency can be easily detected when all the instances share the hash of the policy they received at the beginning and find any mismatches among the hashes. As a defense, all the instance will cease and inform the other party to stop the contract.

\paragraph{Detecting biased traffic distribution}. Our design requires a high-speed and fair load-balancer entirely controlled by $S$,  making the traffic distribution prone to $S$'s manipulation for malicious purpose. For example, a biased traffic distribution can affect the rate-limiting decisions made in different instances and tamper the rate-limiting result in the view of the entire system. Luckily, this bias can be detected similarly by sharing the per-traffic-class packet logging information and comparing with each other. We will discuss the consequence of this later.

\paragraph{Generating consolidated proof with multiple signatures}. In the single instance scheme, the proof of contracted work is generated by the \name enclave along with the signature and submitted by $S$ to the \name contract on behalf of the enclave. The same approach still works in the parallel deployment with only one amendment: the proof has to be signed by all the others if no load-balancer misbehaviors are detected. Any missing signature will cause failure of the verification process in the smart contract, and $S$ will not get the reward for the submitted work. 
%---------OLD------------
%\subsection{Tradeoff between accountability granularity and packet processing speed}
%
%\deli{Performance comparison: A Mpps vs B Mpps}

% \paragraph{Privacy-preserving traffic class granularity.}
% For the channel between $M$ and $D$, we use the traffic classes of $D$. 

% This creates a subtle problem. $S$ may attempt to bypass its own traffic class while satisfying $D$'s classes. 
% We argue that this is okay as this act harms the adversary himself only.

% For the channel between the traffic sources and $M$, we use the source IPs.



==> chapters/impl.tex <==
\section{Implementation}
\label{sec:impl}

%In the naive design, the additional copy of each packet unnecessarily increases the workload for packet processing and imposes a high pressure on the limited enclave memory. We have conceptually shown that after rethinking the accountability that \name really requires, only a lightweight copy of certain fields in the header of a packet is sufficient to maintain a secure view of the metadata over the packet's lifetime in the enclave, which avoids the cost both in the time and space from making a full copy. 
In the implementation overview shown in Figure~\ref{fig:impl-overview}, we can see that the enclave allocates a \textit{header memory pool} that caches the header fields necessary for data-plane operations. This makes \name's implementation more cost-efficient and opens more opportunities in the future when handling 10s Gb/s or more traffic.

\subsection{Overview}

\begin{figure*}[!ht]
	\centering
	\includegraphics[width=0.9\textwidth]{figures/impl-sigcomm.pdf}
	\caption{Implementation details of \name.}
	\label{fig:impl-overview}
\end{figure*}

Figure~\ref{fig:impl-overview} shows the main components of \name's implementation. The application runs in the user space that is split into a trusted area and a untrusted area. The trusted area consists of the entire control-plane and a minimal data-plane to ensure the integrity of the policy composition and enforcement. The entire \name and its running environment is built with Intel SGX SDK 1.9\cite{sgxrelease} and DPDK 17.05.2\cite{dpdkrelease}. We also use Intel SGX SSL library\cite{intelsgxssl} to build the remote attestation module within the control-plane as well as the secure channels for communication with other hosts.

We implemented the data-plane functionality based on the \code{qos\_sched} library from DPDK. To support its running within SGX enclave, we further ported DPDK's memory-related libraries (e.g., \code{rte\_mempool}, \code{rte\_ring}, and \code{rte\_malloc}) and other supporting libraries (e.g., \code{rte\_mbuf}) into the enclave. Moreover, we carefully choose the secure boundary in the data-plane so that only a few OCALLs are invoked (when calling the untrusted functions from the enclave) and the amount of data crossing the boundary is minimized. For example, only the packet reference (i.e. pointer) is passed via the OCALLs while the copy of the header fields are done via the direct memory access.

The trusted part of the implementation contains about 7k source lines of code (SLoC) and the compiled signed enclave binary is 1.7 MB in size. The runtime footprint of trusted memory is 68 MB, effectively preventing the enclave from any EPC paging.

\subsection{Control-Plane}

The control-plane serves as a supervisor of \name's trusted part, responsible for interacting with the local operator (i.e. source) and the remote party (i.e. destination) securely. Once the SGX enclave is launched by the operator, it runs remote attestation to ensure the destination that the enclave is established on a trusted CPU. After the trust establishment, An end-to-end secure channel connecting to the destination is created. The secure channel protects the destination's participation in policy composition with the sensitive information (i.e. private policy) securely provisioned. In the end of the policy composition, the composed policy is used to configure the classifier and the token bucket operations in the data-plane.


\paragraph{Remote attestation}. In order to prove to the destination that an untampered \name is running on an SGX-supported CPU, a \textit{quote} is generated by the SGX platform service and delivered to the destination for verification. The destination contacts the Intel Attestation Service (IAS) to verify the signature of the quote using Intel Enhanced Privacy ID (EPID). Once the signature verification is passed, the content in the quote, including the platform state and the enclave information, can be trusted by the destination. 

\paragraph{Secure channel}. As a building block, the remote attestation is suitable for bootstrapping the secure channel establishment, which performs 3-way handshake to setup the TLS session. The first handshake message is piggybacked on the quote sent to the destination, and the rest of handshake and the key exchange is done afterwards.

\subsection{Data-Plane}

The data-plane follows a pipeline model consisting of three threads inside enclave, a \textit{RX thread}, a \textit{rate-limiter thread}, and a \textit{TX thread}.
Three enclave threads run on individual CPU cores and the packets are passed between cores via DPDK lockless rings. 
The entire flow of packet processing in \name is split into three threads, and every thread runs a small loop polling the hardware or software buffer in the previous stage, processes a batch of the packets, and passes it on to next stage in the pipeline. 

\paragraph{RX thread}. The main tasks of RX thread include receiving the packets from the NIC receive queues and making the secure copy of the header fields for each packet in preparation for future usage in the enclave. With the header securely copied, the input logger can effectively update the per-source-IP counter using count-min sketch algorithm and the classifier will also pre-compute classification result (i.e., traffic class) to release the burden of the rate-limiter thread.

\paragraph{rate-limiter thread}. We adapt the DPDK's \code{qos\_sched} framework to satisfy the our requirement on functionality. We further simplifies the hierarchical token bucket of 5 levels to a simple two-level hierarchy. It supports up to 1024 traffic classes (or queues) with the underlying token bucket runtime parameters properly stored in a cache-friendly manner for fastest retrieving and updating. The time source, CPU TSC timestamp, originally used by \code{qos\_sched} for high-resolution rate calculation is not considered safe given the architectural limitation of SGX. Thus, we use the trusted but coarse-grained time source \code{sgx\_get\_trusted\_time} from SGX SDK as an additional time source to monitor and detect any attempt of clock time modification.

\paragraph{TX thread}. There are two software rings the TX thread needs to accept the packet references from, the \code{tx\_ring} for packets to be forwarded and the \code{drop\_ring} for the packets to be dropped. Either of them marks the end of the packet lifetime within the enclave, so the space used for the secure header copy is recycled to the enclave memory. However, the packet is treated differently according to the rate limiter decision. For the packets to be dropped, DPDK runtime frees the memory of the packet (by reference). For other packets to be forwarded, the output logger updates the per-traffic-class counter and passes the packets to DPDK runtime for transmitting via the NIC.

\subsection{Optimizations}

In the current implementation, we deploy several optimizations to further increase the throughput performance towards the line-rate packet processing. These optimizations reduce the overhead brought by the architectural limitation from SGX, such as the EPC size restriction, the MME operation overhead and the context switch overhead between secure/insecure worlds.

\paragraph{Avoiding EPC paging.}
Depending on the BIOS setting, the isolated secure memory (i.e., EPC) has a fixed size of 64 MB or 128 MB. Except the memory used by SGX SDK, the maximum available EPC for \name instances is approximately 92 MB~\cite{brenner2016securekeeper}. On Linux platform, the SGX can provide larger EPC with the help of paging support from kernel. We carefully control the heap memory usage to reduce the chance of paging and eventually achieve less than 68 MB enclave memory usage.

\paragraph{Reducing the number of context switches.}
The overhead of context switches comes from the saving and restoring of the execution environment (i.e., registers) between trusted and untrusted modes, which slows down the code paths for per-packet processing. In the RX and TX threads, we use batch processing to amortize the cost of one context switch among a number of packets, effectively reducing the overhead imposed by per-packet processing. In the rate-limiter thread where OCALLs are made for CPU timestamps, we also reduce the frequency of invocation  of the time stamps with a reasonable sacrifice of the accuracy of token bucket operations.

\paragraph{Increasing the cache locality.}
The rate-limiter thread runs the highly optimized code that carefully aligns the memory access to the cache line size and pre-fetches the data structures to hide the cache miss penalty. We defer the OCALL of any packet memory operation (mostly free operation for the dropped packets) to the TX thread to avoid disturbing the cache owned by the CPU that runs the rate-limiter thread. This also offers another benefits as the TX thread also focuses on the packet memory operation and has a better cache locality over the packet memory pool.

% \subsection{SGX Primer}
% \label{subsec:sgx-primer}

% Intel SGX is an ISA extension aiming to offer trusted execution environment without relying on dedicated hardwares except the CPU pakcage itself. It transparently create an {\em isolated} memory region, called \textit{enclave}, consisiting of Enclave Page Cache (EPC) and protected by Memory Encryption Engine (MEE), in which the confidentiality and the integrity of the code and the data are guaranteed. It supports enclave execution at user-level privilege and prohibits any other user-mode program or privilege mode (e.g., operating system or OS) from accessing its EPC. SGX also prevents hardware access attempts such as memory bus snooping and monitoring. Moreover, serving as a root trust from CPU package, it allows secure measurements of all the loaded EPC memory, ensuring an unmodified booting stage with verified code and data, which is usually called \textit{attestation}.

% In SGX application design, the application code is divided and placed into the enclave memory region or untrusted memory region, depending on the security requirements of different functions. The interactions between trusted code and untrusted code are recongized as \textit{ECALL} and \textit{OCALL}, where ECALL denotes the untrusted codes calling the trusted ones, and vice versa for OCALL. Both of them require a context switch at CPU level, involving saving and restoring of internal states, and sometimes checking of the passed parameters.

% In our \name implementation, SGX 
% (1) protects sensitive system parameters, such as input filtering policies, the composite policy, or rate-limiting configurations, from direct, unauthorized access and modification by a malicious OS; and
% (2) prevents the operation of \name from being modified by a malicious OS and allows remote third parties to attest the verified version of \name codes. 
%:
%(1) The policy from source, destination or the composed one cannot be read by any unauthroized entities via either software acessses or hardware tappings; (2) The same set of policy and the code of middlebox function cannot be modified by any others in terms of subverting the rate-limiting decisions or creating advantages in leaking any targeted information. (3) The users can be assured that the enclave executes a verified version of code since its lifetime and any modification to the binary before running will not deceive the users into interacting with a untrusted version, and thus leaking information.

%In spite of the advantages a SGX-enabled middlebox can enjoy, there are also a few unpleasant things it faces. The availability of the middlebox can be largely affected by any Denial-of-Service attacks as the underlying OS is not controlled by the middlebox. However, in our service model, the platform contracts closely with the victim flooded by traffic and the victim expects to see the policed traffic transmitted within a secure tunnel, thus rendering any DoS attacks visible directly to the victim.

%\subsection{Baseline design using SGX}
%We first present a baseline \name design with SGX as a simple but realistic design point for general middlebox design using SGX.
%First, all of its control-plane functions (e.g., policy composition $\phi$) are implemented completely within the SGX enclave to protect their sensitive data and code.
%Second, the core, sensitive data-plane operations, such as the classification function, the parallel rate limiters, and the packet encryption function, are also implemented in the enclave for secure operations.
%Third, all user data packets are copied into the enclave because they need to be securely processed (e.g., classified, rate-limited, dropped/forwarded) within the enclave.

%to highlight the challenges 
%Consider a simple implementation of rate-limiting for different classes of traffic, two strategies are immediately realized: (1) In order to hide the fact about dropping individual packets, the survived packets are retrived into TEE and encryption is done in the trusted memory; (2) The multi-class rate-limiting are supported by naturaly running indepedent rate-limiting algorithm (i.e., token bucket algorithm) for each class. Note that the first strategy has been used in Slick\cite{?}, where only the packets that are necessary for further sensitive processing are copied into SGX enclave, which also serves as a performance optimization for avoiding uncessary costly operations (such as packet copying).

%\subsection{Security/Performance Dilemma}
%Our \name implementation has desired security and performance properties.
%In particular, the rate limiting operations should not be tampered with and accessed by a malicious operator of the middlebox.
%This security property is achieved through the careful data flow design with the SGX features; e.g., any sensitive operation is executed within the SGX enclave. 
%Also, line-rate (e.g., 10 Gbps) packet processing is desired since our middlebox is most useful when it can handle and rate limit overwhelming incoming traffic volume. 
%
%In our baseline design, however, we immediately face a {\em security/performance dilemma}. That is, it seems nearly impossible to achieve the strong security for the data-plane operations of \name while processing packets at line rate (e.g., 10 Gbps). 
%The main challenge arises from the two very different (thus conflicting) packet processing requirements for the SGX support (for security) and the DPDK support (for performance). 
%On one hand, for secure packet processing operations (e.g., rate limiting functions, packet encryption), all the incoming data packets {\em must be copied} into the enclave. 
%Note that we cannot selectively copy only a subset of data packets (e.g., only the packets that will be ultimately forwarded to $D$) into the enclave since such memory access behaviors will leak the rate-limiting patterns to the malicious operator. 
%On the other hand, high-performance packet processing in commodity hardware, such as DPDK~\cite{DPDK} or netmap~\cite{netmap}, requires the \textit{zero-copy} memory optimization.
%That is, our middlebox should {\em not make copies} of incoming data packets for line-rate processing.
%Unfortunately, it appears to be challenging satisfy the two conflicting packet copy policies.

% \subsection{Near Zero-Copy Implementation with SGX}
% \label{subsec:our-approach}

% \begin{itemize}
% 	\item Per-class byte counter --- for outgoing packets
% 	\item Count-min sketch --- for incoming packets
% \end{itemize}

%Our approach to implement a secure, line-rate \name middlebox is simple. We decide to support {\em only} authenticity to our data-plane operations but {no} confidentiality, which makes us to maintain our data-plane operations {\em nearly zero copy}, thus achieving line-rate performance. 
%This seemingly a significant sacrifice on the security of the data-plane operations, however, is in fact OKAY. 
%The main reasons are as follows:
%First, offering data-plane confidentiality is not sufficient to address the data-plane side-channel attacks. There are other ways (e.g., probe packets) to infer data-plane operations. It seems it is impossible to remove the side channel anyway. 
%Second, lack of data-plane confidentiality does not reveal the data-plane operations immediately but still requires non-trivial attack cost. For example, comparing incoming/outgoing packets to/from the middlebox requires high performance deep packet inspection, which is not significantly cheaper than other inevitable (or unstoppable) attacks (e.g., probe packets and return packet analysis).
%Third, an authentication mechanism, particularly MAC tagging over packet headers, is sufficient to make the middlebox's data-plane operations {\em non-bypassable} for any packet from $S$ to $D$. 

%\subsection{Non-bypassable data-plane operations}
%
%Non-bypassability requires preventions for three violations (1) packet injection (via replaying tags), (2) packet deletion (via dropping tagged packet), and (3) packet pre-filtering,
%
%\textbf{Header-only MAC}. To support near zero-copy processing, for every packet, the middlebox only reads and copies the packet header, inspecting the most representive metadata, which describe the {\em uniqueness} and {\em shape} of a packet. Hence, with a MAC tag calculated over the header, packet's shape (i.e., length) is bound to a unqiue packet header, eventually ensuring the overall traffic volume, regardless of the content being delivered. This MAC tag also servers as a secure token, any packet injection without MAC can be detected immediately at the receiver side.
%
%\textbf{One-time HMAC}. It is possible that the adversary reuse a generated MAC tag and inject arbritary-content packet with same length into the link. This may work because the 'shape' is same and the packet uniqueness is not good enough (Since we admit that benigh packets may have exact same header). Luckily, this can be prevented by using one-time HMAC. Internally, the middlebox maintains a counter $C$ to record the number of passed packets. Every MAC tag now is calculated by $HMAC(k, c)$, where $k$ is the secret key, $c$ is the current counter value and , $HMAC(\cdot)$ is keyed-hash-based MAC. This largely improves the uniqueness of every passed packet, thus making the MAC tag replay-resistant against packet injection attacks. Additionally, the internal counter can be used to detect packet deletion since the counter value can be synced to the victim out of band periodically. 
%
%\textbf{Packet logging and witness querying}. To prevent packet pre-filtering, the traffic removal done by the malicious source beforehand, the middlebox uses bloom filter to record each incoming packet header and answer the query of witnessing a packet header with a tolerable false postive rate (can be kept as low as possible). Two parallel running bloom filters are used (See Fig.~\ref{fig:packet-log}, each of which will be on (accept insertion) for a period of $T$ and off (stop and reset) for a period of $S$ repeatedly. The difference is one bloom filter's schedule is always behind the other one by $D$, where $D = (S + T) / 2$. At any time, the arrived packet header will be logged either in the only active bloom filter, or the one has longer remaining lifetime. This guarantees that each evidence is kept in one of the bloom filter and will be queryable for at least a period of $D$. This machansim is the realization that the evidence should not be kept forever due to enclave memory limit, however a reasonable query window for each packet is necessary.

%\begin{figure}[!bt]
%\centering
%\includegraphics[width=0.7\columnwidth]{figures/bloomfilter}
%\caption{Packet logging with two overlapped bloom filters}
%\label{fig:packet-log}
%\end{figure}


% HMAC(K, C)

% --------------------------------
% | IP Header | TCP Header | MAC |
% --------------------------------
%
%
% - non-bypassability requires (1) prevention for packet injection (via replaying tags), (2) packet removal, (3) packet pre-filtering. 


%Second, SGX-based applications often involve frequent switching between the trusted and untrusted components, which indeed incurs significant amount of context switches. 
%Our threat model poses challenges on the design of a secure middlebox, even when TEE technology like Intel SGX is adopted. We will discuss these challenges separately, with further realization of the adversary's capabilities and the strengths and limitations in either a generic TEE or a specific one, Intel SGX.

%\subsubsection{Data-plane side-channel information}
%Although a malicious OS that hosts $M(S,D)$ cannot directly access the composite policy $P_{S,D}$, it can observe and even manipulate its data-plane operations: the OS can read, write, and inject any incoming packets to $M(S,D)$ because the input data packets (unlike cryptographically authenticated policy inputs $P_S$ and $P_D$) are unauthenticated, any Internet traffic from source hosts behind the ISP $S$; the OS cannot even read the outgoing packets from $M(S,D)$ due to per-packet encryption performed by $M(S,D)$ but it can still read the aggregate volume of the outgoing traffic.
%
%The baseline design has two realistic side-channel attacks. 
%First, the adversary can monitor the memory access pattern, thus revealing which packets are copied into the enclave for trusted operations, which eventually reveal the set of packet being allowed or dropped. 
%Second, the adversary can monitor the behavior of a rate limiter for a particular traffic class and infer the rate-limiting parameters (e.g., the average rate and burst size of a token bucket)~\cite{sigcomm-16-paper?} and use it to infer the composite policy $P_{S,D}$ indirectly. For the inference, the adversary can carefully craft the input to effectively test a single rate limiter and observe the output volume (even encrypted).

%\subsubsection{Line rate support with secure packet processing} 
%Line-rate (e.g., 10 Gbps) packet processing is necessary since our middlebox is most useful when there exist overwhelming incoming traffic volume. 
%High-performance packet processing in commodity hardware has been widely discussed and developed recently~\cite{DPDK,netmap}.
%In general, line-rate packet processing relies on the two optimization techniques: \textit{zero context switch} (i.e., eliminating unnecessary switches between user and kernel modes) and \textit{zero copy} (i.e., eliminating file copies from the kernel to user space). 
%Unfortunately, it appears to be challenging to achieve the two optimizations when the majority of packet processing must be securely conducted with the SGX support.
%First, for some secure packet processing operations (e.g., packet encryption), a non-negligible percentage of data packets must be copied into the enclave, which violates the zero-copy principle and results in significant data-rate loss.
%Second, SGX-based applications often involve frequent switching between the trusted and untrusted components, which indeed incurs significant amount of context switches. 
%By design, it is not straightforward to minimize the context switching overhead since there is no easy way to split the application as the trusted part versus the untrusted part.

%From Section~\ref{} to Section~\ref{}, we highlight the \name middlebox's main security and performance features. 

% \subsection{Secure packet filtering architecture}

% The baseline design is subject to source's memory inspection on which packets are copied. To simply overcome this, we will simply copy all the packets, regardless of dropping or passing decision made by the rate-limiter, and only encrypt the non-filtered packets inside the enclave. The to-be-dropped packets, although having an excess copy, will neither be encrypted nor occupy the limited memory space inside enclave. The space used for accomplishing the covering copy will be immediately reclaimed and reused as a free space. Ideally, the space wasted on the extra copies is temporary and will only incur one waste of the packet size if only one extra copy is maded at the same time.

% (a figure of overview goes here)
% \subsection{Work-conserving rate-limiters}

% In the baseline design the traffic rate set for a individual rate-limiter can be easily inferred by a malicous source testing the target rate-limiter and observing the volume of encrypted output. By repeating this step, the source learned the parameters for every class's rate-limiter. To overcome this drawback, we enable work-conserving rate-limiting which saturates the output link and keep the overall output volume at a const number.

% This work-conserving mechanism is implemented by allowing token borrowing among different token bucket. The principle is that once any rate-limiter is not consuming any tokens (giving pass decision to the packets), the unused tokens are immediately borrowed by any other working rate-limiters. To ensure fairness, we redistribute these unused tokens with a global view on the working set of rate-limiters. For example, for a system with $n$-class rate-limiters having token refill rates as $r_1$, $r_2$, ... ,$r_n$ respectively, if any time a rate-limiter $u$ is not consuming its $r_u$ tokens per a unit time (say it consume at $r'_u$), these $r_u - r'_u$ tokens are prorated over other running rate-limiters. So a certain working rate-limiter $w$ will obtain $\frac{r_w}{L - r_u} (r_u - r'_u)$ bonus tokens per unit time, where $L$ is the total traffic limit predefined and is the sum of all $r_i$.

% The above work-conserving mechanism applies on any number of underused rate-limiters, which gives us a gurantee that the output volume is constant whenever \name is enabled. Note that \name's activatin condition is when the input traffic exceeds the predefined rate $L$.

% \subsection{Context-switch reducing with SGX}

% To fully respect the lesson learned from zero context switch, we reduce the number of OCALL and ECALL at two dimension in the data-plane: First, the number of designed interfaces for OCALL and ECALL are reduced; Second, the number of invocations on OCALL and ECALL are minimized;

% In data-plane, the only heavily invoked OCALLs are two functions that interacts with the DPDK Poll Mode Driver for network cards, one OCALL asks the driver to receive a batch of packets from physical port, store them in untrusted memory pool, and hand over a list of references (pointers) to enclave, and the other OCALL does similar processes but in a reverse order to inform the driver to transmit the non-filtered packets (in encryption form).

% We fully utilize the benefits of enclave code directly accessing the untrusted memory. Unlike OCALL and ECALL, these accesses are by design allowed by SGX and have no overhead of context switch because the entire virtual memory space (untrusted memory region and enclave memory region) of the process is transparently acessible to enclave code (note that it is not true for untrusted code). In this way, the enclave code and the untrusted code are communicate and synchronize with each other via memory sharing, cutting the potential overhead if OCALL and ECALL are used for communcation.

% \subsection{Scaling \name for 100s Gbps rate}

% \begin{itemize}
% 	\item How to make an array of \name instances to support 100s Gbps rate?
% 	\item How to check biased load balancer efficiently?
% \end{itemize}

% \subsection{Scaling-out for line rate support}

% With the restriction on SGX resources (at most 4 physical cores for Intel SGX CPU, at most roughtly 94MB EPC shared by all enclaves on one machine), achieving line-rate packet filtering on one single machine seems unrealistic, given that the baseline design already requires a lot of copy (memory-consuming) and encryption (both memory-consuming and CPU-consuming). Hence, we propose a scale-out solution that leverages multiple SGX machines and load-balances the incoming line-rate traffic so that the SGX middlebox cluster can still meet the processing requirement and preserve the privacy guarantees achieved on a single SGX middlebox.

% Assume the data-plane on a single machine can only support the processing of input traffic rate at $X$. this suggests that we should duplicate the same configuration of middlebox by $\lceil \frac{I}{X} \rceil$, if the real input traffic rate is $I$. This simple replication relies on the infrastructure's cooperation on offering a fair load-balancer, which may be unsafe to assume since the adversary tends to manipulate the balancing mechanism to gain advantages when conducting traffic manipulation attacks.

% TODO(Deli: not finished yet)

% Therefore, a SGX middlebox should be deployed to load-balance the traffic fairly and randomly, in order to support this scaling scheme. The load-balancer (LB) middlebox will 

% \subsection{Effective and secure accountable enclave}

% From a network persepective, our proposed solution is simply dropping the excess traffic, which will have side affect of interrupting the normal users's communication. This can be exploited by a source adversary since she will be able to filter the packets in advance and shift the blame of packet loss to the middlebox. To overcome this, we implement an effective packet logging mechanism and query service to the system. The former one saves the fact of witness of individual packets in the inbound traffic, while the latter one offers an interface to the users, answering the request about the witness of certain packet. 

% Running a full-fledged packet logging database is impossible as per the discussion of restrictions of SGX. In instead, we will use bloom filter for such packet occurrence test, which is both time-efficient and space-efficient. The false positives brought by this is acceptable because (1) false positive rate can be controlled by many known solutions \cite{X} (2) false positives are not exploitable by the adversary who wants to pre-filter a specific class of traffic.

% To be specific, a bloom filter will insert every packet (whole content) once it arrives and after a period of time the bloom filter is discarded and refreshed as the evidence of witnessing the individual packet doesn't need to be kept for a long time. But if we naively peridically refresh one bloom filter, the lifetime of the evidence vary from zero to the refresh cycle. To have a lower bound of the evidence lifetime for every packets, we can have two carefully overlapped bloom filter, each of them will be alive and accept insertions for a period of $T$ and will then be offline and cleared for a period of $S$. The start time of alive period for two bloom filters has a gap time of $D = (T + S) / 2$. This ensures any evidence is queryable during a lifetime between $D$ and $T$.

%             T                S                 T
% |----------------------|          |----------------------|
% <-----  D  ----->               
%                  |----------------------|          |----------------------|
%                              T                 S                T


% T - D + T + S = D + T

% 2D = T + S
% D = (T + S) / 2

% \subsection{Non-bypassable tagging}

% The encryption for every passed packets (the ones not dropped by rate-limiter) apparently violates the zero-copy principle, and in fact it brings two additional full-packet copy operations for each passed one, of which one is copying plaintext packet from untrusted memory into the enclave and the other one is copying the encrypted packet from the enclave to the untrusted memory. These copies are unavoidable because the encryption has to be done inside the enclave in order to protect the encryption key and the information we want to hide.

% Behind the huge overhead brought by the encryption, the protection we mostly want is hiding the dropping decision made for each individual packet. If we choose to compromise on this and this information is no longer protected, the encryption would immediately become an overkill for providing the other secure properties we originally wanted, which are:

% \begin{itemize}
%     \item P1. bounded overall traffic rate
%     \item P2. bounded traffic rate for each traffic class, if per-class rate-limiter are all saturated.
%     \item P3. Fairness of the work-conserving mechansim        
% \end{itemize}

% It is worth noting that all these properties are more closely relatd to integrity of the decision made by middlebox, which is about the policy enforcement of the traffic class (packet classification) and traffic rate (packet length). A closer look on the rate-limiting function reveals that the decision making process only needs to read the packet header for the purpose of classifying the packet and calculating the tokens consumed.

% We also notice that there is no strong need for confidentiality, if we choose to compromise the protection on dropping decisions. Another supportive observation is that the packet content, which is usually considered confidential, is anyway accessible by the adversary in our threat model. In fact, the adversary is even free to manipulate any bit of the packet sent to the middlebox.

% So far, the initial realization is that, in this fierce environment where a strong adversary controls the input traffic, the most realistic claim we can make is ..

% Based on the understanding that the dropping information can be revealed, we will show a more cost-effecient way to only protect the integrity of the essential parts. This lightweight \textit{secure sketching} technique essentially find a way to let the victim detect any violation of the aforementioned integrity properties. At high-level, the middlebox periodically makes sketchs of the headers of the output packets and sync them with the victim in a out-of-band secure channel so that the victim can be aware of the following violations:

% Now, we will show that, a secure sketching mechanism can make the same claim in a more cost-efficient way, if we no longer protect the true/false information of packet dropping.

% To get rid of the huge overhead brought by IPsec encryption, which actually is an overkill for hiding the information of dropping decision on individual packets, we first admit that the source adversary is so powerful even with the output encryption enabled, and then we consider dropping this heavy defense and think about other lightweight mechansim. A immediate first thought is, this lightweight mechansim still needs to provide certain security property, although it is not comparable to a full encryption.

% As a traffic removal application, one utility goal from the victim's view is to lower the traffic rate coming from the source ISP to a bound (say $L$). Another goal is since the rate-limiter has already shaped the traffic according to the composed policy, the traffic shape should not be influenced by the attacker in any way after the processing.

% Note that the rate-limiter only checks the packet header to classify and make the passing/dropping decision. This checks involves two things: (1) class definition, and (2) packet size, where the class definition decides which class-level rate-limiter should be queried for this ongoing packet, and the packet size affects the number of tokens to be consumed if the packets is allowed. Both of them influence the final shape of the traffic in terms of the volume distribution among different class, which is specified in the composed policy and should be enforced.

% Our secure tag is used as a certificated pass for the packet under the specific class and with specific size. This pass should not be either discarded by the attacker to decrease the volume, or abused by the attacker to increase the volume. This secure tag ensures the integrity of the shape for individual packets, eventually guaranteeing the integrity of the shape for the overall traffic.

% (1) what is tagging idea, (2) what security property it provides (e.g., only integrity on partial bits of packets), (3) why this limited integrity property and lack of confidentiality is okay for our application.

% First, the secure sketching can be used to detect insertion and deletion of tags.

% Second, we have to show that 

==> chapters/inflation.tex <==
\section{Open Inter-ISP Filtering Market: Economic Incentive}
\label{sec:econ-incentive}
%\section{Handling Billing Inflation}

We argue that in addition to the non-economic incentive, it is necessary to provide economic incentives to source ISPs with direct fungible payment from $D$ to $S$. 
First, without a payment mechanism, the source-end filtering service by $S$ can be exploited. For example, even when it is not under attack $D$ may attempt to save its operating cost by asking the packet filtering operations to $S$. Since $S$ in general cannot verify the necessity of packet filtering (e.g., existence of attacks), such exploitation is hard to detect. Thus, direct payment scheme can be an effective deterrence mechanism for such exploitation.
Second, if $S$ receives multiple \name requests from multiple destination ISPs, it needs to carefully determine how to use its limited filtering capability. The payment scheme with negotiable pricing can make \name further increase the economic incentive for $S$ (since $S$ can ask for higher pricing) while more efficiently using its limited resource (since more desperate destinations will use the filtering service).

To remove any additional trusted third party and flexible payment schemes, we propose to use Ethereum smart contracts. This generates the permanent, immutable records of \name services on the Ethereum blockchain. 
Such high level of transparency of \name services in the public domain naturally generates an open inter-ISP filtering market since all the pricing and the results are publicly available. As a result, the reasonable market prices may naturally emerge. Also, misbehaviors can be deterred as misbehaving ISPs are easily recognized in the immutable records. 

\subsection{Flexible payment scheme from $D$ to $S$}

- Protocol figure. 

\paragraph{Proof of contracted work.}

- SGX based proof of contracted work

\paragraph{\name contract.}

- Details… 

\paragraph{Verification and payout.}

\subsection{Transparency and inflation deterrence}

- Impose limits to handle inflation attacks. 

- Transparency: untampered, permanent record of contracts and their 
results. Can create reputation. Can deter inflation attacks. 

\subsection{Economic Analysis}

- Incentive for good behavior. Disincentive for misbehavior. 

- How???? Refer to IKP paper's analysis?

\subsection{Privacy (move to Discussion)?}

Tradeoff? 


------- OLD --------

\msk{\name provides accountable billing, which guarantees correct bandwidth measurement. This establishes a strong economic incentive to source ASes. }

\msk{However, a source AS is able to inflate the bill by creating dummy packets to the \name system. }

\msk{We need to answer to ``how can we handle the bandwidth inflation attacks?''}

- we up front admit that this is an open problem. It is equivalent to S launching DDoS attacks to increae the billing. As long as the cost of generating traffic is lower than the economic reward expected for the increase traffic, there is incentive to launch this attack. 

- In the worst case, our economic incentive end up encouraging ISPs to increase attack volume (either via poor network security checks or even generating new attack traffic) and get paid. 

- In order to handle this serious issue, we propose multiple layers of defense mechanisms that limits the attacker's advantages and ultimately have strong deterrence effect. 

- the underlying theme is transparency. we make the decision made by S transparent and remain untampered in the permanent public database so that S can be responsible for its own actions. 

- in a broader perspective, we create a healthy market place where p2p bilateral filtering is negotiated with the market agreed price and the contract is publicly available for further healthy and attack deterrence market. 

==> chapters/language.tex <==
\section{Policy Abstraction}
\label{sec:policy-abstraction}
%Intro
%- 
%
%Address space agreement
%- Each ISP provides their IP range (set of prefixes they want to include for traffic filtering -- often known information (e.g., peering website)). via $M$, address space agreement. All agree with the address space $U$.
%
%Traffic class partition 
%- why? not comparable
%
%Policy language: what to do with the traffic classes?
%- expressive range: low to high (binary, rank, weight, guarantee/BE) - some combination also possible.
%- binary: too simple. no fairness.
%- weight: too expressive. thus hard to have privacy. (we rule out noise...)
%- rank: right choice.
%
%Distance function
%- important due to the notion of fairness. Closeness or similarity. Semantic.


%The middlebox $M$ should compose the two policies $P_s$ and $P_d$ fairly (thus
%incentivizing the two untrusted parties) and at the same time should limit the
%amount of policy leakage (to the other party) to a certain degree.  In this
%section, we describe the problem space we deal with in the policy composition.
%We will first offer intuitive illustration why there exist an inherent
%trade-off between fairness and privacy in our composition problem.  Then, we
%will discuss the expressive policy languages we may consider for filtering
%policies and corresponding distance definitions. 

%\subsection{Trade-off Between Fairness \& Privacy}
%Intuitively, there is an inherent trade-off between fairness and privacy.
%
%Let us first consider a composition that only aims to maximize the fairness
%metric.  Fairness between two different policies can be interpreted as finding
%a middle point between the two given policy points in the entire policy space,
%which is more clearly defined later.  In other words, the {\em fair} composite
%policy should be equally distanced (the notion of distance is also clearly
%defined later) from the two policies.  Thus, when one policy (either $P_s$ or
%$P_d$) and a middle point ($P_{s,d}$) is given, one can narrow down a number of
%potential the other policies with high accuracy.  This shows that achieving
%fairness naturally undermines the privacy of the other party's policy.
%
%Conversely, a composition that maximizes the privacy metric exclusively
%significantly reduces the fairness.  The strongest privacy implies that when
%one party's policy and the composite policy are given, any possible policy of
%the other party is nearly equally probable.  Indeed, under such strong privacy,
%any extremely unfair composite policy should be allowed since it should be
%equally probable.




%Address space agreement
%- Each ISP provides their IP range (set of prefixes they want to include for traffic filtering -- often known information (e.g., peering website)). via $M$, address space agreement. All agree with the address space $U$.
\subsection{Address space agreement}
Two ISPs $S$ and $D$ first exchange their own IP address spaces that they want
to include for the packet filtering policy composition via the \codename
middlebox.  The ISPs may want to include some or all IP prefixes they directly
own or their direct customers own, which can be verifiable via Resource Public
Key Infrastructure (RPKI)~\cite{rpki}.  The source IP address space determined
by $S$ and the destination IP address space set by $D$ are then combined to
constitute the address space, called $U$, for the policies $P_S$ and $P_D$. 

%Traffic class partition 
%- why? not comparable

%Policy expressiveness (or languages): what to do with the traffic classes?
%- expressive range: low to high (binary, rank, weight, guarantee/BE) - some combination also possible.
%- binary: too simple. no fairness.
%- weight: too expressive. thus hard to have privacy. (we rule out noise...)
%- rank: right choice.
\subsection{Policy Languages}
How one describes and interprets the traffic filtering/policing actions for
defined traffic classes is defined by policy languages.  Two ISPs $S$ and $D$,
and the \codename middlebox $M(S,D)$ must agree on a certain language so that
the actions defined by the ISPs are correctly interpreted by $M(S,D)$.  We can
categorize policy languages by their expressiveness as follows (from the lowest
to higher expressiveness):
\begin{enumerate}
\item {\em Binary allow/block} :ISPs determine whether to allow or drop each
traffic class. This simplest language is easy to use and often expressive
enough to filter out suspicious attack traffic and protect prioritized traffic
classes.  
\item {\em Ranks}: ISPs order traffic classes based on priority and
assign ranks to them. This language is more expressive than the binary one as
it can prioritize among two or more traffic classes.
\item {\em Weights}: ISPs assign normalized weights to traffic classes. This is
more expressive than ranks as it can express fine-grained relative priority
among traffic classes.  
\item {\em Guaranteed bandwidth}: ISPs explicitly
assign desired minimum bandwidth guarantees for traffic classes. This allows
strong bandwidth guarantees to some high-priority traffic classes regardless of
other competing traffic flows. 
\end{enumerate}
These languages can be used in combination (e.g., some traffic classes are
given priority ranks while others are blocked) but for the simplicity of
discussion we do not consider such combinations.  With the above policy
languages, ISPs may agree to allow total desired maximum rate $L$ bps as well. 

\paragraph{Expressiveness and fairness/privacy.}
As we saw in the examples in Section~\ref{sec:prob}, policy expressiveness
affects the notion of fairness and privacy in policy composition.  On one hand,
as we saw in Example 1 in Section~\ref{sec:prob}, the low expressive binary
decision makes the language hard to be fair without being non-deterministic
because the language is too simple to express the `middle point' of the two
policies when they are different.  Non-deterministic composition makes it fair
but it seriously damages the privacy property of the policy composition.  On
the other hand, as we saw in Example 2 in Section~\ref{sec:prob}, the much
highly expressive language with per-class weights can easily offer fair
composition (e.g., via taking average Euclidean distance of the weights);
however, it is hard to achieve adequate level of policy privacy because the
given composite policy is too accurately calculated and expressed for $P_S$ and
$P_D$ and thus the other party's policy can be accurately inferred. 

%Distance function
%- important due to the notion of fairness. Closeness or similarity. Semantic.
\subsection{Distance functions}
Choosing a good distance metric that captures the notion of closeness or
similarity of two policies is important because the notion of fairness relies
on finding the middle (or equally distant) point of the two policies.  Distance
between two policies, $d(P_x,P_y)$, can be defined depending on the policy
languages.  For example, one can use Euclidean distance with the weights of the
rules.  One can also use non-Euclidean metrics, such as the number of pair-wise
order differences between two ordered priority sets.
%
%\subsection{Two Dimensions: Policy Languages \& Distance Definitions}
%There exist two dimensions in our problem space: policy language and distance
%definition. 
%
%\paragraph{Policy Language.} 
%It captures the requirements that the network operators wish to express through
%the filtering operations.  We can imagine a simple binary rules, more complex
%rules with ordered preference, or even with specific per-flow bandwidth
%restrictions.  Regardless of policy languages, any filtering policy has one or
%more traffic classes.  A {\em traffic class} represents a group of packets that
%are treated with the same filtering configuration; e.g., a five-tuple defined
%flow aggregate.  Let us define $U$ as the entire flow space (i.e., any possible
%five-tuple flow definition) from all address space of $S$ to that of $D$.  Let
%$C_{s}$ and $C_{d}$ denote the traffic-class sets defined by the source ISP $S$
%and the destination ISP $D$, respectively.
%Each traffic-class set is an exact cover of $U$; that is, traffic classes in
%$C_{x}$ are pairwise disjoint and the union of all the traffic classes in
%$C_{x}$ is equal to $U$.  {\bf Some figures might be helpful?}
%
%\paragraph{Distance Function.} 
%Accurate distance function should be defined to analyze the fairness and
%privacy of the policy composition since the two properties are measured by the
%distance between policies.  Distance is a numerical description of how far
%apart the two policies are.  Thus distance functions we use in the policy
%composition should be a generalization of the concept of policy similarity;
%that is, the more similar two policies are the lower distance should be
%assigned.  Distance between two policies, $d(P_x,P_y)$, can be defined
%depending on the policy language used and the context.  For example, one can
%use Euclidean distance with the priority rank of the rules (i.e., $k$ for
%$k$-th prioritized flows).  Or, Euclidean distance can be used with any
%assigned per-flow weights (e.g., bandwidth values).  As non-Euclidean example,
%one can also use the difference metrics (e.g., preference order difference or
%binary rule violations) as the distance metric.

\subsection{Proposed Policy Abstraction}
\label{sec:proposed-policy}
Based on our observation on the language expressiveness and the
fairness/privacy properties, in this paper, we propose to use preference-ranked
traffic classes as our policy language.  We observe in the next section that
the level of expressiveness of this policy language offers a good balance
between the fairness and privacy.  For distance function, we use the Kendall
tau distance that is widely used to measure the similarity between two ranking
lists.  Kentall tau distance is a metric that measures the number of pairwise
inversion between two simple policies; the distance between two simple policy
$A$ and $B$ is given $D_{KT}(A, B) = |\{(i, j) | (i, j) \in A \land (j, i) \in
B \}|$.  The minimal distance is $0$ when they are identical and the maximum
distance is $n (n-1) /2$ when they are complete reversed, where $n$ is the
number of traffic classes. 

In the next section, we present a set of algorithms to achieve fair and private
policy composition with a proposed policy abstraction. 


==> chapters/overview-sigcomm.tex <==
\section{Overview}
\label{sec:overview-sigcomm}
This section describes ...

\subsection{Motivation for Yet Another Source-end Filtering}

%Our focus in this paper is {\em not} on how we can introduce new techniques, negotiation protocol (e.g., \cite{ericsson}), or new Internet architecture for better source-end filtering mitigation. 
%Rather, we aim to make this well-studied technique to really be deployed and accepted by actual network operators and used by ISPs when they are under attacks. 

Our investigation of the history of source-end filtering proposals \cite{x,x,x,x,x,x,x,x,x} has clearly shown that, somewhat surprisingly, no studies consider concrete economic or non-economic incentives for the source networks. 
Considering the inherent lack of any incentive for the source\,---\,they are {\em not} the victims of DDoS attacks\,---\,it is evident that strong incentives (preferably in various forms) are desired and we are motivated to close this gap. 

Our quest for strong incentives for source networks quickly comes to a conclusion that accountable filtering operations are necessary for establishing contracts between two ASes. 
Recent study~\cite{} on the importance of accountability in the inter-domain contracts also motivates us to investigate the accountability property of the source-end filtering operations.
%Yet, no existing studies aim to guarantee accountability against active adversary model.


This work is also highly motivated by the recent advances in high-speed packet processing techniques for commodity server platforms. 
We explore in this paper whether we can achieve multiple Giga b/s or higher filtering performance with only a small number of commodity servers with secure processors. 

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.4\textwidth]{figures/overview.pdf}
	\caption{Overview of source-end filtering with \name.}
	\label{fig:overview}
\end{figure}

\subsection{Threat Model}

We consider two distinct networks: a {\em source} AS $S$, which hosts potential attack sources (e.g., botnets) in its and its customers' networks, and a {\em destination} AS $D$, which suffers volumetric DDoS attacks and experiences severe congestion. 
The two ASes $S$ and $D$ may be indirectly connected through one or more transit ASes. 
We consider that $S$ and $D$ are {\em mutually untrusted}. 
This threat model is realistic because the source and destination ASes may seldom have any direct contract between them especially when they are in different geopolitical regions with no direct business relationship.

The untrusted ASes may wish to {\em tamper} with the operation of the \name system. 
By tampering with the filtering operations, two ASes may implement a filtering policy that is more favorable to themselves.
Or, $S$ may wish to modify the recorded amount of filtered bandwidth to overcharge for the filtering service to $D$. 
$S$ also may want to {\em bypass} the \name's filtering logic outside of the \name system to ignore the per-packet decision made by \name.

Note that $S$ has more attack capabilities than $D$ in general since it is the operator that executes and manages the \name system in its own network infrastructure. 
Particularly, we consider that $S$ can control the software/hardware components of \name and even its privileged software (e.g., operating system). 
Moreover, $S$ has the full control (e.g., read, inject, drop) over all the packets entering/leaving \name. 
On the contrary, the destination $D$ can observe only the packets arriving at its network. 

\paragraph{Scope.}
%During the lifetime of a session for mutual collaboration between two ASes $S$ and $D$, we consider that $D$'s filtering policy may change dynamically to adapt to the incoming DDoS attack traffic and the availability of its network and customers. 

$S$'s modification of the packets from $S$ to $D$ outside of the \name system is out of scope of this paper.
In practice, as a Internet service provider, $S$ can always modify any bits of the packets from $S$ to $D$. 
Our \name is a single network function executed in a small subset of the entire network $S$ and we do not (and also cannot) prevent $S$ from modifying the packets it serves.

We consider that other malicious attack sources may generate {\em IP-spoofed} DDoS traffic with the source IPs under the control of a source AS. 
The proposed \name system handles such IP-spoofed attack traffic by simply distinguishing packets with spoofed source IPs and the ones that actually come from the designated source AS. 


\subsection{Intel SGX Overview}

\msk{how widely available.}

\msk{focus on isolated execution, remote attestation.} 

\msk{threat model}

\msk{we trust IAS}

\subsection{Naive Design}

To apply the security guarantees of Intel SGX to our \name design, we borrow some ideas of building user-level applications using the SGX features with a small trusted computing base (TCB) of a few thousands of lines of code~\cite{panopy,scone,royan}. 
To that end, we present a simple design for the \name application, which we will call a {\em naive} design, that immediately offers several useful security properties and handles many of the attacks launched by $S$. 
%Although our naive design of \name may seem already quite useful for closing the gap between the  ideas and the deployment possiblities of source-end filtering proposals, it has several critical security and performance drawbacks, as we see shortly. 

The idea of the naive design is simple. 
We modularize network functions in both the control-plane and data-plane and encapsulate all of them into an SGX enclave. 
Once the functions are enclaved, the integrity of their executions is guaranteed due to the strong execution and the states isolation of the SGX architecture; e.g., even the privileged operating system cannot read/write the execution of the enclaved functions.
Moreover, the remote attestation of the \name ensures that the correct and untampered functions have been loaded and running on the SGX platform.
% has been loaded and running on the platform ensures that the participating ASes the correct and untampered functions operate the \name's filtering operations. 
The full implementation of \name should be open-sourced to public so that the networking community can scrutinize the codes and any participating ASes can attest before making a contract with other ASes. 



In the naive design, we include the following functions into an SGX enclave.

\paragraph{Control plane:}
\begin{itemize}
	\item Secure channel establishment with ASes {\tt est\_sec\_chan()}
	\item Policy composition {\tt compose\_pol()}
	\item Packet logging export {\tt export\_pkt\_log()}
	\item Billing generation and report {\tt gen\_billing()}
\end{itemize}

\paragraph{Data plane:}
\begin{itemize}
	\item Interpretation of composed policy {\tt read\_comp\_pol()}
	\item Packet classification {\tt classify\_pkt()}
	\item Hierarchical token bucket {\tt htb()}
	\item Packet logging for incoming/outgoing traffic {\tt log\_pkt()}
\end{itemize}

The above contro- and data-plane functions are enclaved and exchange control information with $S$ and $D$ and receive/send data packets from $S$ and to $D$ via a set of special SGX functions (e.g., {\tt ECALL} and {\tt OCALL}) that mediate all the interactions of the enclave. 

Note that in Figure~\ref{fig:overview}, the naive \name design includes trusted third-party payment system. 
The payment system checks the validity of the bills submitted by $S$ and makes the payment to $S$ when the bill is verified. 
It also provides an escrow services to $S$ and $D$ so that they can make payment to each other without mutual trust between them. 
As shown in Figure~\ref{fig:overview}, the Intel Attestation Service (IAS) as the trusted third party of the system that verifies the code integrity.
%and the SGX hardware, which becomes the root of trust of the \name system. 
%(\deli{will check the fact about the role of IAS and how the code integrity is guaranteed})

%Security properties offered by the naive design:
%\begin{itemize}
%	\item {\bf Fair policy composition:}
%	\item {\bf Prevention of direct reading of submitted and composed policies:}
%	\item {\bf Accountable packet filtering decision:}
%	\item {\bf Secure packet logging:}
%\end{itemize}

\subsection{Attacks handled by the Naive Design}

The SGX-based naive design already rules out a number of attacks:

\paragraph{Direct reading and tampering of submitted policies:}
$S$ cannot read or tamper with $D$'s policy \PD because $D$ establishes a secure channel with the \name instance via {\tt est\_sec\_chan()} that is isolated from any non-SGX executions (e.g., OS system calls). 
The policy \PD is sent over the secure channel and becomes available only to the \name's {\tt compose\_pol()} function (which is also enclaved) that receives two policies \PS and \PD from $S$ and $D$, respectively, and composes \PSD.

\paragraph{Direct tampering of policy composition:} 
$S$ cannot directly modify the policy composition logic implemented in the {\tt compose\_pol()} function as the function is enclaved.
It is also open-sourced and thus can be publicly verified to ensure that the policy composition is done in a fair manner (whose definition will be defined and analyzed in Section~\ref{}). 
%Moreover, the SGX's remote attestation allows $D$ to always check that the function has not been modified from the open-sourced codebase.

\paragraph{Direct tampering of policy enforcement:}
Similarly, $S$ cannot tamper with how the composed policy \PSD is enforced in the \name's data-plane because all the related data-plane functions {\tt read\_comp\_pol()}, {\tt classify\_pkt()}, and {\tt htb()} are completely enclaved. 
Once {\tt read\_comp\_pol()} receives \PSD from the enclaved function {\tt compose\_pol()}, it configures the other two enclaved functions {\tt classify\_pkt()} and {\tt htb()} for their traffic class definition update and the token bucket parameter setups. 
For each data-plane incoming packets, {\tt classify\_pkt()} and {\tt htb()} perform the specified multi-class rate-limiting operations and decide allow/drop for each packet within the protected SGX enclave. 

\paragraph{Bypassing \name:} 
$S$ may wish to bypass \name when the decision by it is not aligned with $S$'s preference; e.g., $S$ wants a packet $p$ to be delivered to $D$ but \name drops it. 
In the naive design of \name, $S$ can no longer bypass \name without being detected because \name has the untampered logs of all the incoming/forwarded packets in the enclaved {\tt log\_pkt()}. 
\name periodically sends the secure logs to $D$ via another enclaved function {\tt export\_pkt\_log()} over the secure channel. 
At $D$'s side, it also keeps the logs of packets independently and compares with the secure logs from \name to detect any bypass attempt for any packet by $S$. 

\paragraph{Modification of bandwidth measurement:}
$S$ may wish to modify the measured bandwidth by \name to claim unfairly large amount of billing to $D$ at the end of a filtering cycle. 
This threat is prevented since the packet logging function {\tt log\_pkt()} and the billing generation function {\tt gen\_billing()} are both enclaved and thus modification is prevented. 
Therefore, the naive \name implementation ensures that the bandwidth report attached to the final billing is an accurate measured bandwidth of the packets dropped by \name.

\subsection{Challenges}

Despite its useful security properties, especially the verifiably fair policy composition and secure packet logging, the naive \name design appears to be still vulnerable to attacks that happen {\em outside} of the \name system. 
The naive design guarantees the execution integrity of all of its functions only within the SGX enclave; however, the notions of fairness and accountable packet logging between $S$ and $D$ are in fact completely defined outside of \name.
%Thus, the fairness of policy composition and the accountability of packet logging are guaranteed for the {\em given inputs}, such as the submitted policies and incoming packets.
%However, the design does not guarantee the notions of fairness and measurement accountability that are in fact dependent on the inputs to the \name system. 

Let us first consider the notion of fairness in the source-end filtering problem, which is the fundamental guarantee for the incentive to the source ASes in mutual collaborations. 
The fairness between two ASes $S$ and $D$ should describe the quality of being impartial to $S$ and $D$ in filtering policy decision. 
When the genuine policies (say $GP_S$ and $GP_D$) of $S$ and $D$ and their submitted policies (that is, \PS and \PD) are different, the fairness notion cannot be solely guaranteed by the fairness guarantee within the \name system. 
For example, $S$ may send non-genuine policy (i.e., $GP_S \neq P_S$) to \name in the hope that the composed policy \PSD is close to its genuine policy. 
We illustrate this {\em fairness attack} in more detail in Section~\ref{} and address our defense approach. 

%What is subtle in this definition is the implicit gap between the genuine policies (say $GP_S$ and $GP_D$) of the ASes and their submitted policies (that is, \PS and \PD). 
%The naive design guarantees a fairly composed policy \PSD for the given \PS and \PD but there is no way to guarantee that \PSD is the pair policy for the actual genuine policies $GP_S$ and $GP_D$. 
%Since the genuine policies are converted to the submitted policies outside of the SGX-enclaved functions, \name cannot guarantee this broader notion of fairness. 
%Due to this limitation, a malicious AS can send non-genuine policy to the system in the hope that the composed policy is close to its genuine policy. 
%We illustrate this {\em unfair fairness attack} in more detail in Section~\ref{} and address our defense approach. 

Similarly, the accountable logging property relies on the input traffic to the \name system. 
Therefore, when a source AS $S$ manipulates the input traffic, the accountability of the \name system itself may not necessarily guarantee the accurate traffic measurement. 
In a simple example, if $S$ creates high volume dummy packets for the additional input to \name, then our naive design would perform the filtering operations over the dummy packets and finally report much inflated bandwidth measurement report (and thus higher billing to $D$). 
We describe such {\em bandwidth inflation attack} in more detail in Section~\ref{} and our multi-layered systematic defense approaches. 

Moreover, the additional trusted third party for the economic incentive system may become the bottleneck in practical deployment. 
The trusted third party is essential for the verification of the accountable billing (thus, $S$ cannot forge the billing results) and the escrow service for the payment from $D$ to $S$. 
However, in practice, it might be challenging (if not impossible) to find such mutually trusted party in the Internet. 
$S$ and $D$ may very well be located in different geopolitical environment and they may have different sets of trusted parties as the candidate for this job. 
One may suggest to use one of the existing trusted third party services in the inter-domain Internet, such as RPKI; however, such PKI services are not suitable for active verification and escrow services. 
We address this challenge in Section~\ref{} by removing the need for a trusted third party with some reasonable practical assumptions. 

Lastly, the naive design also would likely suffer significant performance overhead, particularly the filtering rate would be much lower than the maximum line rate that typical high-end network interface card can handle (e.g., 10 Gb/s).
The main challenge stems from the intense per-packet secure processing for the verifiably fair packet filtering ({\tt classify\_pkt()} and {\tt htb()}) and the accountable packet logging ({\tt log\_pkt()}) in the enclaved data plane functions. 
Secure processing of all data packets from $S$ to $D$ in the naive design incurs packet copies from the non-enclave memory to the enclave memory, which incurs tremendous overhead for context switching between the non-secure and secure world. 
Worse yet, the available memory size of the secure world is limited up to 128 MB.
The context switching and the small memory size are known to be the main sources of performance overhead especially for high-speed packet processing. 
We discuss how much performance gain can be achieved with architectural optimization in Section~\ref{}.
%\deli{Another performance degradation comes from the paging of insufficient secure memory inside enclave. It is due to the architectural limitation of current SGX version, which only supports up to 128 MB memory within enclave. So the naive implementation of copying all the packets, meaning over 128MB memory footprint, will triger the OS's secure paging with intolerable overhead.}
 


%
%\msk{Three main remaining challenges:}
%
%\msk{(1) Fairness guarantee can be violated if one party can read other's policy and adjust its policy; }
%	
%\msk{(2) Accountable billing without a trusted third party against active adversaries (e.g., bandwidth inflation attacks); and }
%	
%\msk{(3) data-plane must support line-rate speed but it is hard due to per-packet secure operations.}
%
%\msk{We address each point in the following three sections.} 

==> chapters/payment-channel.tex <==
%\subsection{Payment Channels}
%\label{sec:payment-channel}



\name allows source ISPs to charge fees based on the amount of filtering work (which is measured in the refutable invoice) to destination ISPs.
This offers explicit {\em economic incentives} to ISPs for source filtering defense, thereby removing the reliance on ISPs' altruistic motivations~\cite{mahajan2002controlling,argyraki2005active,liu2008filter}.
For monetary transactions, \name may utilize any existing finance infrastructure (e.g., international banks);  yet, in this paper, we choose to use cryptocurrencies for their fast and easy transactions across different countries. 

\begin{figure}[h]
	\centering
	\includegraphics[width=0.40\textwidth]{figures/payment-channels-bitcoin.pdf}
	\vspace{-5pt}
	\caption{A payment channel that utilizes a blockchain (e.g., Bitcoin) as the escrow for the payment and the verifier of the performed filtering work.}
	\vspace{-5pt}
	\label{fig:payment-channels-bitcoin}
\end{figure}

We present an optimized payment channel design that fully utilizes the SGX's security primitives and thus minimizes the reliance on underlying cryptocurrencies. 
Figure~\ref{fig:payment-channels-bitcoin} illustrates the steps:
\begin{packedenumerate}
\item $D$ establishes a \name contract with $S$.
\item $S$ creates an enclaved filter $E$; $E$ creates a fresh cryptocurrency wallet address {\em Addr$_{E}$} and attaches it to its attestation report.
\item $D$ makes a transaction of $X$ coins from its address {\em Addr$_{D}$} to {\em Addr$_{E}$} with the timed lock $T$~\cite{todd2014bip}. This guarantees that the $X$ coins are returned to {\em Addr$_{D}$} if it is not spent after time $T$. 
\item After the filter task, $E$ calculates the fee $Y$ based on the refutable invoice and the negotiated pricing rate, and makes a transaction {\em TX} that includes $Y$ from {\em Addr$_{E}$} to {\em Addr$_{S}$} (as a payout) and $X-Y$ from {\em Addr$_{E}$} to {\em Addr$_{D}$} (as a return).
\item  $S$ submits the transaction {\em TX} to the blockchain to make the final payment. 
\end{packedenumerate}

Note that this model is {\em scalable} because it requires only two regular transactions that can be supported by virtually any cryptocurrencies. 
Moreover, participating ISPs can be ensured that their source filtering activities and payment history remain {\em private} because their public transactions are indistinguishable from other regular transactions.

%An in-depth discussion on alternative payment channel designs (e.g., use of smart contracts) and their advantages and disadvantages are found in Appendix~\ref{sec:payment-channel-appendix}.


==> chapters/payment.tex <==
\section{\name Contracts}
\label{sec:econ-incentive}
%\section{Handling Billing Inflation}

\paragraph{}

\subsection{Trust Anchors for Trust Bootstrapping}

Building trust between two distrusting ISPs is one of the goals in \name contract. Therefore, given that two ISPs may not have any direct relationships before, well-known trusted third parties can be a good starting point for trust bootstrapping. \name contract relies on two external parties, \textit{Resource Public Key Infrastructure} (RPKI) and \textit{Intel Attestation Service} (IAS) and one internal party TESEF whose trust can be extended by the asymmetric cryptography while only the roots certificate need to be unconditionally trusted.

\paragraph{RPKI}. As a free and world-wide service, it is mainly used for securing the Internet routing. While in \name contract, because of the open environment where most ISPs stay and the urgent situaion victim ISP is facing, RPKI can help ISPs reduce the risk of any possible scams and effectively make contact with other legitimate ones who own Internet IP resources related to the ongoing volumetric attacks. For example, as a victim in DDoS, $D$ certainly has a list of ISPs who are the direct upstream of the malicious hosts or controlled botnets. $S$ may also want to confirm the traffic indeed heads towards $D$ instead of a impersonater who ask for arbitrary filtering service.

\paragraph{IAS}. As an important service of the Intel SGX that complete the trust establishment (remote attestation), Intel Attestation Service is a trusted source that responds to any registered remote party who wants to verify a authentic SGX hardware, and provides a verifiable attestation report for public verification (with its signature published). This report is not only accessible to the challenger but also anyone who has the IAS ceritificate and is able to verify the signature in the attestation report. Note that in our \name system, we assume $S$ is both the platform operator who runs the enclave and service provider who attests the running enclave with IAS so anyone including $D$ can knows the enclave's integrity and authenticity status.

\paragraph{TESEF}. We assume that the \name binary will be publicly available along with its source code and the signature. The process that compiles and links the code into binary is securely runs in a trusted environment, so that the private key signing the enclave is also protected to prevent any malicious code injection. Ths signed binary is also an important step required in the SGX security perimeter, which provides a integrity checksum for the enclave initial state after launch and a signature that identify the true author of the entire building process.  

\subsection{Contract initiation and execution}

The contract is nothing but an agreement that $S$ provides $D$ the filtering service by running \name filter to reduce the traffic rate and $D$ makes the payment accordingly. Figure~\cite{contract} shows the essential interactions between $S$, $D$ and other parties ($E$ for enclave and $I$ for IAS) starting from the first contact made by $D$ to the last step of $E$ making the payment onbehalf of $D$. We will further clarify the details later, but first we discuss the notations we used in this section. 

\paragraph{Notations}. The trust establishment is built on top of the asymmetric keys owned by each of the participants and trusted third parties. We use the following notations for the asymmetric keys and its encrypting and signing to ease the illustration throughout this section.

\begin{enumerate}
    \item $\pKey{X}$, $\sKey{X}$: the public and private keys of $X$.
    \item $\enc{A}{\sKey{X}}$: the plaintext of message $A$ along with $X$'s signature.
    \item $\enc{A}{\pKey{X}}$: the ciphertext of message $A$ encrypted by $X$'s public key.
\end{enumerate}

\begin{algorithm}[H]
\floatname{algorithm}{\name Contract}
\renewcommand{\thealgorithm}{}
\caption{Interactions between $S$, $D$, $E$ and $I$}
% \label{}
\begin{algorithmic}[1]
    \State $\mathrlap{S}\hphantom{D}\leftrightarrows\hphantom{D}\mathllap{D}$ : establish a channel through key exchange
    \State $\mathrlap{S}\hphantom{D}\Leftrightarrow\hphantom{D}\mathllap{D}$ : negotiate the contract $F$, $M$, $L$, $P$, $T$ via the channel
    \State $\mathrlap{S}\hphantom{D}\leftarrow\hphantom{D}\mathllap{E}$ : generate quote $Q = \{H_1, H_2, \pKey{E} \}$ with EPID signature
    \State $\mathrlap{S}\hphantom{D}\rightleftarrows\hphantom{D}\mathllap{I}$ : get attestation report $R = \enc{Q}{\sKey{I}}$
    % \State $\mathrlap{S}\hphantom{D}\leftarrow\hphantom{D}\mathllap{I}$ : reply with the attestation report $R = \enc{Q}{\sKey{I}}$
    \State $\mathrlap{S}\hphantom{D}\rightarrow\hphantom{D}\mathllap{D}$ : forward $R$ to $D$ for proving
    % \State $\mathrlap{E}\hphantom{D}\rightarrow\hphantom{D}\mathllap{D}$ : send the policy $\enc{\enc{P_D}{\sKey{D}}}{\pKey{E}}$
    % \State $D\overset{\$}{\dashrightarrow}\hphantom{D}\mathllap{E}$ : entrust the deposit to $E$
    \State $\mathrlap{S}\hphantom{D} \rightarrow \hphantom{D}\mathllap{E} \leftarrow D$ : send $P_S$, $\enc{\enc{P_D}{\sKey{D}}}{\pKey{E}}$ and deposit to $E$
    % \State $\hphantom{D}\mathllap{E}$: compose $P_S$ and $P_D$ into $P_{S,D}$
    \State $\mathrlap{S}\hphantom{D} \leftarrow \hphantom{D}\mathllap{E} \rightarrow D$ : pay $S$ and refund $D$
    \end{algorithmic}
\end{algorithm} 

\paragraph{Channel establishment}. At the beginning, $D$ attempts to contact $S$ via all possible channels to establish a reliable communication channel. The assumption here is that, even facing serious congestions on the main links, ISPs still have the backup plans to guarantee Internet access for urgent situations. We also consider the correct and effective contact of $S$ are public and accessible via $D$'s available channels. The channel establishment follows standard key exchange protocol using the RPKI asymmetric keys and creates an ephemeral symmetric key for the ongoing session. The usage of RPKI authenticates the legitimate identity of participants in the upcoming contract, avoiding any impersonation attacks.

% D initiates key exchange with S and establishes a secure channel with end-to-end encryption (shared symmetric key) and authentication (R’ asymmetric key)

\paragraph{Contract negotiation}. Through the established channel, $S$ and $D$ have the negotation over the contract content and agree on a set of non-sensitive parameters for filtering, including the following things:

\begin{enumerate}
    \item $\mathbf{F}$: The maximum range of the traffic to be filtered.
    \item $\mathbf{M}$: The maximum inbound rate that counts in the bill.
    \item $\mathbf{L}$: The maximum outbound rate that $F$ should be reduced to.
    \item $\mathbf{P}$: The price that $S$ charges $D$ for the traffic removed.
    \item $\mathbf{T}$: The contract expiration time
\end{enumerate}

% D drafts a filtering contract and negotiates with S regarding the content
% F: IP-to-IP flow being filtered, from S to D.
% M: maximum inbound rate that counts towards the bill
% L: outbound rate that the filter reduce the inbound rate to
% P: price that D pays for the traffic removed

\paragraph{Enclave instantiation} 
While the contract negotation is going, $S$ can choose to start deploying \name binary obtained from reliable public source. The SGX CPU will make a trusted measurement (i.e., \texttt{MRENCLAVE}) in the form of 256-bit SHA-2 hash over the entire loading process to ensure the initial state is not tampered. We denote it as $H_1$. $H_1$ is also checked against a special signature structure (i.e., \texttt{SIGSTRUCT}) provided together with the binary, which is generated by the SGX building toolchain. This signature also contains other useful information (i.e. \texttt{MRSIGNER}, \texttt{ISVPRODID}, and \texttt{ISVSVN}) that can be used to identify the specific binary. These informaion is denoted as $H_2$. We will see how $H_1$ and $H_2$ is used to guarantee the code integrity and authenticity and prove to a remote party $D$ later.

\paragraph{Remote attestation}
$S$ starts the remote attestation by requesting a special \textit{quote} (denoted as $Q$) generated by SGX platform service on the same machine, and signed by an \textit{attestation key} (denoted as $A$) that is only verifiable by Intel. The quote $Q$ includes but not limited to these important fields: $H_1$, $H_2$, and $\pKey{E}$, a fresh public key. The quote is sent to IAS for verification and IAS replies a attestation report $R$ is the signature of the quote is verified. IAS also provides the signature as $\enc{R}{\sKey{I}}$, so any one who knows IAS public key $\pKey{I}$ can verify the signature and believe the content, which contains $Q$ and other information. Remember that $Q$ contains $H_1$, $H_2$ and $\pKey{E}$, which ensures one thing: $E$ is runnning a \name filter from a trusted source and holds the private key $\sKey{E}$ securely inside the enclave.

% $S$ presents the quote in the form of $\enc{H_1, H_2, \pkey{E}}{\sKey{A}}$ 

% S boots up the filter, completes the remote attestation, and forwards the attestation report to D for verification
% S launches E with audited and signed TESEF binary
% S obtains the quote from platform service locally with signature signed by an attestation key using EPID technique. The quote has the following facts
% MRENCLAVE: hash over E’s loading procedure as integrity proof
% <MRSIGNER, ISVPRODID, ISVSVN>: TESEF authorship proof
% (KE: E’s ephemeral key)
% S forwards the quote to I for attestation and gets the attestation report with I’s signature. The report contains the quote, hence extending the trust to the quote
\paragraph{\name filtering}. \deli{S routes F to E to start the filtering, with auditability in control-plane and data-plane}
%control-plane: policy composition
%data-plane: rate-limiting and billing

\paragraph{Payment}.
% D makes a deposit, and provisions PD to E with signed and encrypted message. S also presents PS to E to run the control-plane function - policy composition
%The deposit can be made in all manners, with two necessary properties
%E solely controls the fund during operation time (for sake)
%D regains control of the fund after the operation time (for  sake) 

% \msk{(1) Scalable negotiation (i.e., making contracts with many sources at once) with a single contract transaction. (2) Sub-linear blockchain cost increase. (3) Private filtering policy agreement---bilateral collaboration.}

\subsection{Flexible Entrusted Payment from $D$ to $S$}

\deli{show an example of using bitcoin as the payment scheme}

\deli{compare the cost with other choice}
% When D sends PD secretly to E, it also sends the deposit to E’s wallet immediately if it can be ensured that the deposit will be secured by it again after T. This can be guaranteed by a promised transaction from E to D which the blockchain accepts only the operation lock T expires. 
% Deferred Transaction 1 [promised transaction] E to D nLockTime > current block time + T
% Immediate Transaction 2 [deposit transaction] D to E with the deposit
% [operation lasting for T]
% Immediate Transaction [payment transaction] E pays to S, refunds to D in one transaction, which spends the money before the promised transaction, rendering it invalid.
% If anything goes wrong (E fails to execute, or halts in the middle), the deferred transaction will take effect.


% We argue that in addition to the non-economic incentive, it is necessary to provide economic incentives to source ISPs with direct fungible payment from $D$ to $S$. 
% First, without a payment mechanism, the source-end filtering service by $S$ can be exploited by selfish $D$. For example, even when it is not under attack $D$ may attempt to save its operating cost by asking the packet filtering operations to $S$. Since $S$ in general cannot verify the necessity of packet filtering (e.g., existence of attacks), such exploitation is hard to detect. Direct payment scheme can effectively deter such exploitations.
% Second, if $S$ receives too many \name requests, it needs to carefully determine how it should use its limited filtering capability. The payment scheme with negotiable pricing can make \name further increase the economic incentive for $S$ (since $S$ can ask for higher pricing when there is competition) while more efficiently using its limited resource (since more desperate destinations will use the filtering service).

% To remove any additional trusted third party and implement a flexible payment scheme, we propose to use the Ethereum smart contracts. This generates the permanent, immutable records of \name services on the Ethereum blockchain. 
% Such high level of transparency of \name services in the public domain naturally generates an open inter-ISP filtering market since all the pricing and the results are publicly available. As a result, the reasonable market prices may naturally emerge. Also, misbehaviors can be deterred as misbehaving ISPs are easily recognized in the immutable records. 

% \subsection{Contract creation and participation}

% \paragraph{Notations}
% \begin{enumerate}
%     \item $<\pKey{S}, \sKey{S}>, <\pKey{D}, \sKey{D}>$: The RPKI resource certificate key pairs for $S$ and $D$.
%     \item $<\pKey{E}, \sKey{E}>$: \name enclave's fresh key pair
%     \item $<\pWallet{S}, \sWallet{S}>, <\pWallet{D}, \sWallet{D}>$: The Ethereum wallet address and private key for $S$ and $D$.
% \end{enumerate}

% $D$ first initiates the \name contract on Ethereum blockchain with two main types of information, filtering tasks $F$ for disseminating the filtering requesting and trust anchors $T$ for setting the root of the trust in the future verification. 

% \paragraph{Filtering Tasks $F$}. 
% \begin{enumerate}
%     \item The source IP prefixes that require filtering.    
% \end{enumerate}

% \paragraph{Trust Anchors $T$}.

% \begin{enumerate}    
%     \item The trust anchor for SGX platform attestation verification.
%     \item The information for SGX enclave integrity check. (MRENCLAVE, MRSIGNER, ISVPRODID, ISVSVN)
%     \item $D$'s RPKI resource ceritificate key pair.
% \end{enumerate}

% %Note that $D$'s wallet address $\pWallet{D}$ is also included in the signature to bind the Ethereum wallet identity with the RPKI identity. This  
% The last parameter, the signature on its wallet certify the contract is truly created by $D$, as proved by its RPKI certificate.

% \deli{$\pWallet{D}$ calls \textbf{FilterContract<$F$, $T$, $\enc{\pWallet{D}}{\sKey{D}}$>}}


% \paragraph{\texttt{Join()}}

% Once the contract is created, $S$ can choose to join the contract with enough proof, including its owernship of the specified source IPs, and the evidence of running the \name filter on SGX hardwares. Before making any transaction to the contract, $S$ will first check $D$'s signature over $\pWallet{D}$ to make sure no one impersonates $D$.

% Also, before joining happens, $S$ launchs the \name filter on SGX-enabled CPU, finishes the remote attestation and prepare the attestation report with IAS signature to \name contract.

% Eventually, when making the join() call, $S$ add the following information as parameters

% \begin{enumerate}
%     \item $S$'s RPKI public key
%     \item The attetation report signed by IAS
% \end{enumerate}


% The enclave code contains the following hardecoded trust anchors:

% \begin{enumerate}
%     \item RPKI's root certificate
%     \item S'own RPKI
%     \item D's 
% \end{enumerate}

% \subsection{Negotiation}

% Once both parties join the contract, they can start the negotiation via a series of calls of negotiate(). Each of them take turns to modify the pricing details (e.g. IP ranges, filtering price and contract lasting time) until one of them accepts the plan by sending the same details as confirmation.

% Ideally the negotation can be finished with two calls in total and these call can also be merged with the first two calls creation and joining. This will save a lof time time and gas cost.

% \paragraph{Launching the enclave and publishing the contract.}
% Based on the negotiated parameters, $S$ launches the \name enclave in its computing cluster with the SGX-enabled processors.
% In addition to its core data-plane functions (e.g., rate limiting functions and the packet logging functions), the enclave creates  particularly important local data structures when it is initiated. 
% Then, the enclave creates its {\em own Ethereum wallet} by deriving the wallet address from a randomly generated 256-bit private key\cite{wood2014ethereum}. By creating a fresh wallet within the \name enclave, we greatly simplify the process of verifying the contracted work in the \name contract. 
% we greatly simplify the verification of the \name contract.
% That is, instead of directly verifying the message from the enclave (e.g., bandwidth measurements) in the \name contract (e.g., by contacting the Intel Attestation Service (IAS) and verifying the corresponding signatures), we write the enclave's wallet address into the \name contract when it is published as the prover so that the contract can later verify the work submitted is signed by the enclave.
% the enclave's identity (i.e., the corresponding SGX-enclaved \name instance) is checked  
% Note that this design choice is inspired by the smart contract design for the automated PKI compromise detection system~\cite{matsumoto2017ikp}. 

% \paragraph{Negotiating contract parameters}
% Before creating the smart contract, $D$ first negotiates with $S$ to agree on the contract details as seen in Figure~\ref{lst:contract-code}. In the negotiation stage, $D$ checks if $S$ has the authority to police the traffic from the desired source IPs by checking with the RPKI infrastructure to bind $S$ with the AS number and the RPKI public key, and some publicly available peering databases, such as, PeeringDB\footnote{\url{https://www.peeringdb.com/}}, to confirm that $S$ peers with an AS that owns the IPs. Once they agree on the contract, $D$ first publishes the contract including the agreed details and sends the maximum amount of cryptocurrency (e.g., Ether) it is willing to pay. The contract is created only once and $S$'s wallet address is also attached to the open contract so that $S$ also knows that the contract will make the payment to its address. 

% \subsection{Flexibile payment}

% \paragraph{Paying for rate-limiting work.}
% The rate-limiting work done by the \name is logged in the form of an array of average incoming traffic rate during each reporting cycle (i.e. \texttt{reportCycle}). This proof of contracted work is generated by the \name enclave during the operation periodically, and forwarded to $S$ with the signature after the operation. $S$ then sends the proof along with the enclave's signature to the \name contract in a transaction calling the function \texttt{Submit()}. The function checks the identity of the contractor and verifies the signature of the proof, and eventually pays the contractor ($S$) according to the work approved by the accounting function \texttt{Calculating()}.

% \subsection{Flexible payment scheme from $D$ to $S$}
% \label{sec:payment-scheme}

% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{figures/payment.pdf}
% 	\caption{\name contract for flexible payment from $D$ to $S$.}
% 	\label{fig:payment}
% \end{figure}

% \paragraph{\name contract.}
% This contract involves three independent parties: the \texttt{owner}, who initiates the contract, the \texttt{contractor}, who agrees to work under the contract, and the \texttt{prover}, who is unbiased in the measuring and submitting the proof of contracted work done by the \texttt{contractor}. In \name, the \texttt{owner}, \texttt{contractor} and \texttt{prover} are destination ($D$), source ($S$) and \name enclave ($E$) as illustrated in Figure~\ref{fig:payment}. The contract content has the following variables:

% \begin{itemize}
%     \item \textbf{\texttt{maxInputRate}}: the maximum incoming rate that $D$ accepts.
%     \item \textbf{\texttt{outputRate}}: the eventual traffic rate that $D$ requires.
%     \item \textbf{\texttt{reportCycle}}: the time cycle of one proof report.
%     \item \textbf{\texttt{reportLimit}}: the maximum number of reports allowed.
%     \item \textbf{\texttt{price}}: the price per unit bandwidth per unit time.
% \end{itemize}

% The Listing~\ref{lst:contract-code} outlines the \name contract code written in an Ethereum smart contract language, \textit{Solidty}. It details smart contract constructor function \texttt{RateLimiter()}, called by the owner to initialize the contract, and redemption function \texttt{Submit()}, called by the contractor to submit the proof of contracted work with the prover's signature and get the payback.

% % -\msk{Figure X. \name contract for flexible payment from $D$ to $S$.}
% \label{lst:contract-code}
% \begin{lstlisting}[caption={Smart contract code},captionpos=b]
% contract RateLimiterContract {
%     address public owner; address public prover; address public contractor;
%     uint64 maxInputRate; uint64 outputRate; 
%     uint256 price; uint64 reportCycle; uint64 reportLimit;
%     uint64[] inputRates;
    
%     function RateLimiterContract(address s, address e, uint64 p, uint64 c, uint64 t, uint64 i, uint64 o)
%         public payable {
%         require(s != 0x0 && e != 0x0);
%         owner = msg.sender;
%         contractor = s;
%         prover = e;
%         reportCycle = c;
%         reportLimit = t;
%         price = p;
%         maxInputRate = i;
%         outputRate = o;
%     }
    
%     function Calculate(uint64[] rates) internal returns (uint256) {
%         uint256 trafficRemoved = 0;
%         for(uint64 t = 0; t < rates.length && t < reportLimit; t++) {
%             if (rates[t] < outputRate)
%                 continue;
%             if (rates[t] > maxInputRate)
%                 trafficRemoved += maxInputRate;
%             else
%                 trafficRemoved += rates[t];
%         }
%         return trafficRemoved * price * reportCycle;
%     }
    
%     function Submit(uint64[] rates, bytes32 hash, uint8 v, bytes32 r, bytes32 s) public {
%         require(msg.sender == contractor);
%         address signer = ecrecover(hash, v, r, s);
%         require(signer == prover);
%         inputRates = rates; /* save the records in the contract */
%         uint256 payout = Calculate(inputRates);
%         uint256 refund = this.balance - payout;
%         contractor.transfer(payout);
%         owner.transfer(refund);
%     }
% }
% \end{lstlisting}


% $S$ can know that she is the only payee of the contract.


%Second, the enclave also creates a local {\em secure time variable} that is  updated only via the secure time source (i.e., {\tt sgx\_get\_trusted\_time()}) from the SGX processors. 
% Using this secure time variable, the bandwidth resource usage measurement report is summarized and the proof of contracted work is calculated. 
% Note that the enclave's wallet, its underlying ECDSA key, and the secure time variable are stored inside the enclave memory and never be copied out.


% volume of traffic removed by the filter is measured by the \name enclave and reported to the \name contract in the form of Ethereum transaction signed by the enclave's address.


%because (1) only the prover can call this function, (2) the transaction is signed by $E$, the wallet address that previously added as the prover.

% \subsection{Transparency and inflation deterrence}

% \paragraph{\name contract records.}
% Since a \name contract is a smart contract in the Ethereum blockchain, its instantiation and final result are written on the chain and cannot be altered or removed once they are confirmed. 
% Therefore all the elements in the contract itself, submitted proof of contracted work, and payout transactions are made publicly available and form the {\em \name contract records} or \name records.
% This creates the transparent records of \name system that can be used as the basis of an open \name market. 

% \paragraph{Useful analysis of \name records.}
% Using the public \name records, one can compile several useful analysis.
% One can easily track the pricing changes (e.g., Ether per unit bandwidth filtering) of the entire \name history, per ISP, or per country. 
% The easy and transparent access to the pricing changes can contribute to the reliable service pricing for the global \name filtering market. 

% The transparent \name records also make us to better understand the DDoS landscape on the Internet. 
% Although DDoS attacks are prevalent and it is often the public's interest to know more about the ongoing DDoS attack campaigns, we often do not have enough information about them except some aggregated information feeds from some privacy companies(e.g., Digital Attack Map\footnote{\url{http://www.digitalattackmap.com/}}). 
% The \name records can be a less biased, more transparent information source that we can use to understand the global DDoS landscape. 
% Note that the \name records do not include too sensitive information about each \name contract, such as filtering policies or private keys. 

% One can also easily reason about the reputation of any ISP for the \name service usage. 
% If an ISP makes too many \name contracts in a regular basis (e.g., always on for several weeks), this could possibly imply that this ISP is exploiting the \name service for its regular traffic filtering or firewall operations, but not for attack mitigation purposes. 
% Transparency in the \name records can be a strong deterrence for such misbehaviors of ISPs. 

% \paragraph{Inflation deterrence.}
% One particularly important misbehavior is a billing inflation where a malicious $S$ creates and sends dummy packets to the \name instance to increase the amount of filtering work (i.e., volume of filtered-out traffic).
% The increased filtered bandwidth is then recorded in the proof of contracted work and used to inflate the final payout to $S$. 
% Although the maximum input bandwidth $S$ can claim is written in its \name contract and thus the amount of maximum claimable payout is limited, $S$ can still continuously increase the dummy packet volume to force $D$ to raise the maximum input bandwidth set by $S$. 

% With the transparent \name contracts in the Ethereum blockchain, such misbehaviors can be deterred because such suspicious behaviors (e.g., continuously increasing attack volumes over a long period time) can easily damage the ISP's reputation. 

==> chapters/policy-bias.tex <==
\subsection{Policy Bias Attack}
\name  allows two ISPs to agree on a certain algorithm, which they agree on, to receive \PS and \PD and compute the final filtering policy \PSD.
The policy composition is inside an enclave and thus accountable and any tampering would be immediately detectable.

However, an attack is possible to bias the computed policy \PSD. 
Either ISPs can bias the final policy favoring its genuine policy.  By submitting a carefully modified policy instead of the genuine one, 

\msk{In this ... we assume a fair policy composition (whose details are not discussed here)}.

\msk{we analyze the adversary capabilities for this attack: know the algorithm, know its own genuine policy, and know the other party's policy.}

\msk{we make the last capability infeasible.}

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.5\textwidth]{figures/fairness.pdf}
	\caption{Fair policy composition and an end-to-end fairness violation attack.}
	\label{fig:fairness}
\end{figure}

The fair policy composition algorithm, unfortunately, is insufficient for the end-to-end fairness between $S$ and $D$.
Figure~\ref{fig:fairness}(b) illustrates how malicious ISPs can still break the fairness guarantee.
In this example, the source ISP $S$ is the adversary.
Just like the benign case, $S$ first translates its security policy written in human-readable language into this policy \PS. % that follows the agreed policy definition (e.g., per-class policing with preference in our case).
Then, the adversary $S$ submits a {\em modified} policy $P_S'$ ($\neq P_S$) to the filtering system so that the final composed policy \PSD is (nearly) identical to its own policy \PS.  
This attack is undetectable because the policy modification (i.e., from \PS to $P_S'$) happens {\em outside} of the fair composition system. % and thus it is hard to detect and prevent. 

%\subsection{Attack Prevention}
%\label{sec:fairness-attack-prevention}
\paragraph{A solution.} It is fortunately possible to prevent such end-to-end fairness violation attacks by removing and limiting the attack capabilities. 
For an effective attack, an adversary requires three attack capabilities: the knowledge of the composition algorithm, the other party's submitted policy, and resubmission of its policy.
The first capability must be given to the adversary for the accountability property of the policy composition logic; yet, the last two capabilities can be removed or significantly limited. 
The re-submission of policies can be limited by enforcing a minimum policy resubmission period, which can be negotiated between $S$ and $D$ and explicitly written in a \name contract (see Section~\ref{sec:econ-incentive}).
In this section, we focus on the \PD inference and how \name effectively prevent it.

%\paragraph{Preventing the accurate policy inference.}
Let us describe how we can prevent the adversary from inferring the submitted policy of the other party.
For ease of discussion, let us consider that $S$ is conducting the end-to-end fairness violation attack. 
Since $S$ has strictly more attack capabilities than $D$, our attack prevention argument applies to the attacks by $S$ as well.

Note first that an adversary $S$ cannot directly read \PD or \PSD due to the confidentiality guarantees of SGX. 
Yet, $S$ can still observe the behaviors of the filtering enforcement (that is, which packet is allowed/dropped) and may infer the policy behind (i.e., \PSD) the packet filtering decision. 
After obtaining \PSD, it is straightforward for $S$ to calculate \PD since the policy composition algorithm is publicly known and reversing with the output (\PSD) and one of the input (\PS) is trivial; see Appendix X for details.
Thus, let us focus on how $S$ can infer \PSD in the naive design of \name system and how we can prevent it.

The high-level idea of \PSD inference is that the external observer of the filtering operations. 
$S$ detects the existence of a rate limiter for a traffic class and their configurations, particularly, their average rates, $S$ effectively reveals \PSD.
A recent measurement study~\cite{flach2016internet} proposes that an effective algorithm that allows external observers of the policed traffic rate of a rate limiter to accurately measure its average rate. 
The algorithm in~\cite{flach2016internet} exploits that a rate limiter demonstrates a steady, flat outgoing traffic rate when the filtering is activated due to the excessive packet arrival. 
%Our adversary $S$ may attempt to use the same attack strategy to search for the steady outgoing rate of the rate limiters and reveal \PSD; however, 
\name can prevent this attack simply by removing this artifact (i.e., steady, flat outgoing rate) of our filtering logics by making our rate limiter implementation less accurate; 
e.g., introducing intentional random noise in the hierarchical token bucket (HTB) implementation. 
%Our HTB design already has token re-distribution logic for the work-conserving operations of large numbers of token buckets in the filtering system and we make it intentionally less accurate.
The details of this design choice is found in Section~\ref{sec:impl}.

==> chapters/policy.tex <==
\section{Fair Filtering in \name Enclave}
\label{sec:fairness}

As we discussed, source ISPs practically have no incentive to participate in source-end filtering, which is the biggest hurdle for adoption of the technology. 
In this paper, we propose both non-economic and economic incentives. 
%
Although economic incentive is useful and necessary (as we later argue in Section~\ref{sec:econ-incentive}), there may be cases where economic incentive is ineffective; e.g., an ISP's business model is not well aligned with chasing external revenue opportunities, a source ISP is under a sanctioned country where payment is not legally allowed.
Thus, we strongly believe that developing non-economic incentive mechanism that is orthogonal to economic incentives is important. 

\subsection{From outsourcing to {\em bilateral collaboration}}
\label{sec:bilateral-collaboration}
Existing source-end filtering mechanisms~\cite{mahajan2002controlling,argyraki2005active,liu2008filter,alwabel2015senss,li2015drawbridge} may have minor technical differences but the core shared primitive is the {\em outsourcing} of filtering operations to nodes closer to attack sources. 
Outsourcing, unfortunately, offers no incentives to the nodes near the attack sources (e.g., $S$) because they are usually not the victims of the attack.  

To that end, we propose a new source-end filtering primitive, which we call {\em bilateral collaboration}, that directly incentivizes $S$ by offering the control to the traffic filtering operation of the source-end filtering logics. 
Note that this primitive cannot be realized without the established trust between mutually untrusted $S$ and $D$, particularly, the integrity property of the bilateral collaboration logic.

To be more specific, \name allows both $S$ and $D$ to submit their own filtering policies \PS and \PD, respectively. 
The two ISPs are not supposed to consult each other in determining their policies but they do it separately and independently only to represent their own filtering rules and preferences. 
Then, the submitted policies \PS and \PD are processed by the \name instance and converged to a final policy \PSD, which is ultimately used to implement the filters for the traffic from $S$ to $D$.

Compared to the traditional outsourcing modeling, bilateral collaboration
offers an explicit control knob to $S$ so that it can actively participate, not just observe, the filtering operations. 
This simple addition can be extremely beneficial to $S$.
First, it allows $S$ to protect certain packets it wishes to prioritize (e.g., connections for mission critical services/premium customers, white-listed IPs) when some of packets must be dropped due to attacks at $D$.
Second, it allows $S$ to apply its own blacklist (e.g., known botnet IPs within its customers) and deprioritize them. 
Lastly, it indirectly implements the user agreement\,---\,a user scheduling outside of the specification of the target system\,---\,between traffic sources, which is proven to be an ideal solution to denial-of-service attacks at a destination~\cite{yu1988formal}. 

For bilateral collaboration, the policy fairness between $S$ and $D$ is the key because two ISPs should be ensured that their policies are respected in a fair manner. 
%We explain how we achieve the fairness in the rest of this section. 
%
%\subsection{End-to-End Fairness Guarantees}
%The bilateral collaboration can be an attractive incentive to $S$ only when the fairness between $S$ and $D$ is guaranteed; that is, the actual filtering rules must be the result of a {\em fair} composition of the two input policies. 
%
The SGX-based \name design guarantees the fair composition between the two submitted policies \PS and \PD by relying on the SGX's isolated execution and integrity guarantees. 
However, we show that the end-to-end fairness between $S$ and $D$ (not just between their submitted policies \PS and \PD) is in fact non-trivial to achieve due to a potential adaptive attack by $S$ (\S\ref{sec:fairness-attack}). 
We present a number of solutions we use in our \name system. % and describe how they effectively prevent these attacks (\S\ref{sec:fairness-attack-prevention}).

Before we discuss the security concerns, let us first describe the notion of fairness in policy composition. % fairness (\S\ref{sec:fair-composition}).%, focusing on the definition of filtering policy and useful functions over them for fairness discussion. 


\subsection{Verifiably Fair Policy Composition}
\label{sec:fair-composition}

\begin{figure}[t!]
\centering
\includegraphics[width=0.5\textwidth]{figures/fairness.pdf}
\caption{Fair policy composition and an end-to-end fairness violation attack.}
\label{fig:fairness}
\end{figure}

%We begin by describing the abstract model of fair policy composition. 
Figure~\ref{fig:fairness}(a) illustrates the end-to-end fair policy composition. 
Both $S$ and $D$ may have their own packet filtering policies written in human-readable language and they are translated into the policy rules \PS and \PD, respectively. %, we later define their specifications. 
The two policies \PS and \PD are then submitted to the filter where a fair composition logic produces one final filtering policy \PSD. 

Intuitively, the fair composition logic searches for the middle ground between the two submitted policies. 
Algorithmically, we search for the equally distanced policy between \PS and \PD for the final policy when we can define the notion of distance between two arbitrary policies. 

Now let us describe the concrete algorithms that compose the filtering policies with a simple but practical policy definition example. 
Filtering policy is a set of filtering rules that specify certain packet or flow drop/allow operation and thus can vary widely depending on the application. 
%For example, filtering rules for enterprise access control logic should be fine grained, often needs to be stateful and modify packets to handle sophisticated network firewall policies. 
In DDoS mitigation applications, we consider relatively coarse grained flow specifications (e.g., 100s or 1000s of traffic classes) and stateless (since our focus is on the volume of traffic).
%Moreover, actions needed for packet filtering can be simple; e.g., rate limiting based on traffic types. 

Let us summarize the following three types of policy definitions, which are not supposed to be exhaustive lists but some simple examples:
\begin{enumerate}
	\item {\em Binary rules}: As the simplest policy definition, \name determines to allow or drop an entire traffic class. 
%	This simplest action is easy to use and often expressive enough to filter out clear attack traffic and protect clear benign traffic;  
	\item {\em Prioritized binary rules}: Traffic classes are ordered with their priorities and packets with higher priority are served strictly earlier than packets with lower priority. 
%	While this allows the operators to express strong preference notion, it creates a hogging problem (e.g., low-priority packets rarely get served when there are many high-priority packets); 
	\item {\em Prioritized per-class policing}: To address the resource hogging problem of the strict prioritization, traffic classes are ordered and each traffic class is policed with different average rates that are determined based on the priority order. 
%	That is, a high-priority class is assigned with a higher rate than a low-priority class.
%	This is similar to the hard preference action but it alleviates the hogging problem as a high-priority traffic class cannot hog all the available bandwidth. 	
\end{enumerate}

Throughout this paper, we use the {\em prioritized per-class policing} policy definition (unless otherwise noted) as it is more expressive than other action types among the four above action examples.
A filtering policy then can be simply expressed as an ordered list of flow specifications; e.g., \{$c_1,c_2,\cdots,c_n$\} where $c_i$ denotes the $i$-th traffic class defined by the five tuple of TCP/IP flows. 

The distance between two policies $P_1$ and $P_2$ can be defined with the Kendall tau rank distance when one policy is a permutation of the other policy.
For example, if $P_1 = \{c_1,c_2,\cdots,c_n\}$ and $P_2 = \texttt{perm}(P_1)$, the Kendall tau distance $d(P_1, P_2) = |\{(i, j) | (i, j) \in P_1 \land (j, i) \in P_2 \}|$ counts the number of pairwise disagreements between two ranking lists. 
The minimal distance is $0$ when they are identical and the maximum
distance is $n (n-1) /2$ when they are complete reversed, where $n$ is the number of traffic classes. 

\paragraph{Fair composition algorithm.}
Let us now describe the fair composition algorithm for the given two policy inputs \PS and \PD. 
The first issue we face is that the two policies are independently generated by the two ISPs and thus their traffic class definitions can be different and thus {\em incomparable}. 
For example, one traffic class $c$ in \PS may not exist in \PD and thus any comparison between the two is not possible. 
%Such two policies with different traffic class definitions are said to be {\em incomparable} and the distance between them cannot be defined.
%
To make the two policies comparable, we partition their traffic classes into smaller flow definitions until the two policies have the same traffic class sets. 
For example, let us assume a toy example with eight atomic flow definitions $f_1,\cdots,f_8$ and the two incomparable traffic class sets $C_S=\{{\{{f_1,f_2}\},\{{f_3,f_4,f_5}\},\{{f_6,f_7,f_8}\}}\}$ and
$C_D=\{{\{{f_1}\},\{{f_2,f_3}\},\{{f_4,f_5,f_6,f_7,f_8}\}}\}$. 
We partition the traffic classes in $C_S$ and $C_D$ until the two sets become identical  $C_{S,D}=\{{\{{f_1}\},\{{f_2}\},\{{f_3}\},\{{f_4,f_5}\},\{{f_6,f_7,f_8}\}}\}$.

Once the two policies become comparable, we compose them and calculate the policy $P_{S,D}$. 
We define the fairness of a composition function $\phi$ as $\mathcal{F}(\phi) =  |d(P_S,P_{S,D}) - d(P_D,P_{S,D})|$, where $d(P_1,P_2)$ denotes the Kendall tau rank distance between $P_1$ and $P_2$. 
Our aim is to find a $\phi$ that minimize $\mathcal{F}(\phi)$ for all possible input policies $P_S$ and $P_D$.
The detailed deterministic algorithm is found in Appendix~\ref{appx:fair-algorithm} 


\subsection{End-to-End Fairness Violation Attacks}
\label{sec:fairness-attack}

The fair policy composition algorithm, unfortunately, is insufficient for the end-to-end fairness between $S$ and $D$.
Figure~\ref{fig:fairness}(b) illustrates how malicious ISPs can still break the fairness guarantee.
In this example, the source ISP $S$ is the adversary.
Just like the benign case, $S$ first translates its security policy written in human-readable language into this policy \PS. % that follows the agreed policy definition (e.g., per-class policing with preference in our case).
Then, the adversary $S$ submits a {\em modified} policy $P_S'$ ($\neq P_S$) to the filtering system so that the final composed policy \PSD is (nearly) identical to its own policy \PS.  
This attack is undetectable because the policy modification (i.e., from \PS to $P_S'$) happens {\em outside} of the fair composition system. % and thus it is hard to detect and prevent. 

%\subsection{Attack Prevention}
%\label{sec:fairness-attack-prevention}
\paragraph{A solution.} It is fortunately possible to prevent such end-to-end fairness violation attacks by removing and limiting the attack capabilities. 
For an effective attack, an adversary requires three attack capabilities: the knowledge of the composition algorithm, the other party's submitted policy, and resubmission of its policy.
The first capability must be given to the adversary for the accountability property of the policy composition logic; yet, the last two capabilities can be removed or significantly limited. 
The re-submission of policies can be limited by enforcing a minimum policy resubmission period, which can be negotiated between $S$ and $D$ and explicitly written in a \name contract (see Section~\ref{sec:econ-incentive}).
In this section, we focus on the \PD inference and how \name effectively prevent it.

%\paragraph{Preventing the accurate policy inference.}
Let us describe how we can prevent the adversary from inferring the submitted policy of the other party.
For ease of discussion, let us consider that $S$ is conducting the end-to-end fairness violation attack. 
Since $S$ has strictly more attack capabilities than $D$, our attack prevention argument applies to the attacks by $S$ as well.

Note first that an adversary $S$ cannot directly read \PD or \PSD due to the confidentiality guarantees of SGX. 
Yet, $S$ can still observe the behaviors of the filtering enforcement (that is, which packet is allowed/dropped) and may infer the policy behind (i.e., \PSD) the packet filtering decision. 
After obtaining \PSD, it is straightforward for $S$ to calculate \PD since the policy composition algorithm is publicly known and reversing with the output (\PSD) and one of the input (\PS) is trivial; see Appendix X for details.
Thus, let us focus on how $S$ can infer \PSD in the naive design of \name system and how we can prevent it.

The high-level idea of \PSD inference is that the external observer of the filtering operations. 
$S$ detects the existence of a rate limiter for a traffic class and their configurations, particularly, their average rates, $S$ effectively reveals \PSD.
A recent measurement study~\cite{flach2016internet} proposes that an effective algorithm that allows external observers of the policed traffic rate of a rate limiter to accurately measure its average rate. 
The algorithm in~\cite{flach2016internet} exploits that a rate limiter demonstrates a steady, flat outgoing traffic rate when the filtering is activated due to the excessive packet arrival. 
%Our adversary $S$ may attempt to use the same attack strategy to search for the steady outgoing rate of the rate limiters and reveal \PSD; however, 
\name can prevent this attack simply by removing this artifact (i.e., steady, flat outgoing rate) of our filtering logics by making our rate limiter implementation less accurate; 
e.g., introducing intentional random noise in the hierarchical token bucket (HTB) implementation. 
%Our HTB design already has token re-distribution logic for the work-conserving operations of large numbers of token buckets in the filtering system and we make it intentionally less accurate.
The details of this design choice is found in Section~\ref{sec:impl}.








==> chapters/privacy.tex <==
\subsection{Privacy Guarantees}
% \subsection{Upper-bound on Privacy}
\label{subsec:algo-fair-privacy}
From our previous discussion in Section~\ref{subsec:metrics-tradeoff}, it is clear
that achieving ideal fairness and privacy goals simultaneously is an elusive goal. 
Instead, we aim to guarantee a user-controlled privacy level (e.g., anonymity
set size) at the cost of reduced fairness. 


%\input{chapters/algo-example-fig}

Let us first evaluate the privacy property of our policy composition $\phi$ 
in Algorithm~\ref{algo:fair-comp} that guarantees the maximum fairness
in a deterministic way. 
In this algorithm, we make a deterministic choice of performing bubble-sort swaps;
i.e., we pick the swap location based on left-to-right sequence of the target that we cant to reach.
Thus, if we want to find midpoint of $P_S=(2, 3, 4, 1)$ and $P_D=(3, 2, 1, 4)$ which are
at a distance of $2$, the algorithm would always chose $P_{S,D}=(3, 2, 4, 1)$.  Note that there is
another choice $(2, 3, 1, 4)$, which is also at a distance of $1$ from the two inputs; 
however, this alternative middle point is not selected by our deterministic algorithm.
%This means that $(3, 2, 1, 4)$ 
This deterministic operation does not utilize all the alternate middle points as the composite policy and thus limits the policy anonymity set significantly.

% because starting from $(2, 3, 4, 1)$, it is the
%one which does the swap on a left pair. Now, in an attack scenario for this
%example. the attacker knows the start point $(2, 3, 4, 1)$ and the middle
%point $(3, 2, 4, 1)$. Using this, he can calculate that the midpoint is at a
%distance $1$ which implies that the other input policy must be at a distance
%$1$ from $(3, 2, 4, 1)$. Now, the attackers job is trivial, because there are
%only two candidate $(3, 4, 2, 1)$ and $3, 2, 1, 4$ which are left-order swaps
%of distance one. Thus, the attackers anonymity set is only $2$ as compared to
%$24$ in the ideal case.

\paragraph{Randomized Composition.}
%We observe that because of our deterministic algorithm, we hit the lower bound
%of anonymity set which fits the attacker's observation. Which implies that our
%algorithm achieves least possible privacy. The next obvious question is, can
%we do better? 
Let us improve our policy composition algorithm to utilize all available potential
composite policies given two input policies. 
Let us consider the sequence of policies that is formed by
swapping adjacent elements as a path between two polices. Then, given any $P_S$ and $P_D$, there can be multiple different paths which are of the same distance.
Each of these paths may have different mid-points
which represents different composite policies which satisfy our goal of
equidistance. 
To exploit all possible paths, we randomly chose one of the positions to perform the swap instead
of the deterministic left-to-right order.

\input{chapters/random-algorithm}

Algorithm~\ref{algo:rand-fair-comp} adds random swapping operations to Algorithm~\ref{algo:fair-comp} (line 7).
In particular, the algorithm randomly chooses one of the positions to perform the swap instead of the deterministic left-to-right order and thus it can select any of the possible fair composite policies. 
For example, $P_S=(1, 2, 3, 4)$ and $P_D=(3, 2, 1, 4)$ have two
different paths of distance 3. Our randomized algorithm can choose one of the
potential midpoints $(3, 1, 2, 4)$, $(1, 3, 2, 4)$,  $(2, 1, 3, 4)$, or $(2, 3, 1, 4)$.

\paragraph{Policy anonymity set.}
As we defined in the early this section, $\mathcal{P}_D(\phi)$ and $\mathcal{P}_S(\phi)$ are the anonymity sets for $P_D$ and $P_S$, respectively. 
Let us describe how we can calculate $\mathcal{P}_D(\phi)$ for given $P_S$ and $P_{S,D}$ when the above randomized algorithm is used.

Given one end point (i.e., $P_S$) and a middle point (i.e., $P_{S,D}$) in the policy space and their distance is $d_1 = d(P_S, P_{S,D})$, we want to find all possible points in the space that satisfy the two conditions: $d(P_D, P_{S,D}) = d_2$ and $d(P_S, P_D) = d_1 + d_2$, where $d_2 \in \{{d_1-1, d_1, d_1+1}\}$.
For example, when we have two input policies $P_S=(1, 2, 3, 4)$ and $P_D=(3, 2, 1, 4)$ (as in the previous example), if $P_{S,D}=(3, 1, 2, 4)$ is chosen, $S$ finds that there exist six potential $P_D$'s that would result in the same $P_{S,D}$: $(3,2,1,4)$, $(3,1,4,2)$, $(3,2,4,1)$, $(3,4,1,2)$, $(3,4,2,1)$, and $(4,3,1,2)$.
Thus, with the given composite policy, 25\% (6 out of 24) of all possible policies are in the anonymity set for the given $P_{S,D}$. 

\paragraph{Guaranteeing an anonymity set size.}
In our policy composition function $\phi$, ISPs can easily negotiate with the desired level of privacy.
We use the anonymity set size as the metric for the privacy-preserving property of $\phi$. 
ISPs $S$ and $D$ can agree on a minimum anonymity set size and $\phi$ enforces it while composing the two input policies from them. 
To guarantee the minimum anonymity set size, $\phi$ may need to execute Algorithm~\ref{algo:rand-fair-comp} multiple times with a relaxed distance constraint in line 2. 
First, $\phi$ executes the unmodified Algorithm~\ref{algo:rand-fair-comp} and then evaluates the anonymity set size of the chosen composite policy $P_{S,D}$. 
If the anonymity set size is smaller than the minimum desired set size, it re-runs the algorithm with a reduced fairness by adding one more distance to the value $dist$ in Algorithm~\ref{algo:rand-fair-comp}. 
Then, $\phi$ repeats this until it finds a composite policy $P_{S,D}$ that has large enough anonymity set.


% In that case, the attacker neither
%knows which path was taken to reach the mid-point nor can it be certain which
%path to chose to move from the mid-point towards the end-point policy.

%For better understanding let us use vertices to denote the simple policy in
%$n$-element permutation and edges to connect each pair of polices that have
%the Kendall tau distance of 1, we can construct a three-dimension polyhedron.
%For example, Figure~\ref{fig:order_4_p_hedron} shows the polyhedron for
%policies of order 4~\footnote{Such a polyhedron is also refereed to as a
%permutohedron or bubble-sort graph}. With the help of this polyhedron of order
%4, the number of paths between any two simple polices can be visualized and
%counted easily. For example, $(1, 2, 3, 4)$ and $(3, 2, 1, 4)$ have two
%different paths of distance 3. Our randomized algorithm can either chose the
%midpoint $(3, 1, 2, 4)$ on one of the paths $(1, 2, 3, 4), (1, 3, 2, 4), (3,
%1, 2, 4), (3, 2, 1, 4)$. Or it can chose $((2, 1, 3, 4))$ which is the mid-
%point on the other path $(1, 2, 3, 4), (2, 1, 3, 4), (2, 3, 1, 4), (3, 2, 1,
%4)$. In fact, if we randomize the choice or using the ceiling or the floor for
%finding the mid-point, we can add more uncertainty to the attackers choices.
%Algorithm~\ref{algo:rand-fair-comp} shows our randomized version of the policy
%composition algorithm.



% \paragraph{Examples.}
% \begin{itemize}
% 	\item {\bf $d = 2$.}
% 	$\phi ((2, 3, 4, 1) (3, 2, 1, 4)) = (3, 2, 4, 1)$ \\
% 	$\mathcal{F}(\phi) = $ \\
% 	$\mathcal{P}(\phi) = 2$ ; $\{(3, 2, 4, 1), (2, 3, 1, 4)\}$
% 	\item {\bf $d = 3$.}
% 	$\phi ((1, 3, 2, 4), (2, 1, 3, 4)) = (1, 2, 3, 4)$ \\
% 	$\mathcal{F}(\phi) = $ \\
% 	$\mathcal{P}(\phi) = 3$ ; $\{(2,1,3,4), (2,1,4,3), (1,2,4,3)\}$
% 	\item {\bf $d = 4$.}
% 	$\phi ((1, 4, 3, 2) (3, 2, 1, 4)) = (3, 1, 4, 2)$ \\
% 	$\mathcal{F}(\phi) = $ \\
% \end{itemize}

==> chapters/problem.tex <==
\section{Applicability of \name}
\label{sec:overview}

\subsection{Overview of \name}
\label{sec:collaborative-filtering-problem}
%\paragraph{Source-end filtering for DDoS mitigation.}
We design our mutual collaboration as a {\em mutual protocol} between two distinct networks: a {\em
source} AS $S$, which hosts potential attack sources (e.g., botnets) in its and its customers' networks, and a {\em destination} AS $D$, which experiences congestion. 
Note that the two ASes may be indirectly connected through one or more transit ASes. 
%In this paper, we focus on a simple bilateral protocol as the fundamental building block for extended collaborative mitigation models, such as multi-party peer-to-peer collaborations or centralized collaboration models; see Section~\ref{} for detailed discussion. 
%
We consider that $D$ first initiates a collaborative filtering {\em session} with $S$. 
We assume that $D$ has already identified the AS $S$ that sends high volume traffic, via coarse-grained traffic analysis tools, such as NetFlow~\cite{netflow} or sFlow~\cite{}. 
Note that $D$ may create more than one session with multiple source ASes (e.g., $S_1,S_2,\cdots$) but the sessions with different source ASes are independently established and operated.
We observe that the number of such parallel filtering sessions would be small and thus manageable (e.g., 10 -- 20 or less) due to the highly unbalanced attack source (e.g., botnets) distribution in most practical attacks; see Section~\ref{} for detailed analysis. 

%The source AS $S$ filters out a subset of packets that are generated by its customers and {\em destined} to the destination AS $D$. 

%\paragraph{Fairness in collaboration.}
%We envision packet filtering operation that is based on the {\em mutual collaboration} between two ASes, {\em not} a mere network function {\em outsourcing}~\cite{liu2008filter,alwabel2015senss}. 
In \name, {\em both} $S$ and $D$ submit their filtering policies: the \textit{source policy} $P_S$ and the \textit{destination policy} $P_D$. 
Collaborative filtering requires these two independently-generated policies $P_S$ and $P_D$ to be {\em fairly} respected in actual packet filtering operations, benefiting both two collaborating parties.
%Since the two policies are generated without coordination, there may be some conflicting filtering rules, such as, $D$ wishes to drop a certain traffic flow whereas $S$ hopes to protect the same flow.
%Such conflicting rules must be reconciled in a fair manner so that neither parties are favored over the other in the packet filtering operation. 

\subsection{Frequently Asked Questions about \name}
Before describing the details of our system design and security properties, we discuss under what conditions and to what extent \name is useful for DDoS mitigations.
We start by informally addressing four commonly asked questions and then characterize our threat model and describe how to achieve the necessary security properties.

\smallskip
\noindent{\bf Q1: }{\em How is it fundamentally different from existing filtering outsourcing proposals? And why is \name is more attractive to source ASes?} 
Unlike outsourced filtering, \name ``requires'' the source AS to submit its filtering policy. 
That is, a source AS is supposed to actively participate in the packet filtering decision, which is not allowed in any existing solutions. 

This additional functionality offers great incentives to the source ASes. 
Let us imagine that a destination AS $D$ simply outsources filtering operations to a source AS $S$.
For $S$, either acceptance (i.e., implementing $D$'s filtering policy) or rejection (i.e., letting $D$ to filter packets) of the outsourced filtering request implies that it lets the destination AS $D$ to have the full control to decide which packet should be allowed or dropped when under DDoS attacks.  
%As an alternative, $S$ may accept the request but overwrite the requested policy with its own policy; however, this only creates the problem of lack of trust between the two ASes and eventually break the inter-domain session. 
Unlike outsource filtering, \name's collaboration request from $D$ is a strictly better option for $S$ to express its own policy (e.g., protecting or deprioritizing flows) when some portion of its traffic have to be dropped due to DDoS incidents. 


\smallskip
\noindent{\bf Q2: }{\em Isn't that both ASes can already perform own filtering without \name by dropping arbitrary packets in their networks?}
Although any AS on the route from $S$ to $D$ can drop any packets based on their own preference, such arbitrary packet drops cannot serve as a reliable policy enforcement for two reasons. 
First, such arbitrary packet drops (without clear evidence of congestion in their own networks) are observed as the violation of service level agreement (SLA) or net neutrality to the customers. 
Second, dropping certain packets does not guarantee the protection of other packets. 
For example, a source AS $S$ may drop flow $x$ in the hope that its another flow $y$ be better treated in the congested destination network.
However, the destination $D$ will not necessarily respect the $S$'s inexplicit policy because flow $x$ and flow $y$ are independent to $D$.\footnote{Unless $D$ implements strict per source AS fairness bandwidth policy, which is uncommon.} 


\smallskip
\noindent{\bf Q3: }{\em What if attack packets have source IPs spoofed to be the source AS $S$'s addresses? Can such attacks be detected?}
\name is not designed to prevent IP spoofing DoS attacks.
Unfortunately, 20-30 \% of ASes are still without proper ingress filtering thus IP spoofing DoS attacks are easy to launch~\cite{}.
However, \name instead is designed to detect IP-spoofing DoS attacks effectively. 
When a destination AS $D$ first establishes a collaborative filtering session with a source AS $S$, they set a point-to-point tunnel (e.g., a GRE tunnel) between them (e.g., between their edge routers) to encapsulate all the packets from $S$ to $D$. 
This simple inter-domain encapsulation allows the destination AS $D$ to detect IP-spoofing DoS attacks effectively; see Section~\ref{sec:bypass}.

\smallskip
\noindent{\bf Q4: }{\em \name claims to effectively detect misbehaviors (e.g., bypassing the \name filtering), but what can one do when a misbehavior of the other party is detected?} 
In \name, two ASes create temporary contract only between them. 
Therefore, any one of them can abort the temporary contract whenever one party detects misbehaviors. 
For example, if a destination AS $D$ detects the misbehavior of a source AS $S$, $D$ can quickly abort the collaborative filtering and start deprioritizing traffic from $S$ as a penalty to the misbehavior.


%\noindent{\bf Q4: }{\em Despite all the merits of mutual collaboration, what if small (e.g., tier-3) ASes may not be able to afford additional operational costs of \name?} 
%First of all, \name is designed to be low-cost and easily incorporated into exiting private computing cluster with commodity platform.
%In case \name is still not affordable to the direct source AS, its upstream AS (e.g., tier-2) may run \name on behalf of the direct source AS; see a detailed discussion in Section~\ref{}.

\section{Threat Model and Desired Security Properties}
\label{sec:prob}

\subsection{Adversary model}
\label{sec:threat-model}
%Collaboration between two ASes is hard because the ASes in practice tend to be {\em mutually untrusted}.
We consider that two ASes are {\em mutually untrusted}. 
This is realistic because the source and destination ASes seldom have any bilateral contract between them especially when they are remote ASes to each other often in different geopolitical regions with no direct business relationship.

The untrusted two ASes may aim to achieve three main attack goals.
First, ASes want to {\em tamper} with the policy composition logic of the \name system to affect the final composed policy and overwrite it with their own preferred policy.
Second, ASes also may want to {\em bypass} the \name's filtering logic outside of the \name system to ignore the per-packet decision made by \name.
Third, ASes may want to {\em learn} the other's policy. The inferred policy can be used for one's own benefit or can be leaked to other interested parties (e.g., a competitor of the policy owner).

Note that $S$ has more attack capabilities than $D$ in general since it is the operator that executes and manages the \name system in its own network infrastructure. 
Particularly, we consider that $S$ can control the software components of \name and even the privileged software (e.g., operating system) of the system. 
Moreover, $S$ has the full control (e.g., read, inject, drop) over all the packets entering/leaving \name. 
On the contrary, the destination $D$ can observe only the packets leaving the \name system. 

\paragraph{Scope.}
We consider that other malicious attack sources may generate {\em IP-spoofed} DDoS traffic with the source IPs under the control of a source AS. 
The proposed \name system handles such IP-spoofed attack traffic by simply distinguishing packets with spoofed source IPs and the ones that actually come from the designated source AS. 

During the lifetime of a session for mutual collaboration between two ASes $S$ and $D$, we consider that $D$'s filtering policy may change dynamically to adapt to the incoming DDoS attack traffic and the availability of its network and customers. 
Yet, we assume a {\em static} policy submission of the source AS $S$ as its filtering policy is not DDoS attack specific but more related to its own policy regarding its customers; e.g., which customer must have higher access priority when the available bandwidth is limited. 



\subsection{TEE based \name Design}
\label{sec:name-overview}

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.48\textwidth,height=0.5\textheight,keepaspectratio]{figures/design.pdf}
	\caption{A high-level view of a \name instance $F(S,D)$ between two ASes $S$ and $D$.}
	\label{fig:design}
\end{figure}

To protect \codename from the direct access of the source AS $S$, we utilize the hardware-based trusted execution environments (TEEs) in \name's design, as shown in Figure~\ref{fig:design}. 
With the TEE protection, \codename can isolate its packet filtering executions from its malicious operator under $S$'s control and prevents it from tampering with the packet filtering (e.g., accessing/altering filtering policies or packet allow/block decisions).
Moreover, the TEE-based design allows the two ASes $S$ and $D$ to individually verify the
correct implementation of the negotiated packet filtering operations before and while they perform collaborative filtering.
In this work, we implement \name using a recent trusted computing capability called Intel SGX~\cite{}. 

We envision a software virtualization technique to create scalable \name instances on-demand based on the required filtering capability and the volume of traffic from $S$ to $D$. 
\name is a low-cost, highly efficient virtual function that runs on commodity computing clusters.
\name is installed inside the source $S$'s private cluster with commodity servers.
The source AS $S$ redirects packets from $S$ to $D$ to the \name functions when the collaborative packet filtering is activated via SDN's dynamic rerouting capability.



As shown in Figure~\ref{fig:design}, the \name instance $F(S,D)$ between $S$ and $D$ accepts the desired received rate $L$ bps from $D$. 
%$M(S,D)$ also receives the two policies $P_S$ and $P_D$ from the two ASes to make fair packet-drop decisions in its packet filtering logic. 
\name is composed of the control- and data-plane
components: a policy composition $\phi(\cdot)$ and a
policy enforcement $\psi(\cdot)$, respectively.  
The {\em policy composition} $\phi$ reconciles the two independent filtering policies $P_S$ and $P_D$ and creates a {\em composite policy} $P_{S,D}$.
The composite policy $P_{S,D}$ is then passed to the data plane function 
$\psi(\cdot)$ that performs packet filtering based on the given composite policy and the desired rate $L$ bps. 
The {\em policy enforcement} $\psi(\cdot)$ is designed to be a generic packet filtering engine that implements various types of filtering policies $P_{S,D}$ .
To that end, we consider a traffic classifier categorizes incoming packets based on the traffic classifications (i.e., groups of packets from $S$ to $D$ that share the same priority rules) of the given policy $P_{S,D}$, followed by a large array of rate limiters (e.g., token bucket) that enforce rate reduction for each traffic class independently. 
The policy enforcement $\psi$ may also log some packet processing results for audits.





\subsection{Design Problems}
As described in Introduction, we have three security goals against the threat model: (1) verifiably fair policy composition and enforcement; (2) negotiable maximum policy leakage; and (3) effective bypass detection. 
In principle, the TEE-based design of \name guarantees the execution integrity and verifiability of the control-plane and data-plane operations of \name. 
This strong guarantee is the baseline security primitive for the three security goals of \name but it is unfortunately insufficient. 
\begin{itemize}
	\item First, TEE protects the composition logic and the enforcement of the composed policy from malicious system operator (e.g., source AS $S$) and makes them verifiable. 
	However, the notion of fairness and the algorithmic model for fair composition for various policy definitions must be defined and developed first (see Section~\ref{sec:policy}). 
	\item Second, TEE protects a privacy negotiation process between two ASes and guarantees their agreed privacy mechanisms. 
	However, due to the undesirable, inherent tradeoff between privacy and fairness, it is tricky to find a right balance between the fairness and privacy. 
%	For the worst case scenario analysis, we also need to understand the strongest privacy attack strategies (e.g., learning the other's policy within a few minutes) and demonstrate the attacks.
	Moreover, we need to build a framework that suggest an adequate level of privacy (e.g., anonymity set size) for given policies and fairness target (see Section~\ref{sec:attacks}). 
	\item Third, TEE enables per-packet validation between untrusted $S$ and $D$, which makes fine-granular bypass detection achievable. 
	However, per-packet validation incurs significant performance overhead due to excessive context switching and thus make line-rate operation difficult (see Section~\ref{sec:bypass}).
\end{itemize}

%Moreover, the fairness property must be defined and chosen in conjunction with their privacy property


%enables the verification in two levels but not trivial what to verify in control plane ... and how to verify in data plane ... without affecting the line-rate packet processing. 

%\begin{itemize}
%	\item {\bf Lack of privacy property.} Although ASes cannot directly read the submitted policies or the composed policy due to the TEE's memory confidentiality, they can still learn some of the sensitive policies by monitoring and/or testing the middlebox's external behaviors. 
%	For example, consider a middlebox that implements a simple rule that drops a certain type of packets.
%	By sending one or more probe packets of the same type and observing the packet-drop decisions, $S$ can easily infer whether this packet type is filtered or not.
%	Once ASes learn the composed policy $P_{S,D}$, they may then attempt to infer the other AS's policy; see Section~\ref{sec:attacks} for detailed attack descriptions.
%	\item {\bf Lack of non-bypassability property.} 
%	The source AS installs and operates the \name middlebox and thus it is easy for $S$ to bypass the middlebox when it wishes to overwrite the filtering decision made by the middlebox. 
%	For example, if $S$ learns that a packet $p$ is allowed by the middlebox, which is against its will, it may want to drop $p$ before (or even after) the middlebox processes it. 
%	Conversely, $S$ can easily force to send the packet $p$ by bypassing the middlebox when the middlebox decides to drop $p$. 
%	Note that the \name middlebox cannot  prevent such bypasses since it has no control over the network operation of the source AS $S$. 
%\end{itemize}
%
%\subsection{Our Contributions}
%Acknowledging the non-trivial challenges of the two security properties, in this paper, we aim to shed light on the {\em security upper-bounds} of the privacy and non-bypassability properties.
%
%\paragraph{Privacy guarantees.}
%First, we analyze the effectiveness of a family of privacy attacks for inferring the composed policy $P_{S,D}$ of the middlebox and subsequently the other AS's internal policy (Section~\ref{sec:attacks}).
%In the inference attack on $P_{S,D}$, we focus on how effectively and efficiently the ASes can exploit the data-plane side channels (i.e., packet filtering decisions observed via monitoring data-plane packets of the middlebox) and infer $P_{S,D}$. 
%In the subsequent inference attack on $P_D$ by $S$ (or $P_S$ by $D$), we analyze the maximum privacy guarantees (e.g., anonymity set) for the AS's internal policies for various policy definitions (e.g., how to express the preferences in the filtering policy) and fairness notions (e.g., how to define and measure fairness of the composed policy).
%Analysis on these policy inference attacks offers us the necessary insights regarding the privacy bounds of the collaborative packet filtering mechanism in a generic setting and suggestions for the choice of policy expressiveness, preference design, and fairness guarantees for the desired degree of policy privacy. 
%
%\paragraph{Non-bypassability guarantees.}
%Second, we propose a lightweight bypass detection mechanism between the middelbox and the destination AS $D$ (Section~\ref{}).
%We then analyze the upper-bound of non-bypassability guarantees by measuring the effectiveness of the bypass detection by the two participating ASes. 
%We analyze the trade-off between the detection accuracy and the performance (e.g., real-time computation/memory overhead) of the detection mechanism and evaluate the attack effectiveness (e.g., number of packets bypassable without being detected).
%
%\paragraph{SGX-based middlebox implementation.}
%Third, we also design and build a prototype of the proposed \name middlebox that supports multi-gigabit bandwidth (e.g., 10 Gbps or higher) throughput on a commodity server platform with the Intel SGX-enabled CPUs (Section~\ref{sec:impl}).
%We particularly address several non-trivial system optimization issues, including SGX integration with heavy data-plane operation. 



==> chapters/random-algorithm.tex <==
\alglanguage{pseudocode}
\begin{algorithm}
\caption{Randomization to find the midpoint of $P_S$ \& $P_D$}
\label{algo:rand-fair-comp}
\begin{algorithmic}[1]
\scriptsize
\Procedure {FairComposition}{$P_S(s_1 .. s_n)$, $P_D(d_1 .. d_n)$} 
\State $dist \gets RAND(\lfloor d(P_S, P_{D}) / 2 \rfloor, \lceil d(P_S, P_{D}) / 2 \rceil)$
\State $P_{SD} \gets P_D$
\For{$i \leftarrow 1, n-1$}
    \For{$j \leftarrow 1, n - i$}
        \If{$s_m > s_n$ where $s_m = d_j, s_n = d_{j+1}$}
            \State {SWAP} RAND({$d_j, d_{j+1}$})
            \State $dist \gets dist - 1$
            \If{$dist = 0$}
                \State $P_{SD} \gets P_D$
            \EndIf
        \EndIf
    \EndFor
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> chapters/recon-algo.tex <==
\subsection{Fair Reconciliation Algorithm}
\label{subsec:algo}

Given our definitions of fairness and privacy, the goal of an ideal $\phi$
function is to generate a composite policy $P_{S,D}$ which is ideally fair as
well as ideally private w.r.t. input policies $P_S$ and $P_D$. 
%Understanding
%the asymmetric nature of the trade-off, that is, strong privacy hurts fairness
%more than strong fairness does to privacy, we design the algorithm centered
%around the fairness and enforce privacy as constraints of the problem. 
We start with an algorithm which maximizes fairness and then try to maximize
the corresponding privacy that we can achieve for it. A fair policy
composition function $\phi$ always finds a policy has following properties:

\begin{itemize}
\item{\bf Equal distant.} 
The composite policy must be at an equal distance from both input policies. For
example, consider the input policies $P_S=(1, 4, 3, 2)$  and $P_D=(3, 1, 4, 2)$.
Then $P_{S,D}=(4, 3, 1, 2)$ is a fair composite policy as it is at a distance of $2$ from both the input policies.
Often, a fair policy is not unique; e.g., $P_{S,D}=(1, 3, 4, 2)$ is also a fair composite policy since it has equal distance of 1 from both inputs. 
\item{\bf Least distant.}
The composite policy is at a minimum distance from both input policies. 
In the above example, we
prefer $P_{S,D}=(1, 3, 4, 2)$ because it has least distance from the inputs.
\end{itemize}

\paragraph{Search Algorithm for Least-distant \& Equidistant Policy.}
When we use the Kendall tau distance function, the fair composite policy is 
at a distance of $d/2$ from the two input policies\footnote{If $d$ is an odd number, 
the composite policy is $\lfloor{d/2}\rfloor$ away from one input and $\lceil{d/2}\rceil$ 
from the other input.}, where $d = d(P_S,P_D)$ denotes the 
distance between the two input policies. 
Note that this simple algorithm guarantees the equal and the least distant properties
because the Kendall tau metric satisfies the triangle inequality; that is, $d(x,z)\le d(x,y) + d(y,z)$, when $x$, $y$, and $z$ are the filtering policies.

In our algorithm, we start from one of
the input policy and keep making $d$ ranking swaps (e.g., from $(1,2)$ to $(2,1)$) until 
we reach the other input policy. For example, consider that we have two policies $P_S=(1, 4, 3, 2)$ and
$P_D=(3, 2, 1, 4)$ which are at a distance of $4$. We can start from $(1, 4, 3, 2)$
and traverse the path by using a bubble-sort style swapping from left-to-right:
$(1, 4, 3, 2) \rightarrow (1, 3, 4, 2) \rightarrow (3, 1, 4, 2) \rightarrow (3,
1, 2, 4) \rightarrow (3, 2, 1, 4)$. Since our ideal policy is at a
distance of $d/2$ on this path, we can easily determine $P_{S,D}=(3, 1, 4, 2)$.

\input{chapters/algorithm}

Algorithm~\ref{algo:fair-comp} is a deterministic process that implements the
logic we described above. First, we assign the floored half of the Kendall tau distance
between $P_S$ and $P_D$ as the midpoint $dist=\lfloor d(P_S, P_{D}) / 2 \rfloor$ 
(line 2) which is our search target. Next, we assume $P_S$ as a start
point and start bubble-sorting swaps towards
$P_{D}$ (line 6-7). For
every swap of the adjacent elements in $P_{S, D}$, we decrement $dist$ by
$1$ (line 8). We stop the process, when we have done $\lfloor d(P_S, P_{D}) / 2 \rfloor$, 
where we fine the fair policy point $P_{S,D}$.

==> chapters/refutable-invoice.tex <==
%\subsection{Inflation Resistant Refutable Invoicing}
%\label{sec:refutable-invoice}

Refutable invoice is important for the payment systems. 
Intuitively, the work of a filter can be measured by the amount of traffic that has been filtered out for a duration of time. 
As Sekar and Maniatis argue in~\cite{ccsw11}, a verifiable source accounting system should verify not only the accurate amount of consumed resources but also their {\em necessity}. 
In our traffic filter application, however, it is hard to prove the necessity of filtered traffic because a malicious source network can always create unnecessary dummy packets that are indistinguishable from other packets to inflate the bandwidth usage and the invoice. 

\begin{table}[h]
\begin{threeparttable}
	\centering
	\caption{Memory footprint examples of four filter rule sets with two different rule set sizes and two types of rule distributions: concentrated (i.e., rules are adjacent) and dispersed (i.e., rules are widely separated).}
	\label{tbl:mem-footprint}
	\begin{tabular}{c c c}
		\toprule
		&\multicolumn{2}{c}{\textbf{Rule distributions}}\\
		\textbf{Number of rules}  & {concentrated} & {dispersed} \\
		\midrule
		% \hline
		%    300 & 50,432 B & 169,088 B \\
		300 & 50 KByte & 169 KByte \\
		% \hline
		%    3000 & 440,016 B & 1,632,816 B \\
		3,000 & 440 KByte & 1,633* KByte \\
		\bottomrule
	\end{tabular}
	\begin{tablenotes}
		\small
		\item * This only reflects the size of the runtime lookup table, and does not include the huge memory consumption (over 48 MB for 3000 rules) during the building phase of the lookup table.
	\end{tablenotes}
\end{threeparttable}
\end{table}
Instead, we propose a new metric as a proxy for the executed work of the \name filters. 
Our new invoice metric is composed of two values that are resistant to bandwidth inflation.
First, we use the {\em memory footprint} of filtering rules of the filtering task. 
The memory footprint is a proxy for the average lookup cost for each packet filtering operation. 
As we see in Table~\ref{tbl:mem-footprint}, different filtering policies with the same number of rules may have significantly different memory footprints (e.g., 3--4 times difference). 
Second, we also use the {\em expected bandwidth} that will be filtered by the installed rules that are {\em negotiated} during the initial negotiation between the two ISPs (see Step 1 in Figure~\ref{fig:overview}). 
Once the two values are measured, they are written in the contract, which is signed by the two ISPs and the \name enclave. 
Then the final metric for the executed work is the multiplication of the two values and the time duration of the filtering round; that is,
\begin{align}
\text{ExecutedWork} = ~&\text{FilterRuleMemFootprint}~\times\nonumber\\ 
&\text{EstimatedFilteredBandwidth} ~\times\nonumber\\ 
&\text{DurationOfFiltering}
\end{align}



==> chapters/sec-analysis.tex <==
\subsection{Set Intersection Attacks}
\label{subsec:security}

%\paragraph{Set Intersection Attacks.}
If the attacker is allowed to adaptively change his policy and make
observations for each candidate input policy it selects, then our algorithm is
susceptible to another class of attacks. Specifically, we know that for a
given pair of input policies, the size of anonymity set is fixed. Given a
$P_D$ that the attacker wants to recover, he can first send his $P_S$ and
observes resulting $P_{SD}$. Then the attacker can start doing adaptive
attack, where by it changes the $P_S$ to an equidistant $P_S$ from the first
observed $P_{SD}$. It then recovers all the corresponding $P_{SD}$. Once the
attacker has collected all possible $P_{SD}$, it performs an intersection of
all the anonymity sets to get the actual $P_D$.

As an example, lets say that the input policies are $(1, 4, 3, 2)$ which is
known to the attacker and $(3, 4, 2, 1)$ which is the policy that the attacker
wants to learn. When the algorithm executes for the first time, it selects
$(3, 1, 4, 2)$ as the composite policy. Figure~\ref{fig:eg2} shows the 
sub-graph  of the polyhedron for this composition. After the first run, the
attacker's anonymity set comprises of $(3, 4, 2, 1), (3, 2, 1, 4)$ which
satisfy the constraints of being at a distance of $2$ from input $(1, 4, 3,
2)$ and at a distance of $1$ from the mid-point policy $(3, 1, 4, 2)$. To
learn which of these policies is the one that was given by the victim, the
attacker adapts it input. Specifically, it choses one of the polices from the
anonymity set as the new input policy. Lets say in this case, it choses $(3,
4, 2, 1)$ as its new policy. The algorithm now as to compute the composition
of attacker chosen policy $(3, 4, 2, 1)$ and victim's policy $(3, 4, 2, 1)$,
which results in $(3, 4, 2, 1)$ being the new composite policy. As soon as the
attacker observes that the new $P_{SD}$ is the same as the one it chose
adaptively, it knows that the victim has the exact same policy.  On the other
hand, if the attacker had chosen  $(3, 2, 1, 4)$ as its new adaptive input
policy, the algorithm would generate $(3, 1, 4, 2)$ as the new $P_{SD}$ which
is the same as the original composite policy. This would have told the
attacker that the it is not the victim's  policy, which in turn would have
implied that the other policy in the anonymity set (i.e., $(3, 4 , 2, 1)$) is
the victim's policy.

% \paragraph{Generic Attacks.}
% So far, we have assumed that the attacker (source ISP or destination ISP)
% knows the composite policy $P_{s,d}$ computed by any one of our algorithms.
% Here we show how this is possible. We know that each class in the order-based
% policy comprises of IP addresses. When the middlebox sees a packet, it first
% identifies which class the packet belongs to and then refers to the composite
% policy to probabilistically decide whether to drop or keep the packet. The
% rate of dropping a packet is directly defined by the rank of that packet's
% class in the policy.  The attacker knows that the output rate of the packets
% being transmitted is capped to a $L$ bps  pre-specified and known to both the
% ISPs.

% If the source ISP is the attacker, it controls the types and number of packets
% it can deliver to the middlebox. To learn the composite policy, the source ISP
% starts adaptively pre-filtering the traffic it sends to the middlebox.
% Specifically, it starts filtering all the traffic and floods the middle box
% only say 2L packets which belong to one class $C_3$ whose class rate is
% $P_{C_3}$. The middlebox consults the policy and drops $(2L) * (1 - P_{C_3})$
% of the input packets. The attacker measures the number of total packets that
% are being forwarded which is $(SL) * P_{C_3}$. The attacker can easily reverse
% engineer that the class-rate for $C_3$ is $P_{C_3}$. The attacker can repeat
% this process for all the traffic classes and learn all the $P_{C_i}$. This
% directly leaks the composite policy $P_{s, d}$ being deployed by the middlebox.








==> chapters/tesef_details.tex <==
\subsection{Deployment Example}
\label{sec:deployment-example}

%\msk{End-to-end deployment?}

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.40\textwidth]{figures/overview-sigcomm.pdf}
	\vspace{-5pt}
	\caption{A deployment example of \name. (NOC: Network Operations Center, RPKI: Resource Public Key Infrastructure, and IAS: Intel Attestation Service.)}
	\vspace{-15pt}
	\label{fig:overview}
\end{figure}

Figure~\ref{fig:overview} shows an example deployment scenario.
%Here is a summary of the scenario in multiple steps. 
%s found in : % in Section~\ref{sec:architecture-overview}.
%The eight steps are explained as follows:

% Figure~\ref{fig:steps} illustrates the steps needed to establish trust between $S$ and $D$ with the \name system:
% \begin{figure}[h]
% 	\noindent\fbox{\begin{minipage}{\columnwidth}
% 			\footnotesize
			\begin{packedenumerate}
				\item[(1)] {\bf Secure channel establishment:} $D$ contacts $S$ via an out-of-band channel to establish a secure channel.
				They rely on the RPKI infrastructure to authenticate each other.
				$D$ may choose the direct origin of the source IP address it wants to filter or the immediate one-hop upstream of the origin. 
				\item[(2)] {\bf Contract parameter negotiation:} $S$ and $D$ negotiate on  high-level parameters (e.g., pricing, bandwidth limit) in one or more rounds of message exchanges.
				\item[(3)] {\bf Enclave creation:} $S$ creates a enclave for a traffic filter and obtains the enclave quote from quoting enclave. 
				For scalable filtering bandwidth, $S$ may create multiple enclaves as described in Section~\ref{sec:optimization-multiple-enclaves} and \ref{sec:attestation-multiple-enclaves}. %; see Section~\ref{sec:data-plane-design}.
				\item[(4)] {\bf Attestation:} $S$ contacts the IAS and verifies the attestation report.
				\item[(5)] {\bf Attestation report sharing:} $S$ sends the attestation report to $D$ so that it can verify the report locally.
				\item[(6)] {\bf Policy submission:} Both $S$ and $D$ submit their filtering policies to the policy calculation logic. A final policy is computed  inside the enclave.
				\item[(7)] {\bf Packet filtering:} The filter in the enclave is activated and traffic destined to $D$ is routed to the filter. 
				\item[(8)] {\bf Refutable invoice:} The amount of the executed work is sent to $S$ and $D$.
			\end{packedenumerate}
% 	\end{minipage}}
% 	\caption{The \name's steps.}
% 	\label{fig:steps}
% \end{figure}

%\msk{The full end-to-end deployment in Appendix?}

% \paragraph{Secure channel establishment (Step 1):} 
% When $D$ detects a volumetric DDoS attack, it first identifies the IP addresses/prefixes that it wishes to rate limit (e.g., via NetFlow analysis~\cite{netflow}). 
% Then, $D$ determines one or more source ISPs that it wishes to install traffic filters. 
% $D$ may contact the owners of the detected IP addresses/prefixes or their immediate upstream ISPs. 
% The ownership of IP prefixes and the peering relationship can be obtained from various public database (e.g., RPKI~\cite{rpki}, RIPE~\cite{ripedb}, PeeringDB~\cite{peeringdb}). %  infrastructure and the peering relationship can be obtained from various public peering database, such as PeeringDB}.


% Then, $D$ contacts one or more willing source ISPs and establish secure point-to-point channels with them independently. 
% Consider $D$ (with a RPKI public key $K_D$) creates a channel with a willing ISP $S$ (with a RPKI key $K_S$).
% $D$ may directly contact via $S$'s contact information found in the public database (e.g., $S$'s RIPE record often lists email addresses).
% Alternatively, $D$ can publicly announce that it wishes to establish a filtering contract with $S$ in one or more well-known public bulletin boards, network administrator forums, regional network operator group's mailing list (e.g., NANOG mailing list), or highly available web platform (e.g., IPFS\footnote{\url{https://ipfs.io/}}). 
% %In either case, $D$ needs to attach its RPKI  key signature. 
% Then, a wiling $S$ can respond with its own RPKI signature to begin the channel establishment. 
% Similar to other X.509 certificates, RPKI can be used to establish an ephemeral session key between $S$ and $D$ within a few of interactions (e.g., TLS key exchanges~\cite{rfc5246}).

%\paragraph{Assumptions.}
In this example, we assume both source and destination ISPs participate in a common public key infrastructure (PKI) system that binds their AS numbers and IP addresses.
In this paper, we consider the use of the Resource Public Key Infrastructure (RPKI)~\cite{lepinski2012infrastructure} for the origin authentication of ISPs~\cite{rpki}; see Section~\ref{sec:multiple-session-rpki} on how this assumption affects the effectiveness of \name defense. 
We also assume the Internet connectivity of a network operations center (NOC) of an ISP even when it is under DDoS attack.
It is based on the observation that ISPs traditionally have maintained out-of-band channels (e.g., external email servers, telephone lines~\cite{dots-slides}) and ISPs contact other ISPs when hit by large-scale DDoS attacks for manual collaboration defense schemes (e.g., large-scale ISP coordination during the ProtonMail attack~\cite{protonmail}).
Completely independent out-of-band channels, such as cellular Internet connectivity, can be also assumed for the NOCs' backup connectivity during the worst DDoS attacks.


%
%
%
%There are multiple ways: (1) $D$ may rely on some reputable public databases (e.g., RIPE database\footnote{\url{https://www.ripe.net/manage-ips-and-asns/db}}) to obtain the contact information (e.g., email address) of source ISPs
%$D$ may directly sends the initial messages to the contacts in the public RPKI  database \msk{details?}. 
%Or, we can imagine one or more reliable bulletine boards that ISPs can send and receive messages (perhaps openly). 
%
%Secure channel, session key.



% a realistic assumption is the alternative communication line at NOCs. 
%
%$D$ first attempts to make contact with $S$ through the open Internet. For example, anyone can find ISPs contact details in public database such as RIPE\cite{ripe}. Taking these open contact as a starting point, $D$ and $S$ makes a key exchange following the standard protocol (e.g., Diffie-Hellman\cite{}) to create a emphemeral session key for encrypted communication. Also, Their RPKI resource certificates are used to authenticate each other, avoiding any impersonation by attackers or non-ISPs. After the key exchange and authentication, $S$ and $D$ can use the established channel for exchanging information that should be kept private between them.

% \paragraph{Parameter negotiation (Step 2):}. 
% $S$ and $D$ negotiate on the contract parameters. We outline the three parameters: {\bf\em f}, {\bf\em p}, and {\bf\em t}. {\bf\em f} specifies the range of the traffic that should be filtered, which describes IP-prefix level traffic originating from $S$ and destined to $D$. 
% This corase-grained traffic description is sufficient for negotation and more detailed filtering rules will be exchanged privately only after when \name enclave is launched. 
% {\bf\em p} is a pricing rate and will be used in $D$'s payment to $S$ and {\bf\em t} sets a time limit for \name contract and \name filter.
% %   

%<<<<<<< HEAD
% \begin{figure}[h]
%    \begin{framed}
%        \raggedright
%        $\mathrlap{\mathbf{f}}\hphantom{\mathbf{M}}$:  maximum range of the traffic to be filtered. \\
%        $\mathbf{m}$:  maximum inbound rate that counts in the bill. \\
%        $\mathrlap{\mathbf{l}}\hphantom{\mathbf{M}}$:  maximum outbound rate that $F$ should be reduced to. \\
%        $\mathrlap{\mathbf{p}}\hphantom{\mathbf{M}}$:  price that $S$ charges $D$ for the traffic removed. \\
%        $\mathrlap{\mathbf{t}}\hphantom{\mathbf{M}}$:  contract expiration time
%    \end{framed}
%    \caption{\name contract parameters\msk{a table would look better?}}
%    \label{fig:contract-param}
% \end{figure}

%\begin{table}
%\small
%  \caption{\name contract parameters}
%  \label{tab:contract-param}
%  \begin{tabular}{ cl }
%    \toprule
%    % \hline
%    % \multicolumn{2}{c}{\name contract parameters} \\
%    {\bf \em f} & maximum range of the traffic to be filtered \\
%%    {\bf \em m}& maximum inbound rate that counts in the bill \\
%%    {\bf \em l} & maximum outbound rate that $F$ should be reduced to \\
%    {\bf \em p} & price that $S$ charges $D$ for the traffic removed \\
%    {\bf \em t} & contract expiration time \\
%    \bottomrule
%  \end{tabular}  
%\end{table}
%
%\paragraph{Enclave creation and remote attesattion (Step 3, 4, 5):}. In preparation for proceeding the contract, $S$ is responsible for launching the auditable \name filter within its network, and presents $D$ with a proof - the \textit{attestation report} that obtained from IAS after the remote attestation. First, $S$ launches the \name filter's enclave ($E$), and then asks the quoting enclave for a special data structure called \textit{quote}, which collects the information regarding $E$'s creations including but not limited to: the secure \textit{measurement} over the enclave loading process, the enclave \textit{certificate} issued by its author and the \textit{user data} such as a fresh symmetric key pair generated inside the enclave.
%%=======
%%\begin{figure}[h]
%%    \begin{framed}
%%        \raggedright
%%        $\mathrlap{\mathbf{F}}\hphantom{\mathbf{M}}$: The maximum range of the traffic to be filtered. \\
%%        $\mathbf{M}$: The maximum inbound rate that counts in the bill. \\
%%        $\mathrlap{\mathbf{L}}\hphantom{\mathbf{M}}$: The maximum outbound rate that $F$ should be reduced to. \\
%%        $\mathrlap{\mathbf{P}}\hphantom{\mathbf{M}}$: The price that $S$ charges $D$ for the traffic removed. \\
%%        $\mathrlap{\mathbf{T}}\hphantom{\mathbf{M}}$: The contract expiration time
%%    \end{framed}
%%    \caption{\name contract parameters}
%%    \label{fig:contract-param}
%%\end{figure}

% \paragraph{Enclave creation and remote attestation (Step 3, 4, and 5):}. 
% %In preparation for proceeding the contract, $S$ is responsible for launching the auditable \name filter within its network, and presents $D$ with the proof --- the \textit{attestation report} that can be obtained from IAS after the remote attestation. 
% First, $S$ launches the \name filter's enclave ($E$), and then asks the quoting enclave for a special data structure called \textit{quote}, which collects the information regarding $E$'s creations including but not limited to: the secure \textit{measurement} over the enclave loading process, the enclave \textit{certificate} issued by its author and the \textit{user data} such as a fresh symmetric key pair generated inside the enclave.
% %
% The quoting enclave is a trusted component developed by Intel and running on the same hardware as part of the SGX platform service. It owns a EPID~\cite{brickell2009enhanced} member private key whose signature can only be verified by Intel with the corresponding EPID group public key. $S$ has to sends the quote to IAS in exchange for the {\em attestation report} to convince $D$ about the prepared \name filter. This report has IAS's signature so that $D$  can verify the report and ensure the untampered \name filter running on a trusted hardware and $E$'s public key for identifying it.

% \paragraph{Policy composition and execution (Step 6 and 7):} 
% The \name filter receives two policies \PS and \PD from $S$ and $D$, respectively. 
% $S$ and $D$ signs their policies with their RPKI private keys and encrypt them with $E$'s public key.
% The specifications of policies \PS and \PD are negotiated between $S$ and $D$, and we make no assumption on their types.
% $S$ and $D$ agree on the composition algorithm that combines \PS and \PD into \PSD.
% %When two policies have conflicting rules, the algorithm has to resolve them and create a reconciled rule. 
% %For example, when $S$ wishes to allow packet $x$ but $D$ wishes to block it, the algorithm decides the final rule that is actually implemented. 
% The specific algorithm that determines the composition (e.g., perfectly fair reconciliation) is also determined during the negotiation. %; see Section~\ref{}. 

%\begin{figure}[t!]
%	\centering
%	\includegraphics[width=0.4\textwidth]{figures/metering.pdf}
%	\caption{An example of the metering}
%	\label{fig:metering}
%\end{figure}

% \paragraph{Refutable invoice (Step 8):} 
%$S$ receives direct payment from $D$ for the amount of filtering work (e.g., volume of traffic that has been removed). 
% We rely on the enclave $E$ for metering the amount of traffic removed by the filter since neither $S$ nor $D$ can convince the other side regarding this measurement. 
% The invoice is created inside the enclave $E$ and sent to the source ISP. 
% The source ISP then can use this as the invoice claim for the task requested by the destination and requests compensation via an external payment channel. %; see Section~\ref{}.
%$D$ is required to transfer enough funds to $E$' wallet $W_E$ as the deposit and let $E$ make the direct payment fully according to the actual work it measured during the operation. 
%Three paramters ({\bf\em m}, {\bf\em l}, {\bf\em p}) in the contract affect the payout as well as the actual incoming rate towards the \name filter. The measurement is made as follows: only the moment when the incoming rate is between {\bf\em l} and {\bf\em m} counts towards the final summary and any rate over {\bf\em m} is capped at {\bf\em m} and any rate below {\bf\em l} is not considered. 
%Figure~\ref{fig:metering} illustrates this: the shaded area in  is the actual work admitted by $E$ given that the curve is the actual incoming rate variation. 
%The final payment to $D$ is the product of this quantity and the price $P$.
%
%To efficiently realize this guaranteed payment mechanism, as an example, we use a cryptocurrency for the deposit and the payout. 
%Let us consider that $W_S$, $W_D$, and $W_E$ are the cryptocurrency addresses. 
%Particularly, $W_E$ is a fresh address securely generated inside the \name enclave. 
% example of showing the automatic and guaranteed payment, the digital coins such as Bitcoin really show the benefits in terms of safety, digitalization and transparency. Before making any Bitcoin trasancation, $S$, $D$ and $E$ need to generate its own wallet address (equivalently a pair of public key and private key) in private to either accepts the payment or holds the balance safely. And, they also identify each other wallet address by signing the wallet address with the RPKI public key ($S$ or $D$) or the newly generated but verified key ($E$).
%
%$D$ first makes a transaction to $W_E$ with sufficient deposit in order to convince $S$.
%This transaction (Step 6') is locked (e.g., Bitcoin's \texttt{nLockTime}\cite{nlocktime}) so that the deposit can be automatically refunded to $D$ when $E$ does not make the payout (e.g., $E$ is destroyed or blocked) by the time deadline set by $S$. 
%
%However, to complement the fund safety, before any transaction happens, $E$ first construct a \textit{promised} transaction (implemented by setting the parameter \texttt{nLockTime}\cite{nlocktime}) that cannot be included in the blockchain before time $T$.
%This trasancation acts as a fail-safe mechanism that guarantees $D$'s control of the deposit after time $T$.
%%that making a deposit transaction to $E$ has no risks such as deposit being buried on the blockchain due to $E$ being terminated accidentally (no one can spend the money).
%Note that this promised transaction is needless to be published immediately by $E$ after signing the trasaction. Instead, it is sent to $D$ in exchange for $D$'s deposit transaction.
%
%Once $S$ finds the deposit transaction, the traffic $F$ is redirected to $E$ for filtering and any work done by the \name filter is correctly measured.
%Eventually before time $T$, $E$ will make one public transaction to arrange the payment to $S$ and refund $D$ at the same time.
%If anything unexpeted happens and $E$ could not publish the final transaction, $D$ may consider that $S$ is not running \name filter accordingly and advertise the promised trasaction to get its money back.



==> chapters/trust-establishment.tex <==
\section{\name: A Source Filtering System}
\label{sec:overview}

In this section, we introduce a new source filtering system, called \name\footnote{\name stands for `Trust Establishment for Source-end Filtering.'}, and overview its architecture focusing on the high-level goals it is designed to achieve and the considered threat model. 













%We do not consider the denial-of-service attack against the underlying blockchain overlay network (e.g., flooding the majority of 32,000 Ethereum nodes distributed across thousands ASes\footnote{AS distribution of Ethereum nodes from \url{https://www.ethernodes.org/network/1}. \msk{TODO.}}), which would involve much larger DDoS attacks than the attack we handle in this paper.


%\subsection{Desired Properties of \name}
%We summarize the remaining key technical challenges to achieving the two desired properties for the \name's vision.
%In the rest of this paper, we focus on the following properties:
%
%\begin{itemize}
%	\item {\bf Scalable and indirect contract establishment (\S\ref{sec:econ-incentive}). }	
%	To handle large numbers of pairwise filtering contract between many ISPs we design a compact \name contract.
%	We minimize the number of on-chain transactions and the estimated gas of the contract by a lightweight contract design.
%	We show that we can support xx thousand pairwise contracts concurrently, which only amount to less than yy percent of gas allowed per block. 
%	We also design an indirect smart contract structure that removes direct inter-ISP message exchanges when establishing contracts in the middle of flooding attacks. 
%
%
%	\item {\bf Scalable line-rate data-plane design (\S\ref{sec:data-plane-design}). }	
%	The \name enclave should support line-rate data-plane performance while conducting per-packet secure processing.
%	Moreover, when the attack volume from $S$ and $D$ exceeds the bandwidth capacity of a single \name enclave (e.g., 10 Gb/s), \name must be extended with parallel \name enclaves and handle large volume traffic (e.g., 60 Gb/s or higher) while preserving the same level of security guarantees.
%\end{itemize}

\input{chapters/tesef_details}


==> figures/attack-overview.tex <==

\tikzstyle{function} = [circle, draw, dashed, text width=2em, text badly centered, inner sep=0pt]
\tikzstyle{block} = [rectangle, draw, 
text width=2em, text centered, minimum height=1em]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{attack} = [draw, -latex', color=red]

\begin{figure}[th]
    \centering
    \begin{tikzpicture}[node distance = 5em, auto]
        % Place nodes
        \node [block] (ps) {$P_S$};
        \node [block, below of=ps, node distance=3em] (pd) {$P_D$};
        \node [function, right of=ps, yshift=-1.5em] (phi) {$\phi$};
        \node [block, right of=phi] (psd) {$P_{S, D}$};
        \node [function, right of=psd] (psi) {$\psi$};
        \node [block, right of=psi] (rl_param) {$c_i, r_i$};
        \coordinate [below of=psi, node distance = 1.5em] (A1);
        \coordinate [left of=phi, node distance = 2em] (A2);
        \coordinate [below of=phi, node distance = 1.5em] (A3);
        % % Draw edges
        \path [line] (ps) -- (phi);
        \path [line] (pd) -- (phi);
        \path [line] (phi) -- (psd);
        \path [line] (psd) -- (psi);
        \path [line] (psi) -- (rl_param);
        \path [attack] (rl_param) .. controls (A1) .. node[below]{(1) learn $P_{S, D}$} (psd);
        \path [attack] (ps) .. controls (A2) .. (pd);
        \path [attack] (psd) .. controls (A3) .. node[below]{(2) learn $P_D$} (pd);
    \end{tikzpicture}
    \caption{Adversary $S$ inferring $D$'s policy}
    \label{fig:attack-overview}
\end{figure}

==> paper 2/Makefile <==
export TEXINPUTS:=.:formatting:$(TEXINPUTS)

CROSSTEX := crosstex
CROSSTEX_ARGS := --titlecase lower --add-in --short=author --short=conference

BIBTEX   := bibtex

FIGFIGS :=
EPSFIGS := 
PNGFIGS :=
PDFFIGS :=
SVGFIGS := 
GNUPLOTFIGS :=
FIGS    := $(FIGFIGS) $(EPSFIGS) $(PDFFIGS) $(SVGFIGS) $(GNUPLOTFIGS) \
           $(PNGFIGS)

TEX_SOURCES := paper.tex 

.SUFFIXES:

all: 
	pdflatex -shell-escape paper
	bibtex paper
	pdflatex -shell-escape paper
	
pdf: paper.pdf

commit: 
	git commit -m "Added stuff" -a
	git push origin master


spell: $(TEX_SOURCES)
	detex $^ | spell | env LANG=C sort -u | env LANG=C comm -23 - ok-words

clean:
	rm -f *~ *.log *.bbl *.dvi paper.pdf *.blg *.aux *.ps *.out


==> paper 2/algo/inference-attack.tex <==
\begin{algorithm}[t]
	\footnotesize
	\caption{\PSD Inference Attack}
	\label{algo:class-boundary-search}
	\begin{algorithmic}[1]
		\Function{InferenceAttack}{}
		\State $C \gets$ SearchClassBoundary()
		\State $R \gets$ MeasureAverageRates($C$)
		\State \Return $C$, $R$
		\EndFunction		\Function{SearchClassBoundary}{}
		\State $U \gets \{0, 1\}^H, C \gets \emptyset, R \gets \emptyset$
		\While{$|U| > 0$}
		\State $h \overset{\$}{\gets} U$, $C \gets c \cup C$, $c \gets$ FindClass($h$), $U \gets U - c$
		\EndWhile
		\State \Return $C$
		\EndFunction
		\Function{FindClass}{$h$}
		\State $b \gets 0$                              \Comment{bitmask}
		\For{$i \gets 0$ to $H-1$}
		\State $h' \gets h \mathrel{\oplus} 2^i$    \Comment{flip the bit (bitwise xor)}
		\If{PairwiseFlooding($h$,$h'$) $= 1$}
		\State $b \gets b \mathrel{|} 2^i$      \Comment{mark the bit (bitwise or)}
		\EndIf
		\EndFor
		\State \Return $c \gets \{x | \text{ $x$ is coverd by header $h$ and mask $b$} \}$
		\EndFunction
		\Function{MeasureAverageRates}{$C$}
		\State $R \gets \emptyset, W \gets \emptyset$
		\State select a random class $c_0$ from $C$ \Comment{choose the reference class}
		\For{each class $c_i$ in $C$}
			\State choose a random header $h_i$ from $c_i$, $h_0$ from $c_0$
			\State $w_i \gets \textrm{PairwiseFlooding}(h_0, h_i)$
			\State $W \gets W \cup \{w_i\}$
		\EndFor
		\State $w_{\textrm{total}} = \sum\nolimits_{w_i \in W} w_i$
		\For{each class $w_i$ in $W$}
			\State $R \gets R \cup \{\frac{w_i}{w_{\textrm{total}}}L\}$ \Comment{$L$ is the total throughput limit}
		\EndFor
		\State \Return $R$
		\EndFunction
		\Function{PairwiseFlooding}{$h$,$h'$}
		\State Flood with packets of header $h$ and $h'$. Measure their rates $m$ and $m'$.
		\State \Return $\frac{m'}{m}$
		% \If{$m = m'$}
		% \State \Return True
		% \Else
		% \State \Return False
		% \EndIf
		\EndFunction		
	\end{algorithmic}    
\end{algorithm}

==> paper 2/chapters/1intro.tex <==
\section{Introduction}
%
%In spite of extensive efforts (e.g.,~\cite{mirkovic2004taxonomy,moore2006inferring,parno2007portcullis}), distributed denial-of-service (DDoS) attacks continue to plague the Internet.  
Over the last few years, we have observed an escalation in {\em volume} of DDoS attack
%traffic; e.g., four times increase in the last three years~\cite{computerworld2013biggest,guardian2016ddos}. This stems from a growing attack-defense cost asymmetry --- generating attack
%traffic now costs much lesser than buying bandwidth to absorb it~\cite{kang2016defending},
%given the proliferation of attack sources (e.g., IoT devices~\cite{guardian2016ddos}).
During a volumetric attack, a victim autonomous system (AS) is flooded with unmanageably large svolume of packets to process.  
A primary defense against DDoS today is {\em filtering} (or blocking) of packets at the destination AS or {\em outsourced} filtering at third-party networks (e.g., cloud-based scrubbing).
%Unlike application-layer DDoS attacks that surgically target a
%particular resource of a targeted server, 
Volumetric attacks
congest bandwidth resources of targeted servers, their networks, and often
one or more of their upstream ASes~\cite{arbornetwork2016}.
Thus, by their very nature, defenses against volumetric attacks often demand {\em inter-domain collaboration} for filtering packets.
In fact, collaborative filtering has long been practiced via manual, on-demand interaction between administrators of ASes~\cite{dots-working-group}.  
Recently, there have been increasing interests in inter-domain collaborative filtering by major carriers (e.g., AT\&T and CenturyLink's collaborative filtering system~\cite{levy2017operationalizing}), a standards organization (e.g., IETF's DOTS~\cite{dots-use-case-7}), and equipment manufacturers (e.g., Huawei's Cloud Clean Alliance~\cite{}).
%
%two large ASes in the
%US\,---\,AT\&T and CenturyLink\,---\,have proposed a systematic,
%automated collaboration system for DDoS mitigation based on their
%institutional trust and pre-negotiated policies~\cite{levy2017operationalizing}.  
%An IETF standard working group called
%the DDoS Open Threat Signalling group (or DOTS) is working on a
%proposal for collaboration between two adjacent ASes with direct peering
%relationships~\cite{dots-use-case-7}.
%Some network equipment manufacturers advocate collaborative filtering among more than two ASes with a trusted third party that orchestrates large-scale DDoS mitigations (see Huawei's Cloud Clean Alliance~\cite{}).

%\paragraph{Source-end filtering.} 
Ideally, inter-domain collaboration is {\em most} effective when an attack-targeted destination AS {\em directly requests} a source AS, which hosts suspicious traffic, to filter suspicious or unwanted packets.  
Such {\em source-end filtering} has
clear technical and economical benefits: (1) it can significantly
reduce the bandwidth waste (thus cost saving for participating ASes) for
suspicious packets that would otherwise unnecessarily traverse to
downstream ASes; (2) ASes near the sources see lower traffic volume
than the destination ASes and thus can perform more complicated,
resource-demanding filtering operations (e.g., finer-grained rate
limiting); and (3) some local contexts about the traffic sources
(e.g., list of historically poorly protected client machines) can be utilized for better DDoS mitigation.  Many prior work has already highlighted these
benefits of source-end filtering~\cite{huawei-CCA,mirkovic2002attacking, liu2008filter,
  alwabel2015senss,zargar2013survey}.


Despite its advantages, however, source-end filtering has {\em not} found
wide-scale deployment due to the security and incentive problems. First, two ASes may
be {\em mutually distrusting} because they are likely to have no direct business relationship. 
Outsourcing filtering operations between untrusted ASes may pose some
security issues; e.g., a source AS may falsely claim that it is performing the 
requested filtering operation correctly, or, it may leak the filtering policy submitted by the destination AS, which may include sensitive information about the destination AS. 
Second, even if two ASes somehow establish some level of trust, there exist
{\em no explicit incentive} for the source ASes to perform filtering operations, which 
incur non-negligible costs, solely on behalf of other ASes. 
Moreover, even if the source AS somehow finds incentive to help (or decided
to be altruistic), it may find some clear risks of being criticized for dropping its own customers' packets without any evidence of congestion in its network, which further disincentivizes such filtering operations. 


\smallskip
%\paragraph{Secure Collaborative Source-End Filtering.} 
In this paper, we propose a novel collaborative source-end filtering framework (which we call {\em \name}) that, perhaps surprisingly, demonstrates that we can effectively filter suspicious or unwanted packets during DDoS attacks while providing {\em strong incentives} to the source AS (which actually performs packet filtering) and nicely handling potential attacks between the {\em mutually-untrusted} source and destination ASes.
Unlike most, if not all, source-end filtering proposals that {\em outsource} the filtering functionality of a destination AS to a source AS, \name requires {\em mutual participation} from two ASes for determining the final filtering policy that is impartial to the both participating ASes.
To be specific, {\em both} the destination and source ASes submit their packet filtering policies to the {\em filtering function} located in the source AS (let us consider a logical function until we clearly define it later). 
Then the filtering function combines the two policies to create and enforces the final policy for filtering packets from the source AS to the destination AS. 

\name can offer unprecedentedly strong {\em incentives} to source ASes becuase it allows a source AS to explicitly control the filtering policy when a remote destination AS is experiencing congestion. 
In existing DDoS mitigation, source ASes are {\em not} allowed to participate in a packet filtering decision but to solely rely on the destination AS's discretion (or cloud scrubber's decision) on which packets should be dropped when congestion occurs. 

%
%\smallskip
%\paragraph{Necessary security properties.}
\name also offers strong {\em security guarantees} against potential attacks between the untrusted ASes:
%\begin{enumerate}
%\item[(1)] {\bf Verifiably fair policy composition and enforcement.}
(1) \name guarantees the {\em verifiably fair policy composition} between untrusted ASes. 
%When the two independently-generated policies are combined, the final composed filtering policy should be a {\em fair} policy between the two. 
%To be specific, two policies may have rules that are conflicting (or even contradictory) to each other and thus both cannot be included in the final policy. 
The \name's policy composition logic guarantees that the final policy is determined as the middle ground between the two, which favors neither parties.
Moreover, \name allows two ASes to verify whether the policy composition is fairly composed and enforced; 
%
%\item[(2)] {\bf Negotiable privacy guarantees.}
(2) \name enables two ASes to {\em negotiate} the desired level of {\em privacy guarantees}. 
Network filtering policies are inherently sensitive information (e.g., policies may include information about private contracts, private white/black policies, or even vulnerable points of the networks) and thus any excessive policy leakages can be detrimental to their businesses. 
In \name, two ASes negotiate the desired upper-bound of the privacy leakage for their policies before they start filtering packets; and
%In particularly, the ASes should be able to sdecide the upper-bound of policy leakages (e.g., minimum anonymity set size) during the negotiation stage. 
% the minimum guaranteed degree of anonymity (e.g., anonymity set size) for the given two policies based on the inherent fairness-anonymity {\em trade-off}\,---\,that is, fairness must decrease to increase the degree of anonymity of the policies. 
%
%\item[(3)] {\bf Effective bypass detection.}
(3) \name effectively {\em detects any circumvention} attempt by source ASes.
A source AS may try to bypass the filtering function outside of the \name system; e.g., detour the \name system via rerouting.
The \name's detection is fast and accurate (e.g., extremely low false alarm rates).  
%\end{enumerate}


To make \name practical for mitigating large-scale DDoS attacks in today's Internet, we utilize several emerging secure hardwares capabilities and network management techniques available for commodity server platforms.  
First, we utilize a {\em trusted execution environment} (TEE) capability available in many CPUs for commodity servers (e.g., ARM TrustZone, Intel SGX).
With the TEE support, \name offers {\em isolated executions} for the filtering operations, protecting them from a potentially malicious source ASes. 
Second, to make it practical for backbone operations (e.g., 10--100 Gb/s packet filtering) with dynamic bandwidth provisioning at a low operational cost, we take advantage of {\em software-defined networking} (SDN) and {\em network functions virtualization} (NFV), which already have been embraced by major industry players (e.g., Verizon, AT\&T)~\cite{1,1,1,1}.

\smallskip
\paragraph{Challenges.} 
However, there are two main practical challenges that need to be addressed to realize a secure and practical defense mechanism with these emerging security and network capabilities:
\begin{enumerate}
	\item {\bf Fairness and privacy dilemma.} 
	First, there exists an undesirable, inherent trade-off between the fairness of policy composition and the privacy guarantees for the input policies. 
	Thus, it is fundamentally hard to achieve both the fairness and privacy of policies. 
	Worse yet, finding a right balance between them is non-trivial.
	Therefore, it is highly desired to build a negotiation protocol that guarantees quantifiably reasonable fairness and privacy bounds for practical operations between two mutually untrusted ASes.
	
	\item {\bf Secure and fast packet processing rate.} 
	Second, the desired security properties require heavy security checks for large volume of traffic.
	Particularly, for bypass detection, per-packet checks in the secure processor become necessary.
	However, such heavy use of secure processors makes it hard to achieve line-rate (e.g., 10s or 100s Gb/s) packet processing in commodity computing platforms.
	
\end{enumerate}

In this paper, we focus on how the TEE-based \name design can address these practical challenges. 
To address (1), \name analyzes the fairness-anonymity trade-off for a selected generic policy language and then presents a negotiation protocol that draws up an agreement on the balanced fairness-anonymity point between two untrusted parties. 
Moreover, to address (2), \name carefully designs the per-packet security checks to minimize the secure/non-secure-world context switching and achieves the near zero-copy operation for line-rate packet processing. 



Seen in a broader network security context, \name is a unique proof point that answers the question ``What is the emerging trusted hardware capability good for Internet security?'' in a wide-area context beyond simple trust extensions to existing distributed applications; e.g.,~\cite{kim2017enhancing,han2017sgx}.
Specifically, \name's TEE-based verifiably fairness, negotiable privacy guarantees, and circumvention detections form the basis for the first secure and practical source-end filtering against volumetric DDoS attacks.   
In the scope of this paper, \name demonstrates the first trusted collaborative filtering only between two ASes; yet, this design philosophy can be easily applied to existing systems (e.g.,~\cite{att}) and protocols (e.g.,~\cite{dots-working-group}), and extended to multiple-AS collaboration platforms (e.g.,~\cite{huawei}).


%TEE capabilities (e.g., isolated executions, remote attestation) of \name enable the two ASes to verify the \name's guarantees (i.e., fair policy composition, negotiated degree of privacy) and to detect bypass attacks.
%However, building an effective TEE based filtering system poses several design challenges. 
%First it requires the rigorous evaluation of privacy leakage of the submitted filtering policies based on adversary's capabilities/strategies and the fairness notions. 
%To be specific, the trade-off between the fairness of the policy composition and the degree of anonymity of the input policies need to be clearly analyzed for different policy definitions (e.g., simple allow/block rule sets, prioritized flow lists). 
%In addition, we should develop attacks that maximize the privacy leakages of the policies and demonstrate their feasibility and effectiveness. 
%
%Furthermore, designing a TEE based collaborative filtering system entails several non-trivial architectural challenges. 
%Particularly, achieving line-rate packet processing (e.g., rate limiting per traffic class, per-packet bypass detection) with per-packet verification operations by securely executed functions in the secure world seems non-viable due to the expected significant context switching overheads. 


\smallskip
\paragraph{Contributions.}
In this paper, we have the following contributions:
\begin{enumerate}
	\item Identify the security and incentivization problems of source-end outsourced filtering.
	\item First proposal. Fair collaboration. that offers new control to source networks.
	\item TEE based design for verifiably fair policy composition.
	\item Privacy guaranteed negotiation. Attacks. Tradeoff.
	\item Accurate and efficient bypass detection. Line rate. 
	\item SDN/NFV implementation. 
\end{enumerate}


==> paper 2/chapters/3attack.tex <==
\section{Privacy Negotiation between Untrusted Autonomous Systems}
\label{sec:privacy}
In \name, there exist clear concerns for privacy when a destination AS hands over its own filtering policy to another untrusted AS~\cite{levy2017operationalizing}. 
Inherently, some filtering policies of an AS can be privacy-sensitive information that can be abused if they are leaked to other untrusted ASes. 
Filtering policies may include information about private contracts (e.g., which customer networks are `premium' subscribers), proprietary algorithms (e.g., mechanisms that prioritize certain services over the others when under congestion), internal white/black policies (e.g., usual suspects, mission-critical services), or even the vulnerable points of the networks (e.g., which links or subnetworks are under attacks).
In this section, we discuss how \name implements strong privacy mechanism that guarantees a certain level of privacy for both ASes based on the negotiation between them. 

\paragraph{Overview of the section.}
In this section, we first spend enough space to describe a number of policy inference attacks.
Privacy properties (e.g., degree of anonymity) are often the direct outcomes of particular attack instances and thus we first analyze privacy attacks in depth, focusing on their effectiveness and the attack outcomes. 
We devise an optimal adversary strategy and analyze the maximum attack effectiveness in terms of the anonymity set size.
Our policy inference attacks first try to learn the composed policy $P_{S,D}$ of \name and then the policy of the other party ($P_D$ in $S$'s perspective and $P_S$ in $D$'s perspecdtive).

Then, we describe how \name guarantees the desired level of privacy that is negotiable between the two ASes.
For this, we analyze the observed fairness-anonymity tradeoff that enables us to design a negotiable anonymity guarantee mechanism at the cost of reduced fairness. 
We demonstrate a simple, verifiable negotiation mechanism that can guarantee adequate level of privacy with limited fairness degradation.


\subsection{Policy inference attacks}
The ultimate goal of policy inference attacks is to accurately infer the other party's private policy ($P_D$ in $S$'s perspective and $P_S$ in $D$'s perspective). 
In more formal terms, the attack goal is to reduce the degree of anonymity of the other party's policy as much as possible. 
For example, a source AS $S$ may begin observing the behavior of \name to finally infer a number of possible policies of $D$, $\widehat{\mathcal{P}_D} = \{P_D^1,\cdots,P_D^n\}$, which constitutes the anonymity set for $P_D$.
We set the goal of the policy inference attacks to reduce the anonymity set size.

\input{figures/attack-overview.tex}

Note that due to the \name's isolated execution of the policy composition, an adversary cannot direct read the policies (that is, \PS, \PD, \PSD). 
Thus, instead, as shown in Figure~\ref{fig:attack-overview}, an adversary takes two-stage approach: 
(1) an adversary first observes the execution $\psi(\cdot)$ of the composed policy $P_{S,D}$ by monitoring packets entering/leaving the \name system and infer $P_{S,D}$ (Section~\ref{sec:PSD-inference-attack}); and
(2) the adversary infers the other party's policy by reversing the known policy composition function $\phi(\cdot)$ with the estimated $P_{S,D}$ and its own policy (Section~\ref{sec:PD-inference-attack}). 

For simpler illustration, in this section, we focus only on the attacks launched by a source AS $S$ to infer the destination AS $D$'s policy $P_D$. 
The vice versa is also possible (though with less attack effectiveness) and is summarized at the end of this section.
Moreover, as we discussed in Section~\ref{sec:policy-languages}, in this paper, we only consider the {\em soft preference} action type of our policy language.

\subsubsection{\bf Attack 1: $P_{S,D}$ inference attack}
\label{sec:PSD-inference-attack}
In this section, we design an effective attack that can accurately measure \PSD.
This, in fact, may sound {\em counter-intuitive} because the policy composition and the execution of it are {\em isolated} and thus no adversary directly read them.
However, with strong adversary capabilities of controlling all the inputs and outputs of our filtering function, adversaries can accurately infer the filtering policy.

Inferring \PSD is essentially the task of estimating the {\em average rates} of the token buckets for each traffic classes. 
Flach et al.~\cite{flach2016internet} recently proposes a simple algorithm to infer the average rates of token buckets only by monitoring the outgoing packets from a rate limiter.
When a constant flat outgoing rate is observed, it is the telltale sign of the specified average rate because it is highly likely that the incoming rate to the rate limiter is higher than the specified average rate and thus the rate has been policed.
Our \PSD inference attack may utilize this estimation technique to infer the average rate of each traffic class (i.e., token bucket) and reconstruct the policy \PSD.

Having said that, inferring \PSD is not trivial due to the following remaining challenges:
(1) the adversary does {\em not} know the {\em exact} traffic-class set \CSD and thus cannot determine which traffic-class identifier (e.g., five tuple) to measure for the flat outgoing rate; and
(2) the passive mechanism may be inaccurate when tokens in multiple token buckets are {\em shared} to achieve some {\em priority} policies (e.g., hard or soft preference among multiple traffic classes).

To that end, we propose a set of algorithms that detect the traffic class definition \CSD and then estimate the average rate of each traffic class.

\paragraph{Algorithm overview.}
Our algorithm picks one specific five-tuple identifier $h$ (say, $srcIP$=100.100.100.51, $dstIP$=200.200.200.133\footnote{For simplicity of discussion, we consider only IP addresses.}) at a time and tries to find if a slightly different identifier $h'$ (say, $srcIP$=100.100.100.38, $dstIP$=200.200.200.70) is also in the same traffic class or not (see below for details) until identifying the class definition $h$ is included in (say, $srcIP$=100.100.100.0/24, $dstIP$=200.200.200.0/24).
The algorithm continues until it finds all traffic classes specified in \PSD.
In the last step, it measures the average rates of all the identified traffic classes and then finally reconstructs \PSD.


\input{algo/inference-attack}

The full algorithms of the \PSD inference attack is described in Algorithm~\ref{algo:class-boundary-search}. 
The algorithm first runs the function \textsc{SearchClassBoundary} to accurately detect the traffic class definition of \PSD, that is, \CSD. 
The function random selects a flow identifier $h$ from the not-yet-classified flow identifier set ($U$) and then finds its class definition via the function \textsc{FindClass}.
Then, the algorithm brute-forces the position of masked bits of $h$; that is, for each bit in $h$, the algorithm flips the bit, obtains a new header $h'$, and tests whether $h$ and $h'$ are of same class.
To test, in the function \textsc{PairwiseFlooding} the algorithm floods \name with large enough input traffic rate with only packets of two types: $h$ and $h'$.
Then, it measures the output rates $m$ for $h$ and $m'$ for $h'$. 
If they are close enough, the algorithm determines that they are in the same traffic class (i.e., equally treated by \name); otherwise, they are in a different traffic class.
Once the traffic class set \CSD is inferred, the algorithm measures the rates of each traffic class in the function \textsc{MeasureAverageRates($C$)}.


\begin{figure}[ht]
	\centering
	\includegraphics[width=\columnwidth]{figures/attack_cost_analysis.pdf}
	\caption{Time cost evaluation of pairwise flooding (PF) and class boundary searching (CBS)}
	\label{fig:learn_psd_attack_eval}
\end{figure}

This inference attack algorithm is efficient. 
We use the number of calls of the PairwiseFlooding function as the metric for time cost analysis because it is the dominant time-consuming task in the entire algorithm. 
With this metric, the time cost comparison of two attacks is illustrated in Fig.~\ref{fig:learn_psd_attack_eval}. 
The figures shows that the class boundary searching is not only efficient (linear to $H$ and $|C|$) but also practical, even with a growing $H$ and an extremely large $|C|$ (e.g. 1000).
The estimated real time cost for class boundary searching is around 2.7 hours, assuming $|C| = 100$, $H = 100$ and 1s for running flooding-and-measuring once.



\subsubsection{\bf Attack 2: $P_{D}$ inference attack}
\label{sec:PD-inference-attack}

\input{chapters/attack-part2}

\subsection{Negotiation for the desired level of privacy}

As we saw in the policy inference attacks, when the policy composition aims to achieve the fairness between policies, the anonymity of policies can be quite restricted.
In this section, we first analyze this fundamental {\em fairness-anonymity trade-off}; that is, both fairness and anonymity of policies cannot be achieved in their ideal forms and some reduction of one is required to increase the other. 
Then, we utilize this trade-off and achieve much larger anonymity set by compromising relatively small amount of fairness. 

For the guaranteed level of privacy, \name allows untrusted ASes to negotiate on an agreed level of fairness degradation for a desired level of privacy before starting the filtering operation. 
Then, \name lets the two ASes to verify the correct negotiation operations in its control plane $\phi(\cdot)$ throughout the execution of the policies via remote attestation. 

\subsubsection{\bf Fairness-anonymity trade-off}
Let us first illustrate why both the fairness and anonymity properties {\em cannot} be achieved in their ideal forms.
As we saw in the previous section, any policy instance can be mapped into a unique policy point in the entire policy space. 
To achieve the ideal anonymity, when one policy (say, \PS) and the composed policy \PSD are given {\em all} the policy points in the universe must be equally possible for the other policy (say, \PD). 
This essentially implies that our composition function should be a random function that outputs any policy point in the space uniformly at random.
The random function, however, does not guarantee any fairness.
Conversely, to achieve the ideal fairness between \PS and \PD, \name should achieve $\mathcal{F}(\phi) =  |d(P_S,P_{S,D}) - d(P_D,P_{S,D})| = 0$\footnote{Or, $\mathcal{F}(\phi)=1$ when $|d(P_S,P_D)|$ is odd. For simplicity, we assume  $|d(P_S,P_D)|$ is even.} and such strict fairness enforcement allows only a small number of composed policy \PSD.
Therefore when one of the two input policies (say, \PS) and the composed policy \PSD are given, the number of possible \PD's can be quite limited; that is, the anonymity of \PD is limited.

The only way to increase the anonymity set of the input policies is to {\em enlarge} the possible composed policy set beyond the optimally fair policy solutions. 
In other words, \name needs to allow the composition algorithm to choose {\em sub-optimally fair} policies in addition to the optimal ones.

Note that this trade-off is a {\em inherent} property of any policy composition problem and thus cannot be removed via a new composition logic design. 
Instead, in \name, we exploit this trade-off and provide a negotiation mechanism for two untrusted ASes to come to an agreed level of fairness-anonymity trade-off.
Note that all the functions for the policy (i.e., trade-off) negotiation are the control-plane functions of \name and thus can be easily verified by the two ASes.

\subsubsection{\bf Demonstration: guaranteed anonymity set size}
Demonstration of one simple way to implement fairness compromise. Evaluate in various settings -- reasonable anonymity is obtained with reasonable fairness compromise. 



==> paper 2/chapters/abstract.tex <==
\begin{abstract}
% \vspace{-3pt}
In light of ever-increasing scale and sophistication of modern DDoS attacks, it is time to revisit {\em in-network filtering} or the idea of empowering DDoS victims to install in-network traffic filters in the upstream transit networks. 
Recent proposals show that filtering DDoS traffic at a handful of large transit networks can handle volumetric DDoS attacks effectively. 
% However, the in-network filtering primitive makes dropping packets at transit networks, which used to be considered abnormal, a normal network operation, and this can be abused by malicious transit networks.
However, the in-network filtering primitive can also be misused.
Transit networks can use the in-network filtering service as an excuse for any arbitrary packet drops made for their own benefit.
For example, transit networks may intentionally execute filtering services poorly or unfairly to discriminate their competing neighbor ASes while claiming that they drop packets for the sake of DDoS defense.
We argue that it is due to the {\em lack of verifiable filtering}\,---\,i.e., no one can check if a transit network executes the filter rules correctly as requested by the DDoS victims. 
To make in-network filtering a more robust defense primitive, in this paper, we propose a verifiable in-network filtering, called \name, that exploits emerging hardware-based trusted execution environments (TEEs) and offers filtering verifiability to DDoS victims and neighbor ASes.
% We utilize Intel SGX as a feasible root of trust. % of \name. 
Our proof of concept demonstrates that a \name filter implementation on commodity servers with TEE support can handle traffic at line rate (e.g., 10 Gb/s) and execute up to 3,000 filter rules.  
%For larger attack volume (e.g., 100 Gb/s) and complexity
%(e.g., 50,000 filter rules), we propose an efficient filter rule
%distribution algorithm for dynamically reconfiguring large numbers of
%parallel SGX-based filters.  
We show that \name can easily scale to handle larger traffic volume (e.g., 500 Gb/s) and more complex filtering operations (e.g., 150,000 filter rules) by parallelizing the TEE-based filters.
% The system is currently being tested in one of the biggest regional ISPs that spans across multiple countries.
As a practical deployment model, we suggest that Internet exchange points (IXPs) are the ideal candidates for the early adopters of our verifiable filters due to their central locations and flexible software-defined architecture.  
Our large-scale simulations of two realistic attacks (i.e., DNS amplification, Mirai-based flooding) show that only a small number (e.g., 5--25) of large IXPs are needed to offer the \name filtering service to handle the majority (e.g., up to 80--90\%) of DDoS traffic. 
\end{abstract}


==> paper 2/chapters/algo-example-fig.tex <==
\begin{figure}[t]
    \centering
%       \subfloat[Choices of $P_{S,D}$ for given $P_S$ \& $P_D$.]{%
%          \includegraphics[width=0.66\columnwidth]{figures/eg1}%
%          \label{fig:eg1}%
%       } 
%       \subfloat[Choices of $P_D$ for given $P_S$ \& $P_{S,D}$. ]{%
%          \includegraphics[width=0.66\columnwidth]{figures/eg2}%
%          \label{fig:eg2}%
%       }
%       \subfloat[Permutonhedron of order 4.]{%
          \includegraphics[width=0.65\columnwidth]{figures/4-permutohedron-sage}%
          \label{fig:order_4_p_hedron}%
%       }
       \caption{Permutonhedron of order 4.}
%       \label{fig:algo-example}
\end{figure}

==> paper 2/chapters/algorithm.tex <==
\alglanguage{pseudocode}
\begin{algorithm}
\caption{Composition to find the midpoint of $P_S$ and $P_D$}
\label{algo:fair-comp}
\begin{algorithmic}[1]
\scriptsize
\Procedure {FairComposition}{$P_S(a_1, a_2, ..., a_n)$, $P_D(b_1, b_2, ..., b_n)$} 
\State $dist \gets \lfloor d(P_S, P_{D}) / 2 \rfloor$, $P_{S,D} \gets P_D$
\For{$i \leftarrow 1, n-1$}
    \For{$j \leftarrow 1, n - i$}
        \If{$p > q$ where $a_p = b_j, a_q = b_{j+1}$}
            \State {SWAP} {$b_j, b_{j+1}$}, $dist \gets dist - 1$
            \If{$dist = 0$}
                \State $P_{SD} \gets P_D$
                \State \Return
            \EndIf
        \EndIf
    \EndFor
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

%
%\alglanguage{pseudocode}
%\begin{algorithm}
%	\caption{Composition to find the midpoints of $P_S$ and $P_D$}
%	\label{algo:fair-comp}
%	\begin{algorithmic}[1]
%		\scriptsize
%		\Procedure {FairComposition}{$P_S(s_1 .. s_n)$, $P_D(d_1 .. d_n)$} 
%		\State $dist \gets RAND(\lfloor d(P_S, P_{D}) / 2 \rfloor, \lceil d(P_S, P_{D}) / 2 \rceil)$
%		\State $P_{SD} \gets P_D$
%		\For{$i \leftarrow 1, n-1$}
%		\For{$j \leftarrow 1, n - i$}
%		\If{$s_m > s_n$ where $s_m = d_j, s_n = d_{j+1}$}
%		\State {SWAP} RAND({$d_j, d_{j+1}$})
%		\State $dist \gets dist - 1$
%		\If{$dist = 0$}
%		\State $P_{SD} \gets P_D$
%		\EndIf
%		\EndIf
%		\EndFor
%		\EndFor
%		\EndProcedure
%	\end{algorithmic}
%\end{algorithm}

==> paper 2/chapters/as-path.tex <==
\section{Availability of Alternative AS Paths}
\label{sec:as-path}

\updated{As we discussed in Section~\ref{sec:filter-bypass-detection}, the
ASes along the default path from $S$ to $D$ can refuse to forward the traffic,
thus causing {\em false positives} to our bypass detection. Here, we show that
$S$ and $D$ can flexibly choose an alternative AS path rather than sticking
with the default one. In particular, we model the network topology and the BGP
processing using the AS inferred relationships dataset from
CAIDA~\cite{caida}.  Next, we choose $100$ ASes that contain the most number
of Mirai botnets~\cite{mirai} and $100$ ASes that contain the most number of
DNS resolvers~\cite{wessels2014open} and model them as the source ASes. We select Tier-2
ASes, i.e., have providers and customers, to be the destination ASes. For each
source and destination pair, we count the number of available BGP paths
between them. The results in Figure~\ref{fig:as-path}  show that in the
majority of the AS pairs (more than $80\%$), there is at least  one
alternative BGP path between the source and the destination ASes so that they
can move traffic around the intermediate ASes on the default path.}


\begin{figure}[h]
	\centering
	\includegraphics[width=0.40\textwidth]{figures/as-path.pdf}
	\vspace{-5pt}
	\caption{Availability of alternative paths from Mirai-affected ASes and ASes with DNS amplifiers to Tier-2 ASes.}
	\vspace{-5pt}
	\label{fig:as-path}
\end{figure}

==> paper 2/chapters/attack-part2.tex <==
% overview
Once $P_{S, D}$ is learned, the adversary $S$ can use the knowledge of composition algorithm $\phi(\cdot)$ to further recover the destination AS $D$'s policy $P_{D}$. To continue the discussion, we focus on the attack strategy against the soft preference policy and the fair composition algorithm we propose in Section~\ref{sec:policy}. The attack targets only one execution of the composition, i.e., learning $P_D$ according to the corresponding $P_S$ and $P_{S, D}$.

First, the adversary calculates $d(P_D, P_{S, D})$ using the known distance function (e.g., Kendall tau function). It then enumerates all possible \PD's with the condition that can generate $P_{S, D}$ with $P_S$ following the composition algorithm~\ref{algo:fair-comp}. If the there are multiple $P_D$ satisfying the condition, all of the possible \PD's form the anonymity set of \PD.

\input{chapters/algo-example-fig}

%\paragraph{Permutohedron}
% permutohedron
To better illustrate how the attack works, we use \textit{permutohedron} to visualize the policy, the distance metric, and  the composition. Permutohedron is a graph model where each vertex represents one possible policy (one permutation) and each edge represents the transformation between two polices via a single swap of two adjacent elements in the policy. Figure~\ref{fig:order_4_p_hedron} gives an example of permutohedron of order 4, which contains all the possible polices on 4 rules from 1 to 4 and all the possible transformation among each pair of them.

%\paragraph{Attack on deterministic composition}. 
The visualization provides a new way of understanding the deterministic policy composition. The composition algorithm essentially forms a shortest path between $P_S$ and $P_D$ where $P_{S, D}$ is the middle point on the path. When there are multiple shortest paths in the permutohedron for some pairs of $P_S$ and $P_D$, one of the shortest path is selected and its middle point is chosen as the composed policy by the algorithm~\ref{algo:fair-comp}. 
%This deterministic algorithm unfortunately fail to protect the policy $P_D$ since the adversary can always find the correct $P_D$ out of all the possibilities.

%\paragraph{Attack on non-deterministic composition}. 
%For the non-deterministic version of algorithm~\ref{algo:fair-comp} where all the shortest paths are considered and only one is selected randomly, the anonymity set is improved because it is possible that two or more different $P_D$ generates to the same $P_{S, D}$ with the same $P_S$. 
%Now the attacker can only find out the anonymity set instead of the correct $P_D$.

Let us illustrate how an adversary easily compute the anonymity set when \PS and \PSD are known. 
Let say \PS is 1432 ($A$) and \PD is 3214 ($B$), and the algorithm $\phi(\cdot)$ selects \PSD 1324 ($C$). 
Given \PS and \PSD, the adversary can guess that (3214 or 2134) for $\mathcal{F}(\phi) =  |d(P_S,P_{S,D}) - d(P_D,P_{S,D})| = 0$, or (3124, 1234, 3241, 2314, 2143) for $\mathcal{F}(\phi) = 1$ can be \PD. 
Thus, \PD's anonymity set is \{3214, 2134, 3124, 1234, 3241, 2314, 2143\}. 


The anonymity set size varies with different $P_S$ and $P_D$. 
From the permutohedron, one can find that in general the longer distance between $P_S$ and $P_D$, the larger the anonymity set, as there tend to be more equal-length shortest paths. 
Note that in certain extreme cases, the anonymity set may have only one element, which directly reveals \PD; e.g., when \PS is 1432 ($A$) and \PSD is 3124 ($D$), the only possible \PD is 2341 ($E$); i.e., the anonymity has size of 1.

==> paper 2/chapters/attacks-sigcomm.tex <==
\section{Defense against Malicious Sources}
\label{sec:attacks-defenses}

\msk{Three attacks. Occurred outside of the \name enclaves. }

%\input{chapters/policy-bias}

\subsection{Filter Bypass Attack}

\msk{Bypass is possible. $S$ controls the network outside of the \name enclave and thus our system cannot prevent it.}

\msk{We make this detectable via consistancy checks}

\msk{We admit we cannot immediately detect some bypasses}

\msk{In such cases, we let the source hosts detect it instead. Source hosts are the ones who can choose their upstream ISPs (except some places where local ISP market is monopolized.) We believe that this will give reasonable incentives to source ISP not to conduct such bypass.}

This fine-grained packet processing in the enclave is useful for the detection of bypass attacks launched by $S$ to circumvent the \name filtering.
With the per-packet logging functions before and after the rate limiter (see Figure~\ref{fig:near-zero-copy}(a)), the enclave later can proof (1) if it has received a certain packet and (2) if it has allowed/dropped a certain packet. 
For such filtering accountability, one can imagine an memory efficient data structure, such as Bloom filters~\cite{bloom1970space}.
In practice, $D$ can periodically download the secure per-packet logging to match its own logging to detect any bypass (e.g., packet injections or drop outside of the enclave) has been conducted. 
Also, any customer network of $S$ (or even source hosts themselves) can query the enclave to check if their packets have been safely processed without any bypass attempt (e.g., $S$ drops packets before they reach the enclave). 

\subsection{Invoice Inflation Attack}

\msk{We measure `Did I' but not `Should I.'~\cite{ccsw11}. In other words, was the filtering all that necessary? It is hard to answer. In some network functions, this may be answered but not for filtering functions.}

\msk{We admit that measuring Should I is not possible for filtering function}

\msk{Our approach. Make it fully transparent. All the history of sources are recorded in the immutable, write-only log.}

\msk{We admit that we do not provide any proof or analysis of the deterrence. But we believe that this is practically the best approach we could do.}


==> paper 2/chapters/attacks.tex <==
\section{Attacks}
\label{sec:attacks}

In this section, we discuss several generic attacks arising from the current problem settings. To begin with, we first introduce several concepts that are necessary for our discussion.

\begin{itemize}
    \item \textbf{Class}. As we have seen in the motivating examples, \textit{traffic class} groups the packets into a virtual cluster and is a efficient way to express the policy on a large subset of traffic. 
    
    \item \textbf{Action}. The \textit{action} is closely bound to one class, describing the rules or parameters that the rate-limiter should adopt and enforce.
\end{itemize}

According to our observation, we assume that class and action are building blocks in defining policy. We also use \textit{policy language} to denote the principles that different type of policies follow. 

\subsection{Recovering initial policy}
\label{subsec:recover-policy}

% P_S \phi P_D  ---> P_{S, D}.                attack reverses the 
%  | original policy    | composed policy
% class, action/value
The initial policy is the most confidential information and will be destroyed after policy composition. Therefore, the adversary has no way but recovers the initial policy using the information it collects, such as:

\begin{enumerate}
    \item Composition function, $\phi$.
    \item Adversary initial policy, $P_{D}$ or $P_{S}$.
    \item Composite policy, $P_{S, D}$.
\end{enumerate}

Note that (1) and (2) are public to the relevant parties, including the adversary. For (3) composite policy, we assume it is already compromised and fully learned by the adversary, by means we discussed in this paper.

Now we introduce several attacks that target different scenarios. The difficulty of conducting such attacks varies because any factors in policy composition will more or less change the game that adversary is playing. The factors may include the choice of policy language (complexity, expressiveness, completeness), the choice of composition function (fairness, efficiency), and the level of protection on privacy (uncertainty, transparency).

\subsubsection{\textbf{Null- and full-policy attack}}

The adversary uses an empty set of policy (thus the name \textit{null-policy}) to participate the policy composition. A weak composition will immediately output the opponent policy as the composite one, and lets the adversary knows the initial policy. The adversary has zero cost in this attack, making it a free lunch the adversary will anyway try first prior to any other attacks.

Compared to null-policy attack, the other extreme is \textit{full-policy} attack. The fullness is reflected from the size of the policy, because the full-policy abuses the usage of class, treating each individual unit (e.g., packet or flow) as a class. This long list of policy poses a challenge to the composition function: The opponent policy usually has a handful of classes with each covering a large subset of the traffic, so the function has to solve class conflict first. Usually, two strategies are used: (1) It merges some of the single-unit classes according to the classes defined in the opponent policy; (2) It keeps single-unit classes but inevitably assigns same actions to some groups of single-unit classes. Either one reveals at least the class information in the initial policy. On the other hand, the leakage of action information depends on how the adversary codes the action regarding to single-unit classes, which we will not expand here.

\subsubsection{\textbf{Black-and-white attack}}

\textit{Black-and-white} represents the simplest action performed on the class in the policy. For example, ISPs allow or block the traffic belongs to different classes. Such binary decision on each class causes a dilemma in composition when two initial policy have exactly opposite action. Because of this, the \textit{black-and-white attack} exploits the fact that any composition to solve black-and-white conflicts will inevitably reveal the initial policy. A simple example is the adversary will immediately know the opponent initial policy when a black policy on a class eventually turns white in the composite policy.
% \subsubsection{Example 1} \textit{Black-and-white policy}. ISPs use such policy to completely block or allow the traffic falling in certain class. The composition over this policy is never easy as conflicts are common, and they are solved in a way that will aid in reversing the initial policy. Knowing the composition rule, the malicious side can start inferring from the policy that are overwritten, and even create conflicts to its advantage. This inferring is straightforward no matter it is the allow policy overwrites the block policy or vice versa. We can foresee that the policy alike is subject to the reversing attack, simply because the composition is deterministic and reversible.

\subsubsection{\textbf{Inverse function attack}}

\textit{Multi-valued policy} is a direct extension on black-and-white policy, where the policy language allows a range of values associated with the per-class action, such as "block 30\% traffic", "set rate upper bound at 1Gbps", etc. One prominent advantage is such languages permit more flexible merging strategies rather than a binary decision. However, a poorly designed composition is still vulnerable to reversing attack, given that the function $\phi$ has a inverse function $\phi^{-1}$, which will accept $P_{S, D}$ and $P_{S}$ as input and output $P_{D}$ (assume a malicious $S$). This is \textit{inverse function attack}.

In fact, the adversary can construct the inverse function $\phi^{-1}$ using the known information about $\phi$, which compromise a series of naive composition functions like sum, average, or other linear combination of the policy value on  same class. On the other hand, from the composition designer's view, this suggest a defense of running non-reversible or non-deterministic composition functions.

% \subsubsection{Example 2} \textit{Multi-valued policy}. A direct improvement on the policy language is using policy that allows more possibilities with a range over different values. This offers a possibility to have fairness in the composition as a distance function can be defined the quantify the conflicts, and further used to find the middlepoint when solving the conflicts. Yet the attack is still simple given the determinism of the composition.
\subsubsection{\textbf{Adaptive attack}}

The above attacks mostly target one specific composition procedure, whereas the more powerful attack can be mounted when the attack can adaptively change its policy and smartly select the initial policy to recover the opponent one during multiple composition. An assumption here is the target policy will not change frequently during the time of adaptive attack.

Assume the policy language is a rank-based policy where each class is associated to a rank value, and the composition function $\phi$ is supposed to find a fair rank to mediate the difference of two ranks. For example, $(1, 4, 3, 2)$, $(3, 4, 2, 1)$ and $(3, 1, 4, 2)$ are the policies given by the adversary, the opponent, and the composition function $\phi$ respectively. The adversary notice the change after composition, so she launches a second composition using the first composite policy as its input, i.e., $(3, 1, 4, 2)$. The second composite policy is $(3, 4, 1, 2)$, which is close enough to the target. By reusing the composite policy as the input for next iteration, the adversary exploits the fair function $\phi$ that tries to bridge the gap between two diverged policy. Gradually, it approaches the target policy and it can choose to stop the iterations when the composite policy is same as its input or the difference between them is acceptable to the adversary.

% 1432            3421
%     1342     3412
%         3142


\subsection{Learning class and rate}
\label{subsec:learn-class-n-rate}
Another category of attacks appears in the policy enforcement stage, where for each class in the $P_{S, D}$, a rate-limiter is shaping the traffic in the class limited by a per-class rate. The \textit{class partition} and the \textit{per-class rates} are derived secretly from the $P_{S, D}$ and safely used by rate-limiters inside the trusted execution environment, ruling out any direct unauthorized access. However, these parameters are in the adversary's interest. once learned by the adversary, they can be used to infer $P_{S, D}$, eventually resulting in the reversing of the opponent policy (Section \ref{subsec:reverse-policy}).

The main targets are class partition and per-class rates, and the basic tool used by the attacker is traffic \textit{meter}, measuring the traffic rate of a potential class, set according to the guess on the class partition. The meter outputs the rate in real time, plotting the rate variation over time, and if a rate-limiter were set on the same class, one or more horizontal lines pinning at fixed rate would appear on the rate-time plot. This signals a possible right guess of the class and also reveals the rate. Conversely, if there is not capped rate found, the guess could be wrong.

Armed with this observation tool, the adversary could launch various attacks with different difficulty, depending on its capability.

\subsubsection{Enumeration}
For a passive observer watching the output traffic, it can setup per-class meters based on one enumeration of the class partition, whose total number on $n$ elements is given by exponential generating function $\sum_{n=0}^{\infty}{\frac{B_{n}}{n!}}z^{n}=e^{e^{z}-1}$. The attack will succeed once all the meters get the capped rate (and they sum up to the overall limit $L$), meaning that the partition is also found correctly. One can see that this is not a very efficient attack given the huge number of enumeration to make. Note that, the difficulty will continue to increase with \textit{work-conserving} mechanism (Section \ref{}) activated as it allows fluctuation, thus reducing the chances of getting a constant rate.

\subsubsection{Same-rate flooding}
For an active attacker who not only sees the output traffic but also has the ability to control the input, the guessing is not longer necessary. By overwhelming each point with high-volume traffic at a substantially large rate, the work-conserving protection will not take effect because there will be no underutilized bandwidth. Tha adversary then operates meters for every single point, reads the policed rate, and classifies the points having same measured rate into one class. This same-rate clustering works because the bandwidth in same class is equally distributed among every point within the class. The only chance it will fail is when points from different classes happen to have same measured rate, leading to misclassification.

\subsubsection{Partitioned search}


\subsection{Bypassing middlebox}

The third category of attacks, \textit{bypassing middlebox}, mainly carried out by a malicious platform provider, is about manipulating the traffic volume before or after the middlebox. The rate-limiting middlebox is only sensitive to shape-related manipulation as it focuses on the size of packets and only affects the volume of traffic getting through. Any other kinds of manipulation (e.g., packet content manipulation) is no longer only targeting the middlebox but the eventually the recipient of the traffic.

\subsubsection{Pre-filtering} 
The adversary runs its own filters prior to the middlebox, changing the profile of the traffic, or discriminating against the traffic of certain end-users. This pre-filtering is stealthy and runs undercover, since the blame is shifted to the middlebox if the end-users experience any service degradation.

\subsubsection{Probing}
This is another reshaping of the input traffic in a way that not only removes packets but also actively injects to drastically force the profile on input traffic. Usually the probing packets are used for the purpose like inferring the internal state of the middlebox. The more advanced probing has anti-detection measures, (e.g. mirroring traffic, slow rate attack) that evades the monitoring from middlebox or from the receiver of the output traffic.

% traffic addition, traffic deletion.
\subsubsection{Post-manipulating}
At the output side of the middlebox, the adversary is able to inject or remove the traffic mostly for covering up any operations done previously. It can remove the probing traffic or forward the original traffic directly to the output link for a complete bypassing, or inject packets to cancel out any pre-filtering actions.





==> paper 2/chapters/attestation.tex <==
\section{Remote Attestation Performance}
\label{sec:remote-attestation}
% \msk{Shweta?}

The \name filter needs to provide a proof of authenticity to the destination network, before
the destination can trust the filter with the filter rules. 
The filter bootstraps this process by
creating a pair of public and privates keys. It then registers the public key
with the IAS service. At runtime, the destination initiates the remote
attestation process. 
Then the
source enclaved filter creates the attestation report which includes the
enclave measurement, platform security version number, software version,
software vendor security version number, the software configuration and any
other auxiliary information specific to the application.  The filter enclave
then asks the quoting enclave on the same platform to  verify and signs the
report with the attestation (private) key to generate the quote. The source
then forwards this quote to the destination. The destination asks the IAS to
verify the quote. The IAS then uses the initially registered public key of the
filter enclave to verify the signed quote. If the IAS confirms to the
destination that the quote is authentic, the remote attestation process
completes successfully.  

\codename performs remote attestation for each new enclave that the source
launches on its infrastructure. Since \codename is expected to operate under
DDoS attacks, we want to ensure that the launching of multiple-enclaves
on demand does not become the bottleneck for our deployment model. 
Here, we measure
the total amount of time to complete an end-to-end remote attestation
process for one enclave. In our micro-benchmark for remote attestation for the conservative performance tests, we setup the filter enclave
and the destination on a cloud machine hosted in
South Asia, and the IAS service
hosted in Ashburn, Virginia, United States. For an enclave binary of size $1$
MB, the platform takes $28.8$ milliseconds and the total end-to-end latency of $3.04$ seconds with a standard deviation $9.2$ milliseconds.


==> paper 2/chapters/auditable-filter-design.tex <==
\subsection{Stateless Filter Design}
\label{sec:stateless-filter-design}

% We want the victim network and the members of the \name IXP to be able to audit the operation of the filter after it is instantiated by the \name IXP.
% The core part of 
% Our filter implementation is enclosed by an SGX enclave and its internal logic and states can be securely measured and verified via the remote attestation process~\cite{johnson2016intel}. 
%
% We first analyze the conditions for the auditability of the SGX-enclaved filters, derived from the abstract semantics. 
% Then, we propose practical \name filter designs considering the derived requirements and practical filtering properties. % for volumetric attacks.

% \subsubsection{Conditions for Auditability}
% \label{sec:conditions-for-auditability}
% Our filter implementation is enclosed by an SGX enclave where its internal logic and states can be securely measured and verified via the remote attestation process~\cite{johnson2016intel}.
% % The auditability of the enclaved filter relies on the remote attestation to the filter's internal logic.
% However, attestation alone is insufficient because the filtering decisions can be influenced by the inputs to the filter, which is controlled by a malicious \name IXP.

%Let us first describe abstract semantics for our enclaved filter~\cite{panda2015new}.  
%Our model is defined over a potentially infinite set of packets, $P$.
%Each packet contains information about its location (i.e., an input port or an output port of a filter) and the two identical packets $p_1$ and $p_2$ at different locations can be expressed as $p_1 \doteq p_2$.
%Also, $P^*$ represents the set of all sequence of packets.
%The abstract model of the enclaved filter is a function $f$ that takes an arbitrary incoming packet $p \in P$ and a history of all the previous packets $h \in P^*$, and produces either {\tt allowed} or {\tt dropped} decision for each incoming packet. 
%Particularly, the model $f$ can be expressed as,
%
%\begin{align}
%f(p,h) =\left\{
%\begin{array}{ll}
%\{p'\},~p'\doteq p & \textrm{\em if allowed},\\
%\{\} & \textrm{\em if dropped}.
%\end{array}
%\right.
%\end{align}

% We first analyze the dependencies of the enclaved filters, derived from the abstract semantics. 
% Then, we propose practical \name filter designs considering removing the derived requirements and practical filtering properties.
% 
To analyze the dependencies of the enclaved filters, let us first describe an abstract model for our enclaved filter $f$: 
% For general filtering operations (e.g., rate limiting, heavy flow identification), the notion of flow rates (e.g., byte per second or packet per second) is useful. 
% We, thus, express the model with the annotation of packet arrival time $a_i$ for packet $p_i$:
\begin{align}
\{\texttt{ALLOW},\texttt{DROP}\}\leftarrow f\big(\langle{p,a}\rangle, (\langle{p_1,a_1}\rangle, \langle{p_2,a_2}\rangle, \cdots)\big),
\end{align}
where $\langle{p_i,a_i}\rangle$ denotes that packet $p_i$ arrives at the enclaved filter at time $a_i$ (measured by the enclave's internal clock), $\langle{p,a}\rangle$ represents the packet $p$ that is being evaluated and its arrival time $a$, and the following time relationship holds $a > a_1 \ge a_2 \ge \cdots$.

% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[width=0.3\textwidth]{figures/auditability.pdf}
% 	\vspace{-5pt}
% 	\caption{Manipulation of packet arrival time and arbitrary packet injection by a malicious \name IXP.}
% 	\vspace{-10pt}
% 	\label{fig:auditability}
% \end{figure}

% Figure~\ref{fig:auditability} illustrates the two types of manipulations of packets by a malicious \name IXP and how they affect the filtering operations. 
% \muoi{Figure 3 actually can be sacrificed.}

Notice that in this abstract model, the filtering operation of a packet $p$ depends on the packet arrival time and the order of the packets, which can be exploited by the filtering network (see next).
Here, we summarize the two properties that are needed to make \codename filter auditable:
\begin{packeditemize}
    \item {\em Arrival-time independence.} The %auditable 
    filtering decision should be independent of packet-arrival time because it can be easily manipulated by a malicious filtering network (e.g., delaying individual data packets). %, increasing packet arrival times arbitrarily.
    Moreover, a malicious filtering network can delay the time query/response messages to/from the trusted clock source for the enclave~\cite{sgx-forum-trusted-time}, slowing down the enclave's internal time clock.
    % With such arrival time manipulations, a malicious \name IXP may influence the filtering decision without directly tampering with the internal filtering logic.
    \item {\em Packet-injection independence.}
    % Moreover, the \name filter decision should be independent of the injected packets because a malicious \name IXP can also inject any arbitrary packets into the input stream. 
    % Thus, if the filtering decision depends on the previous packets, it can be indirectly controlled by a \name IXP. 
    The filtering decision should not depend on the previous packets since a malicious filtering network can also inject any arbitrary packets into the traffic flow and influence the filtering decision.
\end{packeditemize}



% \paragraph{Stateless filter for auditability.} 
Thus, to ensure that the filtering operations are auditable, the filtering function $f$ can be {\em independent} of all the previous packets and their arrival times; that is,
\begin{align}
f\big(\langle{p,a}\rangle, (\langle{p_1,a_1}\rangle, \langle{p_2,a_2}\rangle, \cdots)\big)=f(p),
\end{align}
which simplifies the filter design to $n$-tuple (e.g., {\tt srcIP, dstIP, srcPort, dstPort, protocol}) per-packet filters.
In other words, the filtering decision of packet $p$ solely relies on $p$, such as five-tuple bits.
While we acknowledge the limitations of such a simple $n$-tuple filter design (e.g., incapable of handling complicated application-level DoS attacks), we note that it is sufficient for handling large volumetric attacks that are in imminent need of in-network filtering.

% \subsubsection{Practical Filter Design Points}
% \label{sec:filter-design-points}

% We also propose several practical design points for our enclaved filter. 
Particularly, for handling volumetric attacks, we allow victim networks to express filter rules for exact-match five-tuple flows (e.g., a specific TCP flow between two hosts) or coarse-grained flow specifications (e.g., HTTP connections from hosts in a /24 prefix).
Details for several practical design points for our enclaved filter are found in Appendix~\ref{sec:filter-design-points}.

% We consider deterministic and non-deterministic filter rule types:
% \begin{packeditemize}
% 	\item A {\em deterministic filter rule} defines a static \{{\tt ALLOW, DROP}\} decision for a specified flow; and
% 	\item A {\em non-deterministic filter rule} expresses only the static probability distribution ($P_{\tt ALLOW}$, $P_{\tt DROP}$, where $P_{\tt ALLOW}+P_{\tt DROP}=1$) for a specified flow and the final filter decision for each exact flows is made by the \name filter.
% 	We guarantee the connection-preserving property in \name filters so that all the packets in a TCP/UDP flow are allowed or dropped together.
% \end{packeditemize}
% %The detailed execution of non-deterministic rules with the connection-preserving property and its performance evaluation is found in Appendix~\ref{sec:connection-preservation}.



% The execution of non-deterministic rules with the {\em connection-preserving property} can be implemented in two different ways:
% \begin{packeditemize}
% 	\item {\bf Hash-based filtering.} For each incoming packet $p$, we compute the cryptographic hash (e.g., SHA-256) of its five-tuple bits and the enclave's secrecy to make filtering decision based on the given probability distribution. For example, packet $p$ is allowed if $H(\texttt{five-tuple-bits}||secrecy) < (2^{256}-1) \times p_{\texttt{ALLOW}}$ with $H(\cdot)=$SHA-256; and
% 	\item {\bf Exact-match rule filtering.} For each TCP/UDP connection, the filter installs an exact-match rule with a filtering decision randomly chosen based on the given probability distribution. %All the subsequent packets in the connection are allowed or dropped based on the installed exact-match rule.
% \end{packeditemize}
% Note that the two design points have different advantages and disadvantages. 
% The hash-based filtering has a smaller memory footprint for lookup table but it incurs per-packet additional latency for cryptographic hash operations. 
% In contrast, the exact-match filter design tends to have shorter per-packet processing time since it executes only one lookup but it requires a larger memory footprint for lookup tables and adds latency for frequent lookup table updates. 
% We propose a {\em hybrid} design where hash-based filtering is performed for new flows until these new flows are installed with exact-match rules at every rule update period (e.g., 5-40 seconds).


% \subsubsection{Mitigation of Filter-Rule Violation Attacks}

% As the \name filter logic is auditable via remote attestation, the two filter-rule violation attacks described in Section~\ref{sec:threat-model} are mitigated with the assumption that all the traffic from the \name IXP to the victim networks is mediated (e.g., {\em no} packet drops outside of the \name filter) by the \name filter; see Section~\ref{sec:bypass-attacks} for the case when this assumption does not hold.
% To violate the filter rules, a malicious \name IXP network has to tamper with the filter's internal logic or modify the requested filter rules, which is prevented by the SGX primitives. 

% \subsubsection{Minimizing Trust on SGX Confidentiality}
% We largely do {\em not} rely on the confidentiality guarantees of the SGX
% architecture due to the known and growing concerns regarding
% side-channels in the current SGX
% architecture~\cite{gotzfried2017cache, last-level-cache, hahnel2017high}. Instead, we rely mainly
% on the integrity guarantees of the SGX and its remote attestation
% property. The only exceptions are (1) the logic that opens a secure channel
% between the enclave at the filtering network and the victim ISP and (2) the cryptographic hashing used for filtering because these components generate and use certain secret keys. Ensuring confidentiality properties
% of a secure channel primitive on SGX is admittedly challenging, but
% one can leverage advances in defenses for
% side-channels~\cite{pigeonhole,gruss2017strong,zerotrace}, constant-timing encryption primitives (e.g., AES-NI~\cite{mowery2012aes}), and
% formal verification techniques~\cite{moat,msr-pldi16} to protect this small number of secrets.



%To further minimize trust on SGX confidentiality, 
%we remove the necessity to store
%private information of the two networks inside the enclave. For example, we do not
%protect the filtering policy submitted by a victim network from
%a source network.  The victim network is advised to maintain the two
%levels of filter rules: a public and a private rule sets, where the
%former set is outsourced to the source network but the latter is enforced inside the victim's local network only.


==> paper 2/chapters/background.tex <==
\section{Background}
\label{sec:background}

\paragraph{Intel SGX.} (.25 page)
--- To be written.
%\msk{Need a short overview of SGX}
%
%
%\msk{how widely available.}
%
%\msk{focus on isolated execution, remote attestation.} 
%
%\msk{threat model}
%
%\msk{we trust IAS}

\paragraph{Blockchain-based Smart Contracts.} (.25 page)
--- To be written.
%\msk{Need a short overview of blockchain, Ethereum, smart contracts}
%
%
%- assets or resources are managed efficiently...
%
%SC.. embodies ... involvement of each party...
%
%SC ... written by a community network operators (e.g., IETF)...
%


==> paper 2/chapters/background_vyas.tex <==
% \section{Background and Motivation}
% %
% We present a case for why in-network filtering is worth reconsidering and why Internet exchange points (IXPs), among other transit infrastructure, are the ideal places to introduce our verifiable in-network filtering.
% We then review recent technical advances in trusted execution environment techniques, specifically, Intel SGX.
%We then describe our threat model with a number of attack strategies and an accountability problem in source filtering between two mutually distrusting ISPs. % and desired security properties. % our problem statement for the \name system design and outline its architecture overview. 

% \subsection{Case for In-network Filtering}
% \label{sec:case-for-source-filtering}

% \muoi{Move this subsection to Intro?}

% The idea in-network filtering has been the core idea of
% many DDoS mitigation proposals.  There are two prominent approaches to
% implementation: dynamic filtering and capability-based
% approaches.
% %
% Dynamic filtering suggests that the destination ISP requests the ISPs on the forwarding paths to install 
% filter rules at the time of
% attack, for instance as proposed in
% Pushback~\cite{mahajan2002controlling},
% D-WARD~\cite{mirkovic2002attacking}, AITF~\cite{argyraki2005active},
% StopIt~\cite{liu2008filter}.
% Capability-based approaches embed capabilities in the packet flows, which can
% be controlled by the destination hosts to authorize flows in upstream, as proposed in SIFF~\cite{yaar2004siff}, TVA~\cite{yang2005limiting},
% and Portcullis~\cite{parno2007portcullis}. 

% Closest to our work is the recent SENSS defense architecture by Ramanathan et al.~\cite{ramanathan2018senss}. 
% SENSS proposes to install DDoS-victim submitted filters at a small number of major ISPs. 
% Ramanathan et al. show that in-network filtering at only four major ISPs in the US would have stopped the Dyn attack happened in 2016~\cite{york2016dyn}.
% SENSS also suggests an automated payment channel between a DDoS victim and a filtering ISP so that the ISP can get compensation for the extra filtering tasks. 
% Although the idea is solid and evaluation is promising, the SENSS proposal lacks the filtering verifiability and thus allows several undetectable misbehaviors of the filtering ISPs.\footnote{Ramanathan et al.~\cite{ramanathan2018senss} sketch a reputation-based mitigation, which can be used together with our \name proposal.}

% The predominant DDoS defense in practice today is an overlay-based filtering approach, such as cloud-based scrubbing services, that performs outsourced filtering in a third-party network on behalf of the DDoS victims (e.g., AWS-Shield~\cite{aws-shield}, Radware DefensePro~\cite{radware}).
% Overlay-based filtering approaches are popular particularly because they require {\em no} changes to current Internet
% architecture. Recent works have proposed advances in such overlay
% filtering using middleboxes~\cite{liu2016middlepolice,gilad2016cdn} and proposals
% have discussed large-scale filtering locally at
% ISPs~\cite{fayaz2015bohatei}.
% However, end users are not satisfied with the status quo. Reports
% suggest that relying on third-party providers centralizes the DDoS
% marketplace~\cite{gilad2016cdn}; costs for small and medium-size victims
% are high and services are left to the discretion of large service
% providers~\cite{guardian2016ddos,gilad2016cdn}.

% \paragraph{ISP's interests in source filtering.}
% From our personal conversations with two ISPs, we have learned the ISPs' strong interests in monitoring and reducing malicious activities in their networks for their reputation.
% Particularly, one major ISP in our region (say ISP $A$) has been using an automated detection for suspicious hosts under its network using flow-based analysis.
% Yet, ISP $A$ performs {\em no coordination} with the traffic destination networks.
% ISP $A$'s such a non-coordinated source filtering is ineffective in reducing attack traffic because ISP $A$ rarely filters its suspicious hosts due to the high risk of banning its own subscribers by mistake. % is too high in practice; e.g., it may end up banning its own benign (but mistakenly identified) customers. 
% %Filtering at the source may be conducted only in some restricted circumstances (such as, suspicious hosts are already Internet-wide blacklisted\footnote{CBL: Composite Blocking List, \url{https://www.abuseat.org/}}) but the effectiveness of source filtering in such cases is questionable. 
% This anecdotal evidence tells us that (1) source ISPs wish to have better source filtering in general; yet, (2) the current practice of non-coordinated source filtering has clear limitations. 
% Our source filtering, namely, \name, enables secure and direct coordination with destination networks.
% With \name, source networks receive the explicit attack indications directly from victim networks, which enables effective filtering at the source networks. % and thus they can handle their own malicious hosts with certainty. %, with only incremental costs being borne by destination networks.} 


% \paragraph{Recent push from industry.}
% In the past few years, there has been a push from industry to realize the idea of in-network filtering. 
% For example, Huawei has been proposing its global inter-ISP platform that enables in-network filtering between participating ISPs via its cloud-based centralized mediator~\cite{huawei2015cca}.
% Team Cymru proposed a volunteer-based filtering service~\cite{cymru}.
% The IETF DDoS Open Threat Signaling (DOTS) working group has developed protocols for outsourced filtering operations between ISPs~\cite{dots-slides}.
% Unfortunately, these initiatives have neglected the issue of lack of verifiability. 
\section{Problem Definition}
\label{sec:problem-definition}

% \muoi{The flow can be: 1) Threat model (attack capability and goals); 2) Desired properties (Auditable filers to defend against the attacks and Scalable design against volumetric attack); 3) Assumption about TEE in general}

In this section, we describe the threat model we consider in this paper (\S\ref{subsec:threat-model}), the desired properties of the \name design, the trusted execution environment model (\S\ref{subsec:trusted-execution-environment}) (\S\ref{sec:desired-filter-verifiability}) and the assumption we make in this work (\S\ref{sec:assumptions}).

\subsection{Threat Model}
\label{subsec:threat-model}

We consider a single malicious transit network that offers in-network filtering services for downstream networks.
In this threat model, the adversary has full control of the control plane and data plane within its network.

% Reliable forwarding operations constitute the primary network service and business model of transit networks, such as IXPs or ISPs. 
Our threat model focuses on the problem of the malicious filtering network manipulating the DDoS-victim-submitted filter rules, which we call as {\em filter rule violation attacks}.
In general, let us consider a filter rule $R$ requested by a victim network.
The malicious filtering network may change $R$ arbitrarily into a different filter rule $R'$ and apply it to all traffic destined to the victim network.
Also, the malicious filtering network may apply different modified rules $R'_1, R'_2, \cdots$ for different traffic flows (e.g., packets delivered via different neighboring ASes).
% This attack capability is already available for filtering IXPs in all existing in-network filtering proposals (e.g, \cite{ramanathan2018senss}) since they do not offer the verification of the filtering operations. %it is the victim and neighboring networks completely entrust the filtering operations at the filtering network.

% Filtering at an IXP can easily disturb the reliable forwarding operations for other nearby networks. 

% o Let us consider a filter rule $R$ is submitted by a DDoS victim. 

% o Filtering network may modify it to $R'$ and apply this for all the traffic it forwards to the victim.

% o Or, the filtering network may have multiple variants of the original rule $R$ and make differnt $R'_1$, $R'_2$, ... $R'_n$ for different traffic groups (e.g., packets delivered via different member ASes). 

% o This manipulation of filter rules are called {\em filter rule violation attacks}.

% o This attack capability is available for filtering networks in all the existing in-network filtering proposals~\cite{ramanathan2018senss}...

% o We present two notable attack goals that ...


% We focus on two {\em filter-rule violation attacks} where the manipulation of traffic filters at the filtering IXPs can seriously disrupt the packet forwarding services for the member ISPs (i.e., direct neighbor ISPs) (\S\ref{sec:attack-members}) and the remote DDoS victim networks (\S\ref{sec:attack-victim}). 
% We emphasize the desired filtering verifiability property of \name (\S\ref{sec:desired-filter-verifiability}) and describe a naive solution and show why it is impractical in current Internet in (\S\ref{sec:impractical-collaboration}).
% Finally, we clearly state the assumptions of our threat model (\S\ref{sec:assumptions}).


% \paragraph{Attack goals}
In the followings, we present two example attack goals, where the manipulation of filter rules at a filtering network can seriously disrupt the packet forwarding services for the neighboring ASes and the remote DDoS victim networks.
In both attacks, we use the same example as in Section~\ref{sec:intro}, i.e., the filtering network manipulates the DDoS-victim-submitted filter rule $R=${\tt [Drop 50\% of HTTP flows destined to victim network]}.

\paragraph{[Goal 1] Discriminating neighboring ASes.}
% \label{sec:attack-members}
ASes expect their traffic to be reliably forwarded by the transit networks.
%packet forwarding from their IXP. 
Yet, when a transit network offers the filtering services for the sake of DDoS defense, the packet forwarding service can be silently degraded differently for different neighboring upstream ASes. % cannot reason about why their packets are dropped by the IXP's filter.
% the member ISPs should expect some packet drops when DDoS victims want to do so. 
% Without any verifiable filtering at the IXP, the member ISPs cannot reason about why their packets are dropped by the IXP's filter. 
% Worse, even when the member ISPs expect some packets drops at the filtering IXP, they cannot check if their traffic is treated indiscriminately.
%
% Let us revisit our example in Section~\ref{sec:intro}; i.e., $R=${\tt [Drop 50\% of HTTP flows destined to victim network]}.
In particular, the filtering network can apply the {modified} filter rules for each neighboring AS based on its own business preference.
% Let us assume two member ISPs $A$ and $B$ in Figure~\ref{fig:venef} send the same amount of HTTP traffic destined to the victim network.
Instead of applying the same original rule $R$, the filtering network may apply $R'_A=${\tt [Drop 20\% of HTTP flows destined to victim network]} for traffic flows delivered by AS $A$ and $R'_B=${\tt [Drop 80\% of HTTP flows destined to victim network]} for traffic flows delivered by AS $B$. 
Such discriminatory filtering is hard to detect because individual neighbor AS $A$ and $B$ do not know the unmodified rule $R$ and, even if they know $R$, they cannot determine if the traffic filter applied to their packets is $R$. 
Each neighbor AS may try to infer the packet drops of the end-to-end path indirectly (e.g., via monitoring TCP sessions); yet, it is {\em insufficient} because pinpointing exact location of packet losses (a.k.a. fault localization) is known to be hard without large-scale network collaboration~\cite{argyraki2010verifiable, basescu2016high}.

%are the correct one that is submitted by the DDoS victim network. 
% Note that such violations can be also effective when the filter rules specifies the source addresses (e.g., {\tt [Drop 40\% of traffic from $A$]}, {\tt [Drop 60\% of traffic from $B$]}) since the IXP can anyway arbitrarily modify and apply them.

% \muoi{Let's move and highlight this in the Intro. Currently the impact of this attack is hidden.} Note that considering that ISPs already often discriminate their neighboring networks by intentionally choking bandwidth of certain peers for their economic benefit~\cite{dispute_level3_comcast}, the above-mentioned discrimination attack is highly anticipated. % with the new near-source filtering services. 

\paragraph{[Goal 2] Reducing operational cost with inaccurate filtering.}
% \label{sec:attack-victim}
% 
To reduce the operational cost, the malicious filtering network may violate the filter rules submitted by the DDoS victims. 
%
% In the same example $R=${\tt [Drop 50\% of HTTP flows destined to the victim network]}, 
For instance, consider that the malicious filtering network wants to use {\em only} 10 Gb/s of its filtering capacity for the rule $R$ while total incoming traffic of 50 Gb/s should be sent to the filters.
To achieve this, the filtering network can send only 10 Gb/s traffic to its filters and execute the unmodified rule $R$.
For the rest of the 40 Gb/s traffic, however, the filtering network can simply allow or drop all
% apply any arbitrary packet drop at the switch fabric 
{\em without} using the filtering capacity.
% (e.g., allow or drop all). 
% Then, for the rest of 
% but apply arbitrary packet drop  perform an {\em insufficient} filtering, that is, filtering only 100Gb/s of the traffic, which resulting in dropping only 50 Gb/s out of 200 Gb/s in total.
% Alternatively, the filtering IXP may perform an {\em excessive} filtering, for example, allowing only 50 Gb/s of traffic to be forwarded to the victim network.
% In the extreme cases, the malicious IXP can allow or drop all the 40 Gb/s traffic.
% In any cases, the filter rule $R$ is not faithfully executed.
Since the victim network has no information about the incoming traffic arrived at the filtering network, it cannot directly detect this attack. 
% the IXP may want to perform much poor filtering, e.g., dropping only 20\% of HTTP flows, while claiming that it executes the requested rule accurately.

% The victim network does not see the incoming traffic to the IXP (e.g., the volume of total HTTP flows arriving at the IXP) and thus cannot directly detect this attack.

% Note that the filtering IXP may have incentive to launch this attack as this attack saves the network and compute resources for the requested filtering tasks. % while claiming the full credit for the work. 

% \muoi{Is this necessary? Involving any 'economic' argument makes the flows more complicated.}
% This attack can be particularly profitable to the filtering IXP when it receives economic compensation for the filtering work from the DDoS victim based on the number of filter rules, as suggested by SENSS~\cite{ramanathan2018senss}.
% Discussion on the economic incentive for the filtering IXPs though is out of the scope of this paper.

\subsection{Desired Properties: Filtering Verifiability and Scalability}
\label{sec:desired-filter-verifiability}

As we introduced in the Introduction, we have the two desired properties of the \codename design. 
% that make it practical for DDoS defense.
First, to remove the attack capabilities required for the filter-rule violation attacks, \codename desires to have the {\em filtering verifiability}.
A filter rule $R$ is said to be verifiable if any modification of the rule $R$ and its execution by the filtering network can be detected by the victim networks or the direct neighboring ASes.
% 
% Note that the filtering verifiability property is beneficial to benign filtering network as well because they can easily provide assurance of the correct filtering operations to their neighboring ASes and DDoS victim networks.
% 
Second, our \name system must be easily {\em scaled up} because DDoS attacks are increasingly scalable in both volume and complexity. 
We have observed an escalation in the volume of DDoS attack
traffic~\cite{computerworld2013biggest,guardian2016ddos} and attacks are getting more sophisticated; e.g., multi-million bots are becoming more common~\cite{mirai}. 
% have been in recent Mirai attacks, an AS has up to 281,686 unique malware infected IPs~\cite{chaos-simulator}.

\subsection{Trusted Execution Environment with Intel SGX}
\label{subsec:trusted-execution-environment}
\codename uses TEEs, particularly Intel SGX in this work, as the feasible hardware-based root of trust.
Intel Software Guard Extensions (SGX) is a recent architectural feature that allows secure execution
of a program on a computing infrastructure in control of
an adversarial operator~\cite{costan2016intel,mckeen2016intel}.
SGX also supports secure execution of a user-level program with no modification of underlying commodity software stacks~\cite{shinde2017panoply,baumann2014shielding,arnautov2016scone}. 
In particular, it offers the isolated execution of the application logic in a protected memory region, called an {\em enclave}, which prevents the operator from tampering it.
Moreover, it supports remote attestation that allows a third party to audit that the correct application and data has been loaded in an enclave.
% for remote audits for the correctness of the logic.
%
% The remote attestation feature allows a third party to be convinced that the correct application code has been loaded in an enclave. 
The attestation process starts when a verifier issues an attestation challenge to the enclaved application. 
The enclave then provides a report, which is cryptographically signed with the attestation key of the SGX hardware. 
Next, the attestation report is verified by the Intel Attestation Service (IAS), which is distributed globally~\cite{johnson2016intel}.
Recently, Intel also allows {\em anyone}, who gets a certificate from Intel, to run their own remote attestation services and verify the attestation report~\cite{vinnie2018intel}.

% \muoi{We should either move this (large-scale collaboration) into the intro or leave it in the discussion. At the moment it doesn't fit the flow.}

% \paragraph{Impractical solution: large-scale collaboration.}
% It is worth noting that it is indeed possible (but {\em impractical}) to detect the filter rule violation attacks without the proposed verifiability property provided by the filter itself. 
% In particular, if {\em all} the member ISPs and the victim networks are honest (i.e., always tell the truth to each other) and they are willing to collaborate, they can verify the filtering operations of the IXP because they collectively see all the incoming/outgoing packets to/from the IXP and know the original filter rules submitted by the victims. 
% However, unfortunately, IXPs easily have hundreds or thousands member ISPs in practice. 
% Furthermore, there would be thousands of potential DDoS victim networks that can use the filtering service of the IXPs due to their central location of the Internet. 
% % Adding to that, we need honest collaboration from any potential DDoS victim networks that may be remote networks from the targeted IXP.
% Considering highly competitive (sometimes adversarial) Internet transit market, such large-scale ISP collaboration has not been observed and will hardly be possible in the near future.  


% \subsection{Intel SGX Summary} 
% \label{sec:net-func-using-sgx}

% Traditional hardware-trust based isolated execution techniques (e.g., TPM based approaches~\cite{mccune2010trustvisor}) enable the secure execution of network functions deployed on the untrusted remote computing platform (e.g., cloud servers).
% More recently, new trusted computing hardware has
% become much easier to use and deploy for user-level applications. 
% Specifically, Intel Software Guard Extention (SGX)~\cite{costan2016intel,mckeen2016intel} (and similar
% primitives) is a recent architectural feature that allows secure execution
% of a program on a computing infrastructure in control of
% an adversarial operator.
% SGX supports secure execution of a user-level program with no modification of underlying commodity software stacks~\cite{shinde2017panoply,baumann2014shielding,arnautov2016scone}. 
% Particularly, it offers isolated execution of the application logic in a protected memory region, called an {\em enclave} memory, and allows remote attestation for remote audits for the correctness of the logic.
% %
% The remote attestation feature allows a third party to be convinced that the correct application code has been loaded in an enclave. 
% In general, a verifier issues an attestation challenge to the enclave application. 
% The enclave then provides a report, which is cryptographically signed with the attestation key of the SGX hardware. 
% Next, the attestation report is verified by the Intel Attestation Service (IAS), which is distributed globally~\cite{johnson2016intel}.
% Recently, Intel also allows {\em anyone}, who gets a certificate from Intel, to run their own remote attestation services and verify the attestation report~\cite{intelsgxdcap}.

%The secure user-level filtering can be nicely incorporated into recent kernel bypass techniques for fast packet processing (e.g., DPDK~\cite{dpdk}, Netmap~\cite{rizzo2012netmap}) with the multi-threaded, multiple-enclave programming support in SGX.

\subsection{Assumptions} 
\label{sec:assumptions}
% In this paper, we use SGX as a feasible hardware based root of trust. 
We assume that ISPs (e.g., victim networks) trust the remote attestation process for the integrity guarantees of the \name enclave. 
% Indeed, the trust of the remote attestation is given by the distributed Intel Attestation Service (IAS)~\cite{johnson2016intel}, or the ISPs can run the attestation services by themselves~\cite{vinnie2018intel}.
% Intel Attestation Service (IAS) for the integrity guarantees of the \name enclave~\cite{johnson2016intel}. 
% Note that, alternatively, the ISPs can run the attestation services by themselves to avoid relying on IAS to verify the attestation report (see Section~\ref{sec:net-func-using-sgx}).
We also assume an idealized implementation of \codename that has no backdoor.
The full implementation of \codename is open-sourced for public scrutiny\footnote{\name is open sourced at \url{https://github.com/InNetworkFiltering/SGX-DPDK}}.
We leave a formal verification of \codename implementation as future work.
% Also, we assume an idealized hardware implementation of SGX; e.g., no backdoors in the SGX implementation. 
We consider all hardware and side-channel attacks (e.g.,\cite{gotzfried2017cache, last-level-cache, hahnel2017high}) as out of scope of this paper since countermeasures to these (e.g.,~\cite{chen2017detecting,gruss2017strong,shih2017t,pigeonhole,costan2016sanctum,song2018towards}) are orthogonal to the design of \codename. 
% Several solutions have been proposed to mitigate the side-channel attacks~\cite{chen2017detecting,gruss2017strong,shih2017t,pigeonhole,costan2016sanctum,song2018towards}.



==> paper 2/chapters/bypass.tex <==
\section{Scalable Filter Implementation}
\label{sec:data-plane-design}

\msk{(1) Single-enclave implementation. Two options: full packet copy vs. near-zero copy.}

\msk{(2) Multi-enclave implementation for scalable bandwidth handling}



Line-rate performance on commodity platform is a necessity for \name design. 
Without it, \name can handle large-scale DDoS only with either highly-specialized hardwares or large numbers of commodity servers and thus can be too costly to source ISPs. 
As more network function virtualization applications require high-speed packet processing on commodity platforms, line-rate on commodity ideas have been extensively studied. Most widely accepted solutions (e.g., DPDK\cite{dpdk}, Netmap\cite{rizzo2012netmap}, PF\_RING ZC\cite{pfring}) implement zero-copy networking and achieve minimum context switching by circumventing the use of kernel network stack. Netmap reports that with a single core of 900 MHz it achieves 14.88 Mpps sending or receiving rate on 10 GbE network adapters. Also, the performance report from DPDK shows the capability of zero packet loss forwarding with various packet size.

However, achieving line-rate speed seems quite challenging when we need to satisfy the two desired security properties of the data-plane operation of \name.

\begin{itemize}
    \item \textbf{Integrity of rate-limiting.} Each data packet's filtering decision (i.e., allow/block) must be made within the enclave to ensure the integrity of the filtering decision. 
    
    \item \textbf{Secure packet logging.} Every packet incoming to and leaving from \name should be recorded within the enclave for accountable billing and bypass detection.
\end{itemize}

The two security properties appear to require per-packet operation within the enclave as we can see in a naive data-plane design.

\subsection{Accountable per-packet processing} 

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.5\textwidth]{figures/near-zero-copy.pdf}
	\caption{Two packet copy approaches for SGX-based accountable rate limiting and logging functions. In the near zero-copy approach, we copy only the memory reference ($\ast$), the five tuple ($5T$), and the size ($s$) of the packet into the enclave.}
	\label{fig:near-zero-copy}
\end{figure}

%As briefly discussed in Section~\ref{sec:overview}, a simple implementation of \name would be to enclose all sensitive filtering operations and private information inside the enclave.
The two main secure functions implemented inside the enclave are the multi-class rate limiters and packet logging. 
To guarantee the accountable operation of these functions, a naive approach would be to make the entire copy of incoming packets into the enclave and operate these functions over the packet copies inside the enclave. 
Figure~\ref{fig:near-zero-copy}(a) illustrates this so-called full packet copy approach. 
Any data-plane packet is copied into the enclave memory for full packet logging and rate limiting operations. 
If the packet is determined to be allowed, it is logged again before being copied once again back to the untrusted memory pool for final forwarding through the NIC.
 
\paragraph{Prevention of bypass attacks with per-packet logging.}
This fine-grained packet processing in the enclave is useful for the detection of bypass attacks launched by $S$ to circumvent the \name filtering.
%The intuition behind this full packet copy approach is clear.
%... want to ... accountability of packet filtering decision and logging per incoming packet. 
%With this ... can detect bypass attempts by $S$. 
With the per-packet logging functions before and after the rate limiter (see Figure~\ref{fig:near-zero-copy}(a)), the enclave later can proof (1) if it has received a certain packet and (2) if it has allowed/dropped a certain packet. 
For such filtering accountability, one can imagine an memory efficient data structure, such as Bloom filters~\cite{bloom1970space}.
In practice, $D$ can periodically download the secure per-packet logging to match its own logging to detect any bypass (e.g., packet injections or drop outside of the enclave) has been conducted. 
Also, any customer network of $S$ (or even source hosts themselves) can query the enclave to check if their packets have been safely processed without any bypass attempt (e.g., $S$ drops packets before they reach the enclave). 

\paragraph{Performance challenges.}
Despite its clear security benefits, the per-packet processing inside the enclave incurs too much overhead for making full packet copies of all the data-plane packets, whose data rate can be even a few Gb/s or more. 
This full packet copy operation also would create too frequent context switching that is too expensive for such high-packet processing requirements.
Our evaluation confirms the poor performance of the per-packet processing approach; see Section~\ref{sec:eval}.

 
%
%\paragraph{Overview}. In this naive implementation, 
%
%\paragraph{Rate-limiting}
%
%\paragraph{Packet logging}
%
%\paragraph{Challenges}
% In this naive detector, our goal to make the each packet's {\em arrival} and {\em departure} (after the packet is processed and allowed) at and from \name {\em verifiable} by the source hosts and the destination ISP $D$, respectively.
% One natural idea is to log {\em all} the packets \name receives and all the packets it forwards to $D$.
% For the memory efficient operations, which are necessary for our high throughput networking applications, we use two sets of Bloom filters $b_{in}$ and $b_{out}$ for incoming packets and outgoing packets, respectively.
% These Bloom filter bit arrays are stored within a secure memory region, e.g., en SGX enclave, to prevent malicious \name operators from manipulating the logging and thus verification.
% We provide two functions, {\tt Add}$_{in}(\cdot)$ and {\tt Query}$_{in}(\cdot)$ also within the secure memory region for $b_{in}$ ({\tt Add}$_{out}(\cdot)$ and {\tt Query}$_{out}(\cdot)$ for $b_{out}$).
% {\tt Add}$_{in}(p)$ function updates $b_{in}$ based on the cryptographic hash outputs of the incoming packet $p$ and {\tt Query}$_{in}(p)$ returns a test result whether $p$ is in the Bloom filter $b_{in}$. {\tt Add}$_{out}(p)$ and {\tt Query}$_{out}(p)$ are similarly defined for the outgoing packet $p$. 

% With the full packet logging mechanism, external verifiers can easily check if a certain packet has been handled by \name by requesting the copy of the Bloom filter bit arrays $b_{in}$ and $b_{out}$ and comparing them with the local filter arrays.
% The destination ISP $D$ may maintain its own local Bloom filter for the packets from $S$ and compare it with the Bloom filter array obtained from \name.
% Provided the accurate time synchronization between \name and $D$\footnote{possible... via a secure channel between them...}, any discrepancy between their Bloom filter arrays indicates a potential bypass attack.
% For example, if an array index is set to 1 in the $D$'s local filter but set to 0 in \name's filter, it indicates the existence of one or more injected packets.
% Or, any index that is set to 0 in the $D$'s local filter but not in \name's filter implies that one ore more packets have been dropped against \name's policy. 
% Note that it is the verifier's discretion to determine these indications as the bypass attacks or the artifacts of normal network operations (e.g., natural bit errors or packet drops happened in the transit networks).

\subsection{Sufficiency of {\em per-traffic-class} processing}
%\subsection{Near zero-copy data-plane}
% \paragraph{Performance challenge.}
% Although the naive full packet logging can effectively detect bypass attacks by the malicious source ISP $S$, there still remains a serious performance challenge\,---\,that is, the {\em per-packet logging} operations of the Bloom filter requires \name to copy {\em all} the packets into the secure memory region, e.g., enclave.
% Such {\em full packet copy} operation is indeed the biggest throughput bottleneck since copying each full packet creates significant context switching overheads.

\paragraph{Per-packet guarantee is unnecessary.}
Regarding the necessity of the expensive per-packet processing in the enclave, we make an observation that even with the secure per-packet processing, $S$ still can affect the rate limiting operations of \name by simply re-ordering the incoming data-plane packets.
Our rate limiter implementation handles multiple traffic classes in individual token buckets and each token bucket maintains the time varying amount of tokens to determine if an incoming packet should be dropped or allowed. 
If $S$ re-orders the packets within the same traffic class, it can affect the filtering decisions of re-ordered packets. 
For example, let say two packets $p_1$ and $p_2$ arrive at \name in this order and only $p_1$ uses the available tokens and $p_2$ is dropped. 
If $S$ flipped the order of the two packets, $p_1$ would be dropped instead. 
Such packet re-ordering can be potentially exploited by $S$ to control the rate limiting decisions within the same traffic class. 
Unfortunately, such packet re-ordering that happens {\em outside} of the enclave cannot be detected by the \name system. 

\paragraph{Per-traffic-class processing is sufficient.}
Instead of building expensive but unnecessary per-packet processing inside the enclave, we choose to build a much coarse-grained, per-traffic-class processing for the enclave operations. 
Figure~\ref{fig:near-zero-copy}(b) illustrates how the per-traffic-class processing works with the enclave memory operation. 
When a packet is received, only a fraction of its header fields (the five tuple fields, $5T$, and the packet size, $s$) are copied into the enclave memory along with the memory reference ($\ast$) of the packet.
The copied fields $<\!5T,s\!>$ are then represents the packet and used for the logging functions and the rate limiter. 
The memory reference $\ast$ is used to perform the corresponding operation (e.g., forward or block) for the packet in the untrusted memory pool depending on the rate limiter decision. 

The per-traffic-class accountability still guarantees the incoming and forwarded traffic volume per traffic class, which is sufficient for bandwidth measurement for billing purposes. 
Moreover, this enables $D$ and the $S$'s customer networks to detect bypass attempts when $S$ violates the per-traffic-class volume enforced by the fairly composed filtering policy \PSD. 
For example, if $S$ drops or injects some packets in a traffic class outside of the enclave, $D$ or the $S$'s customer networks can detect it because the per-traffic-class volume should differ. 
Note that the per-traffic-class accountability allows $S$ to affect the packet filtering decisions within a traffic class (e.g., dropping $p_1$ instead of $p_2$ when both are in the same traffic class); however, as we discussed, this attack is also feasible when we enforce finer-grained, per-packet accountability and it is fundamentally undetectable by \name.
%
%Let us first take a look at a subtle adversary's action called packet modification. 
%So fare we have defined bypass attacks as the source AS's illegal packet removals and injections. 
%Thus, a packet {\em modification} (say packet $p$ is modified to $p'$) by $S$ seems to be considered as bypass attacks (since modification can be expressed as removal followed by injection).
%However, we observe that some packet modifications are in fact {\em not} necessarily considered as bypass of the rate limiting operations. % and thus our bypass detection requirements can be relaxed significantly.
%Let us consider a particular packet modification from $p$ to $p'$ with the two conditions: $p$ and $p'$ are in the same traffic class (i.e., $\texttt{class}(p)=\texttt{class}(p')$) and have the same packet length (i.e., $\texttt{len}(p)=\texttt{len}(p')$).
%
%We observe that this particular packet modification does {\em not} necessarily bypass the rate limiting operation of \name because it does not make any changes to the rate limiting operations. 
%Recalling that our rate limiter operates based on the traffic class and  the packet length of incoming packets, the modification attempt does not effectively bypass any rate limiting operation but only damage the integrity of packets, which we do not aim to guarantee (see Section~X. Packet integrity is a non-goal.)
%
%Note that any other packet modifications (e.g., $p$ and $p'$ are in different traffic class or their lengths are different) are indeed considered as bypass attacks since the modification does bypass the rate limiting decision of \name. 

%\paragraph{Relaxed detection requirements.}
\paragraph{Per-traffic-class operations enables {\em near zero copy}.}
%As we exclude the specific type of packet modifications from our definition of bypass attacks, we can relax our detection requirements significantly.
%Particularly, we can have larger granularity of packet logging as we do not need to consider unnecessary details of each incoming packet but only necessary information for rate limiting operations; i.e., five-tuple bits and packet length.
As Figure~\ref{fig:near-zero-copy}(b) illustrates, the per-traffic-class processing in the enclave significantly reduces the amount of bits we copy into the enclave and thus we achieve a {\em near zero-copy} packet processing. % where only a subset of packet headers (e.g., five tuple bits and packet length) are copied into the trusted memory region and used for per-packet logging.
%We use a simple byte counter per traffic class within a trusted execution environment that maintains the authentic copy of the per-class byte counts at \name. 
%The per-class byte counter values are later sent to the destination AS $D$ and compared with $D$'s own local per-class byte counter values. 
%Any discrepancy between the two implies the potential bypass attempt, as we discussed in the naive full packet logging, with the only difference that we have per-class detection granularity as opposed to per-packet granularity, which is unnecessarily too fine grained.
%
Our near zero-copy operation reduces the byte size of what we copy into the trusted environment significantly (e.g., reduced to about 1\% for 1.5 KByte packets and 20\% for 64 Byte packets).
We evaluate the efficiency of the near zero-copy operation of \name in Section~\ref{sec:eval}.

\subsection{Scalability in parallel deployment}
Given the architectural limitation of secure computing resources in currently available SGX hardware, \name's single-enclave deployment is hardly able to deal with the ever-growing attack volume. Therefore, we extend the \name design to allow a parallel deploying scheme with multiple instances while preserving the same level of security guarantee as in the single one. The core idea is to randomly and equally distribute the traffic load among multiple replicated \name instances - each instance runs independently with same supplied policies and same outbound traffic limit. 
With this design, we believe that the \name system is capable of filtering up to 100 Gb/s undesired traffic, which is a reasonable capacity goal for one \name contract to handle as more contracts can work together to rate-limit the multi-hundred-giga traffic in the real world. 

The idea of replicated instances aims to avoid any additional complexity in the design and to make keeping the security promise a more straightforward task - any bias in the system is detectable because each rate-limiter is intended to start with the same filtering policies and run against roughly same-sized traffic with a similar distribution among different traffic classes. With multiple instances behaving like a single instance of \name, the extended system still keeps the integrity of the per-traffic-class filtering decision even though each instance works independently. 

\paragraph{Parallel Deployment} The extended design consists of multiple \name instances and one load-balancer distributing the traffic among the instances in a random and even manner (see Figure~\ref{}). 
Unlike the \name instance, the load-balancer does not need to run on the trusted hardware, making it possible to handle 100 Gb/s traffic with commodity hardware or any other existing specialized hardware in $S$'s network. Another change is that the instances must identify each other by the Ethereum wallet address with the help of $D$ after their remote attestations with $D$ succeed. Also, they can further establish secure channels with the help of $S$ to ally themselves with others and detect misbehaviors as an alliance.

\paragraph{Detecting diverged policy}. As each instance accepts policies from $S$ and $D$ via separate channels, the polices one receives may differ from the others if any party intends to create difference among the instances, breaking the overall integrity of the policy composition. However, this inconsistency can be easily detected when all the instances share the hash of the policy they received at the beginning and find any mismatches among the hashes. As a defense, all the instance will cease and inform the other party to stop the contract.

\paragraph{Detecting biased traffic distribution}. Our design requires a high-speed and fair load-balancer entirely controlled by $S$,  making the traffic distribution prone to $S$'s manipulation for malicious purpose. For example, a biased traffic distribution can affect the rate-limiting decisions made in different instances and tamper the rate-limiting result in the view of the entire system. Luckily, this bias can be detected similarly by sharing the per-traffic-class packet logging information and comparing with each other. We will discuss the consequence of this later.

\paragraph{Generating consolidated proof with multiple signatures}. In the single instance scheme, the proof of contracted work is generated by the \name enclave along with the signature and submitted by $S$ to the \name contract on behalf of the enclave. The same approach still works in the parallel deployment with only one amendment: the proof has to be signed by all the others if no load-balancer misbehaviors are detected. Any missing signature will cause failure of the verification process in the smart contract, and $S$ will not get the reward for the submitted work. 
%---------OLD------------
%\subsection{Tradeoff between accountability granularity and packet processing speed}
%
%\deli{Performance comparison: A Mpps vs B Mpps}

% \paragraph{Privacy-preserving traffic class granularity.}
% For the channel between $M$ and $D$, we use the traffic classes of $D$. 

% This creates a subtle problem. $S$ may attempt to bypass its own traffic class while satisfying $D$'s classes. 
% We argue that this is okay as this act harms the adversary himself only.

% For the channel between the traffic sources and $M$, we use the source IPs.



==> paper 2/chapters/class-partition.tex <==
\section{Traffic Class Partition}
\label{sebsec:class-partition}

ISPs determine their policies $P_S$ and $P_D$ by translating their internal
traffic management policies; e.g., proprietary agreement for premium access,
higher priority for mission-critical services, black-listed or suspicious
networks.  A resulting filtering policy has one or more traffic classes.  A
{\em traffic class} represents a group of packets (e.g., a five-
tuple\footnote{\{Source IP, destination IP, source port number, destination
port number, and protocol\}.} defined flow aggregate) that are treated with
the same filtering configuration; e.g., any web (port 80 or 443) packet from a
group of hosts in an IP prefix to a group of server clusters.  We require that
each traffic class set ($C_S$ or $C_D$) is an exact cover of $U$ (i.e.,
traffic classes in each set ($C_S$ or $C_D$) are pairwise disjoint and the
union of all the traffic classes in each set is equal to $U$) so that each
policy covers all the flows in the entire address space.

The sets of traffic classes $C_S$ and $C_D$ in two policies $P_S$ and $P_D$,
respectively, are independently decided by the two ISPs and thus they are
likely to be different.  When they are unequal, as in most cases, the \name
middlebox should further partition the traffic classes in $C_S$ and/or $C_D$
until the two sets become identical.  This traffic class partition is
necessary as one cannot easily compare two policies when their traffic class
sets are different.  For example, when we have eight flows ($f_1,\cdots,f_8$),
the two traffic class sets can be differently defined as
$C_S=\{{\{{f_1,f_2}\},\{{f_3,f_4,f_5}\},\{{f_6,f_7,f_8}\}}\}$ and
$C_D=\{{\{{f_1}\},\{{f_2,f_3}\},\{{f_4,f_5,f_6,f_7,f_8}\}}\}$, then the
partitioned traffic class set is calculated as
$C_{S,D}=\{{\{{f_1}\},\{{f_2}\},\{{f_3}\},\{{f_4,f_5}\},\{{f_6,f_7,f_8}\}}\}$.
Two policies $P_S$ and $P_D$ can be expressed with the same traffic class set
$C_{S,D}$ and thus they are comparable.  Note that, as we see in this example,
we want the number of traffic classes in the partitioned set $C_{S,D}$ to be
minimized to remove unnecessary traffic classes.

\subsection{Recovering $C_{victim}$ without a priori information}
\label{subsec:csd-attack-strong}

The attacker wants to learn the victim's policy. This comprises of the traffic
classes and their relationship. For this the attacker first learns the $C_{S,
D}$ and the recovers the rate-limit for each class.

\paragraph{Forcing $C_{SD} = C_{victim}$.}
The attacker specifies a policy where all the points belong to a one class
i.e., $C_{attacker} = C_U$. This policy is an identity policy because it does
not affect the victim's classification. Thus, $\mathcal{C}(C_U, C_{victim}) =
C_{victim}$. For example, lets say that the victim's classification is
$C_{victim} = \{\{f_1,f_2\},\{f_3,f_4,f_5\}\}$ and the attacker choses his
classification as $C_{attacker}=\{\{f_1,f_2, f_3,f_4,f_5\}\}$. The resultant
re-classification $C_{s,d} = \{\{f_1,f_2\},\{f_3,f_4,f_5\}\}$. Thus, the
attacker can always ensure that the classification used by the middlebox is
exactly the same as the victim.

\paragraph{Learning the limit-rate of a class.}
When the middlebox sees a packet, it first identifies which class the packet
belongs to and then refers to the composite policy to probabilistically decide
whether to drop or keep the packet. The rate of dropping a packet is directly
defined by the rate-limiting function and the rank of that packet's class in
the policy.  The attacker knows that the output rate of the packets being
transmitted is capped to a $L$ bps pre-specified and known to both the ISPs.

%without work-conserving rate-limiters
If the source ISP is the attacker, it controls the types and number of packets
it can deliver to the middlebox. To learn the composite policy, the source ISP
starts adaptively pre-filtering the traffic it sends to the middlebox.
Specifically, it starts filtering all the traffic and floods the middle box
only say 2L packets which belong to one class $C_3$ whose class rate is
$P_{C_3}$. The middlebox consults the policy and drops $(2L) * (1 - P_{C_3})$
of the input packets. The attacker measures the number of total packets that
are being forwarded which is $(2L) * P_{C_3}$. The attacker can easily reverse
engineer that the limit-rate for $C_3$ is $P_{C_3}$.

\paragraph{Work-conserving rate-limiters.}
One way to make this attack difficult is to always saturate the output link
and keep the output volume at a constant volume of $L$ bps. Such mechanism is
well known as {\em work-conserving rate-limiters}~\cite{}. Thus, when the
attacker floods the middlebox with $2L$ bps packets from the same class,
instead of limiting the traffic to  the rate limiter with limit the traffic to
$(2L) * P_{C_3}$ bps which is less than $L$, the middle box will send out
packets at the rate of $L$ bps. When such a measure is in place, our attack is
not effective because the attacker only sees a constant encrypted output
traffic of $L$ bps.

\paragraph{Probe packets.}
The attacker can still circumvent the effect of  work-conserving rate-limiters
and learn the rate at which the middlebox is dropping the packets. To do this,
the attacker prepares {\em probe packets}. If a probe packet is delivered to
the victim, the attacker sees a response packet; if the packet is dropped the
attacker does not see any response packet. For example, the attacker prepares
$L$ packets of each class and floods the channel. i.e., if we have $4$ classes
$c_1, c_2, c_3, c_4$, then the attacker creates $4L$ traffic.  He lets the
middlebox filter the traffic to maintain a rate of $L$ and observe $r_1, r_2,
r_3, r_4$ responses per class. Then he learns that the rate for each classes
is $r_i/L$.

\paragraph{Search for partition classes.}

\begin{itemize}
	
	\item {\bf Enumeration.}
	The total number of partitions of an n-element set is given by exponential
	generating function  $\sum_{n=0}^{\infty}{\frac{B_{n}}{n!}}z^{n}=e^{e^{z}-1}$.
	The attacker can enumerate each of these possible partition classes until it
	finds the right partition class of the victim. However, the enumeration size
	quickly grows from $15$ options for $4$ elements to $4140$ options for $8$
	elements.

	\item {\bf Clustering after learning rates for each point.}
	The attacker floods the network with packets with same header $h_i$
	(represents a single point in the header space) and observes what is the
	rate-limit for it, say $r_i$. The attacker does this for all points in the
	header space and collects all the $r_i$ for $0 < i < n$. The it clusters
	all the $i$ which have the same rate. This directly tells the attacker
	that all these $i$ belong to the same class, since they have the same
	rate-limit.
	
	\item {\bf Partitioned Search.}
	The attacker first learns the rate for point 1 to be $r_1$ by sending only
	packets with header $h_1$. The attacker now knows that the rate-limit of
	the class which $h_1$ belongs to, is $r_1$. Then it starts sending equal
	number of packets for $h_1, h_2$ and observes the total output rate. If it
	is $r_1$, then $h_1, h_2$ both belong to the same class. If the new rate
	is $r > r_1$, then $h_2$ belongs to a different class whose rate-limit
	$r_2 = r - r_1$. Now the attacker can repeat this process to check the
	membership of $h_3$: check the rate for $h_1, h_3$ and $h_2, h_3$ to see
	if $h_3$ belongs to $h_1$'s class or $h_2$'s class. This strategy is
	similar to finding the right path in a search graph.

\end{itemize}

\subsection{Recovering $P_{s, d}$}
\label{subsec:psd-attack}

So far, we have assumed that the attacker (source ISP or destination ISP)
knows the composite policy $P_{s,d}$ computed by any one of our algorithms.
Here we show how this is possible. The attacker can repeat the process in
Section~\ref{subsec:csd-attack-strong} for all the traffic classes and learn
all the $P_{C_i}$. This directly leaks the composite policy $P_{s, d}$ being
deployed by the middlebox.

% We know that each class in the order-based policy comprises of IP addresses.
% When the middlebox sees a packet, it first identifies which class the packet
% belongs to and then refers to the composite policy to probabilistically decide
% whether to drop or keep the packet. The rate of dropping a packet is directly
% defined by the rank of that packet's class in the policy.  The attacker knows
% that the output rate of the packets being transmitted is capped to a $L$ bps
% pre-specified and known to both the ISPs.

% If the source ISP is the attacker, it controls the types and number of packets
% it can deliver to the middlebox. To learn the composite policy, the source ISP
% starts adaptively pre-filtering the traffic it sends to the middlebox.
% Specifically, it starts filtering all the traffic and floods the middle box
% only say 2L packets which belong to one class $C_3$ whose class rate is
% $P_{C_3}$. The middlebox consults the policy and drops $(2L) * (1 - P_{C_3})$
% of the input packets. The attacker measures the number of total packets that
% are being forwarded which is $(SL) * P_{C_3}$. The attacker can easily reverse
% engineer that the class-rate for $C_3$ is $P_{C_3}$. The attacker can repeat
% this process for all the traffic classes and learn all the $P_{C_i}$. This
% directly leaks the composite policy $P_{s, d}$ being deployed by the
% middlebox.

==> paper 2/chapters/conclusion.tex <==
\vspace{-5pt}
\section{Conclusion}
% \vspace{-5pt}
In-network filtering has numerous known advantages over other proposed DDoS defenses, but the deployment of any of its variants has been stifled. 
Our proof of concept \name system addresses one of the core, but largely neglected, problems of source filtering---lack of filtering verifiability---and demonstrates that verifiable in-network filtering is indeed possible with a practical hardware root of trust support. 
We hope that our study renews discussion on the deployment of in-network filtering in the IXPs and encourages more sophisticated yet auditable filter designs, such as stateful firewalls.

==> paper 2/chapters/deployment-proposals.tex <==
% \vspace{-5pt}
\section{Practical Deployment at IXP}
\label{sec:deployment-proposals}

\name has a generic architecture designed for any transit networks (e.g., Tier-1 or large Tier-2 ISPs); yet, as the first deployment model, we suggest to deploy it in major Internet exchange points (IXPs).
%
In this section, we present why IXPs, among other transit infrastructure, are the ideal places to introduce our verifiable in-network filtering (\S\ref{sec:ixp-overview}). 
We also provide a deployment example of \name at an IXP (\S\ref{subsec:ixp-deployment}) and then evaluate the effectiveness of \codename at IXPs against DDoS attacks with two real attack source data (\S\ref{subsec:against-ddos-exp}).
Finally, we provide a simple cost analysis for deploying \name service at an IXP for filtering up to 500 Gb/s traffic (\S\ref{subsec:deployment-cost}).

% In the last decade, IXPs have become the central infrastructure of the global Internet connectivity~\cite{ager2012anatomy,chatzis2013there}, with large IXPs handling daily traffic volumes comparable to those carried by the largest Tier-1 ISPs, which makes the IXPs the perfect candidates for our verifiable filtering service~\cite{dietzel2016blackholing}.
% Moreover, unlike the slowly evolving traditional transit ISPs, IXPs are more flexible in integrating with software-defined architecture~\cite{gupta2015sdx}, thus easily providing new value-added services (e.g., fine-grained inter-domain access control~\cite{gupta2016authorizing}, traffic engineering~\cite{dietzel2017sdn}).

% In this section, we provide a deployment example of \name at an IXP.
% We consider the \name IXP has a generic architecture that includes a layer-2 switching fabric, a route server (which is not highlighted in our paper), and a logical central controller for software-defined switches~\cite{gupta2015sdx,gupta2016industrial}.
% We also provide a simple cost analysis for deploying \name service for filtering up to 500 Gb/s traffic.




% \vspace{-5pt}
\subsection{Internet Exchange Points (IXPs)} 
\label{sec:ixp-overview}
% \vspace{-5pt}
% \vyas{you may want to expand a bit more on this subsection for a security audience. maybe take a look at the original IXP paper and the new SDX paper and add a figure or two to explain the concepts. I worry that this may be a new concept for many security readers. Like the main questions -- whats an ixp? how is it diff from regular exchange/peering? what new capabilkities are being offered? why is there excietment in the operational commmunity etc -- the original sigcomm paper would be a good starting point to do this mini tutorial here}


% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[width=0.35\textwidth]{figures/ixp-overview.pdf}
% 	\vspace{-5pt}
% 	\caption{IXP overview.}
% 	\vspace{-15pt}
% 	\label{fig:ixp-overview}
% \end{figure}

IXPs are physical locations where multiple autonomous systems (ASes) peer and exchange traffic and BGP routes. 
% As Figure~\ref{fig:ixp-overview} illustrates, 
Essentially, an IXP is a large layer-2 fabric and connects ASes (e.g., ISPs, content providers, cloud providers) in close proximity. 
IXPs provide great convenience to ASes in making peering relationship with many (e.g., hundreds or thousands) other ISPs without the hassle of individual bilateral agreements. 
% Each participating AS (or a {\em member} AS) exchanges BGP routes and directs traffic to other participants over the layer-2 IXP fabric. 
The Internet currently has more than 600 globally distributed IXPs~\cite{caida-ixp} and some large IXPs serve multi-Tera b/s traffic volume, which is comparable to large Tier-1 ISPs~\cite{ager2012anatomy,chatzis2013there}.

% As an ISP makes a peering connection with an IXP (i.e., becomes a {\em member} of the IXP), the ISP can automatically peer with all other members of the IXP. 
%Usually peering relationship but recently offer new business model (need to check this...).
% IXPs recently have become the central infrastructure of the Internet connectivity with many big IXPs having more than hundreds or thousands members~\cite{ager2012anatomy, caida-ixp}. 

Recently, as more video content providers and large cloud providers rely on IXPs for lower cost but faster transit of their traffic, emerging {\em value-added services} are expected from IXPs; e.g., application-specific peering,  inbound traffic engineering,  wide-area server load balancing, and redirection through middleboxes~\cite{gupta2015sdx}.
% latency  IXPs... more video ... ... content providers, cloud networks, and regional large ISPs. 
% More connectivity and more value-added services thar are not readily available or costly to deploy in traditional transit ISP networks: 
New innovation for these value-added services has been possible because IXPs have a flexible architecture model (especially, compared to traditional transit networks, such as ISPs).
An IXP usually consists of a single data center in a single physical facility;
thus, software-based architecture available for data centers can be easily adopted; see software-defined IXPs~\cite{gupta2015sdx, gupta2016authorizing,gupta2016industrial}.
% New value-added services thus can be easily implemented on the software-based IXP architecture~\cite{gupta2016authorizing,dietzel2017sdn,conti2017blocking}.

% o In short, not only are IXPs the
% right place to begin a revolution in wide-area traffic delivery, but the
% organizations running these IXPs have strong incentives to innovate.

Due to their topological centrality, however, IXPs unfortunately often suffer from collateral damage when other networks are targeted by DDoS attacks~\cite{pospichal2017new}. 
Worse yet, IXPs are sometimes directly targeted by DDoS attacks; see an attack incident in 2016 against multiple IXPs: AMS, LINX, and DE-CIX~\cite{bright2013can}. 
A traffic filtering service could easily be a natural next value-added service for IXPs~\cite{dietzel2016blackholing}.
% It is not hard to imagine the SENSS-like~\cite{ramanathan2018senss} in-network filtering can be easily adopted to major IXPs.

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/ixp-deployment.pdf}
% 	\vspace{-5pt}
	\caption{Deployment example of \name at IXP.}
% 	\vspace{-15pt}
	\label{fig:ixp-deployment}
\end{figure}

\subsection{Deployment example at IXP}
\label{subsec:ixp-deployment}

We consider the \name IXP has a generic architecture that includes a layer-2 switching fabric, a route server (which is not highlighted in our paper), and a logical central controller for software-defined switches~\cite{gupta2015sdx,gupta2016industrial}.
%
Figure~\ref{fig:ixp-deployment} illustrates a deployment example of \name at an IXP.
The filtering IXP sets up one or more commodity servers with SGX support. % and the network interface controllers (NICs) connecting to them.
% Also, the IXP supports remote attestation and filter rules acceptance services in its controller so that a victim network can initiate a \name session and install filtering rules.
% 
% We now describe how a victim network gets its incoming traffic filtered at a \name IXP. 
When a victim network is under DDoS attack, it contacts the controller of the \name IXP via an out-of-band channel.\footnote{We assume this channel is available even when the victim network is under attacks.
ISPs traditionally have maintained out-of-band channels (e.g., external email servers, telephone lines~\cite{dots-slides}) for inter-ISP communication.} % and ISPs contact other ISPs when hit by large-scale DDoS attacks for manual collaboration defense schemes (e.g., large-scale ISP coordination during the ProtonMail attack).
%Completely independent out-of-band channels, such as cellular Internet connectivity, can be also assumed for the backup connectivity during the worst DDoS attacks.}
As suggested in~\cite{ramanathan2018senss}, the victim network can easily authenticate to the IXP via Resource Public Key Infrastructure (RPKI)~\cite{lepinski2012infrastructure}.
% 
The victim network asks the filtering IXP to create one or more SGX filters and audits it by receiving the validation attestation report(s). %; see Section~\ref{sec:net-func-using-sgx}. 
After being convinced that the filters have been set up properly (i.e., the remote attestation is done), the victim network establishes a secure channel with the enclaves (e.g., TLS channels) and submits the filtering rules. % and trigger the rules re-distribution if needed.
The load balancing algorithm at the IXP controller receives the rules from the filter parallelization (see Section~\ref{sec:optimization-multiple-enclaves}) and accordingly controls the switches to distribute traffic destined to the victim network to the enclaved filters.
% In \name, filter rules are {\em not} secret.
The \name IXP eventually learns and analyzes all the rules in this step.
Finally, the enclave filters perform packet filtering based on the submitted rules and forward the allowed traffic to the victim network.


% In step (1), the victim network contacts the \name IXP via an out-of-band channel and establish a secure channel.
% Note that we assume this channel is available even when the victim network is under attacks; see below in this section for more discussion.
% They rely on the Resource Public Key Infrastructure (RPKI) to authenticate each other and their network addresses. 
% In step (2), the \name IXP and the victim network negotiate high-level parameters (e.g., bandwidth limit, pricing) in one or more rounds of message exchanges. 
% In steps (3) to (5), the \name IXP creates one or more filter enclaves, conducts remote attestation, and provides the attestation validation report(s) to the victim network; see Section~\ref{sec:optimization-multiple-enclaves}. 
% In step (6), the victim network securely submits its filtering rules to the filter enclave. 
% In step (7), the enclave performs packet filtering based on the submitted rules and forwards the allowed traffic to the victim network.  
% In step (8), the enclave returns the verifiable report to the \name IXP. 

% o we need commodity servers with SGX support and 10 Gb/s NICs.

% o As we show in the next section... near full line-rate is achieved. 

% o Thus, for handling 500 Gb/s attack traffic, an IXP needs to invest in 50 modest SGX-supporting commodity servers, which would occupy only one or two server racks. 

% o SGX filter initiation (similar to the TESEF setup steps)

\subsection{Effectiveness of \codename at IXPs against DDoS Attacks}
\label{subsec:against-ddos-exp}

\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/IXP-coverage-openres.pdf}
        \vspace{-10pt}
        \caption{Vulnerable DNS resolvers}
        \vspace{-5pt}
        \label{fig:ixp-openres}
    \end{subfigure}
    \begin{subfigure}[t]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/IXP-coverage-mirai.pdf}
        \vspace{-10pt}
        \caption{Mirai botnets}
        \vspace{-5pt}
        \label{fig:ixp-mirai}
    \end{subfigure}
	\vspace{-5pt}
    \caption{The ratio of attack sources that are handled by the \name filters for the two attack source data. $(^*)$: Top-$n$ IXPs denote the $n$ largest IXPs in each of the five regions, see Table~\ref{tab:top-ixps} in {{Appendix~\ref{sec:top-ixp}}}.}
    \vspace{-7pt}
    \label{fig:ixp-coverage}
\end{figure}

% Until now, we have considered a {\em single} \name session between a pair of ISPs.
%Recent major DDoS attacks, however, often involve multi-million bots or amplifiers (or reflectors) that are distributed across large numbers of ASes, which necessitates multiple, concurrent \name sessions with many source ASes. 
%
We analyze how much DDoS attack traffic can be filtered by \name at IXPs with two real attack source data: 3 million vulnerable open DNS resolver IP addresses~\cite{wessels2014open} and 250 thousand Mirai bot IP addresses~\cite{mirai}.

\paragraph{Simulation setup.}
In our inter-domain routing simulation, we use the CAIDA Internet measurement data with the inferred AS business relationship~\cite{caida} and the peering membership of world-wide IXPs~\cite{caida-ixp}.
We randomly choose 1,000 Tier-3 ISPs as the DDoS victims and consider that each victim receives attack traffic from all the attack sources (e.g., open resolvers and bots) in each case.
To determine a traffic forwarding path between autonomous systems (ASes), we assume that each of them applies the following widely adopted BGP routing policies in order~\cite{gill2013survey,gao2001inferring}:
% \begin{packeditemize}
(1) the AS prefers customer links over peer links and peer links over provider links;  (2) the AS prefers the shortest AS-path length route; and
(3) if multiple best paths exist, the AS uses the AS numbers to break the tie. 
% \end{packeditemize}

% Particularly, the first policy guarantees that the created AS-level routes are {\em economically viable} because it ensures that all the ASes on the routes are guaranteed positive revenues.

% For inter-domain route simulation, we ... BGP ... policy... \msk{@muoi, please copy some text from our S\&P submission}.
% IXP data... from CAIDA as well~\cite{caida-ixp}.

We assume that the victim network establishes \name sessions with several largest IXPs (e.g., the biggest IXPs in each of the five regions, as shown in Table~\ref{tab:top-ixps}, see {{Appendix~\ref{sec:top-ixp}}}). 
We compute the ratio of flows from the attack IP addresses to the victim network that are handled by at least one of the established \name filters at the selected IXPs.
A traffic flow is said to be transited at an IXP if it traverses along an AS-path that include two consecutive ASes that are the members of the IXP.

\paragraph{Results.}
Figure~\ref{fig:ixp-coverage} shows how many attack flows can be effectively handled by the in-network filters if installed in some large IXPs.
The box-and-whisker plots show the distribution of the ratio of handled attack IPs when Top 1--5 biggest IXPs in the five regions (thus, 5--25 IXPs globally in total) perform in-network filtering service for DDoS defense. 
In each plot, the solid lines represent the first and the fourth quartile of the data set and the ends of the whisker indicate the 5th- and 95th-percentiles. 
Also, the red band inside the box represents the median.

Even when a single IXP in each region (thus, total five IXPs worldwide) adopts the \name filters, the majority of both attack sources (e.g., vulnerable resolvers, botnet) are handled by the \name IXPs.
Approximately, 60\% of attack mitigation is expected for the median cases, and 70-80\% mitigation can be achieved for the top quarter cases.
As more IXPs adopt the \name filters, even more effective mitigation is achieved.
Particularly, Top-5 IXPs per these regions appear to be sufficient enough to offer more than 75\% attack mitigation for the median cases, and 80-90\% of attack mitigation for the upper quarter cases. 

% Note that our result is not surprising at all.
% It is well-known that some big IXPs already peer with thousands of ISPs and serve multi-Tera b/s traffic volume, which is comparable to large Tier-1 ISPs~\cite{chatzis2013there}.


\subsection{Deployment Cost Analysis}
\label{subsec:deployment-cost}
Let us provide a ballpark estimate of the cost of deploying \name at an IXP to handle 500 Gb/s of traffic.
Note that the 500 Gb/s filter capacity at a {\em single} IXP appears to be sufficient because the attack volume at each IXP can be much lower than the aggregated volume at the victim network.
For instance, it would require only a few \name IXPs with similar capabilities to mitigate the biggest DDoS attack ever recorded with 1.7 Tb/s attack traffic~\cite{zdnet2018ddos}.
% The main bottleneck for this deployment is the bandwidth limit supported by each SGX machine with 4 cores processor is close to 10 Gb/s only, as acknowledged in several existing works (e.g., \cite{naylor2017and}).

Our experiment in Section~\ref{sec:data-plane-performance} shows that a near full line-rate performance of 10 Gb/s per server with four SGX cores is easily achieved. 
% 
Thus, to handle 500 Gb/s attack traffic, an IXP needs to invest in 50 modest SGX-supporting commodity servers, which would require only one or two server racks.
With a commodity server cost is approximately US\$ 2,000, the filtering IXP only needs to spend for one-time investment for US\$ 100K to offer an extremely large defense capability of 500 Gb/s.
% This cost can be further reduced as there are more processors with six or more cores available on the market.~\footnote{List of SGX-enabled processors is available at: \url{ark.intel.com}} % and SGX performance is continuing to be enhanced.
The capital expenditure can be borne by the member ASes (hundreds or thousands) and/or can be amortized by the service fees if the filtering service is economically compensated by the payment from the victims~\cite{ramanathan2018senss}.
% , as suggested by SENSS~\cite{ramanathan2018senss}.
A rigorous economic analysis of \name operations in IXPs is out of the scope of this paper and is left for future work.



% ==================================================================================



% We only need some modest commodity servers (approximately US\$ 2K-3K per server).

% Thus, only 200-300 USD per 1 Gb/s defense capability. 
% For extremely large defense capability 500 Gb/s, only 100K-150K.

% Cost can be borne by the members (hundreds or thousands) and also can be amortized by the service fees if the filtering service is economically compensated by the payment from the victims, as suggested by SENSS~\cite{ramanathan2018senss}.
% We leave more rigourous economic analysis... for future work. 

% --

% In this section, we present an example of bootstrapping a \name filter at an IXP. 
% A DDoS victim network may create multiple \name filters in multiple IXPs by executing the following steps separately. 
% We explain the necessary steps to establish a \name contract with a victim network and execute packet filtering and forwarding during DDoS attacks. % targeting the destination network $D$.

% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[width=0.40\textwidth]{figures/overview-sigcomm.pdf}
% 	\vspace{-5pt}
% 	\caption{\name's bootstrapping example with a DDoS victim network. (NOC: Network Operations Center, RPKI: Resource Public Key Infrastructure, and IAS: Intel Attestation Service.)}
% 	\vspace{-15pt}
% 	\label{fig:overview}
% \end{figure}

% Bootstrapping with IXP members (i.e., neighbor ISPs) is almost identical to the above steps except step (6).

% \updatedlast{
% It is worth noting the three design considerations of our end-to-end deployment: {\em reliance on RPKI}, {\em IP-spoofing detection}, and {\em network availability of $D$}.
% }

% \paragraph{Reliance on RPKI.}
% The \name IXP should not only verify the identity (e.g., AS number) of the victim network but also the address resource to ensure that only the authorized filter rules are executed by the filter enclave.
% As suggested in~\cite{ramanathan2018senss}, we also rely on RPKI~\cite{lepinski2012infrastructure} for the origin authentication and resource validation of ISPs~\cite{rpki-database}.
% See Section~\ref{sec:multiple-session-rpki} to see how the reliance on RPKI affects the effectiveness of \name in practice. 


% \paragraph{IP-spoofing detection.}
% Many volumetric attacks do not send IP-spoofed packets to the victims; e.g., DNS amplification traffic comes from real IP addresses of resolvers.\footnote{Attack queries are IP spoofed but not the responses.} %, multi-million IoT-botnet DDoS attacks often use their real IP addresses. 
% However, IP spoofing is still allowed in many networks~\cite{beverly2013initial} and thus \name needs to still detect IP spoofing effectively.
% Let us consider that a bot in an ISP $A$ sends a packet $p_A$ (i.e., $\texttt{TrueScrIP}(p_A) \in \texttt{AddressSpace}(A)$) to $D$ with the source IPs spoofed with the IPs owned by $S$ (i.e., $\texttt{SpoofedSrcIP}(p_A) \in \texttt{AddressSpace}(S)$).
% When $D$ receives a large number of such spoofed packets, $D$ would contact $S$ ({\em not} $A$ due to the lack of traceback capability) to install a \name filter.
% Since $A$ is not \name controlled, $D$ will continue to receive the spoofed traffic from $A$ even after the \name contract is activated.
% This may confuse $D$ since it cannot determine whether the excessive traffic with the source IPs of $S$ is actually coming from misbehaving $S$ or from other networks that allow source spoofing. 
% \\\indent
% To handle this, \name makes the enclave-processed packets {\em distinguishable} from the IP-spoofed packets.
% We present two potential options.
% First, $S$ and $D$ set one or more point-to-point tunnels (e.g., GRE tunnels) between them to encapsulate the forwarded packets.
% This is a commonly used approach to send the scrubbed traffic back to destination networks by many DDoS scrubbing service providers (e.g., Arbor Networks, Neustar, Incapsula, Level3).
% Second, the \name filters mark a few bits of the forwarded packets with the patterns only known to the filter and the destination network. 
% To mark the packets, \name would need to borrow bits from fields that are not otherwise used.
% Several candidates include 6-bit DS field, 16-bit IP Identification field (when DF flag is set), and 20-bit Flow Label field (only for IPv6)~\cite{fayazbakhsh2014enforcing}.\footnote{
% 	Note that an adversary may generate a large volume of IP-spoofed packets to overwhelm the destination network's local filtering/bandwidth capability. 
% 	Since \name makes the detection of IP-spoofed traffic trivial, the destination network may rely on other orthogonal countermeasures (e.g., BGP-based blackhauling) effectively.}



% \paragraph{Availability of NOC at victim ISP.}
% \updatedlast{
% We assume the Internet connectivity of a network operations center (NOC) of an ISP even when it is under DDoS attack.
% It is based on the observation that ISPs traditionally have maintained out-of-band channels (e.g., external email servers, telephone lines~\cite{dots-slides}) and ISPs contact other ISPs when hit by large-scale DDoS attacks for manual collaboration defense schemes (e.g., large-scale ISP coordination during the ProtonMail attack~\cite{protonmail}).
% Completely independent out-of-band channels, such as cellular Internet connectivity, can be also assumed for the NOCs' backup connectivity during the worst DDoS attacks.
% }

%\input{chapters/tesef_details}



==> paper 2/chapters/design.tex <==
\section{Policy Composition}
\label{sec:policy-composition}

Policy composition takes two input policies $P_S$ and $P_D$, and creates a
resultant composed policy $P_{S,D}$. The \codename middlebox uses this composite
policy to filter incoming packets from the source ISP $S$. 
In our composition, we use the policy abstraction we propose (see Section~\ref{sec:proposed-policy}); 
particularly, traffic classes are marked with preference rankings and Kendall tau metric
is used to define the distance between any two policies.

In this section, we define the fairness and privacy properties we wish to achieve
in more formal terms and define the goals of the policy composition function $\phi$. 
Then, under that proposed policy abstraction, we propose a set of deterministic and non-deterministic algorithms
that maximize the fairness while ensuring an adequate level of policy privacy. 

%The first step in policy
%composition is to calculate the composite traffic classes. \codename
%calculates the composite traffic-class set $C_{s,d}$ by breaking the traffic
%classes in input policies into smaller (i.e., finer-grained) traffic classes
%until both $C_{s}$ and $C_{d}$ can be expressed by $C_{s,d}$.  The number of
%traffic classes in the final composite $C_{s,d}$ is in the range of
%$[\max(|C_s|,|C_d|),|C_s|\times|C_d|]$ (inclusive at both ends). Once
%\codename has converted input policies as order preferences over uniform
%traffic classes, it calculates the composite policy $P_{s,d}$ using a
%composition function $\phi$.

% \subsection{Balancing Fairness \& Privacy}
\subsection{Metrics for Fairness \& Privacy}
\label{subsec:metrics-tradeoff}

%As an example, consider input policies
%$P_S = (1, 3, 2, 4)$ (where $i$-th element represents the rank of the $i$-th traffic class)
%and $P_D = (2, 1, 3, 4)$. 

The fairness and privacy of the resulting composite policy is a sensitive to
the choice of composition algorithms. 
We can express fairness of a composition function $\phi$ as $\mathcal{F}(\phi) =  |d(P_S,P_{S,D}) -
d(P_D,P_{S,D})|^{-1}$. Our aim is to find a $\phi$ that maximizes
$\mathcal{F}(\phi)$ for all possible input policies $P_S$ and $P_D$.
Given $P_S$
and $P_{S,D}$ we can define our privacy function $\mathcal{P}_S(\phi)$  as the
set of unique $P_D$'s such that $\phi(P_S, P_D) = P_{S,D}$. 
Similarly, we define the privacy function $\mathcal{P}_D(\phi)$ for given $P_D$ and $P_{S,D}$ as the 
number of unique $P_S$'s such that $\phi(P_S, P_D) = P_{S,D}$.
Note that $\mathcal{P}_S(\phi)$ ($\mathcal{P}_D(\phi)$) are the anonymity set 
for $D$ ($S$) as the real input policy $P_D$ ($P_S$) can be indistinguishable
within these set of other possible policies.

By these definitions, an ideal composition function $\phi$ is one which
maximizes both fairness $\mathcal{F}(\phi)$ and privacy $\mathcal{P}(\phi)$. 
We can achieve ideal fairness where
$d(P_S,P_{S,D}) = d(P_D,P_{S,D})$ such that $|d(P_S,P_{S,D})- d(P_D,P_{S,D})|
= 0$ then $\mathcal{F}(\phi) = 0^{-1} = \infty$. Thus, an ideal fair $\phi$
function is the one which  finds a policy $P_{S,D}$ that is {\em equidistant} from
both the input policies $P_S$ and $P_D$. Ideal privacy is achieved when the 
composite policy $P_{S,D}$ is completely independent of the input policies i.e., the
attacker's anonymity set size equals all possible policies in the language.
We can say that the
ideal anonymity set of the composite policy is the number of unique policies
possible with a given language and the traffic classes. In case of the policies with
four traffic classes and strictly ordered preference ranks, 
the $\phi$ function which randomly choses a policy from $24$ (or $\mathtt{factorial}({4})$) choices
achieves maximum privacy because by observing the output policy, the attacker
learns nothing about the input policies. As it is evident from this example,
ideal privacy may not preserve any fairness.

\input{chapters/recon-algo}

\input{chapters/privacy}

\input{chapters/sec-analysis}

==> paper 2/chapters/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

We discuss several commonly asked questions regarding the designs and usages of the \name system. % and its potential deployment issues.

%\smallskip
%\paragraph{Will the trust establishment of \name solve the adoption problem of source filtering?}
%As we admit in Introduction, we do {\em not} claim that the lack of trust is the only left necessary condition that has been holding Internet-scale adoption back. 
%From our careful review of the large body of academic work~\cite{mahajan2002controlling,mirkovic2002attacking,argyraki2005active,liu2008filter,alwabel2015senss} and recent industry and standard efforts~\cite{huawei2015cca,cymru,dots-slides,levy2017operationalizing} on source filtering, we conclude that, perhaps to our surprise, the inter-ISP trust issue has been largely neglected.
%We show in this paper that addressing the trust issue addresses several security concerns between ISPs (see Section~\ref{sec:threat-model}). 

%\paragraph{\updated{If both two ISPs have incentives for collaboration, why would the source ISP misbehave?}}
%\updated{Even when the two ISPs collaborate for their own benefits, there is still a need to safeguard against technical operational threats; see Section~\ref{sec:threat-model}.
%\name makes this filtering operation refutable.
%After two ISPs sign a contract to collaborate, \name allows each other to audit the abidance to their agreed filtering policy. TESEF offers ``trustworthiness" of filtering operations, which is an enabler of trust relationships and resolutions of disputes.}


% \paragraph{Incentives for source ISPs.}
% \updatedlast{There exists an additional practical benefit to source ISPs in addition to the economic advantages discussed earlier.
% Our personal conversations with multiple ISPs and campus networks provide anecdotal evidence that source networks have real interests in detecting and stopping DDoS traffic originating from their networks for their reputation. 
% However, the risk for source networks to drop their customer traffic without concrete attack indications would be too high in practice.
% \name effectively enables the explicit attack indications that would help source networks find and handle their own attack hosts easily.
% }

%\smallskip
%\paragraph{Source ISPs won't drop their own customers' packets.}
%Providing Internet access to their customers is the primary job of the ISPs, and any source filtering mechanism can be against this very job of ISPs. 
%\name is the only source filtering system that takes into account this filtering accountability problem (see Section~\ref{sec:threat-model}) and addresses it (see Section~\ref{sec:proof-to-customers}). 


\paragraph{What if victim networks cause denial-of-service by blocking arbitrary packets?}
Malicious victim networks cannot exploit \name and launch new DoS attacks because filter rules are first validated with RPKI. % before installed, which can be validated via RPKI.

\paragraph{Can victim networks exploit \name?}
Even when it is {\em not} under attack, an {\em alleged} DDoS-victim network can make use of \name to filter some flows and reduce its operating cost. 
Regardless of the underlying motivation of \name requests, however, we do not see this as a serious threat to the \name system model.
First, a \name filtering network may also save its operating cost due to the reduced upstream bandwidth usage. 
If not, a \name filtering network can always refuse to serve any \name request. 
Second, a victim network would request filtering of flows that otherwise would be filtered by itself anyway. 
Third, if payment channels exist between the two networks~\cite{ramanathan2018senss}, this is not considered as the abuse of the service but a legitimate outsourced filtering.

\paragraph{Incrementally deployable?}
Incremental deployability of new services is a perennial problem in a global Internet. 
IXPs have been recently highlighted as the practical Internet infrastructure where emerging services can be deployed and used incrementally~\cite{gupta2015sdx,gupta2016industrial}.
A \name instance installed at even single IXP can readily help reduce DDoS traffic by the direct victims with strong verifiability property. 

% \name offers immediate benefits to early adopters because \name does not rely on any support from intermediary networks, such as transit ISPs or cloud providers, for its contract establishment and operation. % but involves only the two participating networks.
%Second, a DDoS victim can filter traffic at the near the attack source so that it can immediately save its upstream bandwidth cost.
%Third, a source network can also reduce the otherwise unnecessarily consumed upstream bandwidth by filtering traffic at its network. 
%Furthermore, \name can offer additional incentives to the source networks with explicit payment via a refutable invoice mechanism (see Appendix~\ref{sec:payment-channel-appendix}).
%Moreover, the deployment of \name is affordable compared to installing specialized, standalone network equipment since \name relies only on COTS servers that are already available for small size computing clusters. 
%
% For even faster deployment of the idea, we envision that Internet exchange points (IXPs) can be used to host the \name filters.
%Although less effective than source ISPs (since farther from traffic sources), 
% In IXPs, technical adoption is easier in conjunction with software-defined Internet exchange architectures~\cite{gupta2015sdx} and traffic is already aggregated at the point. 
% Detailed deployment considerations and security analysis improvement for IXPs remain as future work.  


%\smallskip
\paragraph{Can \name handle any DDoS attacks?}
We do {\em not} claim that in-network filtering can handle all types of DDoS attacks.
\name demonstrates that it can effectively handle volumetric attacks.
However, \name may not be as equally effective against non-volumetric attacks (e.g., application-layer attacks), and thus we suggest that \name is used as an additional layer of defense mechanism, which is orthogonal to existing cloud-based defense solutions. 

%\smallskip


%\smallskip
\paragraph{What does a DDoS victim do when misbehavior is detected?}
In \name, we suggest two networks create a filtering contract only between them. 
Therefore, any one of them can abort the temporary contract whenever one party detects misbehavior. 
%For example, if a DDoS victim detects the misbehavior of a source network, it can quickly abort the filtering contract and start deprioritizing traffic from the source network as a penalty to the misbehavior.

% \paragraph{What if DDoS attacks use spoofed addresses?}
% IP spoofed attack traffic is treated just as other attack traffic because our traffic filters are installed in the transit networks not directly at the source networks. 

% \paragraph{Should all intermediate ISPs be auditable?}
% No, {\em only} \name IXPs are required to be auditable; see Section~\ref{sec:filter-bypass-detection}. 


% %\updated{
% \paragraph{\name is harder to use compared to scrubbing services.}
% Blackbox scrubbing (i.e., a victim blindly delegates the entire DDoS defense to scrubbing services) may be convenient to use but is an unfortunate result of the current lack of auditable filtering.
% With \name, the victims can express any filter rules and have verifiable in-network filtering services.
% Victims who are incapable of creating filter rules for \name may delegate the filter rule generation to a trusted third party.

% \paragraph{Can we apply \name to non-IXP networks?}
% Yes. \name can be deployed as a complementary system to any in-network filtering services (e.g, SENSS~\cite{ramanathan2018senss}) in other transit networks (e.g., Tier-1 or large Tier-2 ISPs). 
% We choose to use IXPs as the first deployment points due to their central locations in the Internet topology and their fast adoption of software-based new services. 
% Thus, \name can be complementary to 

%\paragraph{Amplification attacks.}
%(placeholder)






%\smallskip
%\paragraph{Wouldn't the use of \name violate net neutrality?}
%\name is activated {\em only} when a destination network is under serious volumetric attack and thus should be considered as the packet filtering operations for the victim network's survival, not the preferential classification of traffic. 
%Moreover, whenever there is any controversy, the source network that has performed the filtering tasks can provide the evidence that the tasks have been requested by and performed on behalf of a particular destination victim network.  
%
%\smallskip
%\paragraph{What if the DDoS victims or traffic source hosts are multi-homed?}
%Both DDoS victim hosts and traffic source hosts may be multi-homed (i.e., having more than one upstream ISPs).
%Since \name allow contract establishment between two ISPs on behalf of the DDoS victims and traffic source hosts, the ISPs can make multiple contracts with more than one upstream, multi-homing ISPs. 

% \vyas{you may want to say also that while your design is ixp focused there is also a path to deploy this beyond ixps etc? as in hedge a little bit on generality toward the end. and maybe also talk briefly about this in the intro} 

==> paper 2/chapters/economic-incentive.tex <==
\section{\updated{Opportunities and Pitfalls of Economic Incentives}}
\label{sec:economic-incentive}

%\updated{
%As we argue in Section~\ref{sec:intro} and~\ref{sec:case-for-source-filtering}, {\em well-intentioned} source networks would {\em unilateral} incentives (e.g., reduced upstream cost, monitoring its users/tenants) for non-cooperative filtering and incremental incentives (e.g., filtering with accurate attack attribution) to deploy \name as an add-on service. 
%Thus, additional economic incentive is {\em unnecessary} for them and the \name system can remain as {\em unpaid} service.
%}

Source networks may have multiple internal and external incentives for source filtering.
Irrespective of the types of incentives, \name bootstraps trust between ISPs.
Although the study of incentive models is {\em not} the main scope of this paper, we believe it is worth discussing the feasibility of economic incentive models and their potential pitfalls.


%However, additional economic incentive via {\em payment channels} (e.g., the additional operating costs of destination-specific filtering is paid by the destination ISP) may be useful when source ISPs are willing but unable to bear the operating costs of \name.
%The paid \name service model may have a potential to create a new, economically-driven DDoS defense platform at larger scale.
%may also incentivize indifferent source ISPs that do not have enough unilateral incentive for source filtering because the additional costs of filtering can be compensated by the payment from the destination ISPs. 
%That said, one may consider a paid filtering model, where a destination ISP pays a source ISP for performing certain filter rules. 
For economic incentives, one can consider a {\em paid} \name filtering service, where a DDoS victim network is willing to pay a source network for the measured amount of filtering work. 
%This paid filtering service is indeed possible because of the verifiable filtering operation of \name and, particularly, the accountable billing report from the SGX-based filter design.  
%Without the verifiable \name system between distrusting ISPs, a paid DDoS filtering service is only a wishful thinking. 
Yet, the paid service model, although interesting, must be carefully designed to address two potential pitfalls:
\begin{packeditemize}
\item {\bf Moral hazard.} 
Providing economic incentives for filtering work may end up encouraging rational source ISPs {\em not to fix} the problems in their networks (e.g., compromised hosts, misconfigured DNS servers) because the longer the attack duration, the larger payout the source ISPs can collect. 
To mitigate this, we can strictly limit the economic incentive when the source ISP filters the same attack traffic for the extended period of time.
For example, \name can implement a {\em decreasing pricing scheme} for filtering operations within an SGX-protected billing function. 
This way, the payout for the same traffic filtering work tapers off, thus encouraging the source ISP to fix the underlying problems (e.g., patching compromised hosts, reconfiguring DNS servers).
\item {\bf Attack generating ISPs.} 
A determined malicious source ISP may even generate attack traffic by itself to increase the attack traffic volume and maximize its revenue.
The long-term revenue of the malicious source ISP may not be guaranteed if \name has a defense scheme against the moral hazard problem. 
However, the malicious ISP can still cause short-term bill inflation.
To raise the bar for this attack, we can let the two ISPs to agree on the maximum traffic volume to be filtered with payment and enforce this limit in the SGX-protected billing function.
The malicious source ISP then may have to attack several destination ISPs to maximize its revenue and fully utilize its available attack bandwidth, which may increase the risk of its network being blacklisted. 
%\item {\bf Incentivization for deployment.} 
%The deployment of non-cooperative filtering is justified by the unilateral incentive of source ISPs.
%Only the additional filtering for destination-specific filter rules are required to be paid by the destination ISPs.
%Thus, the payment for the incremental cost cannot be used to incentivize the deployment of the source filter system. 
\end{packeditemize}
We envision that a new line of work on more rigorous economic incentive studies for source filtering will follow.
In this paper, our main interest is in the design of the practical auditable filters, which become an enabling technology for economic incentive models. 

==> paper 2/chapters/evaluation.tex <==
% \vspace{-5pt}
\section{Implementation and Evaluation}
% \vspace{-5pt}
\label{sec:eval}

We implement a proof of concept of the \name filter using SGX and various optimizations (\S\ref{subsec:implementation}) and then evaluate its data-plane (\S\ref{sec:data-plane-performance}) and scalability performance (\S\ref{subsec:eval-scalablability}) for large attack volume and complexity.
% ~\footnote{We plan to release the \name system code.}
% , along with the remote attestation performance.\footnote{We plan to release the \name system code.}
% Moreover, we simulate the effectiveness of \name against DDoS attacks with two real attack source data in the Internet AS topology. % and evaluate the effectiveness of \name against the attacks.
%


% \vspace{-5pt}
\subsection{Implementation}
\label{subsec:implementation}
\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/impl.pdf}
% 	\vspace{-10pt}
	\caption{Implementation details of \name.}
% 	\vspace{-10pt}
	\label{fig:impl-overview}
\end{figure}

\paragraph{Overview}. 
We build the \name filter as a Linux userspace application with Intel SGX SDK 2.1 and DPDK 17.05.2 for high-speed packet processing. Figure~\ref{fig:impl-overview} shows the main components of the \name filter and the minimal trusted computing base (TCB) of code and data inside the enclave, which includes the entire control-plane and the key parts of the data-plane logic (e.g., packet logging and filtering). The control plane performs remote attestation and manages the keys for communication with a DDoS victim. The design of the data plane follows DPDK pipeline model, where three threads (i.e., RX thread, Filter thread, and TX thread) run on individual CPU cores and packets are passed between cores via DPDK lockless rings (i.e., RX ring, DROP ring, and TX ring). Every thread runs a small loop polling the hardware or software buffers in the previous stage, processes a batch of the packets, and passes it to the next stage in the pipeline. 

\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/near-zero-copy.pdf}
	\vspace{-5pt}
	\caption{Two packet copy approaches for the auditable filter and packet logs. In the near zero-copy approach, we copy only the memory reference ($\ast$), the five tuple ($5T$), and the size ($s$) of the packet into the enclave.}
	\vspace{-10pt}
	\label{fig:near-zero-copy}
\end{figure}

\paragraph{Optimization: Near zero-copy design.}
% \subsubsection{Data-Plane Optimization for a Single Enclave}
% \label{sec:optimization-for-single-enclave}
% 
For every incoming data-plane packet, a \name filter logs the packet, filters it based on the given filter rule set, and logs it again if it is allowed by the filter, as shown in Figure~\ref{fig:near-zero-copy}.
Figure~\ref{fig:near-zero-copy}(a) shows a naive approach, where a \name filter makes the entire copy of incoming packets into the enclave and operate these functions over the packet copies inside the enclave.
This {\em full-packet copy} approach can be considered as the baseline packet processing mechanism of other existing SGX-based middlebox applications (e.g., Tor nodes~\cite{kim2017enhancing,shinde2017panoply}, TLS middleboxes~\cite{naylor2017and,han2017sgx,goltzsche18endbox}, inter-domain routing~\cite{prixp,kim2015first}, and IDSs~\cite{trach2018shieldbox,shih2016s,goltzsche18endbox}), where secure operations over the full packet bytes are required (e.g., full packet read or encryption). 
However, this approach may incur too much overhead when performing line-rate processing due to the remaining EPC memory for a \name filter is only about 92 MB.
% as we see later in Section~\ref{sec:data-plane-performance} and \textbf{Appendix~\ref{sec:throughput-performance}}.

We thus minimize the dynamic memory usage and avoid the paging by copying only certain header fields into the enclave, which we call {\em near zero-copy} optimization. 
This allows more memory space for filter rules and the lookup table.
% 
% Instead, we take a {\em near zero-copy} approach, where 
In particular, only a fraction of each packet's header fields (i.e., the five tuple fields, $5T$, and the packet size, $s$) are copied into the enclave memory along with the memory reference ($\ast$) of the packet, as shown in Figure~\ref{fig:near-zero-copy}(b).~\footnote{Such reduction of byte copies is allowed for our auditable filter applications but this does not necessarily apply to any other SGX-based middlebox applications.}
The copied data $\langle 5T,s \rangle$ represents the packet and is used for the logging functions and the filter operation. 
The memory reference $\ast$ is used to perform the corresponding operation (e.g., allow or drop) for the packet in the untrusted memory pool.

With the copied five tuple and the size, we first log each packet using a count-min sketch~\cite{cormode2005improved} (with $2$ independent linear hash functions, $64K$ sketch bins, and $64$ bit counters) for memory efficient (e.g., 1 MB) per-source-IP counters. 
The per-source-IP sketch for the incoming packets enables each neighboring ISPs of the filtering network to detect the `drop before filtering' bypass attack discussed in Section~\ref{sec:filter-bypass-detection}.
For forwarded packets, we also record another count-min sketch based on the full 5-tuple bits so that the victim network can detect bypass attempts.
The latency increased by the two sketch operations is negligible because only 4 linear hash function operations are conducted in the data-plane path.
% The 5-tuple based packet logs still enable the victim networks and IXP's direct neighbors to detect bypass attempts when the malicious IXP intentionally deviates from the given filtering rule set. 
%The implementation is adapted from an open-source project~\cite{cmsketchgithub} and 
Each counter has 64 bits and takes only around 1 MB EPC memory per instance of the count-min sketch.

%Our near zero-copy operation reduces the byte size of what we copy into the trusted environment significantly (e.g., reduced to about 1\% for 1.5 KByte packets and 20\% for 64 Byte packets).
%We evaluate the efficiency of the near zero-copy operation of \name in Section~\ref{sec:eval}.

\paragraph{Optimization: Reducing the number of context switches}. 
Another major overhead stems from the context switches when user application calls the enclave functions (ECall) or the enclaved function calls the outside functions (OCall). 
We address this performance degradation by reducing both types of calls in the filter thread: (1) \name only needs one ECall to launch the filter thread and initiates its polling; and (2) the filter thread makes no OCalls as the communication with other threads relies only on the software rings.

\paragraph{Trusted computing base (TCB).} Beyond the DPDK library containing about 64K source lines of code (SLoC), our \name filter contributes to the TCB only 1,206 SLoC which includes the modification of DPDK \texttt{ip\_pipeline} (1044 SLoC) and the packet logging and near zero-copy functions (162 SLoC).

% The \name filter contributes only 1,206 source lines of code (SLoC) to the TCB beyond the DPDK library of 64K SLoC. 
% In 1,206 SLoC code of our implementation, we have a modified DPDK \texttt{ip\_pipeline} (1044 SLoC) and  the packet logging and near zero-copy functions (162 SLoC).

% \paragraph{Optimizations}. The architectural limitations of Intel SGX (e.g., limited memory and context-switch overhead) challenge the line-rate performance; hence, we implement the following optimizations to address these issues:  

% \begin{packedenumerate}
% 	\item \textbf{Avoiding EPC Paging}. The available remaining EPC memory for a \name filter is approximately 92 MB. Although the Linux version of SGX SDK allows more enclave memory with the paging support from the kernel, it induces significant overhead when performing line-rate processing. We thus minimize the dynamic memory usage and avoid the paging by only copying certain header fields into the enclave, which we call {\em near zero-copy} optimization. This allows more memory space for filter rules and the lookup table, eventually achieving near line-rate (e.g., 8 Gb/s or higher) even with 3,000 filter rules.
% 	\item \textbf{Reducing the number of context switches}. Another major overhead stems from the context switches when user application calls the enclave functions (ECall) or the enclaved function calls the outside functions (OCall). We address this performance degradation by reducing both types of calls in the filter thread: (1) \name only needs one ECall to launch the filter thread and initiates its polling; and (2) the filter thread makes no OCalls as the communication with other threads relies only on the software rings.
% \end{packedenumerate}









\subsection{Line-rate Data-plane Performance}
\label{sec:data-plane-performance}
\paragraph{Testbed Setup}. We test our implementation with two machines: one is a packet generator and one deploys \name filter. 
The packet generator has an Intel E5-2630 v3 CPU (2.40 GHz, 8 cores) and 32 GB memory. 
The filtering machine has an Intel i7-6700 CPU (3.40 GHz, 4 cores) and 8 GB memory. 
Both have 10 GbE Intel X540-AT2 network cards and run Ubuntu 16.04.3 LTS with Linux kernel 4.10. 
On the packet generator machine, we use \texttt{pktgen-dpdk} 3.4.2 to generate the traffic saturating the 10 Gb/s link between the two machines.

%\paragraph{Filter versions???}. We have three different versions of filter implementations:
%(1) a native implementation of filter without using SGX, (2) a naive SGX implementation making full packet copy, and (3) a near-zero-copy SGX implementation making only the header fields copy.


% \begin{figure}[t!]
% 	\centering
% 		\begin{subfigure}[b]{0.5\textwidth}
% 	\includegraphics[width=0.90\textwidth]{figures/throughput_bps.pdf}
% 	\vspace{-5pt}
% 	\caption{Throughput in bit-per-second.}
% 	\label{fig:throughput-bps}
% \end{subfigure}\\
% 		\begin{subfigure}[b]{0.5\textwidth}
% 			\includegraphics[width=0.90\textwidth]{figures/throughput_pps.pdf}
% 			\vspace{-5pt}
% 			\caption{Throughput in packet-per-second.}
% 			\label{fig:throughput-pps}
% 		\end{subfigure}
% 		 %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
% 		%(or a blank line to force the subfigure onto a new line)
% 		\vspace{-15pt}
% 	\caption{Throughput performance for varying packet sizes and 3,000 rules with three implementation versions: (1) Native (no SGX), (2) SGX with full packet copy, and (3) SGX with near zero copy.}
% 	\vspace{-15pt}
% 	\label{fig:throughput}
% \end{figure}

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/throughput_bps.pdf}
	\caption{Throughput performance in bit-per-second for varying packet sizes and 3,000 rules with three implementation versions: (1) Native (no SGX), (2) SGX with full packet copy, and (3) SGX with near zero copy.}
	\vspace{-15pt}
	\label{fig:throughput-bps}
\end{figure}


\paragraph{Throughput Performance.}
We benchmark the maximum throughput performance of the filter with the packet size of 64, 128, 256, 512, 1024, and 1500 bytes for three different versions of the \name filter implementations:
(1) native filter without SGX, 
(2) SGX-based filter with full packet copy, and
(3) SGX-based filter with near zero-copy.
% In our experiments, the near zero-copy implementation demonstrates {\bf 8 Gb/s throughput performance even with 64 Byte packets and 3,000 filter rules} and shows no throughput cap in terms of packet per second.
%, the maximum allowed number of filter rules for a single enclave.
% We present the experiment results of \name throughput performance in details in Appendix~\ref{sec:throughput-performance}.

% Note that the SGX with full packet copy represents the baseline implementation model used in various existing SGX-based NFV middlebox studies (e.g., Tor nodes~\cite{kim2017enhancing,shinde2017panoply}, TLS middleboxes~\cite{naylor2017and,han2017sgx,goltzsche18endbox}, inter-domain routing~\cite{prixp,kim2015first}, and IDSs~\cite{trach2018shieldbox,shih2016s,goltzsche18endbox}).
% Yet, we do not present side-by-side performance comparison with those previous work because
% (1) the resource usages (e.g., number of SGX cores used for packet processing) vary in different proposals\footnote{Sometimes, exact core usage data is missing in the publication; e.g.,~\cite{naylor2017and}.} and thus a fair comparison is hard, and
% (2) some proposals do not have full performance evaluation.

Figure~\ref{fig:throughput-bps} shows the throughput performance for varying packet sizes for the three implementations. 
For the packet sizes of 256 Byte or larger, all the three implementations achieve the full line-rate of 10 Gb/s. 
With small packet sizes, however, we observe some degradation due to the use of SGX.
Particularly, when we make full packet copies for each incoming packet, the filter experiences significant throughput degradation. 
The near zero-copy implementation demonstrates {8 Gb/s throughput performance even with 64 Byte packets and 3,000 filter rules}.
% , the maximum allowed number of filter rules for a single enclave, as shown in Figure~\ref{fig:scalability}. 
Additionally, we present the experiment results of \name evaluation in packet per second metric in Appendix~\ref{sec:throughput-performance}.
% Figure~\ref{fig:throughput-pps} shows the throughput evaluation in packet per second metric. 
% Taking a closer look at the SGX with full packet copy implementation, we notice that the maximum packet processing rate is capped at roughly 6 Mpps, which suggests the inherent capacity limit of the full packet-copy operations.
% Unlike the full packet copy version, the near zero-copy version shows no such throughput cap in terms of packet per second. 
%; see more evaluation results on throughput performance in Appendix~\ref{sec:throughput-pps}. 

\paragraph{Latency Performance.} 
We also measured the latency for the near zero-copy version with various packet size starting from 128 bytes. The results are 34 $\mu$s (128 bytes), 38 $\mu$s (256 bytes), 52 $\mu$s (512 bytes), 80 $\mu$s (1024 bytes), 107 $\mu$s (1500 bytes). All the measurements are average latency over 10-second run with 8 Gb/s constant traffic load, which are reported by \texttt{pktgen}'s latency measurement function.

\paragraph{Connection-Preserving Filtering Performance.}
We evaluate the detailed performance of connection-preserving filtering.
We present the result in Appendix~\ref{sec:connection-performance}.


% As we discussed in Section~\ref{sec:filter-design-points}, the two mechanisms for connection preservation (i.e., hash-based filtering, exact-match rule based filtering) have different advantages and disadvantages.
% Thus, we present a {\em hybrid} design for practical operations.
% For any new flow that does not match any existing exact-match filter rules, the filter allows/drops based on the hash digest of the 5-tuple of the packets and queues this 5-tuple.
% At every filter rule update (e.g., every 5 seconds)\footnote{The rule update period can be synchronized with that of the rule re-configuration for scalable, multiple enclave operations; see Section~\ref{sec:optimization-multiple-enclaves}.}, all the newly received flows since the last update are converted into exact-match rules and inserted to the lookup table. 
% This hybrid design amortizes the cost of lookup table update by batch processing multiple newly observed flows at every update period.
% Also, it limits the per-packet latency increase due to hash operations since newly observed flows should be minority in general. 
% Indeed, our experiments on the performance overhead of the use of hash-based filtering  with various packet sizes show no performance degradation, except with small packet size (see Appendix~\ref{sec:connection-performance} for our full evaluation).


% \begin{table}[t]
% 	\centering
% 	\footnotesize
% 	\caption{Overhead of filter rule batch insertion to a multi-bit trie lookup table.}
% 	\label{tab:batch-insertion}
% 	\begin{tabular}{l r r r r}
% 		\toprule
% 		Number of rules in a batch &  1 & 10 & 100 & 1000  \\
% 		\midrule
% 		Insert time (millisecond) & 50  &  52 & 53 & 75  \\
% 		\bottomrule
% 	\end{tabular}
% 	\vspace{-15pt}
% \end{table}


% Table~\ref{tab:batch-insertion} shows the benchmark on the time taken to insert the batched new exact-match rules to a multi-bit tri-based lookup table. 
% Our test shows that the batch insertion of filter rules is quite efficient and incurs minimal performance overhead even for large batch size; e.g., only 75 milliseconds compared to 5-second rule update period. 







\paragraph{Remote attestation performance.}
Our detailed remote attestation performance can be found in Appendix~\ref{app:remote-attestation-performance}.

% \codename performs remote attestation for each new enclave that the \name IXP
% launches on its infrastructure. Since \codename is expected to operate under
% DDoS attacks, we want to ensure that the launching of multiple-enclaves
% on demand does not become the bottleneck for our deployment model. 
% Here, we measure
% the total amount of time to complete an end-to-end remote attestation
% process for one enclave. In our micro-benchmark for remote attestation for the conservative performance tests, we setup the filter enclave
% and the destination on a cloud machine hosted in
% South Asia, and the IAS service
% hosted in Ashburn, Virginia, United States. For an enclave binary of size $1$
% MB, the platform takes $28.8$ milliseconds and the total end-to-end latency of $3.04$ seconds with a standard deviation $9.2$ milliseconds.

\subsection{Scalable Filter Rule Distribution}
\label{subsec:eval-scalablability}

We evaluate the solving performance of the mixed ILP optimization problem described in Section~\ref{sec:optimization-multiple-enclaves} with the CPLEX solver in a server-grade machine with 20 cores. 
We use 3,000 or more filter rules that would cause the throughput degradation of each \name filter. 
In this evaluation, we consider that the total traffic rate going through the entire VIF filter is 100 Gb/s. 
The incoming traffic distribution across the filter rules follows a lognormal distribution. 

With the number of rules more than 3,000 and the number of enclaves more than 10, we find that the CPLEX's mixed ILP solver cannot return the optimal solutions within any reasonable time period. 
To evaluate the effectiveness of our greedy algorithm in Section~\ref{sec:optimization-multiple-enclaves}, that is, how close it is to the optimal solutions, we use a small number of filter rules ($10\le k \le 15$) and confirm that the difference between the optimal cost function calculated by the CPLEX's mixed ILP solver and the results from our greedy algorithm is only 5.2\%.

\begin{table}[t]
	\centering
	\footnotesize
	\caption{Execution times for the ILP solution and the greedy algorithm solution. The CPLEX's mixed ILP solver is configured to stop when found sub-optimal solutions.}
% 	\vspace{-7pt}
	\label{tab:exe-time-for-ILP-greedy}
	\begin{tabular}{r r r}
		\toprule
		Number of rules ($k$) &  CPLEX (sub-optimal) & Greedy  \\
		\midrule
		5,000  &  210.49s & 0.31s  \\
		10,000 &  772.43s & 0.50s  \\
		15,000 & 1,614.96s & 0.73s  \\
		\bottomrule
	\end{tabular}
% 	\vspace{-15pt}
\end{table}

We now compare the execution time of the CPLEX's mixed ILP solver and our greedy algorithm when the number of rules is between 5,000 and 15,000 and show the results in Table~\ref{tab:exe-time-for-ILP-greedy}.
To measure the execution time of the CPLEX's mixed ILP solver for our optimization problem, we configure the solver to stop earlier when it finds a first, sub-optimal solution. 
As shown in Table~\ref{tab:exe-time-for-ILP-greedy}, the CPLEX solver even requires about 200 -- 1,600 seconds to find the sub-optimal solutions, which are unacceptably slow for the dynamic filter rules redistribution operations.
On the other hand, our greedy algorithm runs {three orders of magnitude faster than the CPLEX solver} with the same number of filter rules.
%Note that the optimal solution would take much more time.


\begin{figure}[t!]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/greedy_solving_time_150k_minsuk.pdf}
% 	\vspace{-5pt}
	\caption{Average time taken (in second) to complete the heuristic algorithm for optimizing filter rules across multiple enclaves for varying number of rules $k$.}
% 	\vspace{-10pt}
	\label{fig:greedy-algo-time}
\end{figure}

Figure~\ref{fig:greedy-algo-time} shows the extended experiments on the execution times of the greedy algorithm for varying number of rules at a much larger range. 
We also run this experiment with the total traffic bandwidth of 500 Gb/s, which follows the log-normal distribution. 
In all the range we test (10K--150K filter rules), the greedy algorithm requires no more than 40 seconds.
This enables a near real-time dynamic filter rule re-distribution for large numbers of \name filters. % that run with the SGX support. 


% \subsection{Large-Scale Inter-domain Simulations}
% \label{sec:multiple-session-rpki}

% % \begin{table*}[t!]
% % 	\centering
% % 	\footnotesize
% % % 	\resizebox{\columnwidth}{!}{%
% % 	\begin{tabular}{clllll}
% % 		\toprule
% % 		Rank & Europe &  North America & South America & Asia Pacific & Africa  \\
% % 	    \midrule
% % 		1 & AMS-IX (1660) & Equinix Ashburn (598)  &  IX.br S\~{a}o Paulo (2082) & Equinix Singapore (504) & NAPAfrica Johannesburg (506) \\
% % 		2 & DE-CIX (1494) & Any2 (557)  &  PTT Porto Alegre (258) & Equinix Sydney (393) & NAPAfrica Cape Town (258) \\
% % 		3 & LINX Juniper (755) & SIX (462) &  PTT Rio de Janeiro (246) & Megaport Sydney (383) & JINX (180) \\
% % 		4 & EPIX Katowice (732) & TorIX (426) &  CABASE-BUE (183) & BBIX Tokyo (286) & NAPAfrica Durban (122) \\
% % 		5 & LINX LON1 (697) & Equinix Chicago (384) &  PTT Curitiba (140) & HKIX (281) & IXPN Lagos (69)  \\
% % 		\bottomrule
% % 	\end{tabular}
% % % 	}
% % 	\caption{Top five IXPs in each of the five regions. Numbers inside the parentheses denote the member sizes of the IXPs.}
% % 	\label{tab:top-ixps}
% % \end{table*}

% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[t]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/IXP-coverage-openres.pdf}
%         \vspace{-10pt}
%         \caption{Vulnerable DNS resolvers}
%         \vspace{-5pt}
%         \label{fig:ixp-openres}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.22\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/IXP-coverage-mirai.pdf}
%         \vspace{-10pt}
%         \caption{Mirai botnets}
%         \vspace{-5pt}
%         \label{fig:ixp-mirai}
%     \end{subfigure}
% 	\vspace{-5pt}
%     \caption{The ratio of attack sources that are handled by the \name filters for the two attack source data. $(^*)$: Top-$n$ IXPs denote the $n$ largest IXPs in each of the five regions, see Table~\ref{tab:top-ixps} in {Appendix~\ref{sec:top-ixp}}.}
%     \vspace{-7pt}
%     \label{fig:ixp-coverage}
% \end{figure}

% % Until now, we have considered a {\em single} \name session between a pair of ISPs.
% %Recent major DDoS attacks, however, often involve multi-million bots or amplifiers (or reflectors) that are distributed across large numbers of ASes, which necessitates multiple, concurrent \name sessions with many source ASes. 
% %
% We analyze the effectiveness of \name at IXPs against DDoS attacks with two real attack source data: 3 million vulnerable open DNS resolver IP addresses~\cite{wessels2014open} and 250 thousand Mirai bot IP addresses~\cite{mirai}.

% \paragraph{Simulation setup.}
% In our inter-domain routing simulation, we use the CAIDA Internet measurement data with the inferred AS business relationship~\cite{caida} and the peering membership of world-wide IXPs~\cite{caida-ixp}.
% We randomly choose 1,000 Tier-3 ISPs as the DDoS victims and consider that each victim receives attack traffic from all the attack sources (e.g., open resolvers and bots) in each case.
% To determine a traffic forwarding path between autonomous systems (ASes), we assume that each of them applies the following widely adopted BGP routing policies in order~\cite{gill2013survey,gao2001inferring}:
% % \begin{packeditemize}
% (1) the AS prefers customer links over peer links and peer links over provider links;  (2) the AS prefers the shortest AS-path length route; and
% (3) if multiple best paths exist, the AS uses the AS numbers to break the tie. 
% % \end{packeditemize}

% % Particularly, the first policy guarantees that the created AS-level routes are {\em economically viable} because it ensures that all the ASes on the routes are guaranteed positive revenues.

% % For inter-domain route simulation, we ... BGP ... policy... \msk{@muoi, please copy some text from our S\&P submission}.
% % IXP data... from CAIDA as well~\cite{caida-ixp}.

% We assume that the victim network establishes \name sessions with several largest IXPs (e.g., the biggest IXPs in each of the five regions, as shown in Table~\ref{tab:top-ixps}, see {Appendix~\ref{sec:top-ixp}}). 
% We compute the ratio of flows from the attack IP addresses to the victim network that are handled by at least one of the established \name filters at the selected IXPs.
% A traffic flow is said to be transited at an IXP if it traverses along an AS-path that include two consecutive ASes that are the members of the IXP.

% \paragraph{Results.}
% Figure~\ref{fig:ixp-coverage} shows how many attack flows can be effectively handled by the in-network filters if installed in some large IXPs.
% The box-and-whisker plots show the distribution of the ratio of handled attack IPs when Top 1--5 biggest IXPs in the five regions (thus, 5--25 IXPs globally in total) perform in-network filtering service for DDoS defense. 
% In each plot, the solid lines represent the first and the fourth quartile of the data set and the ends of the whisker indicate the 5th- and 95th-percentiles. 
% Also, the red band inside the box represents the median.

% Even when a single IXP in each region (thus, total five IXPs worldwide) adopts the \name filters, the majority of both attack sources (e.g., vulnerable resolvers, botnet) are handled by the \name IXPs.
% Approximately, 60\% of attack mitigation is expected for the median cases, and 70-80\% mitigation can be achieved for the top quarter cases.
% As more IXPs adopt the \name filters, even more effective mitigation is achieved.
% Particularly, Top-5 IXPs per these regions appear to be sufficient enough to offer more than 75\% attack mitigation for the median cases, and 80-90\% of attack mitigation for the upper quarter cases. 

% Note that our result is not surprising at all.
% It is well-known that some big IXPs already peer with thousands of ISPs and serve multi-Tera b/s traffic volume, which is comparable to large Tier-1 ISPs~\cite{chatzis2013there}.


% From Figure~\ref{fig:ixp-coverage}, we can see that the IXPs have a large coverage of all traffic and promising potential in filtering attack.
% If \name is deployed at all 25 IXPs (i.e., top 5 IXPs in each region), in 75\% of the tested cases, there will be at most 89\% and 85\% of attack traffic from vulnerable OpenDNS resolvers and Mirai bots, respectively, are handled by \name filters.
% Even when there is only the biggest IXP of each region offers \name service, three fourth of the attack traffic can be filtered in 75\% of all scenarios.


% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[width=0.40\textwidth]{figures/botnet_dist.pdf}
% 	\vspace{-7pt}
% 	\caption{Ratio of attack sources of a DNS amplification attack and a Mirai DDoS attack handled by multiple \name sessions. We vary the number ISPs that execute \name sessions with a DDoS victim. The dashed lines denote the cases where only ISPs with RPKI support are used.}
% 	\vspace{-5pt}
% 	\label{fig:botnet-dist}
% \end{figure}

% Figure~\ref{fig:ixp-coverage} shows the effectiveness of \name (in terms of the ratio of handled attack source IPs) for varying numbers of concurrent \name sessions.
% In both amplification and Mirai DDoS attacks, only a small number of \name sessions (e.g., 10-15) seem to be enough to cover the half of these volumetric attack sources; see the solid lines in Figure~\ref{fig:botnet-dist}.
% This is possible due to highly unbalanced attack source distribution in the Internet, which has been observed before~\cite{CBL}.
% Note that the rest of attack sources can be handled by other orthogonal countermeasures (e.g., local filtering, cloud-based scrubbing) in conjunction with \name.


% \paragraph{Effect of RPKI requirements.}
% % 
% We also calculate the effectiveness when we allow \name sessions only with ASes that support RPKI. 
% As we can see the dashed lines in Figure~\ref{fig:botnet-dist}, interestingly, we confirm that \name is still comparably effective when we limit \name only for ASes with RPKI support~\cite{rpki-database}.
% When establishing small numbers (e.g., 5--15) of \name sessions, we notice that the RPKI restriction causes only minor (e.g., 10--30\%) degradation of the effectiveness.
% This result may seem counter-intuitive since  \name sessions are made with only 10\% of ASes.
% Our investigation discovers that the ASes that host large numbers of bots or vulnerable resolvers are usually large regional service providers and tend to use RPKI much more aggressively than average ASes, making \name works well even with its reliance on RPKI. 



%\subsection{Bypass Detection}

%\subsection{Filtering performance}
%
%We further run a filtering snapshot evaluation on the SGX NZC implementation to show that each traffic class is rate-limited and the total traffic rate is also controlled. Figure~\ref{fig:eval-snapshot} gives a 10-second throughput snapshot for 4 traffic classes taken at the rate-limiter. The traffic generator is configured to generate 10 Gbps traffic with packets of 512 bytes and the traffic class allocation is 60\%, 25\%, 10\%, and 5\%. The rate-limiter has a target rate of 4 Gbps and the allocation is set to 40\%, 30\%, 20\%, and 10\%. They start functioning at 0s and 1s respectively.
%
%\begin{figure}[t!]
%	\centering
%	\includegraphics[width=0.5\textwidth]{figures/snapshot.pdf}
%	\caption{Traffic snapshot}
%	\label{fig:eval-snapshot}
%\end{figure}
%
%The snapshot shows the second-scale bandwidth history of 4 traffic classes as well as the entire traffic flow. We can see that starting from 1s when rate-limiter is on, the traffic rapidly drops to the target rate (4 Gbps) and each class also follows. At 3s, the traffic has a bounce as the token bucket algorithm has a reservation for burst traffic, thus temporarily allowing more than 4 Gbps traffic to pass. One second later, all traffic classes remain stable at its desired rate (2 Gbps, 1.5 Gbps, 1 Gbps and 0.5 Gbps).


% \paragraph{Accuracy of HTB latency}

% \subsection{Information visible to adversary}
% We measure the throughput of our system under 10Gbps incoming traffic generated from packet generator. We allocate three cores for running \name's enclave threads, each of which runs one of the three threads, \texttt{rx\_thread}, \texttt{work\_thread}, and \texttt{tx\_thread}. To ease the measurement and avoid the performance drop brought by statistics collecting code, we directly use the receive rate read from the packet generator as the throughput of the tested \name.

% We compare the following three variants of \name: (1) Native RL, the native implementation supporting work-conserving rate-limiting without SGX, (2) SGX RL, the direct SGX porting of the native RL, (3) SGX RL\_TAG, the full implementation of our approach, as stated in Section~\ref{subsec:our-approach}, especially with the one-time HMAC tagging for each passed packet.

% The result is shown in Figure~\ref{fig:rl_throughput}, we set the overall rate limit for \name as 1Gbps, 2Gbps, 4Gbps, 8Gps. The plot shows the throughput number (read from packet generator) of native RL, SGX RL and, SGX RL\_TAG under these 4 different limit of the output.
% It first shows that native RL can indeed handle line-rate traffic and works as expected. Moreover, the two SGX version have its bottleneck at roughly 2.7Gbps and 1.8Gbps.
% \begin{itemize}
% % \item Baseline without SGX and rate limiter (no packet analysis)
% \item Baseline with rate limiter (due to choice of rate limitinf function implementation)
% \item Perf drop just with SGX (no packet analysis)
% \item Perf drop with both SGX and rate limiter
% \end{itemize}

% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[width=0.5\textwidth,height=0.5\textheight,keepaspectratio]{figures/input-output-throughput.png}
% 	\caption{Line-rate packet filtering performance measurement for varying filtering rates with SGX support.}
% 	\label{fig:rl_throughput}
% \end{figure}

% \subsection{Effectiveness of work-conserving}

%\msk{Attestation Performance? Time only?}



==> paper 2/chapters/filter-bypass-detection.tex <==
% \vspace{-5pt}
\subsection{Filter Bypass Detection}
\label{sec:filter-bypass-detection}
% \vspace{-5pt}

The auditability of the \name filter guarantees that the filter operates correctly for the given packets from a filtering network to a victim network.
However, packets may not be properly filtered when a malicious filtering network configures the traffic to {\em bypass} the \name filter, hence violating the filter rules.
Particularly, the manipulation of the traffic flows happen {\em outside} of the protected enclave and thus cannot be detected by the auditable \name filter itself.
We categorize the filter bypass attacks as follows:
\begin{packeditemize}
	\item {\em Injection after filtering:} The \name filter drops a packet $p$ but the adversary injects a copy of $p$ into the packet stream that is forwarded to the victim;
	\item {\em Drop after filtering:} A packet $p$ is allowed by the filter but the adversary drops $p$ before forwarding it to the victim; and 
	\item {\em Drop before filtering:} The filtering network drops a packet $p$ even before it is processed by the filter.
\end{packeditemize}
% 
% 
% As we discussed in Section~\ref{sec:threat-model}, a \name IXP may have incentives to violate the filter rules requested by a destination ISP by dropping more traffic than it is requested (e.g., to further reduce its bandwidth usage) or allowing (by injecting after filtering) more traffic than it is requested (e.g., to provide unfair filtering experience to different neighbor ISPs).  
%
%
  
Note that, we do {\em not} consider {\em injection before filtering} operations by a filtering network as an attack because it does not affect the filtering decision due to the {\em packet-injection independence} property of the filters (see Section~\ref{sec:stateless-filter-design}).\footnote{Moreover, the detection of packet injections before the enclave operations is hard without explicit coordination with traffic sources.}

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/bypass-detection.pdf}
% 	\vspace{-10pt}
	\caption{Bypass detection. Efficient sketch data structure is used for packet logs.}
% 	\vspace{-3pt}
	\label{fig:bypass-detection}
\end{figure}

\paragraph{Bypass Detection.}
%The desired property against the filter bypass attacks is non-bypassability, which guarantees that every packets from $S$ to $D$ are processed by the auditable filter.
%However, non-bypassability is hard to achieve since the untrusted source network has full control over packets outside of the \name enclave.
%
% We rely on two techniques for bypass detection: (1) an accountable packet logging and (2) inter-domain fault localization protocols~\cite{argyraki2010verifiable,basescu2016high} as illustrated in Figure~\ref{fig:bypass-detection}. % illustrates how bypass is detected via a simple fault localization protocol. 
We allow the victim network and the neighboring ASes of the filtering network to detect such bypass attempts by implementing the {\em accountable packet logs} inside the enclave for incoming and outgoing packet streams, see Figure~\ref{fig:bypass-detection}.
For each packet log, we utilize a sketch, particularly a {\em count-min sketch}, a memory-efficient data structure that stores summaries of streaming data~\cite{cormode2005improved}.
With the sketch-based packet logging, the \name filter keeps only the measurement summary inside an enclave and significantly minimize the memory footprint; e.g., less than 1 MB per each sketch. 
With some additional data-plane optimizations (see Section~\ref{subsec:implementation}), the computational overhead of computing two sketches per packet is negligible (see Section~\ref{sec:data-plane-performance}). 

% The \name enclave logs all the incoming packets, filters them with the given filtering rules, and logs the outgoing packets. 
% The two packet logs for the incoming and outgoing packets are used 
To detect bypass attempts by the filtering network, the victim network queries the authenticated outgoing packet logs from the \codename enclave and compares it with its own local sketch. 
Any discrepancy between the two sketches implies {\em injection after filter} and/or {\em drop after filter} attacks by the filtering network. 
The computation and bandwidth overhead for the logs queries is negligible; i.e., sketching is highly efficient and requires sending only a few MB of sketch memory via the already established channel with the victim network.~\footnote{The computational overhead of the victim network should also be low since it only requires an efficient sketch on a commodity server without SGX overhead.}
%We will analyze this in our final version for varying query frequency.
% For example, if the source ISP injects or drops packets after the filter, the two packet logs in the two ISPs differ and this is detected.
When the victim network detects any bypass attempt, it can decide to abort the ongoing filtering request with the filtering network.
In practice, the \name filtering network should allow a short (e.g., a few minutes) time duration for each filtering round so that victim networks can abort any further request quickly when it detects any bypass attempts. 

Similarly, individual neighbor ASes of the filtering network can detect the {\em drop before filtering} attacks by comparing their own local packet logs with the authenticated incoming packet logs of the \name filter.
% Note that fault localization protocols~\cite{argyraki2010verifiable,basescu2016high} often require some level of inter-domain trust for secure localization of packet drops/injections; however, we rely on the accountable packet logging using SGX to make the bypass detection without the need for inter-domain trust. 
% 
% When the victim network detects any bypass attempt, it can decide to abort the ongoing filtering contract with the \name IXP.
% We let the \name IXPs to allow a short (e.g., a few minutes) time duration for each filtering round so that victim networks can abort any further contracts quickly when it detects any bypass attempts. 
% Unlike the first two types of the bypass attacks, which can be detected by $D$, 
% We note that this {\em drop before filtering} bypass attacks is only detected by individual neighbor ASes. % but not by $D$. 
% Therefore, even when bypass attempts are detected, the filtering contract may not be affected. 
% We argue that \name deters the drop-before-filtering attacks because such bypass attacks can be easily detected by the direct members of the \name IXP and 
As a result, the neighboring ASes can choose another downstream network when they obtain the evidence that their downstream network offers filtering services but intentionally drops their packets before they reach the \name filters. 
% The deterrence can be more effective when there exist many options for upstream ISPs due to stimulated competitions in ISP markets~\cite{isp-market-eu}.


\paragraph{Handling malicious intermediate ASes.}
The bypass detection mechanism may cause {\em false positives} when some packets are dropped after leaving the \name filter but before reaching the victim network. 
When this happens, the victim network cannot accurately pinpoint where the packet drop has happened. 
The packet could have been dropped by one of the {\em intermediate} transit networks between the \name filtering network and the victim network, or by the \name filtering network itself. 
This, often-called, fault localization is known to be difficult unless all the networks (including the \name filtering network, the victim network, and intermediate ASes) collaborate~\cite{argyraki2010verifiable,basescu2016high}.
However, such large-scale collaboration is unlikely in today's Internet. % and also does not comply with our trust model---i.e., no established inter-ISPs trust.

Therefore, instead of locating such packet drops, \name allows the victim network to dynamically {\em test} all the intermediate ASes by rerouting its inbound traffic to avoid each of ASes being tested in a short time using the well-known BGP poisoning-based techniques (e.g., \cite{katz2012lifeguard,smith2018routing}).
Due to the space constraint, we describe the detailed test steps in Appendix~\ref{app:dynamic-test-intermediate-ases}.
% Through the tests, the victim network finds and avoids suspicious ISPs that drop the \name-allowed packets. 
% Particularly, we utilize the well-known BGP {\em poisoning-based} inbound rerouting techniques (e.g., LIFEGUARD~\cite{katz2012lifeguard} and Nyx~\cite{smith2018routing}) to reroute (or detour) inbound traffic and avoid traversing any intermediate ISPs for a short period of time (e.g., a few tens of seconds). 
% These BGP poisoning-based rerouting technologies do {\em not} require any inter-ISP coordination and thus the victim network can independently test if any intermediate ASes drop packets (even without the \name IXP's agreement).

% If misbehavior of an intermediate ISP is detected by the victim network, then the misbehaving ISP can be avoided for the extended period of time (at least during the \name session) for auditable filtering.
% Or, if the victim network continuously witnesses that \name-allowed packets are dropped continuously when dynamically changing the inbound routes, it may conclude that the \name IXP itself has been misbehaving. 
% The victim network can then discontinue the \name contract with the \name IXP at its discretion.

% Note that \name IXP may exercise more complicated strategies (e.g., stop dropping packets when active testing is in progress).
% Or, some malicious intermediate ASes that cannot be avoided (e.g., a malicious upstream ISP of a single-homed victim network) may drop packets. 
% In such extremely adverse conditions, e.g., determined malicious \name IXP or unavoidable malicious intermediate ASes, any coordinated filtering efforts in general seem futile. 
% Thus, \name can be aborted by the victim network when such severe packet drop is detected. 
 




% \subsubsection{Filtering Veriability for IXP Members}
% \label{sec:proof-to-customers}

% % As discussed in Section~\ref{sec:threat-model}, the problem of {\em filtering accountability} may arise when a source ISP $S$ has customers (e.g., subscribers or enterprise networks) under different authorities. 
% A \name IXP provides verifiable evidence that convinces its members (i.e., neighbor ISPs) that 
% (1) a DDoS victim network (not the \name IXP) is accountable for related packet drop policies, and
% (2) actual packet drops have been executed accurately by the \name IXP. 
% The evidence for (1) can be simply the filter rules signed by the victim networks (e.g., RPKI).
% For (2), a \name filter can provide the history of packet logs (both the input and output count-min sketches) with accurate timestamps along with its remote attestation validation report (which has been validated with the help of the Intel Attestation Service). 
% The recipient of the evidence for the latter can verify the integrity of the \name filter and the packet logs, and thus it can check if
% (1) its previous packets have been well received by the filter (i.e., detecting any drop-before-filtering attempts) and
% (2) its packets have been dropped because of the victim-submitted filter rules by the trusted filters.
% We envision that interested IXP members may conduct the verification by themselves.
% Or, some reputable organizations (e.g., Internet Engineering Task Force) may provide a third-party verification service for customers. 


%\msk{@muoi?}
%
%
%
%With the per-packet logging functions before and after the rate limiter (see Figure~\ref{fig:near-zero-copy}(a)), the enclave later can proof (1) if it has received a certain packet and (2) if it has allowed/dropped a certain packet. 
%For such filtering accountability, one can imagine an memory efficient data structure, such as Bloom filters~\cite{bloom1970space}.
%In practice, $D$ can periodically download the secure per-packet logging to match its own logging to detect any bypass (e.g., packet injections or drop outside of the enclave) has been conducted. 
%Also, any customer network of $S$ (or even source hosts themselves) can query the enclave to check if their packets have been safely processed without any bypass attempt (e.g., $S$ drops packets before they reach the enclave). 
%
%
%\msk{(2) Inter-domain protocol: with D and with source hosts.}
%
%Figure~\ref{fig:bypass-detection}...
%
%\msk{In such cases, we let the source hosts detect it instead. Source hosts are the ones who can choose their upstream ISPs (except some places where local ISP market is monopolized.) We believe that this will give reasonable incentives to source ISP not to conduct such bypass.}



%\subsubsection{Data-Plane Optimization}
%
%\begin{figure}[t!]
%	\centering
%	\includegraphics[width=0.43\textwidth]{figures/near-zero-copy.pdf}
%	\caption{Two packet copy approaches for SGX-based accountable filter and packet logging functions. In the near zero-copy approach, we copy only the memory reference ($\ast$), the five tuple ($5T$), and the size ($s$) of the packet into the enclave.}
%	\label{fig:near-zero-copy}
%\end{figure}
%
%A naive approach to log incoming and outgoing packets at the \name filter is to make the entire copy of incoming packets into the enclave and operate these functions over the packet copies inside the enclave, as seen in Figure~\ref{fig:near-zero-copy}(a).
%
%This fine-grained packet processing, however, incurs too much overhead (e.g., too frequent context switching) for making full packet copies of all the data-plane packets. 
%Our evaluation (\S\ref{sec:eval}) confirms the poor performance of the per-packet processing approach.
%
%
%
%\paragraph{Per-traffic-class processing is sufficient.}
%Instead of expensive per-packet processing inside the enclave, we design a much coarse-grained, per-traffic-class processing for the enclave operations.
%As shown in Figure~\ref{fig:near-zero-copy}(b), when a packet is received, only a fraction of its header fields (the five tuple fields, $5T$, and the packet size, $s$) are copied into the enclave memory along with the memory reference ($\ast$) of the packet.
%The copied fields $<\!5T,s\!>$ are then represents the packet and used for the logging functions and the rate limiter. 
%The memory reference $\ast$ is used to perform the corresponding operation (e.g., forward or block) for the packet in the untrusted memory pool.
%
%The per-traffic-class accountability still enables $D$ and the $S$'s customer networks to detect bypass attempts when $S$ violates the per-traffic-class volume enforced by the fairly composed filtering policy \PSD. 
%
%
%Note that the per-traffic-class accountability allows $S$ to affect the packet filtering decisions within a traffic class (e.g., dropping $p_1$ instead of $p_2$ when both are in the same traffic class); however, this attack is also feasible when we enforce finer-grained, per-packet accountability and it is fundamentally undetectable by \name and out of scope of the \name system.
%
%The per-traffic-class processing achieves a {\em near zero-copy} packet processing.
%Our near zero-copy operation reduces the byte size of what we copy into the trusted environment significantly (e.g., reduced to about 1\% for 1.5 KByte packets and 20\% for 64 Byte packets).
%We evaluate the efficiency of the near zero-copy operation of \name in Section~\ref{sec:eval}.


==> paper 2/chapters/filter-design.tex <==
\section{Scalable Filter Implementation}
\label{sec:filter-implementation}

\msk{(1) Single-enclave implementation. Two options: full packet copy vs. near-zero copy.}

\msk{(2) Multi-enclave implementation for scalable bandwidth handling}



Line-rate performance on commodity platform is a necessity for \name design. 
Without it, \name can handle large-scale DDoS only with either highly-specialized hardwares or large numbers of commodity servers and thus can be too costly to source ISPs. 
As more network function virtualization applications require high-speed packet processing on commodity platforms, line-rate on commodity ideas have been extensively studied. Most widely accepted solutions (e.g., DPDK\cite{dpdk}, Netmap\cite{rizzo2012netmap}, PF\_RING ZC\cite{pfring}) implement zero-copy networking and achieve minimum context switching by circumventing the use of kernel network stack. Netmap reports that with a single core of 900 MHz it achieves 14.88 Mpps sending or receiving rate on 10 GbE network adapters. Also, the performance report from DPDK shows the capability of zero packet loss forwarding with various packet size.

However, achieving line-rate speed seems quite challenging when we need to satisfy the two desired security properties of the data-plane operation of \name.

\begin{itemize}
    \item \textbf{Integrity of rate-limiting.} Each data packet's filtering decision (i.e., allow/block) must be made within the enclave to ensure the integrity of the filtering decision. 
    
    \item \textbf{Secure packet logging.} Every packet incoming to and leaving from \name should be recorded within the enclave for accountable billing and bypass detection.
\end{itemize}

The two security properties appear to require per-packet operation within the enclave as we can see in a naive data-plane design.

\subsection{Accountable per-packet processing} 

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.5\textwidth]{figures/near-zero-copy.pdf}
	\caption{Two packet copy approaches for SGX-based accountable rate limiting and logging functions. In the near zero-copy approach, we copy only the memory reference ($\ast$), the five tuple ($5T$), and the size ($s$) of the packet into the enclave.}
	\label{fig:near-zero-copy}
\end{figure}

%As briefly discussed in Section~\ref{sec:overview}, a simple implementation of \name would be to enclose all sensitive filtering operations and private information inside the enclave.
The two main secure functions implemented inside the enclave are the multi-class rate limiters and packet logging. 
To guarantee the accountable operation of these functions, a naive approach would be to make the entire copy of incoming packets into the enclave and operate these functions over the packet copies inside the enclave. 
Figure~\ref{fig:near-zero-copy}(a) illustrates this so-called full packet copy approach. 
Any data-plane packet is copied into the enclave memory for full packet logging and rate limiting operations. 
If the packet is determined to be allowed, it is logged again before being copied once again back to the untrusted memory pool for final forwarding through the NIC.
 
\paragraph{Prevention of bypass attacks with per-packet logging.}
This fine-grained packet processing in the enclave is useful for the detection of bypass attacks launched by $S$ to circumvent the \name filtering.
%The intuition behind this full packet copy approach is clear.
%... want to ... accountability of packet filtering decision and logging per incoming packet. 
%With this ... can detect bypass attempts by $S$. 
With the per-packet logging functions before and after the rate limiter (see Figure~\ref{fig:near-zero-copy}(a)), the enclave later can proof (1) if it has received a certain packet and (2) if it has allowed/dropped a certain packet. 
For such filtering accountability, one can imagine an memory efficient data structure, such as Bloom filters~\cite{bloom1970space}.
In practice, $D$ can periodically download the secure per-packet logging to match its own logging to detect any bypass (e.g., packet injections or drop outside of the enclave) has been conducted. 
Also, any customer network of $S$ (or even source hosts themselves) can query the enclave to check if their packets have been safely processed without any bypass attempt (e.g., $S$ drops packets before they reach the enclave). 

\paragraph{Performance challenges.}
Despite its clear security benefits, the per-packet processing inside the enclave incurs too much overhead for making full packet copies of all the data-plane packets, whose data rate can be even a few Gb/s or more. 
This full packet copy operation also would create too frequent context switching that is too expensive for such high-packet processing requirements.
Our evaluation confirms the poor performance of the per-packet processing approach; see Section~\ref{sec:eval}.

 
%
%\paragraph{Overview}. In this naive implementation, 
%
%\paragraph{Rate-limiting}
%
%\paragraph{Packet logging}
%
%\paragraph{Challenges}
% In this naive detector, our goal to make the each packet's {\em arrival} and {\em departure} (after the packet is processed and allowed) at and from \name {\em verifiable} by the source hosts and the destination ISP $D$, respectively.
% One natural idea is to log {\em all} the packets \name receives and all the packets it forwards to $D$.
% For the memory efficient operations, which are necessary for our high throughput networking applications, we use two sets of Bloom filters $b_{in}$ and $b_{out}$ for incoming packets and outgoing packets, respectively.
% These Bloom filter bit arrays are stored within a secure memory region, e.g., en SGX enclave, to prevent malicious \name operators from manipulating the logging and thus verification.
% We provide two functions, {\tt Add}$_{in}(\cdot)$ and {\tt Query}$_{in}(\cdot)$ also within the secure memory region for $b_{in}$ ({\tt Add}$_{out}(\cdot)$ and {\tt Query}$_{out}(\cdot)$ for $b_{out}$).
% {\tt Add}$_{in}(p)$ function updates $b_{in}$ based on the cryptographic hash outputs of the incoming packet $p$ and {\tt Query}$_{in}(p)$ returns a test result whether $p$ is in the Bloom filter $b_{in}$. {\tt Add}$_{out}(p)$ and {\tt Query}$_{out}(p)$ are similarly defined for the outgoing packet $p$. 

% With the full packet logging mechanism, external verifiers can easily check if a certain packet has been handled by \name by requesting the copy of the Bloom filter bit arrays $b_{in}$ and $b_{out}$ and comparing them with the local filter arrays.
% The destination ISP $D$ may maintain its own local Bloom filter for the packets from $S$ and compare it with the Bloom filter array obtained from \name.
% Provided the accurate time synchronization between \name and $D$\footnote{possible... via a secure channel between them...}, any discrepancy between their Bloom filter arrays indicates a potential bypass attack.
% For example, if an array index is set to 1 in the $D$'s local filter but set to 0 in \name's filter, it indicates the existence of one or more injected packets.
% Or, any index that is set to 0 in the $D$'s local filter but not in \name's filter implies that one ore more packets have been dropped against \name's policy. 
% Note that it is the verifier's discretion to determine these indications as the bypass attacks or the artifacts of normal network operations (e.g., natural bit errors or packet drops happened in the transit networks).

\subsection{Sufficiency of {\em per-traffic-class} processing}
%\subsection{Near zero-copy data-plane}
% \paragraph{Performance challenge.}
% Although the naive full packet logging can effectively detect bypass attacks by the malicious source ISP $S$, there still remains a serious performance challenge\,---\,that is, the {\em per-packet logging} operations of the Bloom filter requires \name to copy {\em all} the packets into the secure memory region, e.g., enclave.
% Such {\em full packet copy} operation is indeed the biggest throughput bottleneck since copying each full packet creates significant context switching overheads.

\paragraph{Per-packet guarantee is unnecessary.}
Regarding the necessity of the expensive per-packet processing in the enclave, we make an observation that even with the secure per-packet processing, $S$ still can affect the rate limiting operations of \name by simply re-ordering the incoming data-plane packets.
Our rate limiter implementation handles multiple traffic classes in individual token buckets and each token bucket maintains the time varying amount of tokens to determine if an incoming packet should be dropped or allowed. 
If $S$ re-orders the packets within the same traffic class, it can affect the filtering decisions of re-ordered packets. 
For example, let say two packets $p_1$ and $p_2$ arrive at \name in this order and only $p_1$ uses the available tokens and $p_2$ is dropped. 
If $S$ flipped the order of the two packets, $p_1$ would be dropped instead. 
Such packet re-ordering can be potentially exploited by $S$ to control the rate limiting decisions within the same traffic class. 
Unfortunately, such packet re-ordering that happens {\em outside} of the enclave cannot be detected by the \name system. 

\paragraph{Per-traffic-class processing is sufficient.}
Instead of building expensive but unnecessary per-packet processing inside the enclave, we choose to build a much coarse-grained, per-traffic-class processing for the enclave operations. 
Figure~\ref{fig:near-zero-copy}(b) illustrates how the per-traffic-class processing works with the enclave memory operation. 
When a packet is received, only a fraction of its header fields (the five tuple fields, $5T$, and the packet size, $s$) are copied into the enclave memory along with the memory reference ($\ast$) of the packet.
The copied fields $<\!5T,s\!>$ are then represents the packet and used for the logging functions and the rate limiter. 
The memory reference $\ast$ is used to perform the corresponding operation (e.g., forward or block) for the packet in the untrusted memory pool depending on the rate limiter decision. 

The per-traffic-class accountability still guarantees the incoming and forwarded traffic volume per traffic class, which is sufficient for bandwidth measurement for billing purposes. 
Moreover, this enables $D$ and the $S$'s customer networks to detect bypass attempts when $S$ violates the per-traffic-class volume enforced by the fairly composed filtering policy \PSD. 
For example, if $S$ drops or injects some packets in a traffic class outside of the enclave, $D$ or the $S$'s customer networks can detect it because the per-traffic-class volume should differ. 
Note that the per-traffic-class accountability allows $S$ to affect the packet filtering decisions within a traffic class (e.g., dropping $p_1$ instead of $p_2$ when both are in the same traffic class); however, as we discussed, this attack is also feasible when we enforce finer-grained, per-packet accountability and it is fundamentally undetectable by \name.
%
%Let us first take a look at a subtle adversary's action called packet modification. 
%So fare we have defined bypass attacks as the source AS's illegal packet removals and injections. 
%Thus, a packet {\em modification} (say packet $p$ is modified to $p'$) by $S$ seems to be considered as bypass attacks (since modification can be expressed as removal followed by injection).
%However, we observe that some packet modifications are in fact {\em not} necessarily considered as bypass of the rate limiting operations. % and thus our bypass detection requirements can be relaxed significantly.
%Let us consider a particular packet modification from $p$ to $p'$ with the two conditions: $p$ and $p'$ are in the same traffic class (i.e., $\texttt{class}(p)=\texttt{class}(p')$) and have the same packet length (i.e., $\texttt{len}(p)=\texttt{len}(p')$).
%
%We observe that this particular packet modification does {\em not} necessarily bypass the rate limiting operation of \name because it does not make any changes to the rate limiting operations. 
%Recalling that our rate limiter operates based on the traffic class and  the packet length of incoming packets, the modification attempt does not effectively bypass any rate limiting operation but only damage the integrity of packets, which we do not aim to guarantee (see Section~X. Packet integrity is a non-goal.)
%
%Note that any other packet modifications (e.g., $p$ and $p'$ are in different traffic class or their lengths are different) are indeed considered as bypass attacks since the modification does bypass the rate limiting decision of \name. 

%\paragraph{Relaxed detection requirements.}
\paragraph{Per-traffic-class operations enables {\em near zero copy}.}
%As we exclude the specific type of packet modifications from our definition of bypass attacks, we can relax our detection requirements significantly.
%Particularly, we can have larger granularity of packet logging as we do not need to consider unnecessary details of each incoming packet but only necessary information for rate limiting operations; i.e., five-tuple bits and packet length.
As Figure~\ref{fig:near-zero-copy}(b) illustrates, the per-traffic-class processing in the enclave significantly reduces the amount of bits we copy into the enclave and thus we achieve a {\em near zero-copy} packet processing. % where only a subset of packet headers (e.g., five tuple bits and packet length) are copied into the trusted memory region and used for per-packet logging.
%We use a simple byte counter per traffic class within a trusted execution environment that maintains the authentic copy of the per-class byte counts at \name. 
%The per-class byte counter values are later sent to the destination AS $D$ and compared with $D$'s own local per-class byte counter values. 
%Any discrepancy between the two implies the potential bypass attempt, as we discussed in the naive full packet logging, with the only difference that we have per-class detection granularity as opposed to per-packet granularity, which is unnecessarily too fine grained.
%
Our near zero-copy operation reduces the byte size of what we copy into the trusted environment significantly (e.g., reduced to about 1\% for 1.5 KByte packets and 20\% for 64 Byte packets).
We evaluate the efficiency of the near zero-copy operation of \name in Section~\ref{sec:eval}.

\subsection{Scalability in parallel deployment}
Given the architectural limitation of secure computing resources in currently available SGX hardware, \name's single-enclave deployment is hardly able to deal with the ever-growing attack volume. Therefore, we extend the \name design to allow a parallel deploying scheme with multiple instances while preserving the same level of security guarantee as in the single one. The core idea is to randomly and equally distribute the traffic load among multiple replicated \name instances - each instance runs independently with same supplied policies and same outbound traffic limit. 
With this design, we believe that the \name system is capable of filtering up to 100 Gb/s undesired traffic, which is a reasonable capacity goal for one \name contract to handle as more contracts can work together to rate-limit the multi-hundred-giga traffic in the real world. 

The idea of replicated instances aims to avoid any additional complexity in the design and to make keeping the security promise a more straightforward task - any bias in the system is detectable because each rate-limiter is intended to start with the same filtering policies and run against roughly same-sized traffic with a similar distribution among different traffic classes. With multiple instances behaving like a single instance of \name, the extended system still keeps the integrity of the per-traffic-class filtering decision even though each instance works independently. 

\paragraph{Parallel Deployment} The extended design consists of multiple \name instances and one load-balancer distributing the traffic among the instances in a random and even manner (see Figure~\ref{}). 
Unlike the \name instance, the load-balancer does not need to run on the trusted hardware, making it possible to handle 100 Gb/s traffic with commodity hardware or any other existing specialized hardware in $S$'s network. 
%Another change is that the instances must identify each other by the Ethereum wallet address with the help of $D$ after their remote attestations with $D$ succeed. 
Also, they can further establish secure channels with the help of $S$ to ally themselves with others and detect misbehaviors as an alliance.

\paragraph{Detecting diverged policy}. As each instance accepts policies from $S$ and $D$ via separate channels, the polices one receives may differ from the others if any party intends to create difference among the instances, breaking the overall integrity of the policy composition. However, this inconsistency can be easily detected when all the instances share the hash of the policy they received at the beginning and find any mismatches among the hashes. As a defense, all the instance will cease and inform the other party to stop the contract.

\paragraph{Detecting biased traffic distribution}. Our design requires a high-speed and fair load-balancer entirely controlled by $S$,  making the traffic distribution prone to $S$'s manipulation for malicious purpose. For example, a biased traffic distribution can affect the rate-limiting decisions made in different instances and tamper the rate-limiting result in the view of the entire system. Luckily, this bias can be detected similarly by sharing the per-traffic-class packet logging information and comparing with each other. We will discuss the consequence of this later.

\paragraph{Generating consolidated proof with multiple signatures}. In the single instance scheme, the proof of contracted work is generated by the \name enclave along with the signature and submitted by $S$ to the \name contract on behalf of the enclave. The same approach still works in the parallel deployment with only one amendment: the proof has to be signed by all the others if no load-balancer misbehaviors are detected. Any missing signature will cause failure of the verification process in the smart contract, and $S$ will not get the reward for the submitted work. 
%---------OLD------------
%\subsection{Tradeoff between accountability granularity and packet processing speed}
%
%\deli{Performance comparison: A Mpps vs B Mpps}

% \paragraph{Privacy-preserving traffic class granularity.}
% For the channel between $M$ and $D$, we use the traffic classes of $D$. 

% This creates a subtle problem. $S$ may attempt to bypass its own traffic class while satisfying $D$'s classes. 
% We argue that this is okay as this act harms the adversary himself only.

% For the channel between the traffic sources and $M$, we use the source IPs.



==> paper 2/chapters/ilp-formal.tex <==
% Knowing that a single enclave has bottlenecks in both bandwidth capacity and rule complexity capacity, the multi-enclave design naturally will divide the load at both the bandwidth level and rule complexity level to avoid any performance degradation. This essentialy becomes an optimization problem.

% Assume we have $k$ firewall rules as $R = \{r_1, r_2, r_3, ..., r_k\}$ and the incoming bandwidth for each rule is $B = \{b_1, b_2, b_3, ..., b_k\}$. Given a single enclave bandwidth capacity is fixed at rate $G$ (e.g. 10 Gb/s) and the EPC memory limit is $M$ (e.g. 94 MB), the rule distribution decides how the rules should be allocated to $n$ enclaves where $n = \lceil \frac{1}{G}\sum_{i = 1}^{k}b_i \rceil$, so that the both $G$ and $M$ for every enclave has full utilization. This rule distribution allocates the rules to $n$ non-overlapping subset $R_j$ so that $R_1 \cup R_2 \cup R_3 \cup ... \cup R_n = R$ and $R_1 \cap R_2 \cap R_3 \cap ... \cap R_n = \emptyset $.

\paragraph{Filter rules calculation optimization problem.} 
In each filter rules redistribution, the master node has to allocate the bandwidth and rules to all enclaved filters.
We consider the calculation of the optimal rule sets for each filter enclave as solving a mixed integer linear programming (ILP) optimization problem. 
% We model the optimal rule allocation an ILP formulation in Figure~\ref{fig:ilp-formal}.
We assume $k$ filter rules as $r_i$ ($1 \leq i \leq k$) and the corresponding incoming bandwidth as $b_i$ ($1 \leq i \leq k$).\footnote{We denote $b_i$ as the incoming bandwidth measured for a filter rule for easier understanding. 
In practice, each enclave would produce byte counts without timestamping them because their individual clock sources are untrusted (see Section~\ref{sec:stateless-filter-design}).
The byte counts are then collected in a timely manner and used for the optimization problem.}
A single enclave has the memory limit $M$ (e.g., 92 MB) and the bandwidth capacity $G$ (e.g., 10 Gb/s) as we have discussed in Section~\ref{sec:bottleneck-rule}. Then, we can decide the minimum number of enclaves as needed as $n_{min} = \lceil \max\left({\frac{1}{G}\sum_{i = 1}^{k}b_i ,\frac{ku}{M-v}}\right)\rceil$. To allow some space for optimization, the number of enclaves is taken as $n =\lceil \max\left({\frac{1}{G}\sum_{i = 1}^{k}b_i ,\frac{ku}{M-v}}\right) \times(1 + \lambda)\rceil$ where $\lambda \ge 0$ is an adjustable parameter for additional enclaves. 
% 
%\paragraph{Decision variables}. 
We define real-valued variables $x_{i,j~(1 \leq i \leq k, 1 \leq j \leq n)}$ denoting the portion of bandwidth $b_i$ allocated to the $j$-th enclave, and binary variables $y_{i,j~(1 \leq i \leq k, 1 \leq j \leq n)}$ representing if rule $r_i$ is installed on the $j$-th enclave (i.e., $y_{i,j} = 1$). 
Based on the allocation plan indicated by $x_{i,j}$ and $y_{i,j}$, we consider $C_j = u \times \sum\limits_{i} y_{i,j} + v$ as the memory cost function, which is a linear function of the number of rules installed (where $u$, $v$ are constants).
Also, $I_j = \sum\limits_{i} x_{i,j}y_{i,j}$ is considered as the allocated bandwidth.
% 
% and $I_j$ as the allocated bandwidth based on the allocation plan indicated by $x_{i,j}$ and $y_{i,j}$. 
% Note that the bandwidth allocation is simply the sum as $I_j = \sum\limits_{i} x_{i,j}y_{i,j}$ while the former one is not a trivial function because of the complexity of the trie structure. 
% We consider a simple version of it as $C_j = u \times \sum\limits_{i} y_{i,j} + v$, which is a linear function of the number of rules installed (where $u$, $v$ are constants).
% 
We present the detailed ILP formulation in Appendix~\ref{app:alp-formulation}.

% Our goal is to fully utilize the available resource on $n$ enclaves in terms of the bandwidth and memory, without triggering the performance degradation. Also, the load on each enclave should be balanced, in order to reduce the chance of any enclave getting closer to the limit of $G$ or $M$. Hence, the maximum $C_j$ and maximum $I_j$ should all be as small as possible, as shown in Equation~\ref{eq:c1}. Note that a constant coefficient $\alpha$ is used to balance two maximums in the sum.
% Because of the capacity limit of a single enclaved filter, any filter should have less than $M$ memory consumption (Equation~\ref{eq:c2}) and less than $G$ bandwidth load (Equation~\ref{eq:c3}).
% Since $b_i$ is distributed to multiple filters, so their allocated bandwidth with respect to rule $i$ should sum up to the value of $b_i$ (Equation~\ref{eq:c4}).
% Two decision variables are not independent since when $y_{i,j} = 0$, $x_{i,j}$ should never be a positive value. (Equation~\ref{eq:c5}).

% \begin{figure}[t]
%   \begin{mdframed}
%   	\footnotesize
%       \raggedright
%       $$\textrm{Minimize}\quad z$$
%       \begin{align}
%         s.t.~~~~~~~~~&\forall p,q: z \geq \alpha \big(u \sum_{i = 1}^{k} y_{i,p} + v \big) + \sum_{i = 1}^{k} x_{i,q}y_{i, q} \label{eq:c1}\\
%         &\forall i: u \cdot \sum_{j = 1}^{n} y_{i,j} + v \leq M \label{eq:c2}\\
%         &\forall j: \sum_{i = 1}^{k} x_{i,j} y_{i,j} \leq G \label{eq:c3}\\
%         &\forall i: \sum_{j = 1}^{n} x_{i,j} = b_i \label{eq:c4}\\
%         &\forall x_{i,j}, y_{i,j}: (1 - y_{i,j}) x_{i,j} = 0 \label{eq:c5}\\
%         &\forall x_{i,j} \geq 0 \quad \textrm{and} \quad \forall y_{i,j} \in \{0, 1\} \label{eq:c6}
%       \end{align}
%   \end{mdframed}
% 	\vspace{-5pt}
%   \caption{ILP formulation for the optimal rule distribution. }
%   \vspace{-15pt}
%   \label{fig:ilp-formal}
% \end{figure}

\paragraph{Greedy algorithm to calculate filter rules}. 
Solving the above-mentioned optimization problem is inherently costly when $k \times n$ is large (e.g. $ > 10K$).
Thus, we propose a greedy algorithm (see Appendix~\ref{sec:greedy-algo}) that finds a sub-optional solution within a reasonably short time period.
The high-level intuition of the greedy algorithm is to pre-compute the two parameters---(1) the number of rules per enclave $h$ and (2) the bandwidth quota per enclave $g$---and arrange the rules and bandwidths for the obtained two parameters heuristically.  

% (e.g., less than 40 seconds for 150K rules, see Figure~\ref{fig:greedy-algo-time}) even with large $k \cdot n$. 

% The time for solving this optimization problem is non-negleible, as the number of decision variables grows linearly when either $k$ or $n$ increases. 


==> paper 2/chapters/impl.tex <==
\section{Implementation}
\label{sec:impl}

%In the naive design, the additional copy of each packet unnecessarily increases the workload for packet processing and imposes a high pressure on the limited enclave memory. We have conceptually shown that after rethinking the accountability that \name really requires, only a lightweight copy of certain fields in the header of a packet is sufficient to maintain a secure view of the metadata over the packet's lifetime in the enclave, which avoids the cost both in the time and space from making a full copy. 
In the implementation overview shown in Figure~\ref{fig:impl-overview}, we can see that the enclave allocates a \textit{header memory pool} that caches the header fields necessary for data-plane operations. This makes \name's implementation more cost-efficient and opens more opportunities in the future when handling 10s Gb/s or more traffic.

\subsection{Overview}

\begin{figure*}[!ht]
	\centering
	\includegraphics[width=0.9\textwidth]{figures/impl-sigcomm.pdf}
	\caption{Implementation details of \name.}
	\label{fig:impl-overview}
\end{figure*}

Figure~\ref{fig:impl-overview} shows the main components of \name's implementation. The application runs in the user space that is split into a trusted area and a untrusted area. The trusted area consists of the entire control-plane and a minimal data-plane to ensure the integrity of the policy composition and enforcement. The entire \name and its running environment is built with Intel SGX SDK 1.9\cite{sgxrelease} and DPDK 17.05.2\cite{dpdkrelease}. We also use Intel SGX SSL library\cite{intelsgxssl} to build the remote attestation module within the control-plane as well as the secure channels for communication with other hosts.

We implemented the data-plane functionality based on the \code{qos\_sched} library from DPDK. To support its running within SGX enclave, we further ported DPDK's memory-related libraries (e.g., \code{rte\_mempool}, \code{rte\_ring}, and \code{rte\_malloc}) and other supporting libraries (e.g., \code{rte\_mbuf}) into the enclave. Moreover, we carefully choose the secure boundary in the data-plane so that only a few OCALLs are invoked (when calling the untrusted functions from the enclave) and the amount of data crossing the boundary is minimized. For example, only the packet reference (i.e. pointer) is passed via the OCALLs while the copy of the header fields are done via the direct memory access.

The trusted part of the implementation contains about 7k source lines of code (SLoC) and the compiled signed enclave binary is 1.7 MB in size. The runtime footprint of trusted memory is 68 MB, effectively preventing the enclave from any EPC paging.

\subsection{Control-Plane}

The control-plane serves as a supervisor of \name's trusted part, responsible for interacting with the local operator (i.e. source) and the remote party (i.e. destination) securely. Once the SGX enclave is launched by the operator, it runs remote attestation to ensure the destination that the enclave is established on a trusted CPU. After the trust establishment, An end-to-end secure channel connecting to the destination is created. The secure channel protects the destination's participation in policy composition with the sensitive information (i.e. private policy) securely provisioned. In the end of the policy composition, the composed policy is used to configure the classifier and the token bucket operations in the data-plane.


\paragraph{Remote attestation}. In order to prove to the destination that an untampered \name is running on an SGX-supported CPU, a \textit{quote} is generated by the SGX platform service and delivered to the destination for verification. The destination contacts the Intel Attestation Service (IAS) to verify the signature of the quote using Intel Enhanced Privacy ID (EPID). Once the signature verification is passed, the content in the quote, including the platform state and the enclave information, can be trusted by the destination. 

\paragraph{Secure channel}. As a building block, the remote attestation is suitable for bootstrapping the secure channel establishment, which performs 3-way handshake to setup the TLS session. The first handshake message is piggybacked on the quote sent to the destination, and the rest of handshake and the key exchange is done afterwards.

\subsection{Data-Plane}

The data-plane follows a pipeline model consisting of three threads inside enclave, a \textit{RX thread}, a \textit{rate-limiter thread}, and a \textit{TX thread}.
Three enclave threads run on individual CPU cores and the packets are passed between cores via DPDK lockless rings. 
The entire flow of packet processing in \name is split into three threads, and every thread runs a small loop polling the hardware or software buffer in the previous stage, processes a batch of the packets, and passes it on to next stage in the pipeline. 

\paragraph{RX thread}. The main tasks of RX thread include receiving the packets from the NIC receive queues and making the secure copy of the header fields for each packet in preparation for future usage in the enclave. With the header securely copied, the input logger can effectively update the per-source-IP counter using count-min sketch algorithm and the classifier will also pre-compute classification result (i.e., traffic class) to release the burden of the rate-limiter thread.

\paragraph{rate-limiter thread}. We adapt the DPDK's \code{qos\_sched} framework to satisfy the our requirement on functionality. We further simplifies the hierarchical token bucket of 5 levels to a simple two-level hierarchy. It supports up to 1024 traffic classes (or queues) with the underlying token bucket runtime parameters properly stored in a cache-friendly manner for fastest retrieving and updating. The time source, CPU TSC timestamp, originally used by \code{qos\_sched} for high-resolution rate calculation is not considered safe given the architectural limitation of SGX. Thus, we use the trusted but coarse-grained time source \code{sgx\_get\_trusted\_time} from SGX SDK as an additional time source to monitor and detect any attempt of clock time modification.

\paragraph{TX thread}. There are two software rings the TX thread needs to accept the packet references from, the \code{tx\_ring} for packets to be forwarded and the \code{drop\_ring} for the packets to be dropped. Either of them marks the end of the packet lifetime within the enclave, so the space used for the secure header copy is recycled to the enclave memory. However, the packet is treated differently according to the rate limiter decision. For the packets to be dropped, DPDK runtime frees the memory of the packet (by reference). For other packets to be forwarded, the output logger updates the per-traffic-class counter and passes the packets to DPDK runtime for transmitting via the NIC.

\subsection{Optimizations}

In the current implementation, we deploy several optimizations to further increase the throughput performance towards the line-rate packet processing. These optimizations reduce the overhead brought by the architectural limitation from SGX, such as the EPC size restriction, the MME operation overhead and the context switch overhead between secure/insecure worlds.

\paragraph{Avoiding EPC paging.}
Depending on the BIOS setting, the isolated secure memory (i.e., EPC) has a fixed size of 64 MB or 128 MB. Except the memory used by SGX SDK, the maximum available EPC for \name instances is approximately 92 MB~\cite{brenner2016securekeeper}. On Linux platform, the SGX can provide larger EPC with the help of paging support from kernel. We carefully control the heap memory usage to reduce the chance of paging and eventually achieve less than 68 MB enclave memory usage.

\paragraph{Reducing the number of context switches.}
The overhead of context switches comes from the saving and restoring of the execution environment (i.e., registers) between trusted and untrusted modes, which slows down the code paths for per-packet processing. In the RX and TX threads, we use batch processing to amortize the cost of one context switch among a number of packets, effectively reducing the overhead imposed by per-packet processing. In the rate-limiter thread where OCALLs are made for CPU timestamps, we also reduce the frequency of invocation  of the time stamps with a reasonable sacrifice of the accuracy of token bucket operations.

\paragraph{Increasing the cache locality.}
The rate-limiter thread runs the highly optimized code that carefully aligns the memory access to the cache line size and pre-fetches the data structures to hide the cache miss penalty. We defer the OCALL of any packet memory operation (mostly free operation for the dropped packets) to the TX thread to avoid disturbing the cache owned by the CPU that runs the rate-limiter thread. This also offers another benefits as the TX thread also focuses on the packet memory operation and has a better cache locality over the packet memory pool.

% \subsection{SGX Primer}
% \label{subsec:sgx-primer}

% Intel SGX is an ISA extension aiming to offer trusted execution environment without relying on dedicated hardwares except the CPU pakcage itself. It transparently create an {\em isolated} memory region, called \textit{enclave}, consisiting of Enclave Page Cache (EPC) and protected by Memory Encryption Engine (MEE), in which the confidentiality and the integrity of the code and the data are guaranteed. It supports enclave execution at user-level privilege and prohibits any other user-mode program or privilege mode (e.g., operating system or OS) from accessing its EPC. SGX also prevents hardware access attempts such as memory bus snooping and monitoring. Moreover, serving as a root trust from CPU package, it allows secure measurements of all the loaded EPC memory, ensuring an unmodified booting stage with verified code and data, which is usually called \textit{attestation}.

% In SGX application design, the application code is divided and placed into the enclave memory region or untrusted memory region, depending on the security requirements of different functions. The interactions between trusted code and untrusted code are recongized as \textit{ECALL} and \textit{OCALL}, where ECALL denotes the untrusted codes calling the trusted ones, and vice versa for OCALL. Both of them require a context switch at CPU level, involving saving and restoring of internal states, and sometimes checking of the passed parameters.

% In our \name implementation, SGX 
% (1) protects sensitive system parameters, such as input filtering policies, the composite policy, or rate-limiting configurations, from direct, unauthorized access and modification by a malicious OS; and
% (2) prevents the operation of \name from being modified by a malicious OS and allows remote third parties to attest the verified version of \name codes. 
%:
%(1) The policy from source, destination or the composed one cannot be read by any unauthroized entities via either software acessses or hardware tappings; (2) The same set of policy and the code of middlebox function cannot be modified by any others in terms of subverting the rate-limiting decisions or creating advantages in leaking any targeted information. (3) The users can be assured that the enclave executes a verified version of code since its lifetime and any modification to the binary before running will not deceive the users into interacting with a untrusted version, and thus leaking information.

%In spite of the advantages a SGX-enabled middlebox can enjoy, there are also a few unpleasant things it faces. The availability of the middlebox can be largely affected by any Denial-of-Service attacks as the underlying OS is not controlled by the middlebox. However, in our service model, the platform contracts closely with the victim flooded by traffic and the victim expects to see the policed traffic transmitted within a secure tunnel, thus rendering any DoS attacks visible directly to the victim.

%\subsection{Baseline design using SGX}
%We first present a baseline \name design with SGX as a simple but realistic design point for general middlebox design using SGX.
%First, all of its control-plane functions (e.g., policy composition $\phi$) are implemented completely within the SGX enclave to protect their sensitive data and code.
%Second, the core, sensitive data-plane operations, such as the classification function, the parallel rate limiters, and the packet encryption function, are also implemented in the enclave for secure operations.
%Third, all user data packets are copied into the enclave because they need to be securely processed (e.g., classified, rate-limited, dropped/forwarded) within the enclave.

%to highlight the challenges 
%Consider a simple implementation of rate-limiting for different classes of traffic, two strategies are immediately realized: (1) In order to hide the fact about dropping individual packets, the survived packets are retrived into TEE and encryption is done in the trusted memory; (2) The multi-class rate-limiting are supported by naturaly running indepedent rate-limiting algorithm (i.e., token bucket algorithm) for each class. Note that the first strategy has been used in Slick\cite{?}, where only the packets that are necessary for further sensitive processing are copied into SGX enclave, which also serves as a performance optimization for avoiding uncessary costly operations (such as packet copying).

%\subsection{Security/Performance Dilemma}
%Our \name implementation has desired security and performance properties.
%In particular, the rate limiting operations should not be tampered with and accessed by a malicious operator of the middlebox.
%This security property is achieved through the careful data flow design with the SGX features; e.g., any sensitive operation is executed within the SGX enclave. 
%Also, line-rate (e.g., 10 Gbps) packet processing is desired since our middlebox is most useful when it can handle and rate limit overwhelming incoming traffic volume. 
%
%In our baseline design, however, we immediately face a {\em security/performance dilemma}. That is, it seems nearly impossible to achieve the strong security for the data-plane operations of \name while processing packets at line rate (e.g., 10 Gbps). 
%The main challenge arises from the two very different (thus conflicting) packet processing requirements for the SGX support (for security) and the DPDK support (for performance). 
%On one hand, for secure packet processing operations (e.g., rate limiting functions, packet encryption), all the incoming data packets {\em must be copied} into the enclave. 
%Note that we cannot selectively copy only a subset of data packets (e.g., only the packets that will be ultimately forwarded to $D$) into the enclave since such memory access behaviors will leak the rate-limiting patterns to the malicious operator. 
%On the other hand, high-performance packet processing in commodity hardware, such as DPDK~\cite{DPDK} or netmap~\cite{netmap}, requires the \textit{zero-copy} memory optimization.
%That is, our middlebox should {\em not make copies} of incoming data packets for line-rate processing.
%Unfortunately, it appears to be challenging satisfy the two conflicting packet copy policies.

% \subsection{Near Zero-Copy Implementation with SGX}
% \label{subsec:our-approach}

% \begin{itemize}
% 	\item Per-class byte counter --- for outgoing packets
% 	\item Count-min sketch --- for incoming packets
% \end{itemize}

%Our approach to implement a secure, line-rate \name middlebox is simple. We decide to support {\em only} authenticity to our data-plane operations but {no} confidentiality, which makes us to maintain our data-plane operations {\em nearly zero copy}, thus achieving line-rate performance. 
%This seemingly a significant sacrifice on the security of the data-plane operations, however, is in fact OKAY. 
%The main reasons are as follows:
%First, offering data-plane confidentiality is not sufficient to address the data-plane side-channel attacks. There are other ways (e.g., probe packets) to infer data-plane operations. It seems it is impossible to remove the side channel anyway. 
%Second, lack of data-plane confidentiality does not reveal the data-plane operations immediately but still requires non-trivial attack cost. For example, comparing incoming/outgoing packets to/from the middlebox requires high performance deep packet inspection, which is not significantly cheaper than other inevitable (or unstoppable) attacks (e.g., probe packets and return packet analysis).
%Third, an authentication mechanism, particularly MAC tagging over packet headers, is sufficient to make the middlebox's data-plane operations {\em non-bypassable} for any packet from $S$ to $D$. 

%\subsection{Non-bypassable data-plane operations}
%
%Non-bypassability requires preventions for three violations (1) packet injection (via replaying tags), (2) packet deletion (via dropping tagged packet), and (3) packet pre-filtering,
%
%\textbf{Header-only MAC}. To support near zero-copy processing, for every packet, the middlebox only reads and copies the packet header, inspecting the most representive metadata, which describe the {\em uniqueness} and {\em shape} of a packet. Hence, with a MAC tag calculated over the header, packet's shape (i.e., length) is bound to a unqiue packet header, eventually ensuring the overall traffic volume, regardless of the content being delivered. This MAC tag also servers as a secure token, any packet injection without MAC can be detected immediately at the receiver side.
%
%\textbf{One-time HMAC}. It is possible that the adversary reuse a generated MAC tag and inject arbritary-content packet with same length into the link. This may work because the 'shape' is same and the packet uniqueness is not good enough (Since we admit that benigh packets may have exact same header). Luckily, this can be prevented by using one-time HMAC. Internally, the middlebox maintains a counter $C$ to record the number of passed packets. Every MAC tag now is calculated by $HMAC(k, c)$, where $k$ is the secret key, $c$ is the current counter value and , $HMAC(\cdot)$ is keyed-hash-based MAC. This largely improves the uniqueness of every passed packet, thus making the MAC tag replay-resistant against packet injection attacks. Additionally, the internal counter can be used to detect packet deletion since the counter value can be synced to the victim out of band periodically. 
%
%\textbf{Packet logging and witness querying}. To prevent packet pre-filtering, the traffic removal done by the malicious source beforehand, the middlebox uses bloom filter to record each incoming packet header and answer the query of witnessing a packet header with a tolerable false postive rate (can be kept as low as possible). Two parallel running bloom filters are used (See Fig.~\ref{fig:packet-log}, each of which will be on (accept insertion) for a period of $T$ and off (stop and reset) for a period of $S$ repeatedly. The difference is one bloom filter's schedule is always behind the other one by $D$, where $D = (S + T) / 2$. At any time, the arrived packet header will be logged either in the only active bloom filter, or the one has longer remaining lifetime. This guarantees that each evidence is kept in one of the bloom filter and will be queryable for at least a period of $D$. This machansim is the realization that the evidence should not be kept forever due to enclave memory limit, however a reasonable query window for each packet is necessary.

%\begin{figure}[!bt]
%\centering
%\includegraphics[width=0.7\columnwidth]{figures/bloomfilter}
%\caption{Packet logging with two overlapped bloom filters}
%\label{fig:packet-log}
%\end{figure}


% HMAC(K, C)

% --------------------------------
% | IP Header | TCP Header | MAC |
% --------------------------------
%
%
% - non-bypassability requires (1) prevention for packet injection (via replaying tags), (2) packet removal, (3) packet pre-filtering. 


%Second, SGX-based applications often involve frequent switching between the trusted and untrusted components, which indeed incurs significant amount of context switches. 
%Our threat model poses challenges on the design of a secure middlebox, even when TEE technology like Intel SGX is adopted. We will discuss these challenges separately, with further realization of the adversary's capabilities and the strengths and limitations in either a generic TEE or a specific one, Intel SGX.

%\subsubsection{Data-plane side-channel information}
%Although a malicious OS that hosts $M(S,D)$ cannot directly access the composite policy $P_{S,D}$, it can observe and even manipulate its data-plane operations: the OS can read, write, and inject any incoming packets to $M(S,D)$ because the input data packets (unlike cryptographically authenticated policy inputs $P_S$ and $P_D$) are unauthenticated, any Internet traffic from source hosts behind the ISP $S$; the OS cannot even read the outgoing packets from $M(S,D)$ due to per-packet encryption performed by $M(S,D)$ but it can still read the aggregate volume of the outgoing traffic.
%
%The baseline design has two realistic side-channel attacks. 
%First, the adversary can monitor the memory access pattern, thus revealing which packets are copied into the enclave for trusted operations, which eventually reveal the set of packet being allowed or dropped. 
%Second, the adversary can monitor the behavior of a rate limiter for a particular traffic class and infer the rate-limiting parameters (e.g., the average rate and burst size of a token bucket)~\cite{sigcomm-16-paper?} and use it to infer the composite policy $P_{S,D}$ indirectly. For the inference, the adversary can carefully craft the input to effectively test a single rate limiter and observe the output volume (even encrypted).

%\subsubsection{Line rate support with secure packet processing} 
%Line-rate (e.g., 10 Gbps) packet processing is necessary since our middlebox is most useful when there exist overwhelming incoming traffic volume. 
%High-performance packet processing in commodity hardware has been widely discussed and developed recently~\cite{DPDK,netmap}.
%In general, line-rate packet processing relies on the two optimization techniques: \textit{zero context switch} (i.e., eliminating unnecessary switches between user and kernel modes) and \textit{zero copy} (i.e., eliminating file copies from the kernel to user space). 
%Unfortunately, it appears to be challenging to achieve the two optimizations when the majority of packet processing must be securely conducted with the SGX support.
%First, for some secure packet processing operations (e.g., packet encryption), a non-negligible percentage of data packets must be copied into the enclave, which violates the zero-copy principle and results in significant data-rate loss.
%Second, SGX-based applications often involve frequent switching between the trusted and untrusted components, which indeed incurs significant amount of context switches. 
%By design, it is not straightforward to minimize the context switching overhead since there is no easy way to split the application as the trusted part versus the untrusted part.

%From Section~\ref{} to Section~\ref{}, we highlight the \name middlebox's main security and performance features. 

% \subsection{Secure packet filtering architecture}

% The baseline design is subject to source's memory inspection on which packets are copied. To simply overcome this, we will simply copy all the packets, regardless of dropping or passing decision made by the rate-limiter, and only encrypt the non-filtered packets inside the enclave. The to-be-dropped packets, although having an excess copy, will neither be encrypted nor occupy the limited memory space inside enclave. The space used for accomplishing the covering copy will be immediately reclaimed and reused as a free space. Ideally, the space wasted on the extra copies is temporary and will only incur one waste of the packet size if only one extra copy is maded at the same time.

% (a figure of overview goes here)
% \subsection{Work-conserving rate-limiters}

% In the baseline design the traffic rate set for a individual rate-limiter can be easily inferred by a malicous source testing the target rate-limiter and observing the volume of encrypted output. By repeating this step, the source learned the parameters for every class's rate-limiter. To overcome this drawback, we enable work-conserving rate-limiting which saturates the output link and keep the overall output volume at a const number.

% This work-conserving mechanism is implemented by allowing token borrowing among different token bucket. The principle is that once any rate-limiter is not consuming any tokens (giving pass decision to the packets), the unused tokens are immediately borrowed by any other working rate-limiters. To ensure fairness, we redistribute these unused tokens with a global view on the working set of rate-limiters. For example, for a system with $n$-class rate-limiters having token refill rates as $r_1$, $r_2$, ... ,$r_n$ respectively, if any time a rate-limiter $u$ is not consuming its $r_u$ tokens per a unit time (say it consume at $r'_u$), these $r_u - r'_u$ tokens are prorated over other running rate-limiters. So a certain working rate-limiter $w$ will obtain $\frac{r_w}{L - r_u} (r_u - r'_u)$ bonus tokens per unit time, where $L$ is the total traffic limit predefined and is the sum of all $r_i$.

% The above work-conserving mechanism applies on any number of underused rate-limiters, which gives us a gurantee that the output volume is constant whenever \name is enabled. Note that \name's activatin condition is when the input traffic exceeds the predefined rate $L$.

% \subsection{Context-switch reducing with SGX}

% To fully respect the lesson learned from zero context switch, we reduce the number of OCALL and ECALL at two dimension in the data-plane: First, the number of designed interfaces for OCALL and ECALL are reduced; Second, the number of invocations on OCALL and ECALL are minimized;

% In data-plane, the only heavily invoked OCALLs are two functions that interacts with the DPDK Poll Mode Driver for network cards, one OCALL asks the driver to receive a batch of packets from physical port, store them in untrusted memory pool, and hand over a list of references (pointers) to enclave, and the other OCALL does similar processes but in a reverse order to inform the driver to transmit the non-filtered packets (in encryption form).

% We fully utilize the benefits of enclave code directly accessing the untrusted memory. Unlike OCALL and ECALL, these accesses are by design allowed by SGX and have no overhead of context switch because the entire virtual memory space (untrusted memory region and enclave memory region) of the process is transparently acessible to enclave code (note that it is not true for untrusted code). In this way, the enclave code and the untrusted code are communicate and synchronize with each other via memory sharing, cutting the potential overhead if OCALL and ECALL are used for communcation.

% \subsection{Scaling \name for 100s Gbps rate}

% \begin{itemize}
% 	\item How to make an array of \name instances to support 100s Gbps rate?
% 	\item How to check biased load balancer efficiently?
% \end{itemize}

% \subsection{Scaling-out for line rate support}

% With the restriction on SGX resources (at most 4 physical cores for Intel SGX CPU, at most roughtly 94MB EPC shared by all enclaves on one machine), achieving line-rate packet filtering on one single machine seems unrealistic, given that the baseline design already requires a lot of copy (memory-consuming) and encryption (both memory-consuming and CPU-consuming). Hence, we propose a scale-out solution that leverages multiple SGX machines and load-balances the incoming line-rate traffic so that the SGX middlebox cluster can still meet the processing requirement and preserve the privacy guarantees achieved on a single SGX middlebox.

% Assume the data-plane on a single machine can only support the processing of input traffic rate at $X$. this suggests that we should duplicate the same configuration of middlebox by $\lceil \frac{I}{X} \rceil$, if the real input traffic rate is $I$. This simple replication relies on the infrastructure's cooperation on offering a fair load-balancer, which may be unsafe to assume since the adversary tends to manipulate the balancing mechanism to gain advantages when conducting traffic manipulation attacks.

% TODO(Deli: not finished yet)

% Therefore, a SGX middlebox should be deployed to load-balance the traffic fairly and randomly, in order to support this scaling scheme. The load-balancer (LB) middlebox will 

% \subsection{Effective and secure accountable enclave}

% From a network persepective, our proposed solution is simply dropping the excess traffic, which will have side affect of interrupting the normal users's communication. This can be exploited by a source adversary since she will be able to filter the packets in advance and shift the blame of packet loss to the middlebox. To overcome this, we implement an effective packet logging mechanism and query service to the system. The former one saves the fact of witness of individual packets in the inbound traffic, while the latter one offers an interface to the users, answering the request about the witness of certain packet. 

% Running a full-fledged packet logging database is impossible as per the discussion of restrictions of SGX. In instead, we will use bloom filter for such packet occurrence test, which is both time-efficient and space-efficient. The false positives brought by this is acceptable because (1) false positive rate can be controlled by many known solutions \cite{X} (2) false positives are not exploitable by the adversary who wants to pre-filter a specific class of traffic.

% To be specific, a bloom filter will insert every packet (whole content) once it arrives and after a period of time the bloom filter is discarded and refreshed as the evidence of witnessing the individual packet doesn't need to be kept for a long time. But if we naively peridically refresh one bloom filter, the lifetime of the evidence vary from zero to the refresh cycle. To have a lower bound of the evidence lifetime for every packets, we can have two carefully overlapped bloom filter, each of them will be alive and accept insertions for a period of $T$ and will then be offline and cleared for a period of $S$. The start time of alive period for two bloom filters has a gap time of $D = (T + S) / 2$. This ensures any evidence is queryable during a lifetime between $D$ and $T$.

%             T                S                 T
% |----------------------|          |----------------------|
% <-----  D  ----->               
%                  |----------------------|          |----------------------|
%                              T                 S                T


% T - D + T + S = D + T

% 2D = T + S
% D = (T + S) / 2

% \subsection{Non-bypassable tagging}

% The encryption for every passed packets (the ones not dropped by rate-limiter) apparently violates the zero-copy principle, and in fact it brings two additional full-packet copy operations for each passed one, of which one is copying plaintext packet from untrusted memory into the enclave and the other one is copying the encrypted packet from the enclave to the untrusted memory. These copies are unavoidable because the encryption has to be done inside the enclave in order to protect the encryption key and the information we want to hide.

% Behind the huge overhead brought by the encryption, the protection we mostly want is hiding the dropping decision made for each individual packet. If we choose to compromise on this and this information is no longer protected, the encryption would immediately become an overkill for providing the other secure properties we originally wanted, which are:

% \begin{itemize}
%     \item P1. bounded overall traffic rate
%     \item P2. bounded traffic rate for each traffic class, if per-class rate-limiter are all saturated.
%     \item P3. Fairness of the work-conserving mechansim        
% \end{itemize}

% It is worth noting that all these properties are more closely relatd to integrity of the decision made by middlebox, which is about the policy enforcement of the traffic class (packet classification) and traffic rate (packet length). A closer look on the rate-limiting function reveals that the decision making process only needs to read the packet header for the purpose of classifying the packet and calculating the tokens consumed.

% We also notice that there is no strong need for confidentiality, if we choose to compromise the protection on dropping decisions. Another supportive observation is that the packet content, which is usually considered confidential, is anyway accessible by the adversary in our threat model. In fact, the adversary is even free to manipulate any bit of the packet sent to the middlebox.

% So far, the initial realization is that, in this fierce environment where a strong adversary controls the input traffic, the most realistic claim we can make is ..

% Based on the understanding that the dropping information can be revealed, we will show a more cost-effecient way to only protect the integrity of the essential parts. This lightweight \textit{secure sketching} technique essentially find a way to let the victim detect any violation of the aforementioned integrity properties. At high-level, the middlebox periodically makes sketchs of the headers of the output packets and sync them with the victim in a out-of-band secure channel so that the victim can be aware of the following violations:

% Now, we will show that, a secure sketching mechanism can make the same claim in a more cost-efficient way, if we no longer protect the true/false information of packet dropping.

% To get rid of the huge overhead brought by IPsec encryption, which actually is an overkill for hiding the information of dropping decision on individual packets, we first admit that the source adversary is so powerful even with the output encryption enabled, and then we consider dropping this heavy defense and think about other lightweight mechansim. A immediate first thought is, this lightweight mechansim still needs to provide certain security property, although it is not comparable to a full encryption.

% As a traffic removal application, one utility goal from the victim's view is to lower the traffic rate coming from the source ISP to a bound (say $L$). Another goal is since the rate-limiter has already shaped the traffic according to the composed policy, the traffic shape should not be influenced by the attacker in any way after the processing.

% Note that the rate-limiter only checks the packet header to classify and make the passing/dropping decision. This checks involves two things: (1) class definition, and (2) packet size, where the class definition decides which class-level rate-limiter should be queried for this ongoing packet, and the packet size affects the number of tokens to be consumed if the packets is allowed. Both of them influence the final shape of the traffic in terms of the volume distribution among different class, which is specified in the composed policy and should be enforced.

% Our secure tag is used as a certificated pass for the packet under the specific class and with specific size. This pass should not be either discarded by the attacker to decrease the volume, or abused by the attacker to increase the volume. This secure tag ensures the integrity of the shape for individual packets, eventually guaranteeing the integrity of the shape for the overall traffic.

% (1) what is tagging idea, (2) what security property it provides (e.g., only integrity on partial bits of packets), (3) why this limited integrity property and lack of confidentiality is okay for our application.

% First, the secure sketching can be used to detect insertion and deletion of tags.

% Second, we have to show that 

==> paper 2/chapters/inflation.tex <==
\section{Open Inter-ISP Filtering Market: Economic Incentive}
\label{sec:econ-incentive}
%\section{Handling Billing Inflation}

We argue that in addition to the non-economic incentive, it is necessary to provide economic incentives to source ISPs with direct fungible payment from $D$ to $S$. 
First, without a payment mechanism, the source-end filtering service by $S$ can be exploited. For example, even when it is not under attack $D$ may attempt to save its operating cost by asking the packet filtering operations to $S$. Since $S$ in general cannot verify the necessity of packet filtering (e.g., existence of attacks), such exploitation is hard to detect. Thus, direct payment scheme can be an effective deterrence mechanism for such exploitation.
Second, if $S$ receives multiple \name requests from multiple destination ISPs, it needs to carefully determine how to use its limited filtering capability. The payment scheme with negotiable pricing can make \name further increase the economic incentive for $S$ (since $S$ can ask for higher pricing) while more efficiently using its limited resource (since more desperate destinations will use the filtering service).

To remove any additional trusted third party and flexible payment schemes, we propose to use Ethereum smart contracts. This generates the permanent, immutable records of \name services on the Ethereum blockchain. 
Such high level of transparency of \name services in the public domain naturally generates an open inter-ISP filtering market since all the pricing and the results are publicly available. As a result, the reasonable market prices may naturally emerge. Also, misbehaviors can be deterred as misbehaving ISPs are easily recognized in the immutable records. 

\subsection{Flexible payment scheme from $D$ to $S$}

- Protocol figure. 

\paragraph{Proof of contracted work.}

- SGX based proof of contracted work

\paragraph{\name contract.}

- Details… 

\paragraph{Verification and payout.}

\subsection{Transparency and inflation deterrence}

- Impose limits to handle inflation attacks. 

- Transparency: untampered, permanent record of contracts and their 
results. Can create reputation. Can deter inflation attacks. 

\subsection{Economic Analysis}

- Incentive for good behavior. Disincentive for misbehavior. 

- How???? Refer to IKP paper's analysis?

\subsection{Privacy (move to Discussion)?}

Tradeoff? 


------- OLD --------

\msk{\name provides accountable billing, which guarantees correct bandwidth measurement. This establishes a strong economic incentive to source ASes. }

\msk{However, a source AS is able to inflate the bill by creating dummy packets to the \name system. }

\msk{We need to answer to ``how can we handle the bandwidth inflation attacks?''}

- we up front admit that this is an open problem. It is equivalent to S launching DDoS attacks to increae the billing. As long as the cost of generating traffic is lower than the economic reward expected for the increase traffic, there is incentive to launch this attack. 

- In the worst case, our economic incentive end up encouraging ISPs to increase attack volume (either via poor network security checks or even generating new attack traffic) and get paid. 

- In order to handle this serious issue, we propose multiple layers of defense mechanisms that limits the attacker's advantages and ultimately have strong deterrence effect. 

- the underlying theme is transparency. we make the decision made by S transparent and remain untampered in the permanent public database so that S can be responsible for its own actions. 

- in a broader perspective, we create a healthy market place where p2p bilateral filtering is negotiated with the market agreed price and the contract is publicly available for further healthy and attack deterrence market. 

==> paper 2/chapters/intro-sigcomm.tex <==

\vspace{-5pt}
\section{Introduction}
\label{sec:intro}
\vspace{-5pt}

% \muoi{From Usenix 2019, footnotes are discouraged, please remember to use endnotes, not footnotes!}

Distributed denial-of-service (DDoS) attacks are highly prevalent. %, globally accounting to about 20,000 attacks per day.\footnote{DDoS Mon: Insight into Global DDoS Threat Landscape, \url{https://ddosmon.net/insight/}.} 
In the last decade, new attack strategies such as amplification~\cite{rossow2014amplification} and new attack sources such as IoT devices~\cite{guardian2016ddos} have surfaced, which have resulted in attacks of extremely high volume~\cite{zdnet2018ddos}.



%Even though a large number of  DDoS defenses have been extensively studied over the past two decades, arguably the most effective defense against the ever-increasing scale of DDoS attacks, also happens to be one of the oldest and simplest ideas; namely {\em source filtering} or pushing traffic filtering nearer to attack sources. 
A large number of  DDoS defenses have been extensively studied over the past two decades.
Among them, an effective defense against the ever-increasing scale of DDoS attacks is {\em in-network filtering} or empowering DDoS victim networks to install in-network traffic filters in the upstream transit networks. 
This idea was proposed in early efforts (e.g., Pushback~\cite{mahajan2002controlling},
D-WARD~\cite{mirkovic2002attacking}, AITF~\cite{argyraki2005active}) and has repeatedly re-surfaced in standardization committees (e.g., see the recent DDoS Open Threat Signaling~\cite{dots-slides}). 

%

%StopIt~\cite{liu2008filter}, SENSS~\cite{alwabel2015senss},
%DrawBridge~\cite{li2015drawbridge}) 

Dropping suspicious packets closer to the attack sources \updated{at the requests of DDoS victims} is desirable because
it (1) reduces wasted traffic on downstream ISPs, thereby reducing overall
network bandwidth and cost of routing malicious traffic; and (2) has the potential to
handle ever-increasing attack volume (e.g., several Tb/s) since attack volume
at each distributed filtering point can be much lower than the aggregated volume at the victim~\cite{argyraki2005active}. 

Unsurprisingly, there is renewed interest in the community on revisiting in-network filtering solutions. Indeed, a recent DDoS defense architecture, called SENSS~\cite{ramanathan2018senss}, suggests that the traffic filters installed at a few large transit ISPs directly by the remote DDoS victims can prevent most of the volumetric attack traffic from flooding the victim networks.
% \muoi{...suggests that the traffic filtering operations installed by the remote DDoS victims at a few large transit ISPs can prevent most of the attack traffic reaching the victim networks.}
% SENSS also proposes an economic compenstation model for the remote filtering service where the DDoS victims may pay the remote filtering service in per-filter rule base. 

% \paragraph{Problem.}
% However, with the in-network filtering primitive, {\em dropping packets} at transit networks, which used to be deemed abnormal, becomes a {\em normal} network operation, and this can be misused by malicious transit networks. 
However, the in-network filtering primitive can be unfortunately misused by malicious transit networks.
Transit networks may claim to provide in-network filtering service on behalf of a remote DDoS victim only to justify any arbitrary packet drops executed for their own benefit.
For example, a transit network that offers in-network filtering service (which we call a {\em filtering network}) can easily compromise a filter rule {\tt [Drop 50\% of HTTP flows destined to the victim network]} requested by a DDoS victim to harm its neighbor networks, as illustrated in Figure~\ref{fig:venef}.
First, the malicious filtering network can silently discriminate its neighbor upstream ASes by applying arbitrarily modified filter rules (e.g., dropping 80\% of HTTP traffic from AS $A$ but only 20\% from AS $B$) based on its business preference (say, AS $A$ is AT\&T and $B$ is Comcast).
Discrimination and dispute among transit ISPs are not a new problem (e.g., a dispute between Level3 and Comcast~\cite{dispute_level3_comcast}); however, it can be easily exacerbated if transit networks start dropping packets for the sake of DDoS defense. 
Worse yet, the filtering network can also perform the requested filter rules inaccurately (e.g., drop only 20\% HTTP traffic on average) to save its filtering resources while claiming the faithful execution of the requested rules.
% Note that packet drops used to be the results of abnormal network operations (e.g., congestion, network failure/misconfiguration, compromised routers).
% However, when in-network filtering is used, transmit networks are {\em allowed} to drop packets in {\em normal} network operations as well and can be misused by malicious transit networks. 
% Unfortunately, the neighbor ASes and the victim networks cannot detect such misbehaviors in practice and thus are only forced to {\em blindly trust} the in-network filtering services. 

We argue that the {\em verifiability} of in-network filtering mitigates such misbehaviors 
% would render the in-network filtering services vulnerable to misbehavior 
by malicious filtering service providers. 
With filtering verifiability, when a filtering network executes a manipulated filter rule, the DDoS victim network who requested the filter rule or the direct neighbor autonomous system (ASes) of the filtering network can detect the misbehavior immediately.
% claims that packets are dropped only based on the requested filter rules, even the DDoS victim network who requested the filter rules {\em cannot} verify if this claim is true. 
% Moreover, there is no clear way for the direct neighbor autonomous systems (ASes) of the filtering network to determine how and why their packets are dropped by the filtering network.
% Therefore, transit networks can conduct some subtle misbehavior for their own benefit. 

In this paper, we offer the first technical means of the strong verifiability of filtering operations and develop a practical and scalable in-network filtering system, called \name.\footnote{\name stands for `Verifiable In-network Filtering'.}
\name has a generic architecture designed for any transit networks (e.g., Tier-1, large Tier-2 ISPs, IXPs).
% As the first deployment model, we suggest to deploy it in major Internet exchange points (IXPs).
% In the last decade, IXPs have become the central infrastructure of the global Internet connectivity~\cite{ager2012anatomy,chatzis2013there}, with large IXPs handling daily traffic volumes comparable to those carried by the largest Tier-1 ISPs, which makes the IXPs the perfect candidates for our verifiable filtering service~\cite{dietzel2016blackholing}.
% Moreover, unlike the slowly evolving traditional transit ISPs, IXPs are more flexible in integrating with software-defined architecture~\cite{gupta2015sdx}, thus easily providing new value-added services (e.g., fine-grained inter-domain access control~\cite{gupta2016authorizing}, traffic engineering~\cite{dietzel2017sdn}).
We exploit software networking functions running on commodity hardware with trusted execution environments (TEEs), such as Intel SGX~\cite{costan2016intel} and Arm TrustZone~\cite{arm2009security}, which are widely available in commercial off-the-shelf (COTS) server platforms; see Microsoft and Google's SGX-based cloud platforms~\cite{russinovich2017azure-sgx,porter2018asylo-sgx}. 

% \paragraph{Challenges.}
% However, NFV and SGX by themselves are not a panacea, but merely enablers for verifiable filters and 
We identify two key technical challenges to realizing the \name vision in practice: 

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.4\textwidth]{figures/venef.pdf}
% 	\vspace{-5pt}
	\caption{Example of in-network filtering in a transit network. \name enables the direct upstream neighbors/the DDoS victim to {\em verify} if the filtering network executes the requested filter rules correctly.}
% 	\vspace{-15pt}
	\label{fig:venef}
\end{figure}


\begin{packeditemize}
	\item {\bf Auditability.} To make the in-network filtering verifiable, we exploit the trusted execution environment with hardware-based root of trust (e.g., Intel SGX) and provide integrity guarantee for filter logic. 
	Yet, achieving auditable filtering operations is not trivial.
	One challenge is that the correct filtering operations are also affected by {\em external} inputs to the filter (e.g., incoming packet order, time clock feeds), which can be controlled by a malicious filtering network.
% 	to indirectly modify the filter operations. 
	Another challenge is that a malicious filtering network can still {\em bypass} the auditable filters by reconfiguring its network and avoid using the auditable filters for adversary-selected packets. 
	\item {\bf Scalability.} To scale out the filter capacity for large volumetric attacks, parallelization with multiple TEE-based auditable filters is required; however, some necessary network components for parallelization (e.g., traffic load balancers) are not directly auditable.
	Moreover, distributing filter rules across multiple auditable filters creates an optimization challenge, which involves two dimensions of resource constraints. 
\end{packeditemize}


\paragraph{Approach and Contributions.} 
% In this paper, we leverage NFV and SGX to develop a practical and scalable source filtering system for IXPs, called \name\footnote{\name stands for `VErifiable NEar-source Filtering.'}, that ensures the verifiable filtering operations at IXPs. 
\name's design makes the following key contributions to address these aforementioned challenges:

\begin{packeditemize}
\item  We analyze the requirements for auditable filters, particularly, their reliance on the external inputs to the filters, which can be controlled by malicious filtering networks (\S\ref{sec:stateless-filter-design}).
Our key insight is that it is sufficient that traffic filters are {\em stateless} for auditable filter operations.
We also implement an effective {\em bypass detection} that relies on the accountable packet logs (with an efficient sketch implementation) measured inside the TEE (\S\ref{sec:filter-bypass-detection}). 
The packet logs can be used to identify packet drops/injections made outside of the auditable filters. % with a simple fault localization protocol; e.g.,~\cite{argyraki2010verifiable}. 
We demonstrate that an efficient {\em line-rate} implementation (nearly 10 Gb/s throughput performance) of the auditable traffic filters with the TEE support is possible with several system optimizations (\S\ref{sec:eval}); and
% Moreover, to minimize the reliance on the confidentiality guarantees of SGX, \name filters are designed to store no private data within an SGX's protected memory region, called {\em enclave}, except a minimal number of session keys;

\item For highly scalable filtering architecture, we implement a dynamic filter rule distribution algorithm across multiple auditable filters and untrusted network components~\cite{patel2013ananta,gandhi2015duet} (\S\ref{sec:scalable-filter-design}). 
We implement a heuristic that can quickly reconfigure a large number of filter rules (e.g., 150,000 filter rules) and a large volume of incoming traffic (e.g., the total volume of 500 Gb/s) with auditable filter instances (e.g., 50 filters). %; and % in real time (e.g., every 40 seconds); and 

% \item To handle bypass attempts, we implement an effective bypass detection that relies on the accountable packet logs (with an efficient sketch implementation) measured inside the SGX enclave (\S\ref{sec:filter-bypass-detection}). The packet logs can be used to identify packet drops/injections outside of the auditable filters with a simple fault localization protocol; e.g.,~\cite{argyraki2010verifiable}. 
\end{packeditemize}

As an early deployment model, we suggest to deploy \name in major Internet exchange points (IXPs) (\S\ref{sec:deployment-proposals}).
In the last decade, IXPs have become the central infrastructure of the global Internet connectivity~\cite{ager2012anatomy,chatzis2013there}, with large IXPs handling daily traffic volumes comparable to those carried by the largest Tier-1 ISPs, which makes the IXPs the perfect candidates for our verifiable filtering service~\cite{dietzel2016blackholing}.
% Moreover, unlike the slowly evolving traditional transit ISPs, IXPs are more flexible in integrating with software-defined architecture~\cite{gupta2015sdx}, thus easily providing new value-added services (e.g., fine-grained inter-domain access control~\cite{gupta2016authorizing}, traffic engineering~\cite{dietzel2017sdn}).
We perform large-scale inter-domain simulations with two realistic attacks (i.e., DNS amplification, Mirai-based DDoS attacks) and show that deploying \name in a small number (e.g., 5--25) of large IXPs is enough to handle the majority (e.g., up to 90\%) of DDoS attacks (\S\ref{subsec:against-ddos-exp}). 

% These results suggest  the technical
% feasibility of the practical and verifiable in-network filtering system at IXPs. We hope that this result can provide the necessary fillip for the renewed interest in practical in-network filtering mechanisms as architectural solutions to ever-increasing DDoS threats.





==> paper 2/chapters/language.tex <==
\section{Policy Abstraction}
\label{sec:policy-abstraction}
%Intro
%- 
%
%Address space agreement
%- Each ISP provides their IP range (set of prefixes they want to include for traffic filtering -- often known information (e.g., peering website)). via $M$, address space agreement. All agree with the address space $U$.
%
%Traffic class partition 
%- why? not comparable
%
%Policy language: what to do with the traffic classes?
%- expressive range: low to high (binary, rank, weight, guarantee/BE) - some combination also possible.
%- binary: too simple. no fairness.
%- weight: too expressive. thus hard to have privacy. (we rule out noise...)
%- rank: right choice.
%
%Distance function
%- important due to the notion of fairness. Closeness or similarity. Semantic.


%The middlebox $M$ should compose the two policies $P_s$ and $P_d$ fairly (thus
%incentivizing the two untrusted parties) and at the same time should limit the
%amount of policy leakage (to the other party) to a certain degree.  In this
%section, we describe the problem space we deal with in the policy composition.
%We will first offer intuitive illustration why there exist an inherent
%trade-off between fairness and privacy in our composition problem.  Then, we
%will discuss the expressive policy languages we may consider for filtering
%policies and corresponding distance definitions. 

%\subsection{Trade-off Between Fairness \& Privacy}
%Intuitively, there is an inherent trade-off between fairness and privacy.
%
%Let us first consider a composition that only aims to maximize the fairness
%metric.  Fairness between two different policies can be interpreted as finding
%a middle point between the two given policy points in the entire policy space,
%which is more clearly defined later.  In other words, the {\em fair} composite
%policy should be equally distanced (the notion of distance is also clearly
%defined later) from the two policies.  Thus, when one policy (either $P_s$ or
%$P_d$) and a middle point ($P_{s,d}$) is given, one can narrow down a number of
%potential the other policies with high accuracy.  This shows that achieving
%fairness naturally undermines the privacy of the other party's policy.
%
%Conversely, a composition that maximizes the privacy metric exclusively
%significantly reduces the fairness.  The strongest privacy implies that when
%one party's policy and the composite policy are given, any possible policy of
%the other party is nearly equally probable.  Indeed, under such strong privacy,
%any extremely unfair composite policy should be allowed since it should be
%equally probable.




%Address space agreement
%- Each ISP provides their IP range (set of prefixes they want to include for traffic filtering -- often known information (e.g., peering website)). via $M$, address space agreement. All agree with the address space $U$.
\subsection{Address space agreement}
Two ISPs $S$ and $D$ first exchange their own IP address spaces that they want
to include for the packet filtering policy composition via the \codename
middlebox.  The ISPs may want to include some or all IP prefixes they directly
own or their direct customers own, which can be verifiable via Resource Public
Key Infrastructure (RPKI)~\cite{rpki}.  The source IP address space determined
by $S$ and the destination IP address space set by $D$ are then combined to
constitute the address space, called $U$, for the policies $P_S$ and $P_D$. 

%Traffic class partition 
%- why? not comparable

%Policy expressiveness (or languages): what to do with the traffic classes?
%- expressive range: low to high (binary, rank, weight, guarantee/BE) - some combination also possible.
%- binary: too simple. no fairness.
%- weight: too expressive. thus hard to have privacy. (we rule out noise...)
%- rank: right choice.
\subsection{Policy Languages}
How one describes and interprets the traffic filtering/policing actions for
defined traffic classes is defined by policy languages.  Two ISPs $S$ and $D$,
and the \codename middlebox $M(S,D)$ must agree on a certain language so that
the actions defined by the ISPs are correctly interpreted by $M(S,D)$.  We can
categorize policy languages by their expressiveness as follows (from the lowest
to higher expressiveness):
\begin{enumerate}
\item {\em Binary allow/block} :ISPs determine whether to allow or drop each
traffic class. This simplest language is easy to use and often expressive
enough to filter out suspicious attack traffic and protect prioritized traffic
classes.  
\item {\em Ranks}: ISPs order traffic classes based on priority and
assign ranks to them. This language is more expressive than the binary one as
it can prioritize among two or more traffic classes.
\item {\em Weights}: ISPs assign normalized weights to traffic classes. This is
more expressive than ranks as it can express fine-grained relative priority
among traffic classes.  
\item {\em Guaranteed bandwidth}: ISPs explicitly
assign desired minimum bandwidth guarantees for traffic classes. This allows
strong bandwidth guarantees to some high-priority traffic classes regardless of
other competing traffic flows. 
\end{enumerate}
These languages can be used in combination (e.g., some traffic classes are
given priority ranks while others are blocked) but for the simplicity of
discussion we do not consider such combinations.  With the above policy
languages, ISPs may agree to allow total desired maximum rate $L$ bps as well. 

\paragraph{Expressiveness and fairness/privacy.}
As we saw in the examples in Section~\ref{sec:prob}, policy expressiveness
affects the notion of fairness and privacy in policy composition.  On one hand,
as we saw in Example 1 in Section~\ref{sec:prob}, the low expressive binary
decision makes the language hard to be fair without being non-deterministic
because the language is too simple to express the `middle point' of the two
policies when they are different.  Non-deterministic composition makes it fair
but it seriously damages the privacy property of the policy composition.  On
the other hand, as we saw in Example 2 in Section~\ref{sec:prob}, the much
highly expressive language with per-class weights can easily offer fair
composition (e.g., via taking average Euclidean distance of the weights);
however, it is hard to achieve adequate level of policy privacy because the
given composite policy is too accurately calculated and expressed for $P_S$ and
$P_D$ and thus the other party's policy can be accurately inferred. 

%Distance function
%- important due to the notion of fairness. Closeness or similarity. Semantic.
\subsection{Distance functions}
Choosing a good distance metric that captures the notion of closeness or
similarity of two policies is important because the notion of fairness relies
on finding the middle (or equally distant) point of the two policies.  Distance
between two policies, $d(P_x,P_y)$, can be defined depending on the policy
languages.  For example, one can use Euclidean distance with the weights of the
rules.  One can also use non-Euclidean metrics, such as the number of pair-wise
order differences between two ordered priority sets.
%
%\subsection{Two Dimensions: Policy Languages \& Distance Definitions}
%There exist two dimensions in our problem space: policy language and distance
%definition. 
%
%\paragraph{Policy Language.} 
%It captures the requirements that the network operators wish to express through
%the filtering operations.  We can imagine a simple binary rules, more complex
%rules with ordered preference, or even with specific per-flow bandwidth
%restrictions.  Regardless of policy languages, any filtering policy has one or
%more traffic classes.  A {\em traffic class} represents a group of packets that
%are treated with the same filtering configuration; e.g., a five-tuple defined
%flow aggregate.  Let us define $U$ as the entire flow space (i.e., any possible
%five-tuple flow definition) from all address space of $S$ to that of $D$.  Let
%$C_{s}$ and $C_{d}$ denote the traffic-class sets defined by the source ISP $S$
%and the destination ISP $D$, respectively.
%Each traffic-class set is an exact cover of $U$; that is, traffic classes in
%$C_{x}$ are pairwise disjoint and the union of all the traffic classes in
%$C_{x}$ is equal to $U$.  {\bf Some figures might be helpful?}
%
%\paragraph{Distance Function.} 
%Accurate distance function should be defined to analyze the fairness and
%privacy of the policy composition since the two properties are measured by the
%distance between policies.  Distance is a numerical description of how far
%apart the two policies are.  Thus distance functions we use in the policy
%composition should be a generalization of the concept of policy similarity;
%that is, the more similar two policies are the lower distance should be
%assigned.  Distance between two policies, $d(P_x,P_y)$, can be defined
%depending on the policy language used and the context.  For example, one can
%use Euclidean distance with the priority rank of the rules (i.e., $k$ for
%$k$-th prioritized flows).  Or, Euclidean distance can be used with any
%assigned per-flow weights (e.g., bandwidth values).  As non-Euclidean example,
%one can also use the difference metrics (e.g., preference order difference or
%binary rule violations) as the distance metric.

\subsection{Proposed Policy Abstraction}
\label{sec:proposed-policy}
Based on our observation on the language expressiveness and the
fairness/privacy properties, in this paper, we propose to use preference-ranked
traffic classes as our policy language.  We observe in the next section that
the level of expressiveness of this policy language offers a good balance
between the fairness and privacy.  For distance function, we use the Kendall
tau distance that is widely used to measure the similarity between two ranking
lists.  Kentall tau distance is a metric that measures the number of pairwise
inversion between two simple policies; the distance between two simple policy
$A$ and $B$ is given $D_{KT}(A, B) = |\{(i, j) | (i, j) \in A \land (j, i) \in
B \}|$.  The minimal distance is $0$ when they are identical and the maximum
distance is $n (n-1) /2$ when they are complete reversed, where $n$ is the
number of traffic classes. 

In the next section, we present a set of algorithms to achieve fair and private
policy composition with a proposed policy abstraction. 


==> paper 2/chapters/overview-sigcomm.tex <==
\section{Overview}
\label{sec:overview-sigcomm}
This section describes ...

\subsection{Motivation for Yet Another Source-end Filtering}

%Our focus in this paper is {\em not} on how we can introduce new techniques, negotiation protocol (e.g., \cite{ericsson}), or new Internet architecture for better source-end filtering mitigation. 
%Rather, we aim to make this well-studied technique to really be deployed and accepted by actual network operators and used by ISPs when they are under attacks. 

Our investigation of the history of source-end filtering proposals \cite{x,x,x,x,x,x,x,x,x} has clearly shown that, somewhat surprisingly, no studies consider concrete economic or non-economic incentives for the source networks. 
Considering the inherent lack of any incentive for the source\,---\,they are {\em not} the victims of DDoS attacks\,---\,it is evident that strong incentives (preferably in various forms) are desired and we are motivated to close this gap. 

Our quest for strong incentives for source networks quickly comes to a conclusion that accountable filtering operations are necessary for establishing contracts between two ASes. 
Recent study~\cite{} on the importance of accountability in the inter-domain contracts also motivates us to investigate the accountability property of the source-end filtering operations.
%Yet, no existing studies aim to guarantee accountability against active adversary model.


This work is also highly motivated by the recent advances in high-speed packet processing techniques for commodity server platforms. 
We explore in this paper whether we can achieve multiple Giga b/s or higher filtering performance with only a small number of commodity servers with secure processors. 

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.4\textwidth]{figures/overview.pdf}
	\caption{Overview of source-end filtering with \name.}
	\label{fig:overview}
\end{figure}

\subsection{Threat Model}

We consider two distinct networks: a {\em source} AS $S$, which hosts potential attack sources (e.g., botnets) in its and its customers' networks, and a {\em destination} AS $D$, which suffers volumetric DDoS attacks and experiences severe congestion. 
The two ASes $S$ and $D$ may be indirectly connected through one or more transit ASes. 
We consider that $S$ and $D$ are {\em mutually untrusted}. 
This threat model is realistic because the source and destination ASes may seldom have any direct contract between them especially when they are in different geopolitical regions with no direct business relationship.

The untrusted ASes may wish to {\em tamper} with the operation of the \name system. 
By tampering with the filtering operations, two ASes may implement a filtering policy that is more favorable to themselves.
Or, $S$ may wish to modify the recorded amount of filtered bandwidth to overcharge for the filtering service to $D$. 
$S$ also may want to {\em bypass} the \name's filtering logic outside of the \name system to ignore the per-packet decision made by \name.

Note that $S$ has more attack capabilities than $D$ in general since it is the operator that executes and manages the \name system in its own network infrastructure. 
Particularly, we consider that $S$ can control the software/hardware components of \name and even its privileged software (e.g., operating system). 
Moreover, $S$ has the full control (e.g., read, inject, drop) over all the packets entering/leaving \name. 
On the contrary, the destination $D$ can observe only the packets arriving at its network. 

\paragraph{Scope.}
%During the lifetime of a session for mutual collaboration between two ASes $S$ and $D$, we consider that $D$'s filtering policy may change dynamically to adapt to the incoming DDoS attack traffic and the availability of its network and customers. 

$S$'s modification of the packets from $S$ to $D$ outside of the \name system is out of scope of this paper.
In practice, as a Internet service provider, $S$ can always modify any bits of the packets from $S$ to $D$. 
Our \name is a single network function executed in a small subset of the entire network $S$ and we do not (and also cannot) prevent $S$ from modifying the packets it serves.

We consider that other malicious attack sources may generate {\em IP-spoofed} DDoS traffic with the source IPs under the control of a source AS. 
The proposed \name system handles such IP-spoofed attack traffic by simply distinguishing packets with spoofed source IPs and the ones that actually come from the designated source AS. 


\subsection{Intel SGX Overview}

\msk{how widely available.}

\msk{focus on isolated execution, remote attestation.} 

\msk{threat model}

\msk{we trust IAS}

\subsection{Naive Design}

To apply the security guarantees of Intel SGX to our \name design, we borrow some ideas of building user-level applications using the SGX features with a small trusted computing base (TCB) of a few thousands of lines of code~\cite{panopy,scone,royan}. 
To that end, we present a simple design for the \name application, which we will call a {\em naive} design, that immediately offers several useful security properties and handles many of the attacks launched by $S$. 
%Although our naive design of \name may seem already quite useful for closing the gap between the  ideas and the deployment possiblities of source-end filtering proposals, it has several critical security and performance drawbacks, as we see shortly. 

The idea of the naive design is simple. 
We modularize network functions in both the control-plane and data-plane and encapsulate all of them into an SGX enclave. 
Once the functions are enclaved, the integrity of their executions is guaranteed due to the strong execution and the states isolation of the SGX architecture; e.g., even the privileged operating system cannot read/write the execution of the enclaved functions.
Moreover, the remote attestation of the \name ensures that the correct and untampered functions have been loaded and running on the SGX platform.
% has been loaded and running on the platform ensures that the participating ASes the correct and untampered functions operate the \name's filtering operations. 
The full implementation of \name should be open-sourced to public so that the networking community can scrutinize the codes and any participating ASes can attest before making a contract with other ASes. 



In the naive design, we include the following functions into an SGX enclave.

\paragraph{Control plane:}
\begin{itemize}
	\item Secure channel establishment with ASes {\tt est\_sec\_chan()}
	\item Policy composition {\tt compose\_pol()}
	\item Packet logging export {\tt export\_pkt\_log()}
	\item Billing generation and report {\tt gen\_billing()}
\end{itemize}

\paragraph{Data plane:}
\begin{itemize}
	\item Interpretation of composed policy {\tt read\_comp\_pol()}
	\item Packet classification {\tt classify\_pkt()}
	\item Hierarchical token bucket {\tt htb()}
	\item Packet logging for incoming/outgoing traffic {\tt log\_pkt()}
\end{itemize}

The above contro- and data-plane functions are enclaved and exchange control information with $S$ and $D$ and receive/send data packets from $S$ and to $D$ via a set of special SGX functions (e.g., {\tt ECALL} and {\tt OCALL}) that mediate all the interactions of the enclave. 

Note that in Figure~\ref{fig:overview}, the naive \name design includes trusted third-party payment system. 
The payment system checks the validity of the bills submitted by $S$ and makes the payment to $S$ when the bill is verified. 
It also provides an escrow services to $S$ and $D$ so that they can make payment to each other without mutual trust between them. 
As shown in Figure~\ref{fig:overview}, the Intel Attestation Service (IAS) as the trusted third party of the system that verifies the code integrity.
%and the SGX hardware, which becomes the root of trust of the \name system. 
%(\deli{will check the fact about the role of IAS and how the code integrity is guaranteed})

%Security properties offered by the naive design:
%\begin{itemize}
%	\item {\bf Fair policy composition:}
%	\item {\bf Prevention of direct reading of submitted and composed policies:}
%	\item {\bf Accountable packet filtering decision:}
%	\item {\bf Secure packet logging:}
%\end{itemize}

\subsection{Attacks handled by the Naive Design}

The SGX-based naive design already rules out a number of attacks:

\paragraph{Direct reading and tampering of submitted policies:}
$S$ cannot read or tamper with $D$'s policy \PD because $D$ establishes a secure channel with the \name instance via {\tt est\_sec\_chan()} that is isolated from any non-SGX executions (e.g., OS system calls). 
The policy \PD is sent over the secure channel and becomes available only to the \name's {\tt compose\_pol()} function (which is also enclaved) that receives two policies \PS and \PD from $S$ and $D$, respectively, and composes \PSD.

\paragraph{Direct tampering of policy composition:} 
$S$ cannot directly modify the policy composition logic implemented in the {\tt compose\_pol()} function as the function is enclaved.
It is also open-sourced and thus can be publicly verified to ensure that the policy composition is done in a fair manner (whose definition will be defined and analyzed in Section~\ref{}). 
%Moreover, the SGX's remote attestation allows $D$ to always check that the function has not been modified from the open-sourced codebase.

\paragraph{Direct tampering of policy enforcement:}
Similarly, $S$ cannot tamper with how the composed policy \PSD is enforced in the \name's data-plane because all the related data-plane functions {\tt read\_comp\_pol()}, {\tt classify\_pkt()}, and {\tt htb()} are completely enclaved. 
Once {\tt read\_comp\_pol()} receives \PSD from the enclaved function {\tt compose\_pol()}, it configures the other two enclaved functions {\tt classify\_pkt()} and {\tt htb()} for their traffic class definition update and the token bucket parameter setups. 
For each data-plane incoming packets, {\tt classify\_pkt()} and {\tt htb()} perform the specified multi-class rate-limiting operations and decide allow/drop for each packet within the protected SGX enclave. 

\paragraph{Bypassing \name:} 
$S$ may wish to bypass \name when the decision by it is not aligned with $S$'s preference; e.g., $S$ wants a packet $p$ to be delivered to $D$ but \name drops it. 
In the naive design of \name, $S$ can no longer bypass \name without being detected because \name has the untampered logs of all the incoming/forwarded packets in the enclaved {\tt log\_pkt()}. 
\name periodically sends the secure logs to $D$ via another enclaved function {\tt export\_pkt\_log()} over the secure channel. 
At $D$'s side, it also keeps the logs of packets independently and compares with the secure logs from \name to detect any bypass attempt for any packet by $S$. 

\paragraph{Modification of bandwidth measurement:}
$S$ may wish to modify the measured bandwidth by \name to claim unfairly large amount of billing to $D$ at the end of a filtering cycle. 
This threat is prevented since the packet logging function {\tt log\_pkt()} and the billing generation function {\tt gen\_billing()} are both enclaved and thus modification is prevented. 
Therefore, the naive \name implementation ensures that the bandwidth report attached to the final billing is an accurate measured bandwidth of the packets dropped by \name.

\subsection{Challenges}

Despite its useful security properties, especially the verifiably fair policy composition and secure packet logging, the naive \name design appears to be still vulnerable to attacks that happen {\em outside} of the \name system. 
The naive design guarantees the execution integrity of all of its functions only within the SGX enclave; however, the notions of fairness and accountable packet logging between $S$ and $D$ are in fact completely defined outside of \name.
%Thus, the fairness of policy composition and the accountability of packet logging are guaranteed for the {\em given inputs}, such as the submitted policies and incoming packets.
%However, the design does not guarantee the notions of fairness and measurement accountability that are in fact dependent on the inputs to the \name system. 

Let us first consider the notion of fairness in the source-end filtering problem, which is the fundamental guarantee for the incentive to the source ASes in mutual collaborations. 
The fairness between two ASes $S$ and $D$ should describe the quality of being impartial to $S$ and $D$ in filtering policy decision. 
When the genuine policies (say $GP_S$ and $GP_D$) of $S$ and $D$ and their submitted policies (that is, \PS and \PD) are different, the fairness notion cannot be solely guaranteed by the fairness guarantee within the \name system. 
For example, $S$ may send non-genuine policy (i.e., $GP_S \neq P_S$) to \name in the hope that the composed policy \PSD is close to its genuine policy. 
We illustrate this {\em fairness attack} in more detail in Section~\ref{} and address our defense approach. 

%What is subtle in this definition is the implicit gap between the genuine policies (say $GP_S$ and $GP_D$) of the ASes and their submitted policies (that is, \PS and \PD). 
%The naive design guarantees a fairly composed policy \PSD for the given \PS and \PD but there is no way to guarantee that \PSD is the pair policy for the actual genuine policies $GP_S$ and $GP_D$. 
%Since the genuine policies are converted to the submitted policies outside of the SGX-enclaved functions, \name cannot guarantee this broader notion of fairness. 
%Due to this limitation, a malicious AS can send non-genuine policy to the system in the hope that the composed policy is close to its genuine policy. 
%We illustrate this {\em unfair fairness attack} in more detail in Section~\ref{} and address our defense approach. 

Similarly, the accountable logging property relies on the input traffic to the \name system. 
Therefore, when a source AS $S$ manipulates the input traffic, the accountability of the \name system itself may not necessarily guarantee the accurate traffic measurement. 
In a simple example, if $S$ creates high volume dummy packets for the additional input to \name, then our naive design would perform the filtering operations over the dummy packets and finally report much inflated bandwidth measurement report (and thus higher billing to $D$). 
We describe such {\em bandwidth inflation attack} in more detail in Section~\ref{} and our multi-layered systematic defense approaches. 

Moreover, the additional trusted third party for the economic incentive system may become the bottleneck in practical deployment. 
The trusted third party is essential for the verification of the accountable billing (thus, $S$ cannot forge the billing results) and the escrow service for the payment from $D$ to $S$. 
However, in practice, it might be challenging (if not impossible) to find such mutually trusted party in the Internet. 
$S$ and $D$ may very well be located in different geopolitical environment and they may have different sets of trusted parties as the candidate for this job. 
One may suggest to use one of the existing trusted third party services in the inter-domain Internet, such as RPKI; however, such PKI services are not suitable for active verification and escrow services. 
We address this challenge in Section~\ref{} by removing the need for a trusted third party with some reasonable practical assumptions. 

Lastly, the naive design also would likely suffer significant performance overhead, particularly the filtering rate would be much lower than the maximum line rate that typical high-end network interface card can handle (e.g., 10 Gb/s).
The main challenge stems from the intense per-packet secure processing for the verifiably fair packet filtering ({\tt classify\_pkt()} and {\tt htb()}) and the accountable packet logging ({\tt log\_pkt()}) in the enclaved data plane functions. 
Secure processing of all data packets from $S$ to $D$ in the naive design incurs packet copies from the non-enclave memory to the enclave memory, which incurs tremendous overhead for context switching between the non-secure and secure world. 
Worse yet, the available memory size of the secure world is limited up to 128 MB.
The context switching and the small memory size are known to be the main sources of performance overhead especially for high-speed packet processing. 
We discuss how much performance gain can be achieved with architectural optimization in Section~\ref{}.
%\deli{Another performance degradation comes from the paging of insufficient secure memory inside enclave. It is due to the architectural limitation of current SGX version, which only supports up to 128 MB memory within enclave. So the naive implementation of copying all the packets, meaning over 128MB memory footprint, will triger the OS's secure paging with intolerable overhead.}
 


%
%\msk{Three main remaining challenges:}
%
%\msk{(1) Fairness guarantee can be violated if one party can read other's policy and adjust its policy; }
%	
%\msk{(2) Accountable billing without a trusted third party against active adversaries (e.g., bandwidth inflation attacks); and }
%	
%\msk{(3) data-plane must support line-rate speed but it is hard due to per-packet secure operations.}
%
%\msk{We address each point in the following three sections.} 

==> paper 2/chapters/payment-channel.tex <==
%\subsection{Payment Channels}
%\label{sec:payment-channel}



\name allows source ISPs to charge fees based on the amount of filtering work (which is measured in the refutable invoice) to destination ISPs.
This offers explicit {\em economic incentives} to ISPs for source filtering defense, thereby removing the reliance on ISPs' altruistic motivations~\cite{mahajan2002controlling,argyraki2005active,liu2008filter}.
For monetary transactions, \name may utilize any existing finance infrastructure (e.g., international banks);  yet, in this paper, we choose to use cryptocurrencies for their fast and easy transactions across different countries. 

\begin{figure}[h]
	\centering
	\includegraphics[width=0.40\textwidth]{figures/payment-channels-bitcoin.pdf}
	\vspace{-5pt}
	\caption{A payment channel that utilizes a blockchain (e.g., Bitcoin) as the escrow for the payment and the verifier of the performed filtering work.}
	\vspace{-5pt}
	\label{fig:payment-channels-bitcoin}
\end{figure}

We present an optimized payment channel design that fully utilizes the SGX's security primitives and thus minimizes the reliance on underlying cryptocurrencies. 
Figure~\ref{fig:payment-channels-bitcoin} illustrates the steps:
\begin{packedenumerate}
\item $D$ establishes a \name contract with $S$.
\item $S$ creates an enclaved filter $E$; $E$ creates a fresh cryptocurrency wallet address {\em Addr$_{E}$} and attaches it to its attestation report.
\item $D$ makes a transaction of $X$ coins from its address {\em Addr$_{D}$} to {\em Addr$_{E}$} with the timed lock $T$~\cite{todd2014bip}. This guarantees that the $X$ coins are returned to {\em Addr$_{D}$} if it is not spent after time $T$. 
\item After the filter task, $E$ calculates the fee $Y$ based on the refutable invoice and the negotiated pricing rate, and makes a transaction {\em TX} that includes $Y$ from {\em Addr$_{E}$} to {\em Addr$_{S}$} (as a payout) and $X-Y$ from {\em Addr$_{E}$} to {\em Addr$_{D}$} (as a return).
\item  $S$ submits the transaction {\em TX} to the blockchain to make the final payment. 
\end{packedenumerate}

Note that this model is {\em scalable} because it requires only two regular transactions that can be supported by virtually any cryptocurrencies. 
Moreover, participating ISPs can be ensured that their source filtering activities and payment history remain {\em private} because their public transactions are indistinguishable from other regular transactions.

%An in-depth discussion on alternative payment channel designs (e.g., use of smart contracts) and their advantages and disadvantages are found in Appendix~\ref{sec:payment-channel-appendix}.


==> paper 2/chapters/payment.tex <==
\section{\name Contracts}
\label{sec:econ-incentive}
%\section{Handling Billing Inflation}

\paragraph{}

\subsection{Trust Anchors for Trust Bootstrapping}

Building trust between two distrusting ISPs is one of the goals in \name contract. Therefore, given that two ISPs may not have any direct relationships before, well-known trusted third parties can be a good starting point for trust bootstrapping. \name contract relies on two external parties, \textit{Resource Public Key Infrastructure} (RPKI) and \textit{Intel Attestation Service} (IAS) and one internal party TESEF whose trust can be extended by the asymmetric cryptography while only the roots certificate need to be unconditionally trusted.

\paragraph{RPKI}. As a free and world-wide service, it is mainly used for securing the Internet routing. While in \name contract, because of the open environment where most ISPs stay and the urgent situaion victim ISP is facing, RPKI can help ISPs reduce the risk of any possible scams and effectively make contact with other legitimate ones who own Internet IP resources related to the ongoing volumetric attacks. For example, as a victim in DDoS, $D$ certainly has a list of ISPs who are the direct upstream of the malicious hosts or controlled botnets. $S$ may also want to confirm the traffic indeed heads towards $D$ instead of a impersonater who ask for arbitrary filtering service.

\paragraph{IAS}. As an important service of the Intel SGX that complete the trust establishment (remote attestation), Intel Attestation Service is a trusted source that responds to any registered remote party who wants to verify a authentic SGX hardware, and provides a verifiable attestation report for public verification (with its signature published). This report is not only accessible to the challenger but also anyone who has the IAS ceritificate and is able to verify the signature in the attestation report. Note that in our \name system, we assume $S$ is both the platform operator who runs the enclave and service provider who attests the running enclave with IAS so anyone including $D$ can knows the enclave's integrity and authenticity status.

\paragraph{TESEF}. We assume that the \name binary will be publicly available along with its source code and the signature. The process that compiles and links the code into binary is securely runs in a trusted environment, so that the private key signing the enclave is also protected to prevent any malicious code injection. Ths signed binary is also an important step required in the SGX security perimeter, which provides a integrity checksum for the enclave initial state after launch and a signature that identify the true author of the entire building process.  

\subsection{Contract initiation and execution}

The contract is nothing but an agreement that $S$ provides $D$ the filtering service by running \name filter to reduce the traffic rate and $D$ makes the payment accordingly. Figure~\cite{contract} shows the essential interactions between $S$, $D$ and other parties ($E$ for enclave and $I$ for IAS) starting from the first contact made by $D$ to the last step of $E$ making the payment onbehalf of $D$. We will further clarify the details later, but first we discuss the notations we used in this section. 

\paragraph{Notations}. The trust establishment is built on top of the asymmetric keys owned by each of the participants and trusted third parties. We use the following notations for the asymmetric keys and its encrypting and signing to ease the illustration throughout this section.

\begin{enumerate}
    \item $\pKey{X}$, $\sKey{X}$: the public and private keys of $X$.
    \item $\enc{A}{\sKey{X}}$: the plaintext of message $A$ along with $X$'s signature.
    \item $\enc{A}{\pKey{X}}$: the ciphertext of message $A$ encrypted by $X$'s public key.
\end{enumerate}

\begin{algorithm}[H]
\floatname{algorithm}{\name Contract}
\renewcommand{\thealgorithm}{}
\caption{Interactions between $S$, $D$, $E$ and $I$}
% \label{}
\begin{algorithmic}[1]
    \State $\mathrlap{S}\hphantom{D}\leftrightarrows\hphantom{D}\mathllap{D}$ : establish a channel through key exchange
    \State $\mathrlap{S}\hphantom{D}\Leftrightarrow\hphantom{D}\mathllap{D}$ : negotiate the contract $F$, $M$, $L$, $P$, $T$ via the channel
    \State $\mathrlap{S}\hphantom{D}\leftarrow\hphantom{D}\mathllap{E}$ : generate quote $Q = \{H_1, H_2, \pKey{E} \}$ with EPID signature
    \State $\mathrlap{S}\hphantom{D}\rightleftarrows\hphantom{D}\mathllap{I}$ : get attestation report $R = \enc{Q}{\sKey{I}}$
    % \State $\mathrlap{S}\hphantom{D}\leftarrow\hphantom{D}\mathllap{I}$ : reply with the attestation report $R = \enc{Q}{\sKey{I}}$
    \State $\mathrlap{S}\hphantom{D}\rightarrow\hphantom{D}\mathllap{D}$ : forward $R$ to $D$ for proving
    % \State $\mathrlap{E}\hphantom{D}\rightarrow\hphantom{D}\mathllap{D}$ : send the policy $\enc{\enc{P_D}{\sKey{D}}}{\pKey{E}}$
    % \State $D\overset{\$}{\dashrightarrow}\hphantom{D}\mathllap{E}$ : entrust the deposit to $E$
    \State $\mathrlap{S}\hphantom{D} \rightarrow \hphantom{D}\mathllap{E} \leftarrow D$ : send $P_S$, $\enc{\enc{P_D}{\sKey{D}}}{\pKey{E}}$ and deposit to $E$
    % \State $\hphantom{D}\mathllap{E}$: compose $P_S$ and $P_D$ into $P_{S,D}$
    \State $\mathrlap{S}\hphantom{D} \leftarrow \hphantom{D}\mathllap{E} \rightarrow D$ : pay $S$ and refund $D$
    \end{algorithmic}
\end{algorithm} 

\paragraph{Channel establishment}. At the beginning, $D$ attempts to contact $S$ via all possible channels to establish a reliable communication channel. The assumption here is that, even facing serious congestions on the main links, ISPs still have the backup plans to guarantee Internet access for urgent situations. We also consider the correct and effective contact of $S$ are public and accessible via $D$'s available channels. The channel establishment follows standard key exchange protocol using the RPKI asymmetric keys and creates an ephemeral symmetric key for the ongoing session. The usage of RPKI authenticates the legitimate identity of participants in the upcoming contract, avoiding any impersonation attacks.

% D initiates key exchange with S and establishes a secure channel with end-to-end encryption (shared symmetric key) and authentication (R’ asymmetric key)

\paragraph{Contract negotiation}. Through the established channel, $S$ and $D$ have the negotation over the contract content and agree on a set of non-sensitive parameters for filtering, including the following things:

\begin{enumerate}
    \item $\mathbf{F}$: The maximum range of the traffic to be filtered.
    \item $\mathbf{M}$: The maximum inbound rate that counts in the bill.
    \item $\mathbf{L}$: The maximum outbound rate that $F$ should be reduced to.
    \item $\mathbf{P}$: The price that $S$ charges $D$ for the traffic removed.
    \item $\mathbf{T}$: The contract expiration time
\end{enumerate}

% D drafts a filtering contract and negotiates with S regarding the content
% F: IP-to-IP flow being filtered, from S to D.
% M: maximum inbound rate that counts towards the bill
% L: outbound rate that the filter reduce the inbound rate to
% P: price that D pays for the traffic removed

\paragraph{Enclave instantiation} 
While the contract negotation is going, $S$ can choose to start deploying \name binary obtained from reliable public source. The SGX CPU will make a trusted measurement (i.e., \texttt{MRENCLAVE}) in the form of 256-bit SHA-2 hash over the entire loading process to ensure the initial state is not tampered. We denote it as $H_1$. $H_1$ is also checked against a special signature structure (i.e., \texttt{SIGSTRUCT}) provided together with the binary, which is generated by the SGX building toolchain. This signature also contains other useful information (i.e. \texttt{MRSIGNER}, \texttt{ISVPRODID}, and \texttt{ISVSVN}) that can be used to identify the specific binary. These informaion is denoted as $H_2$. We will see how $H_1$ and $H_2$ is used to guarantee the code integrity and authenticity and prove to a remote party $D$ later.

\paragraph{Remote attestation}
$S$ starts the remote attestation by requesting a special \textit{quote} (denoted as $Q$) generated by SGX platform service on the same machine, and signed by an \textit{attestation key} (denoted as $A$) that is only verifiable by Intel. The quote $Q$ includes but not limited to these important fields: $H_1$, $H_2$, and $\pKey{E}$, a fresh public key. The quote is sent to IAS for verification and IAS replies a attestation report $R$ is the signature of the quote is verified. IAS also provides the signature as $\enc{R}{\sKey{I}}$, so any one who knows IAS public key $\pKey{I}$ can verify the signature and believe the content, which contains $Q$ and other information. Remember that $Q$ contains $H_1$, $H_2$ and $\pKey{E}$, which ensures one thing: $E$ is runnning a \name filter from a trusted source and holds the private key $\sKey{E}$ securely inside the enclave.

% $S$ presents the quote in the form of $\enc{H_1, H_2, \pkey{E}}{\sKey{A}}$ 

% S boots up the filter, completes the remote attestation, and forwards the attestation report to D for verification
% S launches E with audited and signed TESEF binary
% S obtains the quote from platform service locally with signature signed by an attestation key using EPID technique. The quote has the following facts
% MRENCLAVE: hash over E’s loading procedure as integrity proof
% <MRSIGNER, ISVPRODID, ISVSVN>: TESEF authorship proof
% (KE: E’s ephemeral key)
% S forwards the quote to I for attestation and gets the attestation report with I’s signature. The report contains the quote, hence extending the trust to the quote
\paragraph{\name filtering}. \deli{S routes F to E to start the filtering, with auditability in control-plane and data-plane}
%control-plane: policy composition
%data-plane: rate-limiting and billing

\paragraph{Payment}.
% D makes a deposit, and provisions PD to E with signed and encrypted message. S also presents PS to E to run the control-plane function - policy composition
%The deposit can be made in all manners, with two necessary properties
%E solely controls the fund during operation time (for sake)
%D regains control of the fund after the operation time (for  sake) 

% \msk{(1) Scalable negotiation (i.e., making contracts with many sources at once) with a single contract transaction. (2) Sub-linear blockchain cost increase. (3) Private filtering policy agreement---bilateral collaboration.}

\subsection{Flexible Entrusted Payment from $D$ to $S$}

\deli{show an example of using bitcoin as the payment scheme}

\deli{compare the cost with other choice}
% When D sends PD secretly to E, it also sends the deposit to E’s wallet immediately if it can be ensured that the deposit will be secured by it again after T. This can be guaranteed by a promised transaction from E to D which the blockchain accepts only the operation lock T expires. 
% Deferred Transaction 1 [promised transaction] E to D nLockTime > current block time + T
% Immediate Transaction 2 [deposit transaction] D to E with the deposit
% [operation lasting for T]
% Immediate Transaction [payment transaction] E pays to S, refunds to D in one transaction, which spends the money before the promised transaction, rendering it invalid.
% If anything goes wrong (E fails to execute, or halts in the middle), the deferred transaction will take effect.


% We argue that in addition to the non-economic incentive, it is necessary to provide economic incentives to source ISPs with direct fungible payment from $D$ to $S$. 
% First, without a payment mechanism, the source-end filtering service by $S$ can be exploited by selfish $D$. For example, even when it is not under attack $D$ may attempt to save its operating cost by asking the packet filtering operations to $S$. Since $S$ in general cannot verify the necessity of packet filtering (e.g., existence of attacks), such exploitation is hard to detect. Direct payment scheme can effectively deter such exploitations.
% Second, if $S$ receives too many \name requests, it needs to carefully determine how it should use its limited filtering capability. The payment scheme with negotiable pricing can make \name further increase the economic incentive for $S$ (since $S$ can ask for higher pricing when there is competition) while more efficiently using its limited resource (since more desperate destinations will use the filtering service).

% To remove any additional trusted third party and implement a flexible payment scheme, we propose to use the Ethereum smart contracts. This generates the permanent, immutable records of \name services on the Ethereum blockchain. 
% Such high level of transparency of \name services in the public domain naturally generates an open inter-ISP filtering market since all the pricing and the results are publicly available. As a result, the reasonable market prices may naturally emerge. Also, misbehaviors can be deterred as misbehaving ISPs are easily recognized in the immutable records. 

% \subsection{Contract creation and participation}

% \paragraph{Notations}
% \begin{enumerate}
%     \item $<\pKey{S}, \sKey{S}>, <\pKey{D}, \sKey{D}>$: The RPKI resource certificate key pairs for $S$ and $D$.
%     \item $<\pKey{E}, \sKey{E}>$: \name enclave's fresh key pair
%     \item $<\pWallet{S}, \sWallet{S}>, <\pWallet{D}, \sWallet{D}>$: The Ethereum wallet address and private key for $S$ and $D$.
% \end{enumerate}

% $D$ first initiates the \name contract on Ethereum blockchain with two main types of information, filtering tasks $F$ for disseminating the filtering requesting and trust anchors $T$ for setting the root of the trust in the future verification. 

% \paragraph{Filtering Tasks $F$}. 
% \begin{enumerate}
%     \item The source IP prefixes that require filtering.    
% \end{enumerate}

% \paragraph{Trust Anchors $T$}.

% \begin{enumerate}    
%     \item The trust anchor for SGX platform attestation verification.
%     \item The information for SGX enclave integrity check. (MRENCLAVE, MRSIGNER, ISVPRODID, ISVSVN)
%     \item $D$'s RPKI resource ceritificate key pair.
% \end{enumerate}

% %Note that $D$'s wallet address $\pWallet{D}$ is also included in the signature to bind the Ethereum wallet identity with the RPKI identity. This  
% The last parameter, the signature on its wallet certify the contract is truly created by $D$, as proved by its RPKI certificate.

% \deli{$\pWallet{D}$ calls \textbf{FilterContract<$F$, $T$, $\enc{\pWallet{D}}{\sKey{D}}$>}}


% \paragraph{\texttt{Join()}}

% Once the contract is created, $S$ can choose to join the contract with enough proof, including its owernship of the specified source IPs, and the evidence of running the \name filter on SGX hardwares. Before making any transaction to the contract, $S$ will first check $D$'s signature over $\pWallet{D}$ to make sure no one impersonates $D$.

% Also, before joining happens, $S$ launchs the \name filter on SGX-enabled CPU, finishes the remote attestation and prepare the attestation report with IAS signature to \name contract.

% Eventually, when making the join() call, $S$ add the following information as parameters

% \begin{enumerate}
%     \item $S$'s RPKI public key
%     \item The attetation report signed by IAS
% \end{enumerate}


% The enclave code contains the following hardecoded trust anchors:

% \begin{enumerate}
%     \item RPKI's root certificate
%     \item S'own RPKI
%     \item D's 
% \end{enumerate}

% \subsection{Negotiation}

% Once both parties join the contract, they can start the negotiation via a series of calls of negotiate(). Each of them take turns to modify the pricing details (e.g. IP ranges, filtering price and contract lasting time) until one of them accepts the plan by sending the same details as confirmation.

% Ideally the negotation can be finished with two calls in total and these call can also be merged with the first two calls creation and joining. This will save a lof time time and gas cost.

% \paragraph{Launching the enclave and publishing the contract.}
% Based on the negotiated parameters, $S$ launches the \name enclave in its computing cluster with the SGX-enabled processors.
% In addition to its core data-plane functions (e.g., rate limiting functions and the packet logging functions), the enclave creates  particularly important local data structures when it is initiated. 
% Then, the enclave creates its {\em own Ethereum wallet} by deriving the wallet address from a randomly generated 256-bit private key\cite{wood2014ethereum}. By creating a fresh wallet within the \name enclave, we greatly simplify the process of verifying the contracted work in the \name contract. 
% we greatly simplify the verification of the \name contract.
% That is, instead of directly verifying the message from the enclave (e.g., bandwidth measurements) in the \name contract (e.g., by contacting the Intel Attestation Service (IAS) and verifying the corresponding signatures), we write the enclave's wallet address into the \name contract when it is published as the prover so that the contract can later verify the work submitted is signed by the enclave.
% the enclave's identity (i.e., the corresponding SGX-enclaved \name instance) is checked  
% Note that this design choice is inspired by the smart contract design for the automated PKI compromise detection system~\cite{matsumoto2017ikp}. 

% \paragraph{Negotiating contract parameters}
% Before creating the smart contract, $D$ first negotiates with $S$ to agree on the contract details as seen in Figure~\ref{lst:contract-code}. In the negotiation stage, $D$ checks if $S$ has the authority to police the traffic from the desired source IPs by checking with the RPKI infrastructure to bind $S$ with the AS number and the RPKI public key, and some publicly available peering databases, such as, PeeringDB\footnote{\url{https://www.peeringdb.com/}}, to confirm that $S$ peers with an AS that owns the IPs. Once they agree on the contract, $D$ first publishes the contract including the agreed details and sends the maximum amount of cryptocurrency (e.g., Ether) it is willing to pay. The contract is created only once and $S$'s wallet address is also attached to the open contract so that $S$ also knows that the contract will make the payment to its address. 

% \subsection{Flexibile payment}

% \paragraph{Paying for rate-limiting work.}
% The rate-limiting work done by the \name is logged in the form of an array of average incoming traffic rate during each reporting cycle (i.e. \texttt{reportCycle}). This proof of contracted work is generated by the \name enclave during the operation periodically, and forwarded to $S$ with the signature after the operation. $S$ then sends the proof along with the enclave's signature to the \name contract in a transaction calling the function \texttt{Submit()}. The function checks the identity of the contractor and verifies the signature of the proof, and eventually pays the contractor ($S$) according to the work approved by the accounting function \texttt{Calculating()}.

% \subsection{Flexible payment scheme from $D$ to $S$}
% \label{sec:payment-scheme}

% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{figures/payment.pdf}
% 	\caption{\name contract for flexible payment from $D$ to $S$.}
% 	\label{fig:payment}
% \end{figure}

% \paragraph{\name contract.}
% This contract involves three independent parties: the \texttt{owner}, who initiates the contract, the \texttt{contractor}, who agrees to work under the contract, and the \texttt{prover}, who is unbiased in the measuring and submitting the proof of contracted work done by the \texttt{contractor}. In \name, the \texttt{owner}, \texttt{contractor} and \texttt{prover} are destination ($D$), source ($S$) and \name enclave ($E$) as illustrated in Figure~\ref{fig:payment}. The contract content has the following variables:

% \begin{itemize}
%     \item \textbf{\texttt{maxInputRate}}: the maximum incoming rate that $D$ accepts.
%     \item \textbf{\texttt{outputRate}}: the eventual traffic rate that $D$ requires.
%     \item \textbf{\texttt{reportCycle}}: the time cycle of one proof report.
%     \item \textbf{\texttt{reportLimit}}: the maximum number of reports allowed.
%     \item \textbf{\texttt{price}}: the price per unit bandwidth per unit time.
% \end{itemize}

% The Listing~\ref{lst:contract-code} outlines the \name contract code written in an Ethereum smart contract language, \textit{Solidty}. It details smart contract constructor function \texttt{RateLimiter()}, called by the owner to initialize the contract, and redemption function \texttt{Submit()}, called by the contractor to submit the proof of contracted work with the prover's signature and get the payback.

% % -\msk{Figure X. \name contract for flexible payment from $D$ to $S$.}
% \label{lst:contract-code}
% \begin{lstlisting}[caption={Smart contract code},captionpos=b]
% contract RateLimiterContract {
%     address public owner; address public prover; address public contractor;
%     uint64 maxInputRate; uint64 outputRate; 
%     uint256 price; uint64 reportCycle; uint64 reportLimit;
%     uint64[] inputRates;
    
%     function RateLimiterContract(address s, address e, uint64 p, uint64 c, uint64 t, uint64 i, uint64 o)
%         public payable {
%         require(s != 0x0 && e != 0x0);
%         owner = msg.sender;
%         contractor = s;
%         prover = e;
%         reportCycle = c;
%         reportLimit = t;
%         price = p;
%         maxInputRate = i;
%         outputRate = o;
%     }
    
%     function Calculate(uint64[] rates) internal returns (uint256) {
%         uint256 trafficRemoved = 0;
%         for(uint64 t = 0; t < rates.length && t < reportLimit; t++) {
%             if (rates[t] < outputRate)
%                 continue;
%             if (rates[t] > maxInputRate)
%                 trafficRemoved += maxInputRate;
%             else
%                 trafficRemoved += rates[t];
%         }
%         return trafficRemoved * price * reportCycle;
%     }
    
%     function Submit(uint64[] rates, bytes32 hash, uint8 v, bytes32 r, bytes32 s) public {
%         require(msg.sender == contractor);
%         address signer = ecrecover(hash, v, r, s);
%         require(signer == prover);
%         inputRates = rates; /* save the records in the contract */
%         uint256 payout = Calculate(inputRates);
%         uint256 refund = this.balance - payout;
%         contractor.transfer(payout);
%         owner.transfer(refund);
%     }
% }
% \end{lstlisting}


% $S$ can know that she is the only payee of the contract.


%Second, the enclave also creates a local {\em secure time variable} that is  updated only via the secure time source (i.e., {\tt sgx\_get\_trusted\_time()}) from the SGX processors. 
% Using this secure time variable, the bandwidth resource usage measurement report is summarized and the proof of contracted work is calculated. 
% Note that the enclave's wallet, its underlying ECDSA key, and the secure time variable are stored inside the enclave memory and never be copied out.


% volume of traffic removed by the filter is measured by the \name enclave and reported to the \name contract in the form of Ethereum transaction signed by the enclave's address.


%because (1) only the prover can call this function, (2) the transaction is signed by $E$, the wallet address that previously added as the prover.

% \subsection{Transparency and inflation deterrence}

% \paragraph{\name contract records.}
% Since a \name contract is a smart contract in the Ethereum blockchain, its instantiation and final result are written on the chain and cannot be altered or removed once they are confirmed. 
% Therefore all the elements in the contract itself, submitted proof of contracted work, and payout transactions are made publicly available and form the {\em \name contract records} or \name records.
% This creates the transparent records of \name system that can be used as the basis of an open \name market. 

% \paragraph{Useful analysis of \name records.}
% Using the public \name records, one can compile several useful analysis.
% One can easily track the pricing changes (e.g., Ether per unit bandwidth filtering) of the entire \name history, per ISP, or per country. 
% The easy and transparent access to the pricing changes can contribute to the reliable service pricing for the global \name filtering market. 

% The transparent \name records also make us to better understand the DDoS landscape on the Internet. 
% Although DDoS attacks are prevalent and it is often the public's interest to know more about the ongoing DDoS attack campaigns, we often do not have enough information about them except some aggregated information feeds from some privacy companies(e.g., Digital Attack Map\footnote{\url{http://www.digitalattackmap.com/}}). 
% The \name records can be a less biased, more transparent information source that we can use to understand the global DDoS landscape. 
% Note that the \name records do not include too sensitive information about each \name contract, such as filtering policies or private keys. 

% One can also easily reason about the reputation of any ISP for the \name service usage. 
% If an ISP makes too many \name contracts in a regular basis (e.g., always on for several weeks), this could possibly imply that this ISP is exploiting the \name service for its regular traffic filtering or firewall operations, but not for attack mitigation purposes. 
% Transparency in the \name records can be a strong deterrence for such misbehaviors of ISPs. 

% \paragraph{Inflation deterrence.}
% One particularly important misbehavior is a billing inflation where a malicious $S$ creates and sends dummy packets to the \name instance to increase the amount of filtering work (i.e., volume of filtered-out traffic).
% The increased filtered bandwidth is then recorded in the proof of contracted work and used to inflate the final payout to $S$. 
% Although the maximum input bandwidth $S$ can claim is written in its \name contract and thus the amount of maximum claimable payout is limited, $S$ can still continuously increase the dummy packet volume to force $D$ to raise the maximum input bandwidth set by $S$. 

% With the transparent \name contracts in the Ethereum blockchain, such misbehaviors can be deterred because such suspicious behaviors (e.g., continuously increasing attack volumes over a long period time) can easily damage the ISP's reputation. 

==> paper 2/chapters/policy-bias.tex <==
\subsection{Policy Bias Attack}
\name  allows two ISPs to agree on a certain algorithm, which they agree on, to receive \PS and \PD and compute the final filtering policy \PSD.
The policy composition is inside an enclave and thus accountable and any tampering would be immediately detectable.

However, an attack is possible to bias the computed policy \PSD. 
Either ISPs can bias the final policy favoring its genuine policy.  By submitting a carefully modified policy instead of the genuine one, 

\msk{In this ... we assume a fair policy composition (whose details are not discussed here)}.

\msk{we analyze the adversary capabilities for this attack: know the algorithm, know its own genuine policy, and know the other party's policy.}

\msk{we make the last capability infeasible.}

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.5\textwidth]{figures/fairness.pdf}
	\caption{Fair policy composition and an end-to-end fairness violation attack.}
	\label{fig:fairness}
\end{figure}

The fair policy composition algorithm, unfortunately, is insufficient for the end-to-end fairness between $S$ and $D$.
Figure~\ref{fig:fairness}(b) illustrates how malicious ISPs can still break the fairness guarantee.
In this example, the source ISP $S$ is the adversary.
Just like the benign case, $S$ first translates its security policy written in human-readable language into this policy \PS. % that follows the agreed policy definition (e.g., per-class policing with preference in our case).
Then, the adversary $S$ submits a {\em modified} policy $P_S'$ ($\neq P_S$) to the filtering system so that the final composed policy \PSD is (nearly) identical to its own policy \PS.  
This attack is undetectable because the policy modification (i.e., from \PS to $P_S'$) happens {\em outside} of the fair composition system. % and thus it is hard to detect and prevent. 

%\subsection{Attack Prevention}
%\label{sec:fairness-attack-prevention}
\paragraph{A solution.} It is fortunately possible to prevent such end-to-end fairness violation attacks by removing and limiting the attack capabilities. 
For an effective attack, an adversary requires three attack capabilities: the knowledge of the composition algorithm, the other party's submitted policy, and resubmission of its policy.
The first capability must be given to the adversary for the accountability property of the policy composition logic; yet, the last two capabilities can be removed or significantly limited. 
The re-submission of policies can be limited by enforcing a minimum policy resubmission period, which can be negotiated between $S$ and $D$ and explicitly written in a \name contract (see Section~\ref{sec:econ-incentive}).
In this section, we focus on the \PD inference and how \name effectively prevent it.

%\paragraph{Preventing the accurate policy inference.}
Let us describe how we can prevent the adversary from inferring the submitted policy of the other party.
For ease of discussion, let us consider that $S$ is conducting the end-to-end fairness violation attack. 
Since $S$ has strictly more attack capabilities than $D$, our attack prevention argument applies to the attacks by $S$ as well.

Note first that an adversary $S$ cannot directly read \PD or \PSD due to the confidentiality guarantees of SGX. 
Yet, $S$ can still observe the behaviors of the filtering enforcement (that is, which packet is allowed/dropped) and may infer the policy behind (i.e., \PSD) the packet filtering decision. 
After obtaining \PSD, it is straightforward for $S$ to calculate \PD since the policy composition algorithm is publicly known and reversing with the output (\PSD) and one of the input (\PS) is trivial; see Appendix X for details.
Thus, let us focus on how $S$ can infer \PSD in the naive design of \name system and how we can prevent it.

The high-level idea of \PSD inference is that the external observer of the filtering operations. 
$S$ detects the existence of a rate limiter for a traffic class and their configurations, particularly, their average rates, $S$ effectively reveals \PSD.
A recent measurement study~\cite{flach2016internet} proposes that an effective algorithm that allows external observers of the policed traffic rate of a rate limiter to accurately measure its average rate. 
The algorithm in~\cite{flach2016internet} exploits that a rate limiter demonstrates a steady, flat outgoing traffic rate when the filtering is activated due to the excessive packet arrival. 
%Our adversary $S$ may attempt to use the same attack strategy to search for the steady outgoing rate of the rate limiters and reveal \PSD; however, 
\name can prevent this attack simply by removing this artifact (i.e., steady, flat outgoing rate) of our filtering logics by making our rate limiter implementation less accurate; 
e.g., introducing intentional random noise in the hierarchical token bucket (HTB) implementation. 
%Our HTB design already has token re-distribution logic for the work-conserving operations of large numbers of token buckets in the filtering system and we make it intentionally less accurate.
The details of this design choice is found in Section~\ref{sec:impl}.

==> paper 2/chapters/policy.tex <==
\section{Fair Filtering in \name Enclave}
\label{sec:fairness}

As we discussed, source ISPs practically have no incentive to participate in source-end filtering, which is the biggest hurdle for adoption of the technology. 
In this paper, we propose both non-economic and economic incentives. 
%
Although economic incentive is useful and necessary (as we later argue in Section~\ref{sec:econ-incentive}), there may be cases where economic incentive is ineffective; e.g., an ISP's business model is not well aligned with chasing external revenue opportunities, a source ISP is under a sanctioned country where payment is not legally allowed.
Thus, we strongly believe that developing non-economic incentive mechanism that is orthogonal to economic incentives is important. 

\subsection{From outsourcing to {\em bilateral collaboration}}
\label{sec:bilateral-collaboration}
Existing source-end filtering mechanisms~\cite{mahajan2002controlling,argyraki2005active,liu2008filter,alwabel2015senss,li2015drawbridge} may have minor technical differences but the core shared primitive is the {\em outsourcing} of filtering operations to nodes closer to attack sources. 
Outsourcing, unfortunately, offers no incentives to the nodes near the attack sources (e.g., $S$) because they are usually not the victims of the attack.  

To that end, we propose a new source-end filtering primitive, which we call {\em bilateral collaboration}, that directly incentivizes $S$ by offering the control to the traffic filtering operation of the source-end filtering logics. 
Note that this primitive cannot be realized without the established trust between mutually untrusted $S$ and $D$, particularly, the integrity property of the bilateral collaboration logic.

To be more specific, \name allows both $S$ and $D$ to submit their own filtering policies \PS and \PD, respectively. 
The two ISPs are not supposed to consult each other in determining their policies but they do it separately and independently only to represent their own filtering rules and preferences. 
Then, the submitted policies \PS and \PD are processed by the \name instance and converged to a final policy \PSD, which is ultimately used to implement the filters for the traffic from $S$ to $D$.

Compared to the traditional outsourcing modeling, bilateral collaboration
offers an explicit control knob to $S$ so that it can actively participate, not just observe, the filtering operations. 
This simple addition can be extremely beneficial to $S$.
First, it allows $S$ to protect certain packets it wishes to prioritize (e.g., connections for mission critical services/premium customers, white-listed IPs) when some of packets must be dropped due to attacks at $D$.
Second, it allows $S$ to apply its own blacklist (e.g., known botnet IPs within its customers) and deprioritize them. 
Lastly, it indirectly implements the user agreement\,---\,a user scheduling outside of the specification of the target system\,---\,between traffic sources, which is proven to be an ideal solution to denial-of-service attacks at a destination~\cite{yu1988formal}. 

For bilateral collaboration, the policy fairness between $S$ and $D$ is the key because two ISPs should be ensured that their policies are respected in a fair manner. 
%We explain how we achieve the fairness in the rest of this section. 
%
%\subsection{End-to-End Fairness Guarantees}
%The bilateral collaboration can be an attractive incentive to $S$ only when the fairness between $S$ and $D$ is guaranteed; that is, the actual filtering rules must be the result of a {\em fair} composition of the two input policies. 
%
The SGX-based \name design guarantees the fair composition between the two submitted policies \PS and \PD by relying on the SGX's isolated execution and integrity guarantees. 
However, we show that the end-to-end fairness between $S$ and $D$ (not just between their submitted policies \PS and \PD) is in fact non-trivial to achieve due to a potential adaptive attack by $S$ (\S\ref{sec:fairness-attack}). 
We present a number of solutions we use in our \name system. % and describe how they effectively prevent these attacks (\S\ref{sec:fairness-attack-prevention}).

Before we discuss the security concerns, let us first describe the notion of fairness in policy composition. % fairness (\S\ref{sec:fair-composition}).%, focusing on the definition of filtering policy and useful functions over them for fairness discussion. 


\subsection{Verifiably Fair Policy Composition}
\label{sec:fair-composition}

\begin{figure}[t!]
\centering
\includegraphics[width=0.5\textwidth]{figures/fairness.pdf}
\caption{Fair policy composition and an end-to-end fairness violation attack.}
\label{fig:fairness}
\end{figure}

%We begin by describing the abstract model of fair policy composition. 
Figure~\ref{fig:fairness}(a) illustrates the end-to-end fair policy composition. 
Both $S$ and $D$ may have their own packet filtering policies written in human-readable language and they are translated into the policy rules \PS and \PD, respectively. %, we later define their specifications. 
The two policies \PS and \PD are then submitted to the filter where a fair composition logic produces one final filtering policy \PSD. 

Intuitively, the fair composition logic searches for the middle ground between the two submitted policies. 
Algorithmically, we search for the equally distanced policy between \PS and \PD for the final policy when we can define the notion of distance between two arbitrary policies. 

Now let us describe the concrete algorithms that compose the filtering policies with a simple but practical policy definition example. 
Filtering policy is a set of filtering rules that specify certain packet or flow drop/allow operation and thus can vary widely depending on the application. 
%For example, filtering rules for enterprise access control logic should be fine grained, often needs to be stateful and modify packets to handle sophisticated network firewall policies. 
In DDoS mitigation applications, we consider relatively coarse grained flow specifications (e.g., 100s or 1000s of traffic classes) and stateless (since our focus is on the volume of traffic).
%Moreover, actions needed for packet filtering can be simple; e.g., rate limiting based on traffic types. 

Let us summarize the following three types of policy definitions, which are not supposed to be exhaustive lists but some simple examples:
\begin{enumerate}
	\item {\em Binary rules}: As the simplest policy definition, \name determines to allow or drop an entire traffic class. 
%	This simplest action is easy to use and often expressive enough to filter out clear attack traffic and protect clear benign traffic;  
	\item {\em Prioritized binary rules}: Traffic classes are ordered with their priorities and packets with higher priority are served strictly earlier than packets with lower priority. 
%	While this allows the operators to express strong preference notion, it creates a hogging problem (e.g., low-priority packets rarely get served when there are many high-priority packets); 
	\item {\em Prioritized per-class policing}: To address the resource hogging problem of the strict prioritization, traffic classes are ordered and each traffic class is policed with different average rates that are determined based on the priority order. 
%	That is, a high-priority class is assigned with a higher rate than a low-priority class.
%	This is similar to the hard preference action but it alleviates the hogging problem as a high-priority traffic class cannot hog all the available bandwidth. 	
\end{enumerate}

Throughout this paper, we use the {\em prioritized per-class policing} policy definition (unless otherwise noted) as it is more expressive than other action types among the four above action examples.
A filtering policy then can be simply expressed as an ordered list of flow specifications; e.g., \{$c_1,c_2,\cdots,c_n$\} where $c_i$ denotes the $i$-th traffic class defined by the five tuple of TCP/IP flows. 

The distance between two policies $P_1$ and $P_2$ can be defined with the Kendall tau rank distance when one policy is a permutation of the other policy.
For example, if $P_1 = \{c_1,c_2,\cdots,c_n\}$ and $P_2 = \texttt{perm}(P_1)$, the Kendall tau distance $d(P_1, P_2) = |\{(i, j) | (i, j) \in P_1 \land (j, i) \in P_2 \}|$ counts the number of pairwise disagreements between two ranking lists. 
The minimal distance is $0$ when they are identical and the maximum
distance is $n (n-1) /2$ when they are complete reversed, where $n$ is the number of traffic classes. 

\paragraph{Fair composition algorithm.}
Let us now describe the fair composition algorithm for the given two policy inputs \PS and \PD. 
The first issue we face is that the two policies are independently generated by the two ISPs and thus their traffic class definitions can be different and thus {\em incomparable}. 
For example, one traffic class $c$ in \PS may not exist in \PD and thus any comparison between the two is not possible. 
%Such two policies with different traffic class definitions are said to be {\em incomparable} and the distance between them cannot be defined.
%
To make the two policies comparable, we partition their traffic classes into smaller flow definitions until the two policies have the same traffic class sets. 
For example, let us assume a toy example with eight atomic flow definitions $f_1,\cdots,f_8$ and the two incomparable traffic class sets $C_S=\{{\{{f_1,f_2}\},\{{f_3,f_4,f_5}\},\{{f_6,f_7,f_8}\}}\}$ and
$C_D=\{{\{{f_1}\},\{{f_2,f_3}\},\{{f_4,f_5,f_6,f_7,f_8}\}}\}$. 
We partition the traffic classes in $C_S$ and $C_D$ until the two sets become identical  $C_{S,D}=\{{\{{f_1}\},\{{f_2}\},\{{f_3}\},\{{f_4,f_5}\},\{{f_6,f_7,f_8}\}}\}$.

Once the two policies become comparable, we compose them and calculate the policy $P_{S,D}$. 
We define the fairness of a composition function $\phi$ as $\mathcal{F}(\phi) =  |d(P_S,P_{S,D}) - d(P_D,P_{S,D})|$, where $d(P_1,P_2)$ denotes the Kendall tau rank distance between $P_1$ and $P_2$. 
Our aim is to find a $\phi$ that minimize $\mathcal{F}(\phi)$ for all possible input policies $P_S$ and $P_D$.
The detailed deterministic algorithm is found in Appendix~\ref{appx:fair-algorithm} 


\subsection{End-to-End Fairness Violation Attacks}
\label{sec:fairness-attack}

The fair policy composition algorithm, unfortunately, is insufficient for the end-to-end fairness between $S$ and $D$.
Figure~\ref{fig:fairness}(b) illustrates how malicious ISPs can still break the fairness guarantee.
In this example, the source ISP $S$ is the adversary.
Just like the benign case, $S$ first translates its security policy written in human-readable language into this policy \PS. % that follows the agreed policy definition (e.g., per-class policing with preference in our case).
Then, the adversary $S$ submits a {\em modified} policy $P_S'$ ($\neq P_S$) to the filtering system so that the final composed policy \PSD is (nearly) identical to its own policy \PS.  
This attack is undetectable because the policy modification (i.e., from \PS to $P_S'$) happens {\em outside} of the fair composition system. % and thus it is hard to detect and prevent. 

%\subsection{Attack Prevention}
%\label{sec:fairness-attack-prevention}
\paragraph{A solution.} It is fortunately possible to prevent such end-to-end fairness violation attacks by removing and limiting the attack capabilities. 
For an effective attack, an adversary requires three attack capabilities: the knowledge of the composition algorithm, the other party's submitted policy, and resubmission of its policy.
The first capability must be given to the adversary for the accountability property of the policy composition logic; yet, the last two capabilities can be removed or significantly limited. 
The re-submission of policies can be limited by enforcing a minimum policy resubmission period, which can be negotiated between $S$ and $D$ and explicitly written in a \name contract (see Section~\ref{sec:econ-incentive}).
In this section, we focus on the \PD inference and how \name effectively prevent it.

%\paragraph{Preventing the accurate policy inference.}
Let us describe how we can prevent the adversary from inferring the submitted policy of the other party.
For ease of discussion, let us consider that $S$ is conducting the end-to-end fairness violation attack. 
Since $S$ has strictly more attack capabilities than $D$, our attack prevention argument applies to the attacks by $S$ as well.

Note first that an adversary $S$ cannot directly read \PD or \PSD due to the confidentiality guarantees of SGX. 
Yet, $S$ can still observe the behaviors of the filtering enforcement (that is, which packet is allowed/dropped) and may infer the policy behind (i.e., \PSD) the packet filtering decision. 
After obtaining \PSD, it is straightforward for $S$ to calculate \PD since the policy composition algorithm is publicly known and reversing with the output (\PSD) and one of the input (\PS) is trivial; see Appendix X for details.
Thus, let us focus on how $S$ can infer \PSD in the naive design of \name system and how we can prevent it.

The high-level idea of \PSD inference is that the external observer of the filtering operations. 
$S$ detects the existence of a rate limiter for a traffic class and their configurations, particularly, their average rates, $S$ effectively reveals \PSD.
A recent measurement study~\cite{flach2016internet} proposes that an effective algorithm that allows external observers of the policed traffic rate of a rate limiter to accurately measure its average rate. 
The algorithm in~\cite{flach2016internet} exploits that a rate limiter demonstrates a steady, flat outgoing traffic rate when the filtering is activated due to the excessive packet arrival. 
%Our adversary $S$ may attempt to use the same attack strategy to search for the steady outgoing rate of the rate limiters and reveal \PSD; however, 
\name can prevent this attack simply by removing this artifact (i.e., steady, flat outgoing rate) of our filtering logics by making our rate limiter implementation less accurate; 
e.g., introducing intentional random noise in the hierarchical token bucket (HTB) implementation. 
%Our HTB design already has token re-distribution logic for the work-conserving operations of large numbers of token buckets in the filtering system and we make it intentionally less accurate.
The details of this design choice is found in Section~\ref{sec:impl}.








==> paper 2/chapters/privacy.tex <==
\subsection{Privacy Guarantees}
% \subsection{Upper-bound on Privacy}
\label{subsec:algo-fair-privacy}
From our previous discussion in Section~\ref{subsec:metrics-tradeoff}, it is clear
that achieving ideal fairness and privacy goals simultaneously is an elusive goal. 
Instead, we aim to guarantee a user-controlled privacy level (e.g., anonymity
set size) at the cost of reduced fairness. 


%\input{chapters/algo-example-fig}

Let us first evaluate the privacy property of our policy composition $\phi$ 
in Algorithm~\ref{algo:fair-comp} that guarantees the maximum fairness
in a deterministic way. 
In this algorithm, we make a deterministic choice of performing bubble-sort swaps;
i.e., we pick the swap location based on left-to-right sequence of the target that we cant to reach.
Thus, if we want to find midpoint of $P_S=(2, 3, 4, 1)$ and $P_D=(3, 2, 1, 4)$ which are
at a distance of $2$, the algorithm would always chose $P_{S,D}=(3, 2, 4, 1)$.  Note that there is
another choice $(2, 3, 1, 4)$, which is also at a distance of $1$ from the two inputs; 
however, this alternative middle point is not selected by our deterministic algorithm.
%This means that $(3, 2, 1, 4)$ 
This deterministic operation does not utilize all the alternate middle points as the composite policy and thus limits the policy anonymity set significantly.

% because starting from $(2, 3, 4, 1)$, it is the
%one which does the swap on a left pair. Now, in an attack scenario for this
%example. the attacker knows the start point $(2, 3, 4, 1)$ and the middle
%point $(3, 2, 4, 1)$. Using this, he can calculate that the midpoint is at a
%distance $1$ which implies that the other input policy must be at a distance
%$1$ from $(3, 2, 4, 1)$. Now, the attackers job is trivial, because there are
%only two candidate $(3, 4, 2, 1)$ and $3, 2, 1, 4$ which are left-order swaps
%of distance one. Thus, the attackers anonymity set is only $2$ as compared to
%$24$ in the ideal case.

\paragraph{Randomized Composition.}
%We observe that because of our deterministic algorithm, we hit the lower bound
%of anonymity set which fits the attacker's observation. Which implies that our
%algorithm achieves least possible privacy. The next obvious question is, can
%we do better? 
Let us improve our policy composition algorithm to utilize all available potential
composite policies given two input policies. 
Let us consider the sequence of policies that is formed by
swapping adjacent elements as a path between two polices. Then, given any $P_S$ and $P_D$, there can be multiple different paths which are of the same distance.
Each of these paths may have different mid-points
which represents different composite policies which satisfy our goal of
equidistance. 
To exploit all possible paths, we randomly chose one of the positions to perform the swap instead
of the deterministic left-to-right order.

\input{chapters/random-algorithm}

Algorithm~\ref{algo:rand-fair-comp} adds random swapping operations to Algorithm~\ref{algo:fair-comp} (line 7).
In particular, the algorithm randomly chooses one of the positions to perform the swap instead of the deterministic left-to-right order and thus it can select any of the possible fair composite policies. 
For example, $P_S=(1, 2, 3, 4)$ and $P_D=(3, 2, 1, 4)$ have two
different paths of distance 3. Our randomized algorithm can choose one of the
potential midpoints $(3, 1, 2, 4)$, $(1, 3, 2, 4)$,  $(2, 1, 3, 4)$, or $(2, 3, 1, 4)$.

\paragraph{Policy anonymity set.}
As we defined in the early this section, $\mathcal{P}_D(\phi)$ and $\mathcal{P}_S(\phi)$ are the anonymity sets for $P_D$ and $P_S$, respectively. 
Let us describe how we can calculate $\mathcal{P}_D(\phi)$ for given $P_S$ and $P_{S,D}$ when the above randomized algorithm is used.

Given one end point (i.e., $P_S$) and a middle point (i.e., $P_{S,D}$) in the policy space and their distance is $d_1 = d(P_S, P_{S,D})$, we want to find all possible points in the space that satisfy the two conditions: $d(P_D, P_{S,D}) = d_2$ and $d(P_S, P_D) = d_1 + d_2$, where $d_2 \in \{{d_1-1, d_1, d_1+1}\}$.
For example, when we have two input policies $P_S=(1, 2, 3, 4)$ and $P_D=(3, 2, 1, 4)$ (as in the previous example), if $P_{S,D}=(3, 1, 2, 4)$ is chosen, $S$ finds that there exist six potential $P_D$'s that would result in the same $P_{S,D}$: $(3,2,1,4)$, $(3,1,4,2)$, $(3,2,4,1)$, $(3,4,1,2)$, $(3,4,2,1)$, and $(4,3,1,2)$.
Thus, with the given composite policy, 25\% (6 out of 24) of all possible policies are in the anonymity set for the given $P_{S,D}$. 

\paragraph{Guaranteeing an anonymity set size.}
In our policy composition function $\phi$, ISPs can easily negotiate with the desired level of privacy.
We use the anonymity set size as the metric for the privacy-preserving property of $\phi$. 
ISPs $S$ and $D$ can agree on a minimum anonymity set size and $\phi$ enforces it while composing the two input policies from them. 
To guarantee the minimum anonymity set size, $\phi$ may need to execute Algorithm~\ref{algo:rand-fair-comp} multiple times with a relaxed distance constraint in line 2. 
First, $\phi$ executes the unmodified Algorithm~\ref{algo:rand-fair-comp} and then evaluates the anonymity set size of the chosen composite policy $P_{S,D}$. 
If the anonymity set size is smaller than the minimum desired set size, it re-runs the algorithm with a reduced fairness by adding one more distance to the value $dist$ in Algorithm~\ref{algo:rand-fair-comp}. 
Then, $\phi$ repeats this until it finds a composite policy $P_{S,D}$ that has large enough anonymity set.


% In that case, the attacker neither
%knows which path was taken to reach the mid-point nor can it be certain which
%path to chose to move from the mid-point towards the end-point policy.

%For better understanding let us use vertices to denote the simple policy in
%$n$-element permutation and edges to connect each pair of polices that have
%the Kendall tau distance of 1, we can construct a three-dimension polyhedron.
%For example, Figure~\ref{fig:order_4_p_hedron} shows the polyhedron for
%policies of order 4~\footnote{Such a polyhedron is also refereed to as a
%permutohedron or bubble-sort graph}. With the help of this polyhedron of order
%4, the number of paths between any two simple polices can be visualized and
%counted easily. For example, $(1, 2, 3, 4)$ and $(3, 2, 1, 4)$ have two
%different paths of distance 3. Our randomized algorithm can either chose the
%midpoint $(3, 1, 2, 4)$ on one of the paths $(1, 2, 3, 4), (1, 3, 2, 4), (3,
%1, 2, 4), (3, 2, 1, 4)$. Or it can chose $((2, 1, 3, 4))$ which is the mid-
%point on the other path $(1, 2, 3, 4), (2, 1, 3, 4), (2, 3, 1, 4), (3, 2, 1,
%4)$. In fact, if we randomize the choice or using the ceiling or the floor for
%finding the mid-point, we can add more uncertainty to the attackers choices.
%Algorithm~\ref{algo:rand-fair-comp} shows our randomized version of the policy
%composition algorithm.



% \paragraph{Examples.}
% \begin{itemize}
% 	\item {\bf $d = 2$.}
% 	$\phi ((2, 3, 4, 1) (3, 2, 1, 4)) = (3, 2, 4, 1)$ \\
% 	$\mathcal{F}(\phi) = $ \\
% 	$\mathcal{P}(\phi) = 2$ ; $\{(3, 2, 4, 1), (2, 3, 1, 4)\}$
% 	\item {\bf $d = 3$.}
% 	$\phi ((1, 3, 2, 4), (2, 1, 3, 4)) = (1, 2, 3, 4)$ \\
% 	$\mathcal{F}(\phi) = $ \\
% 	$\mathcal{P}(\phi) = 3$ ; $\{(2,1,3,4), (2,1,4,3), (1,2,4,3)\}$
% 	\item {\bf $d = 4$.}
% 	$\phi ((1, 4, 3, 2) (3, 2, 1, 4)) = (3, 1, 4, 2)$ \\
% 	$\mathcal{F}(\phi) = $ \\
% \end{itemize}

==> paper 2/chapters/problem.tex <==
\section{Applicability of \name}
\label{sec:overview}

\subsection{Overview of \name}
\label{sec:collaborative-filtering-problem}
%\paragraph{Source-end filtering for DDoS mitigation.}
We design our mutual collaboration as a {\em mutual protocol} between two distinct networks: a {\em
source} AS $S$, which hosts potential attack sources (e.g., botnets) in its and its customers' networks, and a {\em destination} AS $D$, which experiences congestion. 
Note that the two ASes may be indirectly connected through one or more transit ASes. 
%In this paper, we focus on a simple bilateral protocol as the fundamental building block for extended collaborative mitigation models, such as multi-party peer-to-peer collaborations or centralized collaboration models; see Section~\ref{} for detailed discussion. 
%
We consider that $D$ first initiates a collaborative filtering {\em session} with $S$. 
We assume that $D$ has already identified the AS $S$ that sends high volume traffic, via coarse-grained traffic analysis tools, such as NetFlow~\cite{netflow} or sFlow~\cite{}. 
Note that $D$ may create more than one session with multiple source ASes (e.g., $S_1,S_2,\cdots$) but the sessions with different source ASes are independently established and operated.
We observe that the number of such parallel filtering sessions would be small and thus manageable (e.g., 10 -- 20 or less) due to the highly unbalanced attack source (e.g., botnets) distribution in most practical attacks; see Section~\ref{} for detailed analysis. 

%The source AS $S$ filters out a subset of packets that are generated by its customers and {\em destined} to the destination AS $D$. 

%\paragraph{Fairness in collaboration.}
%We envision packet filtering operation that is based on the {\em mutual collaboration} between two ASes, {\em not} a mere network function {\em outsourcing}~\cite{liu2008filter,alwabel2015senss}. 
In \name, {\em both} $S$ and $D$ submit their filtering policies: the \textit{source policy} $P_S$ and the \textit{destination policy} $P_D$. 
Collaborative filtering requires these two independently-generated policies $P_S$ and $P_D$ to be {\em fairly} respected in actual packet filtering operations, benefiting both two collaborating parties.
%Since the two policies are generated without coordination, there may be some conflicting filtering rules, such as, $D$ wishes to drop a certain traffic flow whereas $S$ hopes to protect the same flow.
%Such conflicting rules must be reconciled in a fair manner so that neither parties are favored over the other in the packet filtering operation. 

\subsection{Frequently Asked Questions about \name}
Before describing the details of our system design and security properties, we discuss under what conditions and to what extent \name is useful for DDoS mitigations.
We start by informally addressing four commonly asked questions and then characterize our threat model and describe how to achieve the necessary security properties.

\smallskip
\noindent{\bf Q1: }{\em How is it fundamentally different from existing filtering outsourcing proposals? And why is \name is more attractive to source ASes?} 
Unlike outsourced filtering, \name ``requires'' the source AS to submit its filtering policy. 
That is, a source AS is supposed to actively participate in the packet filtering decision, which is not allowed in any existing solutions. 

This additional functionality offers great incentives to the source ASes. 
Let us imagine that a destination AS $D$ simply outsources filtering operations to a source AS $S$.
For $S$, either acceptance (i.e., implementing $D$'s filtering policy) or rejection (i.e., letting $D$ to filter packets) of the outsourced filtering request implies that it lets the destination AS $D$ to have the full control to decide which packet should be allowed or dropped when under DDoS attacks.  
%As an alternative, $S$ may accept the request but overwrite the requested policy with its own policy; however, this only creates the problem of lack of trust between the two ASes and eventually break the inter-domain session. 
Unlike outsource filtering, \name's collaboration request from $D$ is a strictly better option for $S$ to express its own policy (e.g., protecting or deprioritizing flows) when some portion of its traffic have to be dropped due to DDoS incidents. 


\smallskip
\noindent{\bf Q2: }{\em Isn't that both ASes can already perform own filtering without \name by dropping arbitrary packets in their networks?}
Although any AS on the route from $S$ to $D$ can drop any packets based on their own preference, such arbitrary packet drops cannot serve as a reliable policy enforcement for two reasons. 
First, such arbitrary packet drops (without clear evidence of congestion in their own networks) are observed as the violation of service level agreement (SLA) or net neutrality to the customers. 
Second, dropping certain packets does not guarantee the protection of other packets. 
For example, a source AS $S$ may drop flow $x$ in the hope that its another flow $y$ be better treated in the congested destination network.
However, the destination $D$ will not necessarily respect the $S$'s inexplicit policy because flow $x$ and flow $y$ are independent to $D$.\footnote{Unless $D$ implements strict per source AS fairness bandwidth policy, which is uncommon.} 


\smallskip
\noindent{\bf Q3: }{\em What if attack packets have source IPs spoofed to be the source AS $S$'s addresses? Can such attacks be detected?}
\name is not designed to prevent IP spoofing DoS attacks.
Unfortunately, 20-30 \% of ASes are still without proper ingress filtering thus IP spoofing DoS attacks are easy to launch~\cite{}.
However, \name instead is designed to detect IP-spoofing DoS attacks effectively. 
When a destination AS $D$ first establishes a collaborative filtering session with a source AS $S$, they set a point-to-point tunnel (e.g., a GRE tunnel) between them (e.g., between their edge routers) to encapsulate all the packets from $S$ to $D$. 
This simple inter-domain encapsulation allows the destination AS $D$ to detect IP-spoofing DoS attacks effectively; see Section~\ref{sec:bypass}.

\smallskip
\noindent{\bf Q4: }{\em \name claims to effectively detect misbehaviors (e.g., bypassing the \name filtering), but what can one do when a misbehavior of the other party is detected?} 
In \name, two ASes create temporary contract only between them. 
Therefore, any one of them can abort the temporary contract whenever one party detects misbehaviors. 
For example, if a destination AS $D$ detects the misbehavior of a source AS $S$, $D$ can quickly abort the collaborative filtering and start deprioritizing traffic from $S$ as a penalty to the misbehavior.


%\noindent{\bf Q4: }{\em Despite all the merits of mutual collaboration, what if small (e.g., tier-3) ASes may not be able to afford additional operational costs of \name?} 
%First of all, \name is designed to be low-cost and easily incorporated into exiting private computing cluster with commodity platform.
%In case \name is still not affordable to the direct source AS, its upstream AS (e.g., tier-2) may run \name on behalf of the direct source AS; see a detailed discussion in Section~\ref{}.

\section{Threat Model and Desired Security Properties}
\label{sec:prob}

\subsection{Adversary model}
\label{sec:threat-model}
%Collaboration between two ASes is hard because the ASes in practice tend to be {\em mutually untrusted}.
We consider that two ASes are {\em mutually untrusted}. 
This is realistic because the source and destination ASes seldom have any bilateral contract between them especially when they are remote ASes to each other often in different geopolitical regions with no direct business relationship.

The untrusted two ASes may aim to achieve three main attack goals.
First, ASes want to {\em tamper} with the policy composition logic of the \name system to affect the final composed policy and overwrite it with their own preferred policy.
Second, ASes also may want to {\em bypass} the \name's filtering logic outside of the \name system to ignore the per-packet decision made by \name.
Third, ASes may want to {\em learn} the other's policy. The inferred policy can be used for one's own benefit or can be leaked to other interested parties (e.g., a competitor of the policy owner).

Note that $S$ has more attack capabilities than $D$ in general since it is the operator that executes and manages the \name system in its own network infrastructure. 
Particularly, we consider that $S$ can control the software components of \name and even the privileged software (e.g., operating system) of the system. 
Moreover, $S$ has the full control (e.g., read, inject, drop) over all the packets entering/leaving \name. 
On the contrary, the destination $D$ can observe only the packets leaving the \name system. 

\paragraph{Scope.}
We consider that other malicious attack sources may generate {\em IP-spoofed} DDoS traffic with the source IPs under the control of a source AS. 
The proposed \name system handles such IP-spoofed attack traffic by simply distinguishing packets with spoofed source IPs and the ones that actually come from the designated source AS. 

During the lifetime of a session for mutual collaboration between two ASes $S$ and $D$, we consider that $D$'s filtering policy may change dynamically to adapt to the incoming DDoS attack traffic and the availability of its network and customers. 
Yet, we assume a {\em static} policy submission of the source AS $S$ as its filtering policy is not DDoS attack specific but more related to its own policy regarding its customers; e.g., which customer must have higher access priority when the available bandwidth is limited. 



\subsection{TEE based \name Design}
\label{sec:name-overview}

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.48\textwidth,height=0.5\textheight,keepaspectratio]{figures/design.pdf}
	\caption{A high-level view of a \name instance $F(S,D)$ between two ASes $S$ and $D$.}
	\label{fig:design}
\end{figure}

To protect \codename from the direct access of the source AS $S$, we utilize the hardware-based trusted execution environments (TEEs) in \name's design, as shown in Figure~\ref{fig:design}. 
With the TEE protection, \codename can isolate its packet filtering executions from its malicious operator under $S$'s control and prevents it from tampering with the packet filtering (e.g., accessing/altering filtering policies or packet allow/block decisions).
Moreover, the TEE-based design allows the two ASes $S$ and $D$ to individually verify the
correct implementation of the negotiated packet filtering operations before and while they perform collaborative filtering.
In this work, we implement \name using a recent trusted computing capability called Intel SGX~\cite{}. 

We envision a software virtualization technique to create scalable \name instances on-demand based on the required filtering capability and the volume of traffic from $S$ to $D$. 
\name is a low-cost, highly efficient virtual function that runs on commodity computing clusters.
\name is installed inside the source $S$'s private cluster with commodity servers.
The source AS $S$ redirects packets from $S$ to $D$ to the \name functions when the collaborative packet filtering is activated via SDN's dynamic rerouting capability.



As shown in Figure~\ref{fig:design}, the \name instance $F(S,D)$ between $S$ and $D$ accepts the desired received rate $L$ bps from $D$. 
%$M(S,D)$ also receives the two policies $P_S$ and $P_D$ from the two ASes to make fair packet-drop decisions in its packet filtering logic. 
\name is composed of the control- and data-plane
components: a policy composition $\phi(\cdot)$ and a
policy enforcement $\psi(\cdot)$, respectively.  
The {\em policy composition} $\phi$ reconciles the two independent filtering policies $P_S$ and $P_D$ and creates a {\em composite policy} $P_{S,D}$.
The composite policy $P_{S,D}$ is then passed to the data plane function 
$\psi(\cdot)$ that performs packet filtering based on the given composite policy and the desired rate $L$ bps. 
The {\em policy enforcement} $\psi(\cdot)$ is designed to be a generic packet filtering engine that implements various types of filtering policies $P_{S,D}$ .
To that end, we consider a traffic classifier categorizes incoming packets based on the traffic classifications (i.e., groups of packets from $S$ to $D$ that share the same priority rules) of the given policy $P_{S,D}$, followed by a large array of rate limiters (e.g., token bucket) that enforce rate reduction for each traffic class independently. 
The policy enforcement $\psi$ may also log some packet processing results for audits.





\subsection{Design Problems}
As described in Introduction, we have three security goals against the threat model: (1) verifiably fair policy composition and enforcement; (2) negotiable maximum policy leakage; and (3) effective bypass detection. 
In principle, the TEE-based design of \name guarantees the execution integrity and verifiability of the control-plane and data-plane operations of \name. 
This strong guarantee is the baseline security primitive for the three security goals of \name but it is unfortunately insufficient. 
\begin{itemize}
	\item First, TEE protects the composition logic and the enforcement of the composed policy from malicious system operator (e.g., source AS $S$) and makes them verifiable. 
	However, the notion of fairness and the algorithmic model for fair composition for various policy definitions must be defined and developed first (see Section~\ref{sec:policy}). 
	\item Second, TEE protects a privacy negotiation process between two ASes and guarantees their agreed privacy mechanisms. 
	However, due to the undesirable, inherent tradeoff between privacy and fairness, it is tricky to find a right balance between the fairness and privacy. 
%	For the worst case scenario analysis, we also need to understand the strongest privacy attack strategies (e.g., learning the other's policy within a few minutes) and demonstrate the attacks.
	Moreover, we need to build a framework that suggest an adequate level of privacy (e.g., anonymity set size) for given policies and fairness target (see Section~\ref{sec:attacks}). 
	\item Third, TEE enables per-packet validation between untrusted $S$ and $D$, which makes fine-granular bypass detection achievable. 
	However, per-packet validation incurs significant performance overhead due to excessive context switching and thus make line-rate operation difficult (see Section~\ref{sec:bypass}).
\end{itemize}

%Moreover, the fairness property must be defined and chosen in conjunction with their privacy property


%enables the verification in two levels but not trivial what to verify in control plane ... and how to verify in data plane ... without affecting the line-rate packet processing. 

%\begin{itemize}
%	\item {\bf Lack of privacy property.} Although ASes cannot directly read the submitted policies or the composed policy due to the TEE's memory confidentiality, they can still learn some of the sensitive policies by monitoring and/or testing the middlebox's external behaviors. 
%	For example, consider a middlebox that implements a simple rule that drops a certain type of packets.
%	By sending one or more probe packets of the same type and observing the packet-drop decisions, $S$ can easily infer whether this packet type is filtered or not.
%	Once ASes learn the composed policy $P_{S,D}$, they may then attempt to infer the other AS's policy; see Section~\ref{sec:attacks} for detailed attack descriptions.
%	\item {\bf Lack of non-bypassability property.} 
%	The source AS installs and operates the \name middlebox and thus it is easy for $S$ to bypass the middlebox when it wishes to overwrite the filtering decision made by the middlebox. 
%	For example, if $S$ learns that a packet $p$ is allowed by the middlebox, which is against its will, it may want to drop $p$ before (or even after) the middlebox processes it. 
%	Conversely, $S$ can easily force to send the packet $p$ by bypassing the middlebox when the middlebox decides to drop $p$. 
%	Note that the \name middlebox cannot  prevent such bypasses since it has no control over the network operation of the source AS $S$. 
%\end{itemize}
%
%\subsection{Our Contributions}
%Acknowledging the non-trivial challenges of the two security properties, in this paper, we aim to shed light on the {\em security upper-bounds} of the privacy and non-bypassability properties.
%
%\paragraph{Privacy guarantees.}
%First, we analyze the effectiveness of a family of privacy attacks for inferring the composed policy $P_{S,D}$ of the middlebox and subsequently the other AS's internal policy (Section~\ref{sec:attacks}).
%In the inference attack on $P_{S,D}$, we focus on how effectively and efficiently the ASes can exploit the data-plane side channels (i.e., packet filtering decisions observed via monitoring data-plane packets of the middlebox) and infer $P_{S,D}$. 
%In the subsequent inference attack on $P_D$ by $S$ (or $P_S$ by $D$), we analyze the maximum privacy guarantees (e.g., anonymity set) for the AS's internal policies for various policy definitions (e.g., how to express the preferences in the filtering policy) and fairness notions (e.g., how to define and measure fairness of the composed policy).
%Analysis on these policy inference attacks offers us the necessary insights regarding the privacy bounds of the collaborative packet filtering mechanism in a generic setting and suggestions for the choice of policy expressiveness, preference design, and fairness guarantees for the desired degree of policy privacy. 
%
%\paragraph{Non-bypassability guarantees.}
%Second, we propose a lightweight bypass detection mechanism between the middelbox and the destination AS $D$ (Section~\ref{}).
%We then analyze the upper-bound of non-bypassability guarantees by measuring the effectiveness of the bypass detection by the two participating ASes. 
%We analyze the trade-off between the detection accuracy and the performance (e.g., real-time computation/memory overhead) of the detection mechanism and evaluate the attack effectiveness (e.g., number of packets bypassable without being detected).
%
%\paragraph{SGX-based middlebox implementation.}
%Third, we also design and build a prototype of the proposed \name middlebox that supports multi-gigabit bandwidth (e.g., 10 Gbps or higher) throughput on a commodity server platform with the Intel SGX-enabled CPUs (Section~\ref{sec:impl}).
%We particularly address several non-trivial system optimization issues, including SGX integration with heavy data-plane operation. 



==> paper 2/chapters/random-algorithm.tex <==
\alglanguage{pseudocode}
\begin{algorithm}
\caption{Randomization to find the midpoint of $P_S$ \& $P_D$}
\label{algo:rand-fair-comp}
\begin{algorithmic}[1]
\scriptsize
\Procedure {FairComposition}{$P_S(s_1 .. s_n)$, $P_D(d_1 .. d_n)$} 
\State $dist \gets RAND(\lfloor d(P_S, P_{D}) / 2 \rfloor, \lceil d(P_S, P_{D}) / 2 \rceil)$
\State $P_{SD} \gets P_D$
\For{$i \leftarrow 1, n-1$}
    \For{$j \leftarrow 1, n - i$}
        \If{$s_m > s_n$ where $s_m = d_j, s_n = d_{j+1}$}
            \State {SWAP} RAND({$d_j, d_{j+1}$})
            \State $dist \gets dist - 1$
            \If{$dist = 0$}
                \State $P_{SD} \gets P_D$
            \EndIf
        \EndIf
    \EndFor
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> paper 2/chapters/recon-algo.tex <==
\subsection{Fair Reconciliation Algorithm}
\label{subsec:algo}

Given our definitions of fairness and privacy, the goal of an ideal $\phi$
function is to generate a composite policy $P_{S,D}$ which is ideally fair as
well as ideally private w.r.t. input policies $P_S$ and $P_D$. 
%Understanding
%the asymmetric nature of the trade-off, that is, strong privacy hurts fairness
%more than strong fairness does to privacy, we design the algorithm centered
%around the fairness and enforce privacy as constraints of the problem. 
We start with an algorithm which maximizes fairness and then try to maximize
the corresponding privacy that we can achieve for it. A fair policy
composition function $\phi$ always finds a policy has following properties:

\begin{itemize}
\item{\bf Equal distant.} 
The composite policy must be at an equal distance from both input policies. For
example, consider the input policies $P_S=(1, 4, 3, 2)$  and $P_D=(3, 1, 4, 2)$.
Then $P_{S,D}=(4, 3, 1, 2)$ is a fair composite policy as it is at a distance of $2$ from both the input policies.
Often, a fair policy is not unique; e.g., $P_{S,D}=(1, 3, 4, 2)$ is also a fair composite policy since it has equal distance of 1 from both inputs. 
\item{\bf Least distant.}
The composite policy is at a minimum distance from both input policies. 
In the above example, we
prefer $P_{S,D}=(1, 3, 4, 2)$ because it has least distance from the inputs.
\end{itemize}

\paragraph{Search Algorithm for Least-distant \& Equidistant Policy.}
When we use the Kendall tau distance function, the fair composite policy is 
at a distance of $d/2$ from the two input policies\footnote{If $d$ is an odd number, 
the composite policy is $\lfloor{d/2}\rfloor$ away from one input and $\lceil{d/2}\rceil$ 
from the other input.}, where $d = d(P_S,P_D)$ denotes the 
distance between the two input policies. 
Note that this simple algorithm guarantees the equal and the least distant properties
because the Kendall tau metric satisfies the triangle inequality; that is, $d(x,z)\le d(x,y) + d(y,z)$, when $x$, $y$, and $z$ are the filtering policies.

In our algorithm, we start from one of
the input policy and keep making $d$ ranking swaps (e.g., from $(1,2)$ to $(2,1)$) until 
we reach the other input policy. For example, consider that we have two policies $P_S=(1, 4, 3, 2)$ and
$P_D=(3, 2, 1, 4)$ which are at a distance of $4$. We can start from $(1, 4, 3, 2)$
and traverse the path by using a bubble-sort style swapping from left-to-right:
$(1, 4, 3, 2) \rightarrow (1, 3, 4, 2) \rightarrow (3, 1, 4, 2) \rightarrow (3,
1, 2, 4) \rightarrow (3, 2, 1, 4)$. Since our ideal policy is at a
distance of $d/2$ on this path, we can easily determine $P_{S,D}=(3, 1, 4, 2)$.

\input{chapters/algorithm}

Algorithm~\ref{algo:fair-comp} is a deterministic process that implements the
logic we described above. First, we assign the floored half of the Kendall tau distance
between $P_S$ and $P_D$ as the midpoint $dist=\lfloor d(P_S, P_{D}) / 2 \rfloor$ 
(line 2) which is our search target. Next, we assume $P_S$ as a start
point and start bubble-sorting swaps towards
$P_{D}$ (line 6-7). For
every swap of the adjacent elements in $P_{S, D}$, we decrement $dist$ by
$1$ (line 8). We stop the process, when we have done $\lfloor d(P_S, P_{D}) / 2 \rfloor$, 
where we fine the fair policy point $P_{S,D}$.

==> paper 2/chapters/refutable-invoice.tex <==
%\subsection{Inflation Resistant Refutable Invoicing}
%\label{sec:refutable-invoice}

Refutable invoice is important for the payment systems. 
Intuitively, the work of a filter can be measured by the amount of traffic that has been filtered out for a duration of time. 
As Sekar and Maniatis argue in~\cite{ccsw11}, a verifiable source accounting system should verify not only the accurate amount of consumed resources but also their {\em necessity}. 
In our traffic filter application, however, it is hard to prove the necessity of filtered traffic because a malicious source network can always create unnecessary dummy packets that are indistinguishable from other packets to inflate the bandwidth usage and the invoice. 

\begin{table}[h]
\begin{threeparttable}
	\centering
	\caption{Memory footprint examples of four filter rule sets with two different rule set sizes and two types of rule distributions: concentrated (i.e., rules are adjacent) and dispersed (i.e., rules are widely separated).}
	\label{tbl:mem-footprint}
	\begin{tabular}{c c c}
		\toprule
		&\multicolumn{2}{c}{\textbf{Rule distributions}}\\
		\textbf{Number of rules}  & {concentrated} & {dispersed} \\
		\midrule
		% \hline
		%    300 & 50,432 B & 169,088 B \\
		300 & 50 KByte & 169 KByte \\
		% \hline
		%    3000 & 440,016 B & 1,632,816 B \\
		3,000 & 440 KByte & 1,633* KByte \\
		\bottomrule
	\end{tabular}
	\begin{tablenotes}
		\small
		\item * This only reflects the size of the runtime lookup table, and does not include the huge memory consumption (over 48 MB for 3000 rules) during the building phase of the lookup table.
	\end{tablenotes}
\end{threeparttable}
\end{table}
Instead, we propose a new metric as a proxy for the executed work of the \name filters. 
Our new invoice metric is composed of two values that are resistant to bandwidth inflation.
First, we use the {\em memory footprint} of filtering rules of the filtering task. 
The memory footprint is a proxy for the average lookup cost for each packet filtering operation. 
As we see in Table~\ref{tbl:mem-footprint}, different filtering policies with the same number of rules may have significantly different memory footprints (e.g., 3--4 times difference). 
Second, we also use the {\em expected bandwidth} that will be filtered by the installed rules that are {\em negotiated} during the initial negotiation between the two ISPs (see Step 1 in Figure~\ref{fig:overview}). 
Once the two values are measured, they are written in the contract, which is signed by the two ISPs and the \name enclave. 
Then the final metric for the executed work is the multiplication of the two values and the time duration of the filtering round; that is,
\begin{align}
\text{ExecutedWork} = ~&\text{FilterRuleMemFootprint}~\times\nonumber\\ 
&\text{EstimatedFilteredBandwidth} ~\times\nonumber\\ 
&\text{DurationOfFiltering}
\end{align}



==> paper 2/chapters/related.tex <==
\vspace{-5pt}
\section{Related Work}
%\vspace{-5pt}
\label{sec:rw}

Network DDoS attacks and defenses have been extensively studied in the last 2--3 decades~\cite{mirkovic2004taxonomy}. 
Here, we summarize a few categories of DDoS defenses and related projects.

\vspace{-5pt}
\subsection{In-network Filtering}

The idea in-network filtering has been the core idea of many DDoS mitigation proposals.  
There are two prominent approaches to implementation: dynamic filtering and capability-based approaches.
Dynamic filtering suggests that the destination ISP requests the ISPs on the forwarding paths to install filter rules at the time of attack, for instance as proposed in
Pushback~\cite{mahajan2002controlling}, D-WARD~\cite{mirkovic2002attacking}, AITF~\cite{argyraki2005active}, StopIt~\cite{liu2008filter}.
Capability-based approaches embed capabilities in the packet flows, which can be controlled by the destination hosts to authorize flows in upstream, as proposed in SIFF~\cite{yaar2004siff}, TVA~\cite{yang2005limiting}, and Portcullis~\cite{parno2007portcullis}. 

Closest to our work is the recent SENSS defense architecture by Ramanathan et al.~\cite{ramanathan2018senss}.  
SENSS proposes to install DDoS-victim submitted filters at a small number of major ISPs. 
Ramanathan et al. show that in-network filtering at only four major ISPs in the US would have stopped the Dyn attack happened in 2016~\cite{york2016dyn}.
SENSS also suggests an automated payment channel between a DDoS victim and a filtering ISP so that the ISP can get compensation for the extra filtering tasks. 
Although the idea is solid and evaluation is promising, the SENSS proposal lacks the filtering verifiability and thus allows several undetectable misbehaviors of the filtering ISPs.\footnote{Ramanathan et al.~\cite{ramanathan2018senss} sketch a reputation-based mitigation, which can be used together with our \name proposal.}

%\vspace{-5pt}
% In the earlier Section~\ref{sec:case-for-source-filtering}, we review the families of DDoS defense proposals, focusing on in-network filtering mechanisms. 
% Please refer to that section for general discussions.

% \paragraph{Inter-domain protocols for in-network filtering.}
% Particularly, in the past few years, there have been several proposals to design inter-domain protocols that establish filtering contracts between a DDoS victim and a network in the upstream paths.
% SENSS~\cite{alwabel2015senss} proposes a generic inter-domain protocol to install filters in any willing ISPs on the Internet, enabling early attack identification and mitigation.
% Huawei envisions a global association of trusted ISPs that enable in-network filtering between the member ISPs; see Huawei's Cloud Clean Alliance project~\cite{huawei2015cca}.
% Team Cymru also proposes a similar idea called Unwanted Traffic Removal Service~\cite{cymru}.
% IETF's DDoS Open Threat Signaling (DOTS) working group~\cite{dots-slides} has been working on the standard channels for inter-domain filtering operations.
% More recently, one study utilizes the Ethereum's smart contracts for in-network filtering contract establishment between two ISPs~\cite{rodrigues2017blockchain}. 

Unlike previous in-line filtering proposals, our system \name focuses on the highly desired but yet-unaddressed security property for in-network filtering system, i.e., the verifiable filter, and demonstrates its feasibility and scalability.



%
%Several solutions and systems have been proposed in the last 15 years to realize the source-end mitigation for various DDoS attacks.
%Mirkovic et al. propose D-WARD, an automated system that detects flooding attacks via anomaly detection mechanisms and automatically installs filters at the source ISPs~\cite{mirkovic2002attacking}. 
%In D-WARD, the receiver has no control over the detection and filtering of flooding traffic.
%Moreover, D-WARD can be easily bypassed by attackers who can control their traffic to be within a normal range.
%Liu et al. propose StopIt, a hybrid source-end filtering system, that enables each destination host to install a network filter at the source host or source ISPs that blocks the undesirable traffic it receives~\cite{liu2008filter}. 
%In StopIt, destination hosts (or destination ISPs) can express their filtering policies but it has serious security and privacy concerns. 
%First, destination hosts or ISPs cannot check whether their policies are correctly applied and enforced by the source hosts (or source ISPs). 
%Moreover, destination policies are forced to be revealed to the source hosts or ISPs, thus offering no privacy for their internal proprietary policies. 
%More recently, Alwabel et al. present SENSS, a distributed filtering system that allows destinations express their policies in traffic filters distributed across many ASes in the Internet~\cite{alwabel2015senss}.
%SENSS allows not only the source ISPs but also any transit ISPs to install filters and offer outsourced traffic filtering services to the destination ISPs. 
%Although SENSS partially addresses incentive problems (e.g., lack of economic incentives for installing filters for others), it still shares the same security and privacy concerns of the previous solutions, such as StopIt.  
%
%Furthermore, all the existing source-end packet filtering schemes lack accountable packet filtering and thus when a packet is dropped by the source ISP, the corresponding source host cannot understand the cause of the packet drops. 
%\name is the first source-end packet filtering mechanism that offers security and privacy properties. 

\vspace{-5pt}
\subsection{Network Function Virtualization with Trusted Hardware}
%\vspace{-5pt}
% In the past few years, high-performance outsourced network functions have been proposed and demonstrated using the Intel SGX capability.
We categorize some of them:
\begin{packeditemize}
	\item {\bf Middleboxes:} Various network middleboxes have been tested with the SGX capability. 
	TLS middleboxes~\cite{naylor2017and,han2017sgx} demonstrate that an SGX-protected middlebox can handle thousands of TLS sessions without violating their end-to-end encryption. 
	ShieldBox~\cite{trach2018shieldbox} and Trusted Click~\cite{trusted-click} demonstrate that SGX can protect the Click modular router to implement various trusted network functions.  
	S-NFV~\cite{shih2016s} also discusses general policy, data privacy issues of network functions. 
	LightBox~\cite{lightbox} demonstrates the line-rate performance for simple secure packet processing functions. 
	Snort-SGX~\cite{kuvaiskii2018snort} also demonstrates line-rate performance of Snort 3 along with a DPDK network layer.
	SafeBricks~\cite{poddar2018safebricks} implements a highly modularized and safe network function architecture in the Intel SGX platform.
	
	Our main contribution is not merely an integration of a simple flow filter function and an SGX architecture but more on addressing scalability and filter-rule violations at network layer that are specific to verifiable in-network filtering defense systems. 
	
	\item {\bf Privacy-preserving systems:} 
	Several systems demonstrate that SGX-based network functions can improve the privacy of anonymity systems: SGX-protected Tor nodes~\cite{kim2017enhancing,shinde2017panoply},
% 	Also, an SGX-based cryptocurrency mixer has been proposed~\cite{tran2016obscuro}.
	\item {\bf Inter-domain routing:}  
	Also, several secure inter-domain routing applications have been proposed to exploit the security guarantees of Intel SGX~\cite{prixp,kim2015first}.
	\item {\bf Verifiable accounting:} 
	There also have been some prototype systems that enable the outsource network functions to securely measure the amount of resources used for the requested tasks (e.g., \cite{tople2018vericount} in an SGX platform, \cite{vee13} in a TPM platform).
\end{packeditemize}

With \name we investigate a unique design point of auditable traffic filters. 
Particularly, our contribution of \name is in the design of auditable filters that can handle ever-growing large-scale attack volume and complexity with the SGX support.
%
%SGX-Box~\cite{han2017sgx}
%
%Slick~\cite{trach2017slick}
%
%LightBox~\cite{duan2017lightbox}, 
%
%TruNet~\cite{zhang2011network} %, Assayer(?)
%
%Trusted Click: Overcoming security issues of NFV in the cloud~\cite{trusted-click}
%
%SGX Tor~\cite{kim17enhancing}, ~\cite{kim2015first}
%
%PrIXP~\cite{prixp}

\vspace{-5pt}
\subsection{Cloud-based DDoS Mitigations}
%\vspace{-5pt}


The predominant DDoS defense in practice today is an overlay-based filtering approach, such as cloud-based scrubbing services, that performs outsourced filtering in a third-party network on behalf of the DDoS victims (e.g., AWS-Shield~\cite{aws-shield}, Radware DefensePro~\cite{radware}).
Overlay-based filtering approaches are popular particularly because they require {\em no} changes to the current Internet
architecture. Recent works have proposed advances in such overlay
filtering using middleboxes~\cite{liu2016middlepolice,gilad2016cdn} and proposals
have discussed large-scale filtering locally at
ISPs~\cite{fayaz2015bohatei}.
However, end users are not satisfied with the status quo. Reports
suggest that relying on third-party providers centralizes the DDoS
marketplace~\cite{gilad2016cdn}; costs for small and medium-size victims
are high and services are left to the discretion of large service
providers~\cite{guardian2016ddos,gilad2016cdn}.


% Cloud-based DDoS scrubbing services or replication services are the most widely used DDoS defense solutions today. 
% Gilad {\em et al.} point out that the DDoS mitigation market is dominated by a small number of large cloud providers and thus they are prohibitively expensive for small websites and propose an affordable on-demand usage of cloud infrastructure for contents replication~\cite{gilad2016cdn}.
% MiddlePolice~\cite{liu2016middlepolice} addresses the lack of control over the filtering policy in the current cloud-based scrubbing services and enables DDoS victims to specify filter rules of their preference by installing and controlling middleboxes in the cloud infrastructures. 
% Bohatei~\cite{fayaz2015bohatei} handles large volumetric attacks (e.g., 500 Gb/s) by dynamically scaling out the available commodity server cluster in the local ISP networks. 

Unlike these proposals, \name does not rely on the cloud or the local victim network's capability but directly establishes filtering rules at the transit networks. 

%
%\subsection{End-to-end bandwidth guarantees}
%IntServ, DiffServ, 
%
%SIBRA~\cite{basescu2015sibra}



%\subsection{Privacy-preserving policy composition}
%
%\subsection{Privacy-preserving network function virtualization}
%
%\subsection{Smart Contracts and Blockchain... security work}
%
%potential in establishing de-centralized contracts for handling PKI
%certificate compromises have been
%discussed~\cite{matsumoto2017ikp}. 


==> paper 2/chapters/scalable-filter-design.tex <==
\section{Scalable Filter Design}
\label{sec:scalable-filter-design}

% Scalable enclaved-filter design, though highly desired, is not straightforward because the parallelization of the individually trusted filters necessarily involves an {\em untrusted} facilitating component (e.g., high-bandwidth switching fabric), which can be potentially exploited by a malicious \name IXP for the filter-rule violations.

In this section, we first analyze the performance (e.g., throughput, network I/O) bottlenecks of a single auditable filter (\S\ref{sec:bottleneck-rule}) and then describe a scalable filtering design with multiple enclaved filters running in parallel and an untrusted load balancer (\S\ref{sec:optimization-multiple-enclaves}).

% We first 
%present our data-plane optimization for a single filter enclave (\S\ref{sec:optimization-for-single-enclave}). 
%Then, we 
% analyze the bottlenecks of scaling out the enclaved filters (\S\ref{sec:bottleneck-rule}), and provide dynamic algorithms for scalable, trusted filter design with untrusted network components (\S\ref{sec:optimization-multiple-enclaves}). 
% In this section, we focus on the algorithmic complexity of scalable filter design.
%Readers are encouraged to refer to Appendix~\ref{sec:attestation-multiple-enclaves} for practical attestation mechanisms for multiple enclaved filters.
%\msk{Why is it challenging? Because of untrusted LB!}

%\subsubsection{Data-Plane Optimization for a {\em Single} Enclave}
%\label{sec:optimization-for-single-enclave}
%
%\begin{figure}[t!]
%	\centering
%	\includegraphics[width=0.43\textwidth]{figures/near-zero-copy.pdf}
%	\caption{Two packet copy approaches for SGX-based accountable filter and packet logging functions. In the near zero-copy approach, we copy only the memory reference ($\ast$), the five tuple ($5T$), and the size ($s$) of the packet into the enclave.}
%	\label{fig:near-zero-copy}
%\end{figure}
%For every incoming data-plane packet, a \name filter logs the packet, filters it based on the given policy rule set, and logs it again if it is allowed by the filter, as shown in Figure~\ref{fig:near-zero-copy}.
%Figure~\ref{fig:near-zero-copy}(a) shows a naive approach, where a \name filter makes the entire copy of incoming packets into the enclave and operate these functions over the packet copies inside the enclave.
%%
%This {\em full-packet copy} based processing, however, incurs too much overhead (e.g., too frequent context switching). % for making full packet copies of all the data-plane packets. 
%Our evaluation (\S\ref{sec:eval}) confirms the poor performance of the per-packet processing approach.
%
%
%
%\paragraph{Near zero-copy design.}
%Instead, we take a {\em near zero-copy} approach, where only a fraction of its header fields (i.e., the five tuple fields, $5T$, and the packet size, $s$) are copied into the enclave memory along with the memory reference ($\ast$) of the packet, as shown in Figure~\ref{fig:near-zero-copy}(b).
%The copied data $\langle 5T,s \rangle$ represents the packet and is used for the logging functions and the filter. 
%The memory reference $\ast$ is used to perform the corresponding operation (e.g., forward or block) for the packet in the untrusted memory pool.
%
%With the copied five tuple and the size, we first log each packet using a count-min sketch~\cite{cormode2005improved} for memory efficient per-source-IP counters. 
%The per-source-IP sketch for the incoming packets enables each source host to detect the `drop before filtering' bypass attack discussed in Section~\ref{sec:bypass-attacks}.
%For forwarded packets, we also record another count min sketch based on the full 5-tuple bits so that the DDoS victim to detect bypass attempts.
%%
%The 5-tuple based packet logs still enables $D$ and the $S$'s customer networks to detect bypass attempts when $S$ intentionally deviates from the given filtering rule set. %violates the per-filter-rule volume enforced by the fairly composed filtering policy \PSD. 
%
%
%%Note that the per-filter-rule accountability allows $S$ to affect the packet filtering decisions within a filter rule (e.g., dropping $p_1$ instead of $p_2$ when both are in the same filter rule); however, this is not considered as the violation of correct filtering operations since it conforms to the DDoS victim's filtering policy.
%%this attack is also feasible when we enforce finer-grained, per-packet accountability and it is fundamentally undetectable by \name and out of scope of the \name system.
%%
%%The per-filter-rule processing achieves a {\em near zero-copy} packet processing.
%Our near zero-copy operation reduces the byte size of what we copy into the trusted environment significantly (e.g., reduced to about 1\% for 1.5 KByte packets and 20\% for 64 Byte packets).
%We evaluate the efficiency of the near zero-copy operation of \name in Section~\ref{sec:eval}.



\subsection{Bottlenecks: Maximum Bandwidth and Number of Rules per SGX Filter}
\label{sec:bottleneck-rule}

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/perf_vs_n_rules}
        % \vspace{-10pt}
        \caption{Filter throughput}
        % \vspace{-5pt}
        \label{fig:thruput-bottleneck}
    \end{subfigure}
    \begin{subfigure}[t]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mem_vs_n_rules}
        % \vspace{-10pt}
        \caption{Filter memory footprint}
        % \vspace{-5pt}
        \label{fig:mem-bottlenck}
    \end{subfigure}
% 	\vspace{-5pt}
    \caption{Filter throughput degradation for increasing number of filtering rules}
    % \vspace{-5pt}
    \label{fig:bottleneck}
\end{figure}

Recent works such as mbTLS have demonstrated the 10Gb/s performance per enclave can be reached with a four SGX cores machine~\cite{naylor2017and}.
Although the processors with six or more cores available on the market~\footnote{List of SGX-enabled processors is available at: \url{ark.intel.com}.} may support larger bandwidth, we consider the maximum network I/O performance of each SGX enclave is 10 Gb/s in the rest of the paper.

Since the SGX-based filter must match the installed rules with incoming flows to perform filtering, the number of filter rules naturally becomes the bottleneck of the filter's performance.
Indeed, we measure the throughput of traffic processed by a single enclaved filter with different numbers of filter rules and show the results in Figure~\ref{fig:thruput-bottleneck}.
We can see from Figure~\ref{fig:thruput-bottleneck} that when the number of filter rules exceeds approximately 3,000, the \name filter's throughput performance rapidly degrades.

% Given the architectural limitation of secure computing resources in currently available SGX architecture, \name's single-enclave deployment may not be able to deal with the ever-growing volume and complexity of attacks.
% Particularly, the number of filter rules can easily become the bottleneck of a \name filter's performance.
% Figure~\ref{fig:bottleneck}(a) shows that the \name filter's throughput performance rapidly degrades when the number of filter rules exceeds around 3,000. 
%Note that 3,000 rules per enclaved filter may fall far short of the desired number of unique filter rules for handling real large-scale volumetric attacks (e.g., Mirai attacks using $2.3$ millions bots with unique IPs~\cite{mirai}).
% e.g., in recent Mirai attacks, the number of unique malware infected IPs per AS can be up to 281,686~\cite{chaos-simulator}.
%\msk{Which is insufficient for Mirai...}



% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[t]{0.25\textwidth}
%         \centering
%         \includegraphics[]{figures/perf_vs_n_rules}
%         \caption{Filter throughput degradation for increasing number of filtering rules.}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.25\textwidth}
%         \centering
%         \includegraphics[]{figures/mem_vs_n_rules}
%         \caption{Filter memory footprint for varying number of filtering rules}
%     \end{subfigure}
%     \caption{Caption place holder}
% \end{figure}


% \begin{figure}[t]
% \centering
% 	\includegraphics[width=0.40\textwidth]{figures/perf_vs_n_rules}
% 	\caption{Filter throughput degradation for increasing number of filtering rules.}
% 	\label{fig:bottleneck}
% \end{figure}

% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.40\textwidth]{figures/mem_vs_n_rules}
% 	\caption{Filter memory footprint for varying number of filtering rules}
% 	\label{fig:mem_rules}
% \end{figure}

One of the explanation is that, when the number of filter rules increases, the lookup table for the packet processing inside an SGX enclave also grows accordingly. 
Even when we use the state-of-the-art multi-bit tries data structure for looking up the filter rules (see Section~\ref{sec:eval} for details), the memory size of the lookup table still grows linearly with the number of filter rules, as shown in Figure~\ref{fig:mem-bottlenck}.
This result also confirms the Enclave Page Cache (EPC) limit is around 92 MB, as seen in many other works (e.g.,~\cite{kuvaiskii2018snort}).

% The core data structure for filtering rule lookup is a state-of-the-art multi-bit tries data structure, and the memory size of the lookup table grows linearly or sub-linearly depending on the type of rules. % (as seen in Table~\ref{tbl:mem-footprint} in Appendix~\ref{sec:payment-channel-appendix}).
% Figure~\ref{fig:bottleneck}(b) shows the growing trusted memory footprint with the increasing number of rules. It confirms the Enclave Page Cache (EPC) limit is around 92 MB, as seen in many other works (e.g.,~\cite{kuvaiskii2018snort}).
%Figure~\ref{fig:bottleneck}(b) shows 3,000 rules can be installed without causing any significant performance loss; however, larger than 3,000 rules cause EPC paging on Linux version of SGX SDK to allow more virtual memory use beyond about 92 MB EPC size~\cite{brenner2016securekeeper}.


% The per-EPC rule-size limit measured in our implementation (approximately 3,000) does {\em not} necessarily apply to other middlebox applications because it depends on the types of operations and implementation details. 
% In our DPDK-based filter implementation, the building phase of this data structure consumes an additional amount of memory, beyond the trie structure itself, which should be preserved in preparation of any upcoming rule update with the necessary hot switch support for frequent rule redistribution.


\subsection{Scalable Filtering with Multiple SGX Filters}
\label{sec:optimization-multiple-enclaves}

%\msk{How to scale out the two non-deterministic filter designs?}

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/scalability.pdf}
% 	\vspace{-5pt}
	\caption{Scalable \name architecture. Multiple \name enclaves are parallelized with an untrusted load balancer.}
% 	\vspace{-15pt}
	\label{fig:scalability}
\end{figure}

Given the architectural limitation of secure computing resources in currently available SGX architecture, the single-enclave filtering deployment may not be able to deal with the increasing attack volume and complexity.
Hence, we propose a generic \codename architecture that can easily scale up as the number of filters grows, as shown in Figure~\ref{fig:scalability}.
The scalable \codename design includes multiple enclaved filters running in parallel and some {\em untrusted} facilitating components such as the high-bandwidth switching fabric and the controller.

In the followings, we describe how filter rules are distributed and dynamically adjusted among multiple enclaves and explain why a malicious filtering network cannot exploit the untrusted components to manipulate the filtering operations.

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.30\textwidth]{figures/multi-enclave-protocol.pdf}
	\vspace{-5pt}
	\caption{Protocol for filter rule recalculation and redistribution across three enclaved filters: $E_0$, $E_1$, and $E_2$.}
	\vspace{-10pt}
	\label{fig:multi-enclave-protocol}
\end{figure}

\paragraph{Filter rules distribution protocol.}
Since the traffic flows being filtered are frequently changed, the filter rules also need to be updated and redistributed among filters accordingly.
We consider the filter rules distribution happens in {\em rounds}, i.e., the entire filter rule set is given and does not change until the next rule reconfiguration is executed.
In each round, the filter rules are calculated and redistributed via a simple master-slave topology among multiple enclaved filters.
We illustrate the protocol in Figure~\ref{fig:multi-enclave-protocol}, where we have filter $E_0$ as the master node and $E_1$, $E_2$ as the slave nodes.
In particular, when reconfiguration of filter rules is desired (e.g., traffic volume or the number of filter rules handled by a certain filter exceeds a threshold), any enclaved filter may initiate a rule redistribution round and become the master node.
Then, all the slave nodes upload their filter rule sets ($R_i$ for $E_i$) and the array of the average received flow rates of each rule set $R_i$ ($B_i$ for $E_i$) to the master node.
The master node calculates re-configured filter rules, which then be redistributed to all the slave nodes and the load balancer. 
If the calculation requires the changes to the number of enclaves, necessary additional steps (e.g., creating and attesting more enclaved filters) may be required before the rule redistribution. 

% F ruies calculation.gulrefilter~\ref{fig:multi-enclave-protocol} illustrates how the filter rules in three \name filters ($E_0$, $E_1$, $E_2$) can be calculated and distributed periodically to keep up with the changes in incoming traffic streams and newly inserted rules in each filter.
% We consider a simple master-slave topology among multiple enclaved filters: $E_0$ (master), $E_1$/$E_2$ (slaves).
% %All the enclave nodes have the equivalent filtering functionalities but the master filter additionally runs the rule optimization algorithm and re-distribute them periodically.
% When reconfiguration of filter rules is desired (e.g., traffic volume or the number of filter rules handled by a certain filter exceeds a threshold), a rule redistribution process can be initiated by any filter enclave.
% Then, all the enclave nodes upload their filter rule sets ($R_i$ for $E_i$) and the array of the average received flow rates of each rule set $R_i$ ($B_i$ for $E_i$) to the master node.
% The master node executes the greedy algorithm for the re-configured filter rules, which then be redistributed to all the enclave nodes and the load balancer. 
% If the algorithm requires the changes to the number of enclaves, necessary additional steps (e.g., creating and attesting more enclaved filters) may be required before the rule redistribution. 

% We assume that time synchronization between the enclaves is accurate (which may require a secure time protocol among enclaves; e.g., ~\cite{matetic2017rote}) and filters are supposed to have a short grace period at the boundaries of new rule configuration which can be set according to the maximum time synchronization error. 

% To make the \name filter scalable to increasing attack volume and complexity, we propose a generic scalable \name architecture, as shown in Figure~\ref{fig:scalability}.
% Note that our trusted filter parallelization differs from distributed filter/monitoring proposals (e.g.,~\cite{ioannidis2000implementing,sekar2006lads}) in that (1) it involves an untrusted traffic load balancer with multiple trusted filters and (2) it creates an optimization problem with strict memory limitation that restricts the number of rules per filter implementation, as discussed in Section~\ref{sec:bottleneck-rule}. 
% 
% Note that some filter rules are given by a victim network but some are generated and inserted into the lookup table on demand as data packets enter the filters.
% In our discussion, we first assume that the entire filter rule set is given and does not change until the next rule reconfiguration is executed.
% At the end of this section, we describe how to handle dynamic rule updates (e.g., insertion, deletion) between two rule reconfigurations.




%\msk{ILP formulation}
\input{chapters/ilp-formal}

\paragraph{Detecting misbehavior of untrusted components.}
The load balancer and other components outside of the enclave are untrusted and may misbehave.
For example, the load balancer may redirect to a filter the traffic flows that do not match with the filter rules assigned for that filter.
However, these misbehaviors can be easily detected by each filter by checking if it receives any packets that do {\em not} match the rules it receives from the master node.
Each enclave detects such load-balancing misbehavior, and reports it to the DDoS victim.
%
Note that if the load balancer drops the traffic flows that are supposed to be redirected to an enclave, it can be detected by the bypass detection of the auditable filters (see Section~\ref{sec:filter-design}).

% Our filter parallelization calculates the filter rule sets for each filter enclave (including both {\tt ALLOW} and {\tt DROP} rules) given the filter rules and the incoming traffic volume per each rule.
% Then the filter rule sets are pushed to each filter.
%
% As the filtering operation begins, each filter checks if it receives any packets that do {\em not} match the rules in its enclave, which implies the {\em misbehavior} of the untrusted load balancer. 
% Each enclave detects such load-balancing misbehavior, and reports it to the DDoS victim.
%

%\msk{Heuristic solution? Demonstrate complexity... time to solve it...?}


%In the single instance scheme, the proof of contracted work is generated by the \name enclave along with the signature and submitted by $S$ to the \name contract on behalf of the enclave. The same approach still works in the parallel deployment with only one amendment: the proof has to be signed by all the others if no load-balancer misbehaviors are detected. Any missing signature will cause failure of the verification process in the smart contract, and $S$ will not get the reward for the submitted work. 

==> paper 2/chapters/sec-analysis.tex <==
\subsection{Set Intersection Attacks}
\label{subsec:security}

%\paragraph{Set Intersection Attacks.}
If the attacker is allowed to adaptively change his policy and make
observations for each candidate input policy it selects, then our algorithm is
susceptible to another class of attacks. Specifically, we know that for a
given pair of input policies, the size of anonymity set is fixed. Given a
$P_D$ that the attacker wants to recover, he can first send his $P_S$ and
observes resulting $P_{SD}$. Then the attacker can start doing adaptive
attack, where by it changes the $P_S$ to an equidistant $P_S$ from the first
observed $P_{SD}$. It then recovers all the corresponding $P_{SD}$. Once the
attacker has collected all possible $P_{SD}$, it performs an intersection of
all the anonymity sets to get the actual $P_D$.

As an example, lets say that the input policies are $(1, 4, 3, 2)$ which is
known to the attacker and $(3, 4, 2, 1)$ which is the policy that the attacker
wants to learn. When the algorithm executes for the first time, it selects
$(3, 1, 4, 2)$ as the composite policy. Figure~\ref{fig:eg2} shows the 
sub-graph  of the polyhedron for this composition. After the first run, the
attacker's anonymity set comprises of $(3, 4, 2, 1), (3, 2, 1, 4)$ which
satisfy the constraints of being at a distance of $2$ from input $(1, 4, 3,
2)$ and at a distance of $1$ from the mid-point policy $(3, 1, 4, 2)$. To
learn which of these policies is the one that was given by the victim, the
attacker adapts it input. Specifically, it choses one of the polices from the
anonymity set as the new input policy. Lets say in this case, it choses $(3,
4, 2, 1)$ as its new policy. The algorithm now as to compute the composition
of attacker chosen policy $(3, 4, 2, 1)$ and victim's policy $(3, 4, 2, 1)$,
which results in $(3, 4, 2, 1)$ being the new composite policy. As soon as the
attacker observes that the new $P_{SD}$ is the same as the one it chose
adaptively, it knows that the victim has the exact same policy.  On the other
hand, if the attacker had chosen  $(3, 2, 1, 4)$ as its new adaptive input
policy, the algorithm would generate $(3, 1, 4, 2)$ as the new $P_{SD}$ which
is the same as the original composite policy. This would have told the
attacker that the it is not the victim's  policy, which in turn would have
implied that the other policy in the anonymity set (i.e., $(3, 4 , 2, 1)$) is
the victim's policy.

% \paragraph{Generic Attacks.}
% So far, we have assumed that the attacker (source ISP or destination ISP)
% knows the composite policy $P_{s,d}$ computed by any one of our algorithms.
% Here we show how this is possible. We know that each class in the order-based
% policy comprises of IP addresses. When the middlebox sees a packet, it first
% identifies which class the packet belongs to and then refers to the composite
% policy to probabilistically decide whether to drop or keep the packet. The
% rate of dropping a packet is directly defined by the rank of that packet's
% class in the policy.  The attacker knows that the output rate of the packets
% being transmitted is capped to a $L$ bps  pre-specified and known to both the
% ISPs.

% If the source ISP is the attacker, it controls the types and number of packets
% it can deliver to the middlebox. To learn the composite policy, the source ISP
% starts adaptively pre-filtering the traffic it sends to the middlebox.
% Specifically, it starts filtering all the traffic and floods the middle box
% only say 2L packets which belong to one class $C_3$ whose class rate is
% $P_{C_3}$. The middlebox consults the policy and drops $(2L) * (1 - P_{C_3})$
% of the input packets. The attacker measures the number of total packets that
% are being forwarded which is $(SL) * P_{C_3}$. The attacker can easily reverse
% engineer that the class-rate for $C_3$ is $P_{C_3}$. The attacker can repeat
% this process for all the traffic classes and learn all the $P_{C_i}$. This
% directly leaks the composite policy $P_{s, d}$ being deployed by the middlebox.








==> paper 2/chapters/tesef-filter-design.tex <==
\section{Auditable Filter Design}
\label{sec:filter-design}

The \codename filtering operation is enclosed by an SGX enclave where the integrity of its execution is guaranteed, i.e., a malicious filtering network cannot tamper it.
Furthermore, the filtering internal logic and states are also securely verified via the remote attestation process~\cite{johnson2016intel}.
% The auditability of the enclaved filter relies on the remote attestation to the filter's internal logic.
The isolated execution and remote attestation are useful in realizing the auditable filter; yet, they are insufficient because (1) the filtering decisions can be influenced by the external inputs to the filter such as packet order and time clock feeds, which are controlled by the filtering network; and (2) the malicious filtering network may redirect the traffic within its network to bypass the filtering operations.

To address these two challenges, we propose the filtering operations to be {\em stateless} and hence be independent from the external inputs (\S\ref{sec:stateless-filter-design}) and implement the enclaved packet logs to detect bypassing attempts (\S\ref{sec:filter-bypass-detection}).

% \muoi{Editing this section soon}

% In this section, we address the three challenges (i.e., auditability, scalability, and bypass resistance) of \name.% and then address the corresponding three research questions we have raised in Section~\ref{sec:problem-statement} in the three following subsection. 

% \vyas{one thing that is not obvious to me is the deployment of the hardware inside the ixp. do we envision the ixp owner supporting hardware to run these services or proivde rackspace for the isps wanting to offer this service? isnt the spasce constrained? how muich hardware do they need to add? is this like a small pvt cloud that the isps can use etc? i think we need some sort of a design overview showing what additional componetns need to be added to the IXP why you think it is feasible and not too much of a burden and whether that is consistent with the reaquirements of the hardware/performance we see in eval etc. not quite obvious in the current version}



\input{chapters/auditable-filter-design}
% \input{chapters/scalable-filter-design}
\input{chapters/filter-bypass-detection}


==> paper 2/chapters/tesef_details.tex <==
\subsection{Deployment Example}
\label{sec:deployment-example}

%\msk{End-to-end deployment?}

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.40\textwidth]{figures/overview-sigcomm.pdf}
	\vspace{-5pt}
	\caption{A deployment example of \name. (NOC: Network Operations Center, RPKI: Resource Public Key Infrastructure, and IAS: Intel Attestation Service.)}
	\vspace{-15pt}
	\label{fig:overview}
\end{figure}

Figure~\ref{fig:overview} shows an example deployment scenario.
%Here is a summary of the scenario in multiple steps. 
%s found in : % in Section~\ref{sec:architecture-overview}.
%The eight steps are explained as follows:

% Figure~\ref{fig:steps} illustrates the steps needed to establish trust between $S$ and $D$ with the \name system:
% \begin{figure}[h]
% 	\noindent\fbox{\begin{minipage}{\columnwidth}
% 			\footnotesize
			\begin{packedenumerate}
				\item[(1)] {\bf Secure channel establishment:} $D$ contacts $S$ via an out-of-band channel to establish a secure channel.
				They rely on the RPKI infrastructure to authenticate each other.
				$D$ may choose the direct origin of the source IP address it wants to filter or the immediate one-hop upstream of the origin. 
				\item[(2)] {\bf Contract parameter negotiation:} $S$ and $D$ negotiate on  high-level parameters (e.g., pricing, bandwidth limit) in one or more rounds of message exchanges.
				\item[(3)] {\bf Enclave creation:} $S$ creates a enclave for a traffic filter and obtains the enclave quote from quoting enclave. 
				For scalable filtering bandwidth, $S$ may create multiple enclaves as described in Section~\ref{sec:optimization-multiple-enclaves} and \ref{sec:attestation-multiple-enclaves}. %; see Section~\ref{sec:data-plane-design}.
				\item[(4)] {\bf Attestation:} $S$ contacts the IAS and verifies the attestation report.
				\item[(5)] {\bf Attestation report sharing:} $S$ sends the attestation report to $D$ so that it can verify the report locally.
				\item[(6)] {\bf Policy submission:} Both $S$ and $D$ submit their filtering policies to the policy calculation logic. A final policy is computed  inside the enclave.
				\item[(7)] {\bf Packet filtering:} The filter in the enclave is activated and traffic destined to $D$ is routed to the filter. 
				\item[(8)] {\bf Refutable invoice:} The amount of the executed work is sent to $S$ and $D$.
			\end{packedenumerate}
% 	\end{minipage}}
% 	\caption{The \name's steps.}
% 	\label{fig:steps}
% \end{figure}

%\msk{The full end-to-end deployment in Appendix?}

% \paragraph{Secure channel establishment (Step 1):} 
% When $D$ detects a volumetric DDoS attack, it first identifies the IP addresses/prefixes that it wishes to rate limit (e.g., via NetFlow analysis~\cite{netflow}). 
% Then, $D$ determines one or more source ISPs that it wishes to install traffic filters. 
% $D$ may contact the owners of the detected IP addresses/prefixes or their immediate upstream ISPs. 
% The ownership of IP prefixes and the peering relationship can be obtained from various public database (e.g., RPKI~\cite{rpki}, RIPE~\cite{ripedb}, PeeringDB~\cite{peeringdb}). %  infrastructure and the peering relationship can be obtained from various public peering database, such as PeeringDB}.


% Then, $D$ contacts one or more willing source ISPs and establish secure point-to-point channels with them independently. 
% Consider $D$ (with a RPKI public key $K_D$) creates a channel with a willing ISP $S$ (with a RPKI key $K_S$).
% $D$ may directly contact via $S$'s contact information found in the public database (e.g., $S$'s RIPE record often lists email addresses).
% Alternatively, $D$ can publicly announce that it wishes to establish a filtering contract with $S$ in one or more well-known public bulletin boards, network administrator forums, regional network operator group's mailing list (e.g., NANOG mailing list), or highly available web platform (e.g., IPFS\footnote{\url{https://ipfs.io/}}). 
% %In either case, $D$ needs to attach its RPKI  key signature. 
% Then, a wiling $S$ can respond with its own RPKI signature to begin the channel establishment. 
% Similar to other X.509 certificates, RPKI can be used to establish an ephemeral session key between $S$ and $D$ within a few of interactions (e.g., TLS key exchanges~\cite{rfc5246}).

%\paragraph{Assumptions.}
In this example, we assume both source and destination ISPs participate in a common public key infrastructure (PKI) system that binds their AS numbers and IP addresses.
In this paper, we consider the use of the Resource Public Key Infrastructure (RPKI)~\cite{lepinski2012infrastructure} for the origin authentication of ISPs~\cite{rpki}; see Section~\ref{sec:multiple-session-rpki} on how this assumption affects the effectiveness of \name defense. 
We also assume the Internet connectivity of a network operations center (NOC) of an ISP even when it is under DDoS attack.
It is based on the observation that ISPs traditionally have maintained out-of-band channels (e.g., external email servers, telephone lines~\cite{dots-slides}) and ISPs contact other ISPs when hit by large-scale DDoS attacks for manual collaboration defense schemes (e.g., large-scale ISP coordination during the ProtonMail attack~\cite{protonmail}).
Completely independent out-of-band channels, such as cellular Internet connectivity, can be also assumed for the NOCs' backup connectivity during the worst DDoS attacks.


%
%
%
%There are multiple ways: (1) $D$ may rely on some reputable public databases (e.g., RIPE database\footnote{\url{https://www.ripe.net/manage-ips-and-asns/db}}) to obtain the contact information (e.g., email address) of source ISPs
%$D$ may directly sends the initial messages to the contacts in the public RPKI  database \msk{details?}. 
%Or, we can imagine one or more reliable bulletine boards that ISPs can send and receive messages (perhaps openly). 
%
%Secure channel, session key.



% a realistic assumption is the alternative communication line at NOCs. 
%
%$D$ first attempts to make contact with $S$ through the open Internet. For example, anyone can find ISPs contact details in public database such as RIPE\cite{ripe}. Taking these open contact as a starting point, $D$ and $S$ makes a key exchange following the standard protocol (e.g., Diffie-Hellman\cite{}) to create a emphemeral session key for encrypted communication. Also, Their RPKI resource certificates are used to authenticate each other, avoiding any impersonation by attackers or non-ISPs. After the key exchange and authentication, $S$ and $D$ can use the established channel for exchanging information that should be kept private between them.

% \paragraph{Parameter negotiation (Step 2):}. 
% $S$ and $D$ negotiate on the contract parameters. We outline the three parameters: {\bf\em f}, {\bf\em p}, and {\bf\em t}. {\bf\em f} specifies the range of the traffic that should be filtered, which describes IP-prefix level traffic originating from $S$ and destined to $D$. 
% This corase-grained traffic description is sufficient for negotation and more detailed filtering rules will be exchanged privately only after when \name enclave is launched. 
% {\bf\em p} is a pricing rate and will be used in $D$'s payment to $S$ and {\bf\em t} sets a time limit for \name contract and \name filter.
% %   

%<<<<<<< HEAD
% \begin{figure}[h]
%    \begin{framed}
%        \raggedright
%        $\mathrlap{\mathbf{f}}\hphantom{\mathbf{M}}$:  maximum range of the traffic to be filtered. \\
%        $\mathbf{m}$:  maximum inbound rate that counts in the bill. \\
%        $\mathrlap{\mathbf{l}}\hphantom{\mathbf{M}}$:  maximum outbound rate that $F$ should be reduced to. \\
%        $\mathrlap{\mathbf{p}}\hphantom{\mathbf{M}}$:  price that $S$ charges $D$ for the traffic removed. \\
%        $\mathrlap{\mathbf{t}}\hphantom{\mathbf{M}}$:  contract expiration time
%    \end{framed}
%    \caption{\name contract parameters\msk{a table would look better?}}
%    \label{fig:contract-param}
% \end{figure}

%\begin{table}
%\small
%  \caption{\name contract parameters}
%  \label{tab:contract-param}
%  \begin{tabular}{ cl }
%    \toprule
%    % \hline
%    % \multicolumn{2}{c}{\name contract parameters} \\
%    {\bf \em f} & maximum range of the traffic to be filtered \\
%%    {\bf \em m}& maximum inbound rate that counts in the bill \\
%%    {\bf \em l} & maximum outbound rate that $F$ should be reduced to \\
%    {\bf \em p} & price that $S$ charges $D$ for the traffic removed \\
%    {\bf \em t} & contract expiration time \\
%    \bottomrule
%  \end{tabular}  
%\end{table}
%
%\paragraph{Enclave creation and remote attesattion (Step 3, 4, 5):}. In preparation for proceeding the contract, $S$ is responsible for launching the auditable \name filter within its network, and presents $D$ with a proof - the \textit{attestation report} that obtained from IAS after the remote attestation. First, $S$ launches the \name filter's enclave ($E$), and then asks the quoting enclave for a special data structure called \textit{quote}, which collects the information regarding $E$'s creations including but not limited to: the secure \textit{measurement} over the enclave loading process, the enclave \textit{certificate} issued by its author and the \textit{user data} such as a fresh symmetric key pair generated inside the enclave.
%%=======
%%\begin{figure}[h]
%%    \begin{framed}
%%        \raggedright
%%        $\mathrlap{\mathbf{F}}\hphantom{\mathbf{M}}$: The maximum range of the traffic to be filtered. \\
%%        $\mathbf{M}$: The maximum inbound rate that counts in the bill. \\
%%        $\mathrlap{\mathbf{L}}\hphantom{\mathbf{M}}$: The maximum outbound rate that $F$ should be reduced to. \\
%%        $\mathrlap{\mathbf{P}}\hphantom{\mathbf{M}}$: The price that $S$ charges $D$ for the traffic removed. \\
%%        $\mathrlap{\mathbf{T}}\hphantom{\mathbf{M}}$: The contract expiration time
%%    \end{framed}
%%    \caption{\name contract parameters}
%%    \label{fig:contract-param}
%%\end{figure}

% \paragraph{Enclave creation and remote attestation (Step 3, 4, and 5):}. 
% %In preparation for proceeding the contract, $S$ is responsible for launching the auditable \name filter within its network, and presents $D$ with the proof --- the \textit{attestation report} that can be obtained from IAS after the remote attestation. 
% First, $S$ launches the \name filter's enclave ($E$), and then asks the quoting enclave for a special data structure called \textit{quote}, which collects the information regarding $E$'s creations including but not limited to: the secure \textit{measurement} over the enclave loading process, the enclave \textit{certificate} issued by its author and the \textit{user data} such as a fresh symmetric key pair generated inside the enclave.
% %
% The quoting enclave is a trusted component developed by Intel and running on the same hardware as part of the SGX platform service. It owns a EPID~\cite{brickell2009enhanced} member private key whose signature can only be verified by Intel with the corresponding EPID group public key. $S$ has to sends the quote to IAS in exchange for the {\em attestation report} to convince $D$ about the prepared \name filter. This report has IAS's signature so that $D$  can verify the report and ensure the untampered \name filter running on a trusted hardware and $E$'s public key for identifying it.

% \paragraph{Policy composition and execution (Step 6 and 7):} 
% The \name filter receives two policies \PS and \PD from $S$ and $D$, respectively. 
% $S$ and $D$ signs their policies with their RPKI private keys and encrypt them with $E$'s public key.
% The specifications of policies \PS and \PD are negotiated between $S$ and $D$, and we make no assumption on their types.
% $S$ and $D$ agree on the composition algorithm that combines \PS and \PD into \PSD.
% %When two policies have conflicting rules, the algorithm has to resolve them and create a reconciled rule. 
% %For example, when $S$ wishes to allow packet $x$ but $D$ wishes to block it, the algorithm decides the final rule that is actually implemented. 
% The specific algorithm that determines the composition (e.g., perfectly fair reconciliation) is also determined during the negotiation. %; see Section~\ref{}. 

%\begin{figure}[t!]
%	\centering
%	\includegraphics[width=0.4\textwidth]{figures/metering.pdf}
%	\caption{An example of the metering}
%	\label{fig:metering}
%\end{figure}

% \paragraph{Refutable invoice (Step 8):} 
%$S$ receives direct payment from $D$ for the amount of filtering work (e.g., volume of traffic that has been removed). 
% We rely on the enclave $E$ for metering the amount of traffic removed by the filter since neither $S$ nor $D$ can convince the other side regarding this measurement. 
% The invoice is created inside the enclave $E$ and sent to the source ISP. 
% The source ISP then can use this as the invoice claim for the task requested by the destination and requests compensation via an external payment channel. %; see Section~\ref{}.
%$D$ is required to transfer enough funds to $E$' wallet $W_E$ as the deposit and let $E$ make the direct payment fully according to the actual work it measured during the operation. 
%Three paramters ({\bf\em m}, {\bf\em l}, {\bf\em p}) in the contract affect the payout as well as the actual incoming rate towards the \name filter. The measurement is made as follows: only the moment when the incoming rate is between {\bf\em l} and {\bf\em m} counts towards the final summary and any rate over {\bf\em m} is capped at {\bf\em m} and any rate below {\bf\em l} is not considered. 
%Figure~\ref{fig:metering} illustrates this: the shaded area in  is the actual work admitted by $E$ given that the curve is the actual incoming rate variation. 
%The final payment to $D$ is the product of this quantity and the price $P$.
%
%To efficiently realize this guaranteed payment mechanism, as an example, we use a cryptocurrency for the deposit and the payout. 
%Let us consider that $W_S$, $W_D$, and $W_E$ are the cryptocurrency addresses. 
%Particularly, $W_E$ is a fresh address securely generated inside the \name enclave. 
% example of showing the automatic and guaranteed payment, the digital coins such as Bitcoin really show the benefits in terms of safety, digitalization and transparency. Before making any Bitcoin trasancation, $S$, $D$ and $E$ need to generate its own wallet address (equivalently a pair of public key and private key) in private to either accepts the payment or holds the balance safely. And, they also identify each other wallet address by signing the wallet address with the RPKI public key ($S$ or $D$) or the newly generated but verified key ($E$).
%
%$D$ first makes a transaction to $W_E$ with sufficient deposit in order to convince $S$.
%This transaction (Step 6') is locked (e.g., Bitcoin's \texttt{nLockTime}\cite{nlocktime}) so that the deposit can be automatically refunded to $D$ when $E$ does not make the payout (e.g., $E$ is destroyed or blocked) by the time deadline set by $S$. 
%
%However, to complement the fund safety, before any transaction happens, $E$ first construct a \textit{promised} transaction (implemented by setting the parameter \texttt{nLockTime}\cite{nlocktime}) that cannot be included in the blockchain before time $T$.
%This trasancation acts as a fail-safe mechanism that guarantees $D$'s control of the deposit after time $T$.
%%that making a deposit transaction to $E$ has no risks such as deposit being buried on the blockchain due to $E$ being terminated accidentally (no one can spend the money).
%Note that this promised transaction is needless to be published immediately by $E$ after signing the trasaction. Instead, it is sent to $D$ in exchange for $D$'s deposit transaction.
%
%Once $S$ finds the deposit transaction, the traffic $F$ is redirected to $E$ for filtering and any work done by the \name filter is correctly measured.
%Eventually before time $T$, $E$ will make one public transaction to arrange the payment to $S$ and refund $D$ at the same time.
%If anything unexpeted happens and $E$ could not publish the final transaction, $D$ may consider that $S$ is not running \name filter accordingly and advertise the promised trasaction to get its money back.



==> paper 2/chapters/trust-establishment.tex <==
\section{\name: A Source Filtering System}
\label{sec:overview}

In this section, we introduce a new source filtering system, called \name\footnote{\name stands for `Trust Establishment for Source-end Filtering.'}, and overview its architecture focusing on the high-level goals it is designed to achieve and the considered threat model. 













%We do not consider the denial-of-service attack against the underlying blockchain overlay network (e.g., flooding the majority of 32,000 Ethereum nodes distributed across thousands ASes\footnote{AS distribution of Ethereum nodes from \url{https://www.ethernodes.org/network/1}. \msk{TODO.}}), which would involve much larger DDoS attacks than the attack we handle in this paper.


%\subsection{Desired Properties of \name}
%We summarize the remaining key technical challenges to achieving the two desired properties for the \name's vision.
%In the rest of this paper, we focus on the following properties:
%
%\begin{itemize}
%	\item {\bf Scalable and indirect contract establishment (\S\ref{sec:econ-incentive}). }	
%	To handle large numbers of pairwise filtering contract between many ISPs we design a compact \name contract.
%	We minimize the number of on-chain transactions and the estimated gas of the contract by a lightweight contract design.
%	We show that we can support xx thousand pairwise contracts concurrently, which only amount to less than yy percent of gas allowed per block. 
%	We also design an indirect smart contract structure that removes direct inter-ISP message exchanges when establishing contracts in the middle of flooding attacks. 
%
%
%	\item {\bf Scalable line-rate data-plane design (\S\ref{sec:data-plane-design}). }	
%	The \name enclave should support line-rate data-plane performance while conducting per-packet secure processing.
%	Moreover, when the attack volume from $S$ and $D$ exceeds the bandwidth capacity of a single \name enclave (e.g., 10 Gb/s), \name must be extended with parallel \name enclaves and handle large volume traffic (e.g., 60 Gb/s or higher) while preserving the same level of security guarantees.
%\end{itemize}

\input{chapters/tesef_details}


==> paper 2/figures/attack-overview.tex <==

\tikzstyle{function} = [circle, draw, dashed, text width=2em, text badly centered, inner sep=0pt]
\tikzstyle{block} = [rectangle, draw, 
text width=2em, text centered, minimum height=1em]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{attack} = [draw, -latex', color=red]

\begin{figure}[th]
    \centering
    \begin{tikzpicture}[node distance = 5em, auto]
        % Place nodes
        \node [block] (ps) {$P_S$};
        \node [block, below of=ps, node distance=3em] (pd) {$P_D$};
        \node [function, right of=ps, yshift=-1.5em] (phi) {$\phi$};
        \node [block, right of=phi] (psd) {$P_{S, D}$};
        \node [function, right of=psd] (psi) {$\psi$};
        \node [block, right of=psi] (rl_param) {$c_i, r_i$};
        \coordinate [below of=psi, node distance = 1.5em] (A1);
        \coordinate [left of=phi, node distance = 2em] (A2);
        \coordinate [below of=phi, node distance = 1.5em] (A3);
        % % Draw edges
        \path [line] (ps) -- (phi);
        \path [line] (pd) -- (phi);
        \path [line] (phi) -- (psd);
        \path [line] (psd) -- (psi);
        \path [line] (psi) -- (rl_param);
        \path [attack] (rl_param) .. controls (A1) .. node[below]{(1) learn $P_{S, D}$} (psd);
        \path [attack] (ps) .. controls (A2) .. (pd);
        \path [attack] (psd) .. controls (A3) .. node[below]{(2) learn $P_D$} (pd);
    \end{tikzpicture}
    \caption{Adversary $S$ inferring $D$'s policy}
    \label{fig:attack-overview}
\end{figure}

==> paper 2/tables/black-white-list.tex <==
\begin{table}[]
\centering
\caption{Firewall policy. White-listing and black-listing rules of source and destination for $4$ prefixes.}
\label{tab:black-white-list}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{Header}}                         & \multicolumn{2}{c|}{\textbf{Source}}                                                                                          & \multicolumn{2}{c|}{\textbf{Destination}}                                                                                     & \multicolumn{2}{c|}{\textbf{Composition}}                                                                                     \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}IP /\\ Range\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}White\\ List\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Black\\ List\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}White\\ List\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Black\\ List\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}White\\ List\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Black\\ List\end{tabular}} \\ \hline
$x_1$                                                         &                                                               & \yes                                                          &                                                               & \yes                                                          &                                                               & \yes                                                          \\ \hline
$x_2$                                                         &                                                               & \yes                                                          & \yes                                                          &                                                               &\yes                                                           & \\ \hline
$x_3$                                                         & \yes                                                          &                                                               &                                                               & \yes                                                          &\yes                                                           & \\ \hline
$x_4$                                                         & \yes                                                          &                                                               & \yes                                                          &                                                               & \yes                                                              & \\ \hline
\end{tabular}
\end{table}


==> paper 2/tables/eg_composite_policy.tex <==
\begin{table}[]
\centering
\caption{An example of final policy using root mean square composition function $\phi_{RMS}$.}
\label{table:example-final-policy}
\begin{tabular}{c|c|c|c|c|c|c|}
\cline{2-7}
\multicolumn{1}{l|}{}                                                                         & \multicolumn{2}{c|}{\textbf{Source}}                                                                                                  & \multicolumn{2}{c|}{\textbf{Destination}}                                                                                             & \multicolumn{2}{c|}{\textbf{Composition}}                                                                                                     \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Header \\ Flow\\ $f_i$\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Weight\\ $W_{Si}$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rank\\ $R_{Si}$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Weight\\ $W_{Di}$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rank\\ $R_{Di}$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Weight\\ $W_{\phi_i}$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rank\\ $R_{\phi_i}$\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{$x_1$}                                                                   & 0.50                                                               & 1                                                                & 0.40                                                               & 1                                                                & 0.45                                                                   & 1                                                                    \\ \hline
\multicolumn{1}{|c|}{$x_2$}                                                                   & 0.05                                                               & 4                                                                & 0.30                                                               & 2                                                                & 0.22                                                                   & 3                                                                    \\ \hline
\multicolumn{1}{|c|}{$x_3$}                                                                   & 0.30                                                               & 2                                                                & 0.20                                                               & 3                                                                & 0.25                                                                   & 2                                                                    \\ \hline
\multicolumn{1}{|c|}{$x_4$}                                                                   & 0.15                                                               & 3                                                                & 0.10                                                               & 4                                                                & 0.13                                                                   & 4                                                                    \\ \hline
\end{tabular}
\end{table}

==> paper 2/tables/eg_ip_rate_limiter_policy.tex <==
\begin{table}[th]
\centering
\caption{An example of provider policy}
\label{table:example-provider-policy}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Header Flow} & \textbf{Weight} & \textbf{Preference} \\
\textbf{$f_i$} & \textbf{$W(f_i)$} & \textbf{$R(f_i)$} \\
\hline
\parbox[t]{0.5cm}{
$x_1$ \\
$x_2$ \\
$x_3$ \\ 	
$x_4$ \\ 
} &
\parbox[t]{0.5cm}{
0.50 \\
0.05 \\
0.30 \\
0.15 \\
} &
\parbox[t]{0.5cm}{
1 \\
4 \\
2 \\
3 \\
} \\
\hline
\end{tabular}
\end{table}

==> paper 2/tables/eg_provider_policy.tex <==
\begin{table}[th]
\centering
\caption{An example of provider policy}
\label{table:example-provider-policy}
\begin{tabular}{|c|c|}
\hline
\textbf{Preference Policy $P$} & \textbf{Rank Function $r^P(x_i)$} \\
\hline
\parbox[t]{1cm}{
$x_4$ \\
$x_3$ \\
$x_1, x_2$
} &
\parbox[t]{1cm}{
1 \\
2 \\
3
} \\
\hline
\end{tabular}
\end{table}




==> paper 2/tables/eg_rate_limiter_policy.tex <==
\begin{table}[]
\centering
\caption{An example of provider policy}
\label{table:example-provider-policy}
\begin{tabular}{|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Header Flow\\ $f_i$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Weight\\ $W_i$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rank\\ $R_i$\end{tabular}} \\ \hline
$x_1$                                                                & 0.50                                                            & 1                                                                   \\ \hline
$x_2$                                                                & 0.05                                                            & 4                                                                   \\ \hline
$x_3$                                                                & 0.30                                                            & 2                                                                   \\ \hline
$x_4$                                                                & 0.15                                                            & 3                                                                   \\ \hline
\end{tabular}
\end{table}

==> paper 2/tables/sor-prime.tex <==
\begin{table}[]
\centering
\caption{SoR. the policy list after policy composition}
\label{tab:sor-prime}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Header\\ Class\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$P_A$\\ Rank\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$P_{B'}$\\ Rank\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$\phi{SoR}$\\ Rank\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Normalized\\ Rank\end{tabular}} \\ \hline
$x_1$                                                           & 1                                                             & 2                                                                & 3                                                                   & 1                                                                  \\ \hline
$x_2$                                                           & 2                                                             & 3                                                                & 5                                                                   & 3                                                                  \\ \hline
$x_3$                                                           & 3                                                             & 1                                                                & 4                                                                   & 2                                                                  \\ \hline
$x_4$                                                           & 4                                                             & 4                                                                & 8                                                                   & 4                                                                  \\ \hline
\end{tabular}
\end{table}

==> paper 2/tables/sor.tex <==
\begin{table}[]
\centering
\caption{SoR. the policy list after policy composition}
\label{tab:sor}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}
	Traffic \\
	Class
\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$P_s$\\ Rank\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$P_d$\\ Rank\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$\phi$\\ Rank\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Discretized\\ Rank of $P_{s,d}$\end{tabular}} \\ \hline
$x_1$                                                           & 1                                                             & 1                                                             & 1                                                                   & 1                                                                  \\ \hline
$x_2$                                                           & 2                                                             & 4                                                             & 3                                                                   & 3                                                                  \\ \hline
$x_3$                                                           & 3                                                             & 2                                                             & 2.5                                                                   & 2                                                                  \\ \hline
$x_4$                                                           & 4                                                             & 3                                                             & 3.5                                                                   & 4                                                                  \\ \hline
\end{tabular}
\end{table}

==> paper 2/tables/weight-based.tex <==
\begin{table}[]
\centering
\caption{Weighted Preference Policy. Source's and destination's probabilistic preference to keep the packets of $4$ ranges of IP addresses.}
\label{tab:weight-based}
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{Header}} & \textbf{Source} & \textbf{Destination} & \textbf{Composition} \\ \hline
$x_1$                                 & 0.50            & 0.40                 & 0.45                 \\ \hline
$x_2$                                 & 0.05            & 0.30                 & 0.17                 \\ \hline
$x_3$                                 & 0.30            & 0.20                 & 0.25                 \\ \hline
$x_4$                                 & 0.15            & 0.10                 & 0.13                 \\ \hline
\end{tabular}
\end{table}

==> tables/black-white-list.tex <==
\begin{table}[]
\centering
\caption{Firewall policy. White-listing and black-listing rules of source and destination for $4$ prefixes.}
\label{tab:black-white-list}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{Header}}                         & \multicolumn{2}{c|}{\textbf{Source}}                                                                                          & \multicolumn{2}{c|}{\textbf{Destination}}                                                                                     & \multicolumn{2}{c|}{\textbf{Composition}}                                                                                     \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}IP /\\ Range\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}White\\ List\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Black\\ List\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}White\\ List\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Black\\ List\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}White\\ List\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Black\\ List\end{tabular}} \\ \hline
$x_1$                                                         &                                                               & \yes                                                          &                                                               & \yes                                                          &                                                               & \yes                                                          \\ \hline
$x_2$                                                         &                                                               & \yes                                                          & \yes                                                          &                                                               &\yes                                                           & \\ \hline
$x_3$                                                         & \yes                                                          &                                                               &                                                               & \yes                                                          &\yes                                                           & \\ \hline
$x_4$                                                         & \yes                                                          &                                                               & \yes                                                          &                                                               & \yes                                                              & \\ \hline
\end{tabular}
\end{table}


==> tables/eg_composite_policy.tex <==
\begin{table}[]
\centering
\caption{An example of final policy using root mean square composition function $\phi_{RMS}$.}
\label{table:example-final-policy}
\begin{tabular}{c|c|c|c|c|c|c|}
\cline{2-7}
\multicolumn{1}{l|}{}                                                                         & \multicolumn{2}{c|}{\textbf{Source}}                                                                                                  & \multicolumn{2}{c|}{\textbf{Destination}}                                                                                             & \multicolumn{2}{c|}{\textbf{Composition}}                                                                                                     \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Header \\ Flow\\ $f_i$\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Weight\\ $W_{Si}$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rank\\ $R_{Si}$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Weight\\ $W_{Di}$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rank\\ $R_{Di}$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Weight\\ $W_{\phi_i}$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rank\\ $R_{\phi_i}$\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{$x_1$}                                                                   & 0.50                                                               & 1                                                                & 0.40                                                               & 1                                                                & 0.45                                                                   & 1                                                                    \\ \hline
\multicolumn{1}{|c|}{$x_2$}                                                                   & 0.05                                                               & 4                                                                & 0.30                                                               & 2                                                                & 0.22                                                                   & 3                                                                    \\ \hline
\multicolumn{1}{|c|}{$x_3$}                                                                   & 0.30                                                               & 2                                                                & 0.20                                                               & 3                                                                & 0.25                                                                   & 2                                                                    \\ \hline
\multicolumn{1}{|c|}{$x_4$}                                                                   & 0.15                                                               & 3                                                                & 0.10                                                               & 4                                                                & 0.13                                                                   & 4                                                                    \\ \hline
\end{tabular}
\end{table}

==> tables/eg_ip_rate_limiter_policy.tex <==
\begin{table}[th]
\centering
\caption{An example of provider policy}
\label{table:example-provider-policy}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Header Flow} & \textbf{Weight} & \textbf{Preference} \\
\textbf{$f_i$} & \textbf{$W(f_i)$} & \textbf{$R(f_i)$} \\
\hline
\parbox[t]{0.5cm}{
$x_1$ \\
$x_2$ \\
$x_3$ \\ 	
$x_4$ \\ 
} &
\parbox[t]{0.5cm}{
0.50 \\
0.05 \\
0.30 \\
0.15 \\
} &
\parbox[t]{0.5cm}{
1 \\
4 \\
2 \\
3 \\
} \\
\hline
\end{tabular}
\end{table}

==> tables/eg_provider_policy.tex <==
\begin{table}[th]
\centering
\caption{An example of provider policy}
\label{table:example-provider-policy}
\begin{tabular}{|c|c|}
\hline
\textbf{Preference Policy $P$} & \textbf{Rank Function $r^P(x_i)$} \\
\hline
\parbox[t]{1cm}{
$x_4$ \\
$x_3$ \\
$x_1, x_2$
} &
\parbox[t]{1cm}{
1 \\
2 \\
3
} \\
\hline
\end{tabular}
\end{table}




==> tables/eg_rate_limiter_policy.tex <==
\begin{table}[]
\centering
\caption{An example of provider policy}
\label{table:example-provider-policy}
\begin{tabular}{|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Header Flow\\ $f_i$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Weight\\ $W_i$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rank\\ $R_i$\end{tabular}} \\ \hline
$x_1$                                                                & 0.50                                                            & 1                                                                   \\ \hline
$x_2$                                                                & 0.05                                                            & 4                                                                   \\ \hline
$x_3$                                                                & 0.30                                                            & 2                                                                   \\ \hline
$x_4$                                                                & 0.15                                                            & 3                                                                   \\ \hline
\end{tabular}
\end{table}

==> tables/sor-prime.tex <==
\begin{table}[]
\centering
\caption{SoR. the policy list after policy composition}
\label{tab:sor-prime}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Header\\ Class\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$P_A$\\ Rank\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$P_{B'}$\\ Rank\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$\phi{SoR}$\\ Rank\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Normalized\\ Rank\end{tabular}} \\ \hline
$x_1$                                                           & 1                                                             & 2                                                                & 3                                                                   & 1                                                                  \\ \hline
$x_2$                                                           & 2                                                             & 3                                                                & 5                                                                   & 3                                                                  \\ \hline
$x_3$                                                           & 3                                                             & 1                                                                & 4                                                                   & 2                                                                  \\ \hline
$x_4$                                                           & 4                                                             & 4                                                                & 8                                                                   & 4                                                                  \\ \hline
\end{tabular}
\end{table}

==> tables/sor.tex <==
\begin{table}[]
\centering
\caption{SoR. the policy list after policy composition}
\label{tab:sor}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}
	Traffic \\
	Class
\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$P_s$\\ Rank\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$P_d$\\ Rank\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$\phi$\\ Rank\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Discretized\\ Rank of $P_{s,d}$\end{tabular}} \\ \hline
$x_1$                                                           & 1                                                             & 1                                                             & 1                                                                   & 1                                                                  \\ \hline
$x_2$                                                           & 2                                                             & 4                                                             & 3                                                                   & 3                                                                  \\ \hline
$x_3$                                                           & 3                                                             & 2                                                             & 2.5                                                                   & 2                                                                  \\ \hline
$x_4$                                                           & 4                                                             & 3                                                             & 3.5                                                                   & 4                                                                  \\ \hline
\end{tabular}
\end{table}

==> tables/weight-based.tex <==
\begin{table}[]
\centering
\caption{Weighted Preference Policy. Source's and destination's probabilistic preference to keep the packets of $4$ ranges of IP addresses.}
\label{tab:weight-based}
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{\textbf{Header}} & \textbf{Source} & \textbf{Destination} & \textbf{Composition} \\ \hline
$x_1$                                 & 0.50            & 0.40                 & 0.45                 \\ \hline
$x_2$                                 & 0.05            & 0.30                 & 0.17                 \\ \hline
$x_3$                                 & 0.30            & 0.20                 & 0.25                 \\ \hline
$x_4$                                 & 0.15            & 0.10                 & 0.13                 \\ \hline
\end{tabular}
\end{table}
